Scales in hybrid mice over $\mathbb{R}$

We develop a general theory of strategic mice, prove their condensation properties, and analyze the scales pattern in the stack of $\Theta$-g-organized $\mathcal{F}$-mice over $\mathbb{R}$, Lp$^{G\mathcal{F}}(\mathbb{R})$, for a class of nice operators $\mathcal{F}$.

==> scales_J_premice.tex <==
\section{The fine structural framework}
\label{SigmaMiceOverR}

Given a set $X$, we write $\J(X)$ for the rud closure of $X\un\{X\}$. Standard premice are 
constructed using the function $\J$ to take steps 
at successor stages, adding extenders at certain limits.
One often wants to generalize this picture, replacing $\J$ with 
some \emph{operator} $\Fop$. The resulting structures are \emph{$\Fop$-opremice} (\emph{o} for 
\emph{operator}), which are 
analogous to standard premice,
with the key difference that $\Fop$ is used to take steps at successor stages, instead of $\J$.
(It is more convenient to reserve \emph{$\Fop$-premouse} for a somewhat 
different notion.)

In \S\S\ref{SigmaMiceOverR},\ref{sec:operators}, we will define \emph{$\Fop$-opremice} for a 
fairly 
wide class of operators 
$\Fop$ with nice condensation properties, and develop their basic theory.
(We define \emph{operator} precisely in \S\ref{sec:operators}.)
The theory will reduce to that of standard premice in the case 
that $\Fop=\J$, albeit with somewhat different notation.

This theory has been presented to some extent by others, in the existing literature, but 
there are some problems with those presentations. Here we give a 
(hopefully) complete development of the theory. Much of the theory 
is simply an immediate transcription of the theory of standard premice, so naturally we skip 
such transcriptions and focus on 
what is different. We have tried to develop the theory in a manner which is as compatible as 
possible with the earlier presentations (though in places we have opted for choosing suggestive 
notation and terminology over sticking with tradition). Partly because of this, we develop the 
theory of $\Fop$-opremice more abstractly than what is really necessary for application,
dealing with operators $\Fop$ more general than those given by $\J$-structures.
This does have the cost of increasing somewhat the quantity of work to be completed, and
a reasonable alternative would have been to restrict attention to operators given by 
$\J$-structures, since all applications known to the authors are of this form.
However, it has the advantage of showing what properties of $\J$-structures are most essential 
to the theory.

One class of operators the theory will cover, which makes an illustrative example, are 
\emph{strategy} operators $\Fop_\Sigma$,
such as those with the \emph{least tree hierarchy}, roughly described as follows.
Fix a mouse $P$ and iteration strategy $\Sigma$ for $P$.
Then given an $\Fop_\Sigma$-opremouse $\M$ with associated wellorder $<_\M$,
$\Fop_\Sigma(\M)$ is an amenable structure extending $\M$ which codes
$(\Tt,b)$ where $b=\Sigma(\Tt)$ and $\Tt$ is the $<_\M$-least tree in $\M$, on $P$,
via $\Sigma$, for which $\M$ has no initial segment encoding $(\Tt,b)$.

In \S\ref{SigmaMiceOverR} we will define a series of increasingly focused approximations to 
$\Fop$-opremice.
We first define \emph{hierarchical model}, which describes the most basic structure of 
$\Fop$-opremice.
We refine this by defining \emph{adequate model}, adding some 
semi-fine-structural structural requirements (such as \emph{acceptability}).
We then develop some basic facts regarding adequate models and their cardinal 
structure. From there we can define \emph{potential 
operator premouse \tu{(}potential opm\tu{)}}
(analogous to a potential premouse); this definition makes new restrictions
on the information encoded by the predicates (most significantly that the predicate 
$\hmEdot$ encodes extenders analogous to those of premice), and adds some pre-fine structural 
requirements.
Using the latter, we can define the central fine structural concepts for 
potential opms.
We then define \emph{Q-operator premouse \tu{(}Q-opm\tu{)}} by requiring that every proper segment 
be fully sound,
and show that the first-order content of Q-opm-hood is \emph{almost} expressed by a 
Q-formula.\footnote{As in \cite{fsit}, we consider two cases: type 3, and non-type 3. For example, 
the property of being a non-type 3 Q-opm is expressed by a Q-formula 
modulo transitivity and the Pairing Axiom.}
We then define \emph{operator premouse} (analogous to \emph{premouse}).
We prove various fine structural facts regarding operator premice,
and discuss the basic iterability theory.

In \S\ref{sec:operators}, we introduce \emph{operators} 
$\Fop$, and \emph{$\Fop$-opremice}. In $\Fop$-opremice $\M$, the predicate $\hmEdot$ is used to 
encode an extender, 
$\hmPdot$ to encode auxiliary information given by $\Fop$ (such as the branch $b$ in the 
example above), $\hmSdot$ to encode the sequence of proper initial segments of $\M$, $\hmXdot$ 
to encode the extensions 
of all (not just proper) segments of $\M$, $\hmbdot$ to refer to the coarse 
\emph{base} of $\M$ (a coarse, 
transitive 
set at the bottom of the structure), $\hmpdot$ for the coarse \emph{parameter} of 
$\M$, $\hmmudot$ for the critical point of $\hmEdot$, and 
$\hmedot$ for its largest proper segment.\footnote{\emph{E} is for \emph{extender},
\emph{P} for \emph{predicate}, \emph{S} for \emph{segments}, e\emph{X} for 
\emph{extensions}, \emph{cb} for \emph{coarse base}, \emph{cp} for \emph{coarse parameter},
$\mu$ for \emph{$\mu$easurable}, and \emph{e} for (smaller) \emph{extender}.} An 
$\Fop$-opremouse $\M$ is
\emph{over} its base $A$.
Here $A\in\M$ and 
$A$ is in all proper segments of $\M$.
When considering $\Fop$-opremice over a fixed $A$, all elements of $A\un\{A\}$ will be in all 
hulls 
that we form. However, in some contexts we allow $A$ to vary, and will also be interested in hulls 
which do not include all elements of $A$. In the case, say, of an 
$\Fop_\Sigma$-opremouse for a strategy operator $\Fop_\Sigma$ for a strategy $\Sigma$ for a 
premouse $P$,
we might want our language to be able to refer to $P$ explicitly, and we do this 
using the constant $\hmpdot$. We might, for example, want $A$ to vary while $P$ is fixed,
so it is useful to have both symbols.

We now commence with the details.

\begin{definition}
Let $Y$ be transitive. Then $\varrho_Y:Y\to\rank(Y)$ denotes the rank function.
And $\hat{Y}$ denotes $\trancl(\{(Y,\om,\varrho_Y)\})$.
For $M$ transitive, we say that $M$ is \emph{rank closed} iff for every $Y\in M$,
we have $\hat{Y}\in M$ and $\hat{Y}^{<\om}\in M$. Note that if $M$ is rud closed and rank closed 
then $\rank(M)=\Ord\inter M$.

Let $Y,M$ be transitive structures, with $M$ rud closed, rank closed and
$Y,\om\in M$. The 
\textbf{$\hat{Y}$-coarse projectum of $M$} is the least ordinal
$\rho\geq\om$ 
such that there is
$Z\sub\hat{Y}^{<\om}\cross\rho^{<\om}$ such that $Z$ is definable from parameters over $M$ but 
$Z\notin M$.
\end{definition}


\begin{definition}[Hulls] Let $\Ll=\{\dot{B},\Pvec,\cvec\}$ be a finite first-order language, where 
$\dot{B}$ is a binary predicate, 
$\Pvec=\left<\dot{P}_i\right>_{i<m}$ is a tuple of unary predicates and 
$\cvec=\left<\dot{c}_i\right>_{i<n}$ a tuple of constants.
Let $\N$ be a first-order $\Ll$-structure
and $B=\dot{B}^\N$, etc.
Let $\Gamma$ be a collection of $\Ll$-formulas with ``$x=\dot{c}_i$'' in $\Gamma$ for each $i<n$. 
Let $X\sub\univ{\N}$. Then
\[ \Hull^\N_\Gamma(X)\eqdef(H,B\inter H^2,P_0\inter H,\ldots,P_{m-1}\inter 
H,c_0,\ldots,c_{n-1}), \] where $H$ is the set of all $y\in\univ{\N}$ such that for some 
$\varphi\in\Gamma$ and $\xvec\in 
X^{<\om}$, $y$ is the unique $y'\in\N$ such that $\N\sats\varphi(\xvec,y')$.
If $\N$ is transitive, then
$\C=\cHull^\N_\Gamma(X)$
denotes the $\L$ structure which is the transitive collapse of $\Hull^\N_\Gamma(X)$. (That is,
$\univ{\C}$ is the transitive collapse of $H$, and letting $\pi:\univ{\C}\to H$ be the uncollapse, 
$P_i^\C=\pi^{-1}(P_i)$, etc.)
\end{definition}
\begin{definition}\label{dfn:language_Ll_0}
Let $\Ll_0$ be the language of set theory expanded by unary predicate symbols
$\hmEdot, \hmPdot, \hmSdot$, $\hmXdot$, and constant symbols $\hmbdot$, 
$\hmpdot$, $\hmmudot$, $\hmedot$. Let 
$\Ll_0^-=\Ll_0\cut\{\hmEdot,\hmPdot,\hmmudot,\hmedot\}$.
\end{definition}


\begin{definition}
\label{model}
A \textbf{hierarchical model}
is an $\Ll_0$-structure
\[ \M = (\univ{\M}; \hmE, \hmP, \hmS, \hmX, \hmbv, \hmpv,\hmmu,\hme),\]
where $\hmEdot^\M=\hmE$, etc, $\hmbv=\hmbdot^\M$ and $\hmpv=\hmpdot^\M$, such that for some
ordinal $\lambda>0$, the following hold.
\begin{enumerate}
  \item $\M$ is amenable, $\univ{\M}$ is transitive, rud closed and 
rank closed.
\item (Base, Parameter) $\hmbv=\hat{Y}$ for some transitive $Y$ and $\hmpv\in\J(\hmbv)$; we say 
that 
$\M$ is \emph{over} the 
\emph{\tu{(}coarse\tu{)} base} $\hmbv$
and has \emph{\tu{(}coarse\tu{)} parameter} $\hmpv$.
 \item (Segments) $\hmS = \left<\hmS_\xi\right>_{\xi<\lambda}$ where $\hmS_0=\hmbv$ and for each 
$\xi\in[1,\lambda)$, $\hmS_\xi$ is a hierarchical model over $\hmbv$ with parameter $\hmpv$, with 
$\hmSdot^{\hmS_\xi} = \hmS\rest \xi$.
Let $\hmS_\lambda=\M$.
\item\label{item:limit_union} (Continuity) If $\lambda$ is a limit then 
$\univ{\M}=\bigcup_{\alpha<\lambda}\univ{\hmS_\alpha}$.
\item\label{item:extensions} (Extensions) $\hmX\colon\univ{\M}\to\lambda$, and $\hmX(x)$ is the 
least $\alpha$ such that $x\in\hmS_{\alpha+1}$.
\end{enumerate}
Let $\wl(\M)$ denote 
$\lambda$, the \textbf{length} of $\M$.
For $\alpha\leq\lambda$ let $\M\wupto\alpha=\hmS_\alpha$.
A hierarchical model $\M$ is a \emph{successor} iff $\wl(\M)$ is a successor 
$\xi+1$; in this case let $\M^-=\M\wupto\xi$. If $\wl(\M)$ is a limit, 
let $\M^-=\M$. We say that $\N$ is a 
\emph{whole segment} of $\M$,
and write $\N\wins\M$, iff 
$\N=\M\wupto\alpha$ for some $\alpha\in[1,\lambda]$, and say that $\N$ is a \emph{proper 
whole segment} of $\M$, and write $\N\wpins\M$, iff $\N\wins\M$ and $\N\neq\M$.
(Note that $\M\wupto0=\hmbv\nwins\M$.) We write $E^\M=E$, etc.\footnote{We opted to use 
\emph{cp} instead of just \emph{p} to avoid conflict with notation for standard 
parameters. We use \emph{cb} instead of just \emph{b} because for certain hierarchical models 
$\M$ we will use $b^\M$ to denote a certain branch through a certain iteration tree in $\M$.
Until we discuss strategy premice, $\hmp$ will be unimportant. For better readability, we will 
typically use the variable $A$ to represent $\hmb^\M$.} For any transitive $Y$, let
$\hmb^{\hat{Y}}=\hat{Y}$; so $\hmb^{\M\wupto\alpha}=\M\wupto0$ for all $\alpha$.
\end{definition}

\begin{definition}\label{dfn:adequate}
Let $\M$ be a hierarchical model over $A$.

Let $p\in[\OR(\M)]^{<\om}$. We say that $\M$ is \emph{$(1,p)$-solid} iff for each $i<\lh(p)$,
\[ \Th_{\Sigma_1}^\M(\hmb^\M\un p_i\un\{p\rest i\})\in\M. \]

We say that $\M$ is \emph{soundly projecting} iff 
for every successor $\N\wins\M$, there is $p\in\OR(\N)^{<\om}$ such that $\N$ is $(1,p)$-solid 
and
\[ \N=\Hull_{\Sigma_{1}}^{\N}(\N^-\un\{\N^-, p\}) \]


We say that $\M$ is \emph{acceptable} iff
for every successor $\N\wins\M$,
for every $\tau\in\OR(\N^-)$,
if there is some $X\in\pow(A^{<\om}\cross\tau^{<\om})$ such that $X\in\N\cut 
\N^-$ then in $\N$ there is a map $A^{<\om}\cross\tau^{<\om}\onto\N^-$.

We say that $\M$ is an \emph{adequate model} iff $\M$ an acceptable hierarchical model
and every \emph{proper} whole segment of $\M$ is soundly projecting.
\end{definition}



\begin{definition}\label{dfn:Ll_0-Q-formula} Given a language $\Ll$ extending the language of set 
theory, a \textbf{$\Ll$-simple-Q-formula} is a formula of the form
\[ \varphi(v_0,\ldots,v_{n-1})\ \iff\ \all x\ex y[x\sub y\ \&\ \psi(y,v_0,\ldots,v_{n-1})], \]
for some $\Sigma_1$ formula $\psi$ of $\Ll$. (Here all free variables are displayed; hence, $x$ is 
not free in $\psi$.)

Let $\varphi_{\mathrm{pair}}$ be the Pairing Axiom.
\end{definition}

It is easy to see that neither $\varphi_{\mathrm{pair}}$, nor rud closure, can be expressed, modulo 
transitivity, by a simple-Q-formula.\footnote{If $\Ll$ is a first-order language extending the 
language of 
set theory, and $X,Y$ are rud closed transitive $\Ll$-structures such that $c^X=c^Y$ for each 
constant symbol $c\in\Ll$,
and $P^X=P^Y$ for each predicate symbol $P\in\Ll$ with 
$P\neq\dot{\in}$, then any $\Ll_0$-Q-formula true in both 
$X,Y$ is also true in the ``union'' of $X,Y$.} However:

\begin{lemma}\label{lem:adequate model_almost_Q}
There is an $\Ll_0$-simple-Q-formula $\varphi_{\mathrm{am}}$ such that for all transitive 
$\Ll_0$-structures
$\M$, $\M$ is an adequate model iff $\M\sats[\varphi_{\mathrm{pair}}\ \&\ 
\varphi_{\mathrm{am}}]$.
\end{lemma}
\begin{proof}[Proof Sketch]
 This is a routine calculation, which we omit. (First find an $\Ll_0$-Q-formula 
$\varphi_{\mathrm{rud}}$ such that $[\varphi_{\mathrm{pair}}\ \&\ \varphi_{\mathrm{rud}}]$ 
expresses rud closure;
this uses the the finite basis for rud functions.)
\end{proof}



If $\M$ is an adequate model over $A$ and $\xi<\wl(\M)$ then $\M$ has a map 
\[ A^{<\om}\cross\xi^{<\om}\onto\M\wupto\xi.\]
In fact, by the following lemma, this is true uniformly. Its proof is 
routine, using the sound-projection of proper whole segments of $\M$, much like in the proof 
of the
corresponding fact for $L$.

\begin{lemma}\label{lem:canonical_surjection}
There is a $\Sigma_1$ formula $\varphi$ in $\Ll_0^-$, of two free variables, 
such that for all $A$
and adequate models $\M$ over $A$,
$\varphi$ defines a map $F:\wl(\M)\to\M$, and for $\xi<\wl(\M)$, letting $h_\xi=F(\xi)$, 
we have
\[ h_{\xi}:A^{<\om}\cross\xi^{<\om}\onto\M\wupto\xi\]
and for all 
$\alpha\leq\xi$, we have $h_\alpha\sub 
h_\xi$.
\end{lemma}

\begin{definition}\label{dfn:h^M}
 Given an adequate model $\M$ over $A$ and $\xi<\wl(\M)$, let
$h^\M_\xi$ be the function $h_\xi$ of the preceding lemma.
 Let $h^\M=\bigcup_{\xi<\wl(\M)}h^\M_\xi$.
\end{definition}

\begin{remark}\label{rem:h^M} So $h^\M$ is $\Sigma_1^\M$, uniformly in adequate $\M$,
and
\[ h^\M:A^{<\om}\cross\wl(\M^-)^{<\om}\onto\M^- \]
(recall that if $\M$ is a limit then $\M^-=\M$), and if $\M$ is a successor then 
$h^\M\in\M$.
\end{remark}
\begin{definition}
 Let $\M$ be an adequate model over $A$ and $\lambda=\wl(\M)$.
Let $\rho<\OR(\M)$. Then $\rho$ is an \emph{$A$-cardinal} of $\M$ iff $\M$
has no map $A^{<\om}\cross\gamma^{<\om}\onto\rho$ where $\gamma<\rho$.
We let $\Theta^\M$ denote the least $A$-cardinal of $\M$, if such exists.
We say that $\rho$ is \emph{$A$-regular} in $\M$ iff $\M$ has no map 
$A^{<\om}\cross\gamma^{<\om}\cofto\rho$ where $\gamma<\rho$.
We say that $\rho$ is an \emph{ordinal-cardinal} of $\M$ iff $\M$ has 
no map $\gamma^{<\om}\onto\rho$ where $\gamma<\rho$.
We say that $\rho$ is \emph{relevant} iff $\rho\leq\OR(\M^-)$.
\end{definition}

Using $h^\M_\xi$ we get:

\begin{lemma}
 Let $\M$ be an adequate model over $A$ and $\lambda=\wl(\M)>\xi>0$.
 Let $\kappa$ be an $A$-cardinal of $\M$ such that $\kappa\leq\OR(\M\wupto\xi)$.
 Then $\rank(A)<\kappa\leq\xi$ and $\kappa=\OR(\M\wupto\kappa)$.
\end{lemma}


\begin{lemma}\label{lem:H_Theta^M_etc}
 There is a $\Sigma_1$ formula $\varphi$ in $\Ll_0^-$ such that,
 for any $A$ and adequate model $\M$ over $A$, we have the following.
 
 Suppose $\Theta=\Theta^\M$ exists and is relevant. Then:
 \begin{enumerate}
  \item\label{item:power(a)_unbounded} $\Theta$ is the least 
$\alpha$ such that $\pow(A^{<\om})^\M\sub\M\wupto\alpha$.
  \item\label{item:M_Theta_is_H_Theta} $\univ{\M\wupto\Theta}$ is the set of all $x\in\M$ such that 
$\trancl(x)$ is the surjective image of $A^{<\om}$ in $\M$.
  \item\label{item:uniform_surjections} Over $\M\wupto\Theta$, $\varphi(0,\cdot,\cdot)$ defines 
a function $G:\Theta\to\M\wupto\Theta$ such that for all $\alpha<\Theta$, 
we have $G(\alpha):A^{<\om}\onto\M\wupto\alpha$.
 \item\label{item:Theta_A-regular} $\Theta$ is $A$-regular in $\M$.
\end{enumerate}

 Let $\kappa_0<\kappa_1$ be consecutive relevant $A$-cardinals of $\M$. Then:
 \begin{enumerate}[resume*]
\item $\kappa_1$ is the least $\alpha$ such that 
$\pow(A^{<\om}\cross\kappa_0^{<\om})^\M\sub\M\wupto\alpha$.
\item $\univ{\M\wupto\kappa_1}$ is the set of all $x\in\M$ such that $\trancl(x)$ is the surjective 
image of $A^{<\om}\cross\kappa_0^{<\om}$ in $\M$.
\item Over $\M\wupto\kappa_1$,
$\varphi(\kappa_0,\cdot,\cdot)$ defines a map $G:\kappa_1\to\M\wupto\kappa_1$ such that for all 
$\alpha<\kappa_1$,
we have $G(\alpha):A^{<\om}\cross\kappa_0^{<\om}\onto\M\wupto\alpha$.
\item $\kappa_1$ is $A$-regular in $\M$.
\end{enumerate}
\end{lemma}
\begin{proof}
We just prove parts \ref{item:power(a)_unbounded}--\ref{item:Theta_A-regular}; the others are
similar.

Let $\gamma$ be least such that $\pow(A^{<\om})\inter\M\sub\M\wupto\gamma$.
Then $\gamma$ is a limit ordinal. By acceptability, for every $\alpha<\gamma$,
$\M\wupto\gamma$ has a map $A^{<\om}\onto\M\wupto\alpha$.

Now suppose that $\gamma<\Theta$, and let $g:A^{<\om}\onto\gamma^{<\om}$ be in $\M$.
Let $h=h^\M_\gamma$. Then because $g,h\in\M$, clearly $\M$ has a map
$f:A^{<\om}\onto\M\wupto\gamma$, so there is a surjection 
$f':A^{<\om}\to\pow(A^{<\om})^\M$ in $\M$, a contradiction as usual.

So $\gamma=\Theta$, which gives parts \ref{item:power(a)_unbounded},\ref{item:M_Theta_is_H_Theta}.

Now consider part \ref{item:uniform_surjections}. Let $\alpha<\Theta$.
We will define
$g:A^{<\om}\cross A^{<\om}\onto\M\wupto\alpha$,
and the uniformity in the definition will yield the result.
Let $\beta\in[\alpha,\gamma)$ be least such that
\[ \pow(A^{<\om})\inter\M\wupto\beta\not\sub\M\wupto\alpha.\]
Let $h=h^\M_\beta$. Let $x\in A^{<\om}$ be such that for some $y$, $f=h(x,y)$ is 
such that $f:A^{<\om}\to\M\wupto\alpha$ is a surjection (such $x$ exists by acceptability). Let $y$ 
be least such,
and $f=h(x,y)$. Then for $z\in A^{<\om}$,
define $g(x,z)=f(z)$. For all other $(x,z)$, $g(x,z)=\emptyset$. This completes the definition
of $g$, and the uniformity is clear.

Part \ref{item:Theta_A-regular} now follows.
\end{proof}

\begin{corollary}
 Let $\M$ be an adequate model over $A$ and let $\gamma$ be a relevant $A$-cardinal of $\M$.
 If $\gamma$ is a limit of $A$-cardinals of $\M$ then 
$\M\wupto\gamma$ satisfies Separation and Power Set.
If $\gamma$ is not a limit of $A$-cardinals of $\M$ 
then $\M\wupto\gamma\sats\ZFmin$. In particular, $\M\wupto\Theta^\M\sats\ZFmin$.
\end{corollary}

\begin{lemma}\label{lem:cardinals_equiv}
Let $\M$ be an adequate model over $A$ such that $\Theta^\M$ exists and is relevant.
Let $\kappa\in[\Theta^\M,\OR(\M))$ be relevant.
Then $\kappa$ is an $A$-cardinal of $\M$ iff $\kappa$ is an ordinal-cardinal of $\M$.
\end{lemma}
\begin{proof}
 Suppose $\kappa>\Theta=\Theta^\M$ and $\kappa$ is an ordinal-cardinal,
 but $\M$ has a map 
\[ f:A^{<\om}\cross\gamma^{<\om}\onto\kappa \] where $\gamma<\kappa$.
 For each $y\in\gamma^{<\om}$, let $f_y:A^{<\om}\to\kappa$ be $f_y(x)=f(x,y)$,
 and let $g_y$ be the norm associated to $f_y$
 (that is, $f_y(x)<f_y(x')$ iff $g_y(x)<g_y(x')$, and $\rg(g_y)$ is an ordinal).
Then $g_y\in\M$ and $\rg(g_y)<\Theta$, because the prewellorder 
on 
$A^{<\om}$ determined by $f_y$ is in $\M\wupto\Theta$ and $\M\wupto\Theta\sats\ZFmin$. Similarly, 
the 
function $y\mapsto(f_y,g_y)$ is in $\M$.
 Let
 \[ h:\Theta\cross\gamma^{<\om}\onto\kappa \] be as follows.
 Let $(\alpha,y)\in\Theta\cross\gamma^{<\om}$. If $\alpha\notin\rg(g_y)$ then $h(\alpha,y)=0$;
 otherwise $h(\alpha,y)=f(x,y)$ where $g_y(x)=\alpha$. Then $h\in\M$, a
contradiction.
\end{proof}



\begin{remark}\label{rem:cardinal_successors}
 Let $\M$ be an adequate model over $A$ and let $\kappa<\OR(\M)$.
Then $(\kappa^+)^\M$ denotes either the least ordinal-cardinal $\gamma$ of 
$\M$ such that $\gamma>\kappa$, if there is such, and denotes $\OR(\M)$ otherwise.
By \ref{lem:cardinals_equiv}, if $\wl(\M)$ is a limit and $\Theta^\M\leq\kappa$, then 
$(\kappa^+)^\M$
is the least $A$-cardinal $\gamma$ of $\M$ such that $\gamma>\kappa$,
if there is such, or is $\OR(\M)$ otherwise. This applies when $\hmE^\N\neq\emptyset$ 
in \ref{dfn:potential opm} below.
\end{remark}


\begin{remark}
 We now proceed to the definition of \emph{potential operator-premouse}. We first give some 
motivation for some of the 
finer clauses. \emph{Projectum amenability} ensures that we record all essential segments of a 
potential operator-premouse 
$\N$ in its history $\hmS^\N$. For example, suppose we are forming an $n$-maximal iteration tree 
and 
we wish to apply an extender $E$ to some piece of $\N$, but $E$ is not $\N$-total. 
Projectum amenability will ensure that there is some 
$\M\wpins\N$ such that $E$ is $\M$-total and $\M$ projects to $\crit(E)$. 
The property of \emph{$\Sigma_1$-ordinal-generation} is used in making sense of fine structure; it 
ensures for 
example 
that 
the 1st standard parameter $p_1$ is well-defined. The \emph{stratification} of $\N$ lets us 
establish facts regarding the preservation of fine structure (including the preservation of $p_1$, 
assuming $1$-solidity) under degree $0$ ultrapower maps.
It also ensures that $\Hull_{\Sigma_1}^\N(\hmb^\N\un Y)\elem_1\N$ for any $Y\sub\N$. And 
the existence of 
\emph{$\hmb^\N$-ordinal-surjections}, together with stratification, will be used in proving that 
$\Sigma_1$-ordinal-generation is propogated under degree $0$ ultrapower maps.
\end{remark}


\begin{definition}\label{dfn:potential opm}We say that $\N$ is a \emph{potential operator-premouse 
\tu{(}potential opm\tu{)}}
iff $\N$ is an adequate model, over $A$, such that
for every $\M\wins\N$,
\begin{enumerate}
\item ($\hmP$-goodness) If $\hmP^\M\neq\emptyset$ then $\M$ is a successor and 
$\hmP^\M\sub\M\cut\M^-$.\footnote{The requirement that $\hmP^\M\sub\M\cut\M^-$ does not restrict 
the information that can be encoded in $\hmP^\M$, because given any $X\sub\M$, one can 
always replace it with $\{\M^-\}\cross X$.}
\item ($\hmE$-goodness) If $\hmE^\M=\emptyset$ then $\hmmu^\M=\hme^\M=\emptyset$. If 
$\hmE^\M\neq\emptyset$ then 
$\wl(\M)$ is a limit and there is an extender $F$ over $\M$ such that, letting $\hmS=\hmS^\M$ and 
$\hmE=\hmE^\M$ and $\kappa=\kappa^\M$:
\begin{enumerate}[label=--]
\item $\kappa=\crit(F)$,
\item $F$ is $A\times\gamma$-complete for all $\gamma < \kappa$,
\item the premouse axioms \cite[Definition 2.2.1]{wilson2012contributions} hold for 
$(\univ{\M},\hmS,\hmE)$ (so $\hmE$ is the
amenable code for $F$, as in \cite{steel2010outline}),
\item if $F$ is type $2$ then $\hme^\M$ is the trivial completion of the largest non-type $Z$ 
proper segment of $F$; otherwise $\hme^\M=\emptyset$.\footnote{In \cite{FSIT}, 
the (analogue of) $\hme^\M$ is referred to by its 
code $\gamma^\M$. We use $\hme^\M$ instead because this does not depend 
on having (and selecting) a wellorder of $\M$.}
\end{enumerate}
(It follows that $\M$ has a largest cardinal 
$\delta$, and $\delta\leq i_F(\kappa)$, and $\OR(\M)=(\delta^+)^U$ where $U=\Ult(\M,F)$,
and $i_F(\hmS\rest(\kappa^+)^\M)\rest\OR(\M)=\hmS$.)
\item\label{item:successor_potential opm} If $\M$ is a successor then:
\begin{enumerate}
 \item\label{item:no_early_proj} (Projectum amenability) If $\wl(\M)>1$ and 
$\om,\alpha<\rho^{\M^-}$ then
\[ \pow(A^{<\om}\cross\alpha^{<\om})\inter\M\sub\M^-.\]
 \item\label{item:surjections} (A-ordinal-surjections) For every $x\in\M$ there is $\alpha<\OR(\M)$ 
and $f\in\M$ such that
$f:A^{<\om}\cross\alpha^{<\om}\onto x$.
\item\label{item:M=Hull_1^M(OR)} ($\Sigma_1$-ordinal-generation) 
$\M=\Hull_1^\M(\M^-\un\{\M^-\}\un\OR(\M))$.
 \item\label{item:stratification} (Stratification) There is a limit $\gamma\in\Ord$ and sequence 
$\Mtilde=\left<\Mtilde_\alpha\right>_{\alpha<\gamma}$ such that:
\begin{enumerate}
 \item $\Mtilde$ is a continuous, strictly increasing sequence with $\M^-\in\Mtilde_0$ and
$\M=\bigcup_{\alpha<\gamma}\Mtilde_\alpha$,
\item for each $\alpha<\gamma$, $\Mtilde_\alpha$ is an $\Ll_0$-structure such that 
$\univ{\Mtilde_\alpha}$ is transitive and $\Mtilde_\alpha=\M\rest\univ{\Mtilde_\alpha}$;
that is, $\hmb^{\Mtilde_\alpha}=A$ and $\hmp^{\Mtilde_\alpha}=\hmp^\M$ and 
$\hmE^{\Mtilde_\alpha}=\hmE^{\M}\inter\Mtilde_\alpha$, etc,
 \item\label{item:Ntilde_def} $\Mtilde\rest\alpha\in\M$ for every $\alpha<\gamma$, and the function 
$\alpha\mapsto\Mtilde\rest\alpha$, 
with domain $\gamma$, is 
$\Sigma_1^\M(\{\M^-\})$.\qedhere
\end{enumerate}
\end{enumerate}
\end{enumerate}
\end{definition}


\begin{remark}
Let $\N$ be a potential opm over $A$. Suppose $\hmE^\N$ codes an extender $F$. Clearly 
$\kappa=\crit(F)>\Theta^\M>\rank(A)$. By \cite[Definition 
2.2.1]{wilson2012contributions}, we have 
$(\kappa^+)^\M<\OR(\M)$; cf. \ref{rem:cardinal_successors}. Note that
\emph{we allow $F$ to be of superstrong type} (see 
\ref{someNotations}) in accordance with 
\cite{wilson2012contributions}, not \cite[Definition 2.4]{steel2010outline}.\footnote{The main 
point of permitting superstrong 
extenders is that it simplifies 
certain things. But it complicates others. If the reader prefers, one could 
instead require that $F$ \emph{not} be superstrong, but 
various 
statements throughout the paper regarding condensation would need to be modified, along the lines 
of \cite[Lemma 3.3]{FSIT}.}
\end{remark}

\begin{definition}
\label{someNotations}
Let $\M$ be a potential opm over $A$.
We say that $\M$ is \textbf{$\hmE$-active} iff
$\hmE^\M\neq\emptyset$, and \textbf{$\hmP$-active} iff
$\hmP^\M\neq\emptyset$. \textbf{Active} means either
$\hmE$-active or $\hmP$-active. \textbf{$\hmE$-passive} means not
$\hmE$-active. \textbf{$\hmP$-passive} means not $\hmP$-active. \textbf{Passive}
means not active. \textbf{Type 0} means passive. 
\textbf{Type 4} means $\hmP$-active. \textbf{Type 1, 2} or \textbf{3} 
mean $\hmE$-active, with the usual numerology.

We write $\actext^\M$ for the extender $F$ coded by $\hmE^\M$ (where $F=\emptyset$ if 
$\hmE^\M=\emptyset$).
We write $\es^\M$ for the function with domain $\wl(\M)$, sending 
$\alpha\mapsto\actext^{\M\wupto\alpha}$.
Likewise for $\es^\M_+$, but with domain $\wl(\M)+1$.

If $F=F^\M\neq\emptyset$, we say $\M$, or $F$, is \textbf{superstrong} iff 
$i_F(\crit(F))=\nu(F)$. We say that $\M$ is \textbf{super-small} iff $\M$ has no superstrong 
whole segment.
We define $\M^\sq$ as in \cite{fsit}. (Unless $\M$ is type $3$,
we have $\M^\sq=\M$.)

Suppose $\M$ is a successor.
A \emph{stratification} of $\M$ is a sequence $\Mtilde$ witnessing 
\ref{dfn:potential opm}(\ref{item:stratification}) for $\M$. For a $\Sigma_1$ formula 
$\varphi\in\Ll_0$,
we say that $\M$ is \emph{$\varphi$-stratified} iff $\varphi(\M^-,\cdot)^\M$ defines the set of all 
proper restrictions $\Mtilde\rest\alpha$ of a 
stratification $\Mtilde$ of $\M$.\footnote{The $\varphi$-stratification of $\M$ need not imply that 
every successor $\N\wpins\M$ is $\varphi$-stratified.}

The classes of (non-simple) \textbf{$\Ll_0$-Q-formulas} and \textbf{$\Ll_0$-P-formulas} are 
defined analogously to in \cite[\S\S2,3]{FSIT} (but 
with $\Sigma_1$ in place of the $\rSigma_1$ of \cite{FSIT}).
\end{definition}

\begin{lemma}\label{lem:local_hulls}
Let $\M$ be a successor potential opm, over $A$. Let 
$\Mtilde=\left<\Mtilde_\alpha\right>_{\alpha<\gamma}$ be a stratification of $\M$.
For $\alpha<\gamma$ let 
\[ H_\alpha=\Hull_1^{\Mtilde_\alpha}(A^{<\om}\un\OR(\Mtilde_\alpha)). \]
Then for every $x\in\M$ there is $\alpha<\gamma$ such that $x\sub H_\alpha$.
\end{lemma}
\begin{proof} Use $\Sigma_1$-ordinal-generation and 
$A$-ordinal-surjections.
\end{proof}


\begin{definition}
Let $\N$ be a structure for a finite first-order language $\Ll$. We say that $\N$ is 
\emph{pre-fine} iff:
\begin{enumerate}[label=--]
 \item $\Ll$ is a finite and $\{\dot{\in},\hmbdot\}\sub\Ll$, where 
$\dot{\in}$ is a binary relation symbol and $\hmbdot$ is a constant symbol.
 \item $\N$ is an amenable $\Ll$-structure with transitive, rud closed, rank closed universe 
$\univ{\N}$ and $\dot{\in}^\N={\in}\inter\univ{\N}^2$ and $\hmbdot^\N$ is transitive.
 \item $\N=\Hull_{\Sigma_1}^\N(\hmbdot^\N\un\{\hmbdot^\N\}\un\OR(\N))$.\qedhere
\end{enumerate}
\end{definition}



\begin{definition}[Fine structure]
Let $\N$ be pre-fine for the language $\Ll$. We sketch a description of the \emph{fine structural 
notions} 
for $\M=(\N,\Ll)$. For details refer to \cite{fsit} and/or \cite{outline}. Let $A=\hmb^\N$.

We say that $\M$ is \emph{$0$-sound} and let $\rho_0^\M=\OR(\N)$ and 
$p_0^\M=\emptyset$ and $\core_0(\M)=\N$ and
$\rSigma_{1}^{\M}=\Sigma_1^{\core_0(\M)}$. (Here and in what follows, definability is with respect 
to $\Ll$.) 

Now let $n<\om$ and suppose that $\M=(\N,\Ll)$ is $n$-sound (which will imply that 
$\N=\core_n(\M)$) and that $\om<\rho_n^{\M}$.
We write $\pvec_n^\M=(p_1^\M,\ldots,p_n^\M)$.
Then $\rho=\rho_{n+1}^\M$ is the least ordinal $\rho\geq\om$ such that for some 
$X\sub A^{<\om}\cross\rho^{<\om}$, $X$ is $\bfrSigma_{n+1}^\M$ but $X\notin\univ{\N}$.
And $p_{n+1}^\M$ is the least tuple $p\in\Ord^{<\om}$ such that some such $X$ is 
\[ \rSigma_{n+1}^\M(A\un\rho\un\{p,\pvec^\M_n\}).\]
Here $p_{n+1}^\M$ is well-defined 
by $\Sigma_1$-ordinal-generation. 
For any $X\sub\N$, let
\[ \Hull_{n+1}^\M(X)=\Hull_{\rSigma_{n+1}}^\N(X),\]
and $\cHull_{n+1}^\M(X)$ be 
its transitive collapse.
Then we let
\[ \C=\core_{n+1}(\M)=\cHull_{n+1}^\M(A\un\rho_{n+1}^\M\un\pvec_{n+1}^\M), \]
and the uncollapse map $\pi:\C\to\N$ is the associated \emph{core embedding}.
Define $(n+1)$-\emph{solidity} and $(n+1)$-\emph{universality} for $\M$ as usual (putting the 
parameters in $A$ into every relevant hull).
We say that $\M$ is $(n+1)$-\emph{sound} iff $\M$ is $(n+1)$-solid and $\C=\N$ and $\pi=\id$.

Now suppose that $\M$ is $(n+1)$-sound and $\rho_{n+1}^\M>\om$ (so $\rho_{n+1}^\M>\rank(A)$). 
Define $T=T_{n+1}^\M\sub\core_{n+1}(\M)=\N$ by letting $t\in T$ iff 
for some $q\in\N$ and $\alpha<\rho_{n+1}^\M$,
\[ t=\Th_{\rSigma_{n+1}}^\N(A\un\alpha\un\{q\}). \]
(This denotes the \emph{pure} $\rSigma_{n+1}$ theory, as opposed to the \emph{generalized} 
$\rSigma_{n+1}$ theory of \cite{fsit}.\footnote{As in \cite[\S2]{fsit}, it does not matter which we 
use.}) Define $\rSigma_{n+2}^\M$ from $T$ as 
usual.
\end{definition}

\begin{definition}
 Let $\N$ be a potential opm.
If $\N$ is active type 3 
then $\core_0(\N)$ denotes $\N^\sq$, and otherwise denotes $\N$.
We define the \textbf{fine structural notions} for $\N$ ($n$-soundness,
 $\rho_{n+1}^{\N}$, $\Hull^\N_{n+1}$, etc) as those for 
$\M=(\core_0(\N),\Ll_0)$.
\end{definition}



\begin{remark}
In the proof of the solidity, etc, of iterable opms, one must also deal with 
structures which are almost active opms, except that they may fail the ISC.
The details are immediate modifications of the standard notions, so we leave them to the reader.
\end{remark}

\begin{definition}
Let $\N$ be an $\om$-sound potential opm. We say that $\N$ is \emph{condensing} 
iff for every $k<\om$, for every $(k+1)$-sound potential opm $\M$ which is soundly projecting, 
for every near $k$-embedding 
$\pi:\M\to\N$ such that $\rho=\rho_{k+1}^\M\leq\crit(\pi)$ and 
$\rho<\rho_{k+1}^\N$, we have the following. If $\M\wupto\rho$ is $\hmE$-passive let $\Q=\M$,
and otherwise let $\Q=\Ult(\M\wupto\rho,F^{\M\wupto\rho})$. Then either:
\begin{enumerate}[label=--]
\item $\M\wpins\Q$, or
\item $\M^-\wpins\Q$, and $\M\in\R$ where $\R\wpins\Q$ is such 
that $\R^-=\M^-$.\qedhere
\end{enumerate}
\end{definition}

Note that if we have $\M\in\R$ as above, then $\rho_\om^\M=\rho_\om^{\M^-}$.

\begin{definition}
 A \emph{Q-operator-premouse \tu{(}Q-opm\tu{)}}\footnote{\emph{Q} is for \emph{Q-formula}. We will 
see that the first-order aspects 
of Q-opm-hood are expressible with Q-formulas and P-formulas.} is a potential operator-premouse 
$\M$ such that every $\N\wpins\M$ is $\om$-sound and condensing.
\end{definition}

In \cite{fsit}, premice are not required to have condensing proper segments. We 
make this demand here so that we can avoid stating it as an explicit axiom at certain points later 
(and it holds for the structures we care about).

\begin{lemma}\label{lem:Q-opm_type_Q-formulas} There are $\Ll_0$-Q-formulas 
$\varphi_1,\varphi_2$,
a $\Ll_0$-P-formula $\varphi_3$, an $\Ll_0$-simple-Q-formula $\varphi_{0,\mathrm{limit}}$, 
and for each $\Sigma_1$ formula $\psi\in\Ll_0$ there are $\Ll_0$-simple-Q-formulas 
$\varphi_{0,\psi},\varphi_{4,\psi}$ such that for any adequate model $\N$:
\begin{enumerate}
\item\label{item:passive_limit} $\N\sats\varphi_{\mathrm{0,limit}}$ iff $\N$ is a passive 
Q-opm of limit length.
\item\label{item:B-active} $\N\sats\varphi_{4,\psi}$ iff $\N$ is a $\psi$-stratified $\hmP$-active 
Q-opm.
\item\label{item:passive} $\N\sats\varphi_{0,\psi}$ iff $\N$ is a passive Q-opm and 
either
$\wl(\N)$ is a limit or $\N$ is $\psi$-stratified.
 \item\label{item:active_1,2} $\N\sats\varphi_1$ 
\tu{(}respectively, $\N\sats\varphi_2$\tu{)} iff $\N$ is a type 1 \tu{(}respectively, type 2\tu{)} 
Q-opm.
 \item\label{item:active_3} If $\N=\M^\sq$ for 
a type 3 Q-opm $\M$ then $\N\sats\varphi_3$, and if $\N\sats\varphi_3$ then $\hmE^\N$ 
codes an 
extender 
$F$ over $\N$ and if $\Ult(\N,F)$ is wellfounded then 
$\N=\M^\sq$ for a type 3 Q-opm.
\end{enumerate}
\end{lemma}
\begin{proof}
Part \ref{item:passive_limit} is routine and parts \ref{item:active_1,2}, 
\ref{item:active_3} are straightforward adaptations of their analogues
\cite[Lemma 2.5]{fsit}, \cite[Lemma 3.3]{fsit} respectively, with the added point that we can 
drop the clause ``or $\N$ is of superstrong type'' of \cite[Lemma 
3.3]{fsit}, because we allow extenders of superstrong type.
Part \ref{item:B-active} is an easy adaptation of part \ref{item:passive}, using the fact that if 
$\N$ is $\P$-active then $\P^\N\sub\N\cut\N^-$.
So we just sketch the proof of part \ref{item:passive}.

We leave it to the reader to verify that here is an $\Ll_0$-simple-Q-formula (in fact in $\Ll_0^-$) 
asserting 
that every $\M\wpins\N$ is an $\om$-sound potential opm satisfying internal condensation, and an 
$\Ll_0$-simple-Q-formula asserting 
that 
$\hmP^\N=\hmE^\N=\hmmu^\N=\hme^\N=\emptyset$.
It remains to see that we can assert that \ref{dfn:potential opm}(\ref{item:successor_potential 
opm}) holds for $\M=\N$
(the assertion will include the possibility that $\wl(\N)$ is a limit). For 
\ref{dfn:potential opm}(\ref{item:no_early_proj}), use the formula
``$\all x\ex y[x\sub y\&\varphi(y)]$'',
where $\varphi(y)$ asserts ``either there is $s\in \hmS^\M$ such that $y\in s$ or there are 
$\hmS,A$ 
such that $\hmS=y\inter \hmS^\M$ and $A=\hmb^\M$ and $\hmS$ has a largest element $\P$ and 
for each $\tau<\OR(\P)$, if there is $X\in y\cut\P$ such that $X\sub 
A^{<\om}\cross\tau^{<\om}$, then there is $n<\om$ such that 
$\rho_{n+1}^\P\leq\tau$, as witnessed by a satisfaction relation in 
$y$'' (use the fact that $\N$ is rud closed).

Clause \ref{dfn:potential opm}(\ref{item:surjections}) is easy, and it is fairly straightforward to 
assert that either $\wl(\N)$ is a limit or $\N$ is $\psi$-stratified, identifying candidates for 
$\N^-$ as in the previous paragraph.
We can therefore assert \ref{dfn:potential opm}(\ref{item:M=Hull_1^M(OR)}) as ``$\all x\ex y[x\sub 
y$ 
and there is $\alpha<\gamma$ such that $y\sub H_\alpha$'', where 
$\gamma,H_\alpha$ are defined as in \ref{lem:local_hulls}, using the stratification given by $\psi$.
\end{proof}

One can also prove the above lemma with every instance of \emph{Q-opm} replaced by \emph{potential 
opm}, 
but we 
don't need this observation.

\begin{lemma}\label{lem:Qformula_pres}
The natural adaptations of \tu{\cite[Lemmas 2.4, 3.2]{FSIT}} 
hold.
\end{lemma}

In fact, we can also give a version of those lemmas for weak $0$-embeddings.


\begin{definition}\label{weak0}
Let $\N$ be an adequate model with $\hmE^\N\neq\emptyset$. If $\hmE^\N$ is a set of 
partial extenders over $\N$, all with the same critical point $\mu$, then let $\mu(\hmE^\N)=\mu$.

Let $\M$ be a Q-opm. Let $\R$ be an $\Ll_0$-structure (possibly illfounded). If $\M$ is 
type 3 then let $\pi:\R\to\M^\sq$, and otherwise let $\pi:\R\to\M$.

We say that $\pi$ is an \textbf{weak $0$-embedding} iff $\pi$ is 
$\Sigma_0$-elementary (therefore $\R$ is extensional and wellfounded, so assume $\R$ is 
transitive) and there is $X\sub\R$ such that $X$ is $\in$-cofinal in $\R$ and
$\pi$ is $\Sigma_1$-elementary on elements of $X$, and if $\M$ is type 1 or 2, then letting 
$\mu=\hmmu^\R$,
there is $Y\sub\R\wupto{(\mu^+)^\R}\cross\R$ such that $Y$ is $\in\cross\in$-cofinal in 
$\R\wupto{(\mu^+)^\R}\cross\R$ and $\pi$ is $\Sigma_1$-elementary on 
elements of $Y$.
\end{definition}

\begin{lemma}\label{lem:Qformula_pres_weak0}
Let $\M$ be a Q-opm and let $\pi:\R\to\M$, unless $\M$ is type $3$, in which case let 
$\pi:\R\to\M^\sq$. Suppose that $\pi$ is a weak $0$-embedding.

For any $\Ll_0$-Q-formula $\varphi$, if $\M\sats\varphi$ then $\R\sats\varphi$.
If $\M$ is a type $i$ Q-opm, $i\neq 3$, then $\R$ is also a type $i$ Q-opm.
\footnote{Note though that if $\R,\M$ are passive, then possibly $\M$ is a successor length but
$\R$ a limit.}

Suppose $\M$ is type 3. For any $\Ll_0$-P-formula $\varphi$,
if $\M^\sq\sats\varphi$ then $\R\sats\varphi$.
If $\Ult(\M,F^\M)$ is wellfounded then 
$\R=\N^\sq$ for some type 3 Q-opm $\N$.
\end{lemma}
The proof is routine, so we omit it.

\begin{definition}\label{dfn:k-embedding}
For $k\leq\om$, a \textbf{(near) $k$-embedding} $\pi:\M\to\N$ between $k$-sound Q-opms 
is defined analogously to 
\cite{outline}, and a \textbf{weak $k$-embedding} is analogous to 
\cite[***where?]{copy_con}.\footnote{Note that 
this definition of \emph{weak $k$-embedding} diverges slightly from the definitions given in 
\cite{fsit} and \cite{outline}.} Recall that when $k=\om$, each of these notions are equivalent 
with full elementarity.
(According to the standard convention, if $\M,\N$ are type 3 then
literally $\dom(\pi)=\univ{\M^\sq}$ and $\codom(\pi)=\univ{\N^\sq}$ and the elementarity of $\pi$ 
is 
with respect to $\M^\sq,\N^\sq$.)

We say that $\pi:\M\to\N$ is \textbf{(weakly, nearly) $k$-good} iff $\pi$ is a (weak, near) 
$k$-embedding and $\hmb^\M=\hmb^\N$ and $\pi\rest \hmb^\M=\id$.
\end{definition}
\begin{lemma}
 Let $\M$ be an $n$-sound Q-opm over $A$ with $\om<\rho_n^\M$. Let $X\sub\core_0(\M)$, let
\[ \N=\cHull_{n+1}^\M(A\un X\un\pvec_n^\M) \]
and let $\pi:\N\to\M$ be the uncollapse. Then $\pi$ is nearly $n$-good.
\end{lemma}
\begin{proof}
 Suppose $n=0$; so we just need to see that $\pi$ is $\rSigma_1$-elementary.
 Let $x\in\N$, let $\varphi$ be $\rSigma_0$ and suppose that $\M\sats\ex y\varphi(y,\pi(x))$.
 We want to see that there is some $y\in\rg(\pi)$ such that $\M\sats\varphi(y,\pi(x))$.

Note that $\xi\in\rg(\pi)$, where $\xi$ is least such that $\pi(x)\in\M\wupto(\xi+1)$ and there is 
$y\in\M\wupto(\xi+1)$ such that $\M\sats\varphi(y,\pi(x))$.
Suppose $\xi+1<\lh(\M)$. Let 
$\avec\in A^{<\om}$ be such that there is $\betavec\in(\xi+1)^{<\om}$ such that 
$\M\sats\varphi(y,\pi(x))$ where $y=h^\M_{\xi+1}(\avec,\betavec)$. Taking 
$\betavec$ least such, then $\betavec\in\rg(\pi)$, so $y\in\rg(\pi)$, as required. Now suppose 
instead that $\xi+1=\lh(\M)$. Let $\left<H_\alpha\right>_{\alpha<\gamma}$ be as in 
\ref{lem:local_hulls}, with respect to some stratification $\Mtilde$ of $\M$. Then 
$\alpha\in\rg(\pi)$, where 
$\alpha$ is least such that $\pi(x)\in H_\alpha$ and
there is $y\in H_\alpha$ such that $\M\sats\varphi(y,\pi(x))$ (use here that for each 
$\beta<\gamma$, $\Mtilde_\beta\elem_0\M$).
So as before, there is some such $y\in\rg(\pi)$.

If $n>0$, then the proof for standard premice adapts routinely, using the fact that 
$A\sub\rg(\pi)$ as above.\footnote{The fine structural setup here is a little different 
from that in \cite{fsit}, as we have dropped the use of $u_i^\M$. See \cite{local_prikry} 
for calculations which deal with this difference.}\end{proof}

Using stratifications and standard calculations, we also have:

\begin{lemma}\label{lem:core_embedding}
Let $\pi:\N\to\M$ be nearly $n$-good, and $A=\hmb^\N$. Suppose that $\N\notin\M$ and
$\N=\Hull_{n+1}^\N(A\un\rho\un\{q\})$, where $\rho\in\Ord$ and $\rho\leq\crit(\pi)$.
Then $\pi$ is $n$-good.

If $\N=\core_{n+1}(\M)$ and $\pi$ is the core embedding, then $\pi$ is $n$-good.
\end{lemma}

\begin{definition}
 An \emph{operator-premouse \tu{(}opm\tu{)}} is a soundly projecting Q-opm. For an opm $\M$, 
let $q^\M=p_1^\M\inter(\OR(\M^-),\OR(\M))$
(so if $\M$ is a limit then $q^\M=\emptyset$).
\end{definition}
\begin{definition}
 Let $\M$ be a $k$-sound opm over $A$ and $q\in(\rho_k^\M)^{<\om}$. We say that $\M$ is 
\emph{$(k+1,q)$-solid}
 iff for each $\alpha\in q$, letting $q'=q\cut(\alpha+1)$ and $X=A\un\alpha\un q'\un\pvec_k^\M$, we 
have
$\Th_{\rSigma_{k+1}}^\M(X)\in\M$.
\end{definition}
\begin{lemma}\label{lem:succ_opm_top_param} Let $\M$ be a successor opm and $\wl(\M)=\xi+1$. Let 
$\rho=\rho_\om^{\M^-}$ and $p=p_1^\M\cut\rho$. Then $\M$ is $\rho$-sound and 
$\rho_1^\M\leq\rho$ and either $p\sub\xi+1$ or $p=q^\M$.
Therefore either $\M$ is $\om$-sound and 
$\rho_\om^\M=\rho_\om^{\M^-}$,
or there is $k<\om$ such that $\M$ is $k$-sound and $\rho_{k+1}^\M<\rho_\om^{\M^-}\leq\rho_k^\M$.
\end{lemma}
\begin{proof} If 
$q^\M\neq\emptyset$ then $p\inter[\rho,\OR(\M^-)]=\emptyset$, 
as letting $A=\hmb^\M$,
\[ \M^-\un\{\M^-\}\sub\Hull_1^\M(A\un\rho\un p) \]
as $\hmX^\M$ is 
$\Sigma_1^\M$, and
this suffices since $\M$ is soundly projecting. So suppose $q^\M=\emptyset$.
Then $p$ is the least $r\in(\xi+1)^{<\om}$ such that 
\[ \M^-\in H=\Hull_1^\M(A\un\rho\un r).\]
Moreover, $\M$ is $(1,p)$-solid. For $\M=H$
by sound-projection and since $q^\M=\emptyset$. Therefore 
$p\leq r$. But letting $\alpha\in r$ and 
$r'=r\cut(\alpha+1)$ and
\[ H' = \Hull_1^\M(A\un\alpha\un r'), \]
we have $\M^-\notin H'$, so $H'\sub\M^-$, because $\hmX^\M$ is $\Sigma_1^\M$.
This suffices.\end{proof}





\begin{lemma}\label{lem:Sigma_1_hull_reflects_opm}
 Let $\N$ be a successor operator-premouse and let $\pi:\M\to\N$. Suppose that either
\tu{(}i\tu{)} $\pi$ is $\Sigma_1$-elementary and 
$q^\N=\emptyset$, or \tu{(}ii\tu{)} $\pi$ is $\Sigma_2$-elementary and 
$q^\N\in\rg(\pi)$.
Then $\M$ is an operator-premouse of the same type as $\N$, and $\pi(q^\M)=q^\N$.
\end{lemma}
\begin{proof}
By \ref{lem:Q-opm_type_Q-formulas}, $\M$ is a Q-opm and we may assume that 
that $\N^-\in\rg(\pi)$, so $\M$ is a successor and $\pi(\M^-)=\N^-$, and $\M$ is $\psi$-stratified 
where $\N$ is $\psi$-stratified. In part (i) the 
$\psi$-stratification gives $\M=\Hull_1^\M(\M^-\un\{\M^-\})$. In part (ii) use 
generalized solidity witnesses.
\end{proof}

However, if $\pi$ is just $\Sigma_1$-elementary and $p_1^\N\neq\emptyset$,
$\M$ might not be soundly projecting, even if $p_1^\N\in\rg(\pi)$. Such embeddings arise 
when we take $\Sigma_1$ hulls, like in the proof of $1$-solidity.

Let $X$ be transitive. Then $X^\#$
determines naturally an opm $\M$ over $\hat{X}$ of length $1$, so $U=\Ult_0(\M,F^{X^\#})$ is also a 
Q-opm over $\hat{X}$ of length $1$, but $U$ is not an opm. However, given a successor opm $\N$, 
we will only form ultrapowers of $\N$ with extenders $E$ such that $\crit(E)<\OR(\N^-)$, 
and 
under these circumstances, opm-hood is preserved. In fact, we will only form ultrapowers and 
fine structural hulls under further fine structural assumptions:

\begin{definition}
Let $k\leq\om$. An opm $\M$ is $k$-\emph{relevant} iff
$\M$ is $k$-sound, and either $\M$ is a limit or $k=\om$ or 
$\rho_{k+1}^\M<\rho_\om^{\M^-}$.

A Q-opm $\M$ which is not an opm (so $\M$ is a successor) is \emph{$k$-relevant} iff $k=0$ and 
$\rho_1^\M<\rho_\om^{\M^-}$.
\end{definition}

For the development of the basic fine structure theory of opms, one only need consider 
$k$-stack-maximal iteration trees on $k$-relevant 
opms (and on phalanxes of such structures, and on bicephali and pseudo-premice); see 
\ref{dfn:iteration_trees}. For instance, the following lemma follows from 
\ref{lem:succ_opm_top_param}:

\begin{lemma}\label{lem:non_k-rpm_sound}
Let $k<\om$ and $\M$ be a $k$-sound operator-premouse which is not $k$-relevant. Then $\M$ is 
$(k+1)$-sound.
\end{lemma}








In the following lemma we establish the preservation of fine structure under degree $k$ 
ultrapowers, for $k$-relevant opms.
The proof involves a key use of stratification.

\begin{lemma}\label{lem:Ult_k_pres_fs}
 Let $\M$ be a $k$-relevant opm and $E$ an extender over $\M$, weakly amenable to 
$\M$, 
with 
$\crit(E)<\rho_k^\M$, and $\crit(E)<\rho_\om^{\M^-}$ if $\M$ is a successor. Let $\N=\Ult_k(\M,E)$ 
and $j=i^\M_{E,k}$ be the ultrapower embedding.
Suppose $\N$ is wellfounded.
 Then:
 \begin{enumerate}
  \item\label{item:pres_relevant_opm_type} $\N$ is a $k$-relevant opm of the same type as 
$\M$.
  \item\label{item:ult_pres_psi-strat} $\N$ is a successor iff $\M$ is. If 
$\M$ is a successor then $j(\wl(\M))=\wl(\N)$ and if $\M$ 
is $\psi$-stratified then $\N$ is $\psi$-stratified.
  \item\label{item:i_E_k-embedding} $j$ is $k$-good.
  \item\label{item:pres_solidity} For any $q\in(\rho_k^\M)^{<\om}$, if $\M$ is $(k+1,q)$-solid 
then 
$\N$ is 
$(k+1,j(q))$-solid.
\item\label{item:half_sup_pres_rho} $\rho_{k+1}^\N\leq\sup 
j``\rho_{k+1}^\M$.
  \item\label{item:E_close_sup_pres_rho} If $E$ is close to $\M$ and $\M$ is $(k+1)$-solid then 
$\rho_{k+1}^\N=\sup j``\rho_{k+1}^\M$ and $p_{k+1}^\N=j(p_{k+1}^\M)$ and $\N$ is 
$(k+1)$-solid.
\end{enumerate}
\end{lemma}
\begin{proof}
The fact that $\N$ is a Q-opm of the same type as $\M$ is by \ref{lem:Q-opm_type_Q-formulas}. 
Part \ref{item:i_E_k-embedding} is standard and part 
\ref{item:ult_pres_psi-strat} follows easily. We now verify that $\N$ is soundly projecting; we may 
assume that 
$\M,\N$ are successors. If $k>0$, use elementarity and stratification. Suppose $k=0$. Let 
$\rho=\rho_\om^{\M^-}$ and $q=j(q^\M)$. The fact that $\N$ is $(1,q)$-solid follows by 
an easy adaptation of the usual proof of preservation of the standard parameter, using 
stratification (where in 
the usual proof, one uses the natural stratification of the $\J$-hierarchy).
So it suffices to see that 
$\N=\Hull_1^\N(\N^-\un\{\N^-,q\})$.
But this holds because $\M$ is an opm and
\[ \N=\Hull_1^\N(\rg(j)\un\nu_E) \]
and $\nu_E\sub\N^-$, the latter because $\crit(E)\leq\OR(\N^-)$ (in fact, 
$\crit(E)<\rho_\om^{\N^-}$).



Parts \ref{item:pres_solidity}--\ref{item:E_close_sup_pres_rho}: If $k>0$ the proof for standard 
premice works (see, for example, \cite[Lemmas 4.5, 4.6]{fsit}, and if
$\kappa<\rho_{k+1}^\M$, see the calculations in \cite[Claim 5 of Theorem 6.2]{fsit} and
\cite[***p,rho-pres]{fs_from_normal}.
If $k=0$, again use stratification to adapt the usual proof. (In the case that 
$\wl(\M)$ is a limit, $\M$ is of course ``stratified'' by its proper whole segments.)

By part \ref{item:half_sup_pres_rho}, it follows that $\N$ is $k$-relevant, completing part 
\ref{item:pres_relevant_opm_type}.
\end{proof}

\begin{definition}\label{dfn:iteration_trees}
\textbf{Iteration trees} on opms $\M$ are as for standard premice, except that
for all $\alpha+1\leq\lh(\Tt)$,
$M^\Tt_\alpha$ is an opm, and if $\alpha+1<\lh(\Tt)$ then 
$E^\Tt_\alpha\in\es_+(\M^\Tt_\alpha)$.
\textbf{Putative iteration trees} $\Tt$ are likewise, except that if $\Tt$ has successor length 
then no demand is made on the nature of $M^\Tt_\infty$; in particular, it might be illfounded.

Let $k<\om$ and let $\M$ be a $k$-sound opm. The iteration 
game 
$\G^{\M}(k,\theta)$ is defined completely analogously to the game $\G_k(\M,\theta)$ of 
\cite[\S3.1]{steel2010outline}, forming a (putative) iteration tree as above, except for the 
following difference: Let $\Tt$ be the putative tree being produced. For $\beta+1<\alpha+1$, we 
replace the requirement (on player $\plI$) that 
$\lh(E^\Tt_\beta)<\lh(E^\Tt_\alpha)$ with the requirement that 
$\lh(E^\Tt_\beta)\leq\lh(E^\Tt_\alpha)$. The rest is like in \cite{outline}.

A (putative) iteration tree on $\M$ is \textbf{$k$-maximal} iff it is a partial play 
of $\G^{\M}(k,\infty)$. A \textbf{$(k,\theta)$-iteration strategy} for $\M$ is 
a winning strategy for player $\plII$ in $\G^{\M}(k,\theta)$.

The iteration game 
$\G^{\M}(k,\alpha,\theta)$ is defined by analogy with the game $\G_k(\M,\alpha,\theta)$ 
of \cite[\S4.1]{outline}, except that each round consists of a run of 
$\G^{\Q}(q,\theta)$ for some $\Q,q$.\footnote{Recall that for $\gamma<\alpha$,
after the first $\gamma$ rounds have been played, both players having met their commitments so far,
we have a $\gamma$-sequence $\Ttvec$ of iteration trees, with wellfounded final model 
$M^{\Ttvec}_\infty$ (formed by direct limit if $\gamma$ is a limit); it follows that this 
model is an $n$-sound operator-premouse where $n=\deg^{\Ttvec}(\infty)$. At the beginning of 
round $\gamma$, player $\plI$ chooses some 
$(\Q,q)\wins(\M^{\Ttvec}_\infty,n)$, and round $\gamma$ is a run of 
$\G^{\Q}(q,\theta)$. If round $\gamma$ is won by player $\plII$ and 
the run produces a tree of length $\theta$, then the run of 
$\G^\M(k,\alpha,\theta)$ is won by player $\plII$.} The 
iteration game $\G=\G^{\M}_{\max}(k,\alpha,\theta)$ is 
defined likewise, except that we do not allow player $\plI$ to drop in model or degree at the 
beginnings of rounds. That is, (i) round $0$ of $\G$ is a run of $\G^{\M}(k,\theta)$, 
and (ii) letting $0<\gamma<\alpha$ and $\Ttvec=\left<\Tt_\beta\right>_{\beta<\gamma}$ be the 
sequence of trees played in rounds $<\gamma$ and $\N=M^{\Ttvec}_\infty$ and 
$n=\deg^{\Ttvec}(\infty)$, round $\gamma$ of $\G$ is a run of 
$\G^{\N}(n,\theta)$.

A (putative) iteration tree is \textbf{$k$-stack-maximal} iff it is a partial play of 
$\G^\M_{\max}(k,\infty,\infty)$.
A \textbf{$(k,\alpha,\theta)$-maximal iteration strategy} for $\M$ is a winning strategy 
for player $\plII$ in $\G^{\M}_{\max}(k,\alpha,\theta)$, and a
\textbf{$(k,\alpha,\theta)$-iteration strategy} is likewise for 
$\G^{\M}(k,\alpha,\theta)$.

Now \textbf{$(k,\theta)$-iterability}, \textbf{$(k,\alpha,\theta)$-maximal iterability}, etc, are 
defined by the existence of the appropriate winning 
strategy.
\end{definition}

\begin{remark}
The requirement, in $\G^{\M}(k,\theta)$, that $\lh(E^\Tt_\beta)\leq\lh(E^\Tt_\alpha)$ for 
$\beta<\alpha$, is weaker than requiring that $\lh(E^\Tt_\beta)<\lh(E^\Tt_\alpha)$, 
because opms may have superstrong extenders. For example, we might have that 
$E^\Tt_0$ is type 2 and $E^\Tt_1$ is 
superstrong with $\crit(E^\Tt_1)$ the largest cardinal of $\M^\Tt_0\wupto\lh(E^\Tt_0)$, in which 
case 
$\M^\Tt_2$ is active but $\OR(\M^\Tt_2)=\lh(E^\Tt_1)$, and therefore we might have 
$\lh(E^\Tt_2)=\lh(E^\Tt_1)$.

The preceding example is essentially general. It is easy to show that if $\Tt$ is 
$k$-maximal and $\alpha+1\leq\beta<\lh(\Tt)$ then either 
$\lh(E^\Tt_\alpha)<\OR(M^\Tt_\beta)$ and $\lh(E^\Tt_\alpha)$ 
is a cardinal of $M^\Tt_\beta$, or $\beta=\alpha+1$ and 
$\lh(E^\Tt_\alpha)=\OR(M^\Tt_{\alpha+1})$ and $E^\Tt_\alpha$ is 
superstrong and $M^\Tt_{\alpha+1}$ is type 2. Therefore if $\alpha+1<\beta+1<\lh(\Tt)$ then 
$\nu(E^\Tt_\alpha)<\nu(E^\Tt_\beta)$, and if $\alpha+1\leq\beta<\lh(\Tt)$ then 
$E^\Tt_\alpha\rest\nu(E^\Tt_\alpha)$ is not an initial segment of any extender on 
$\es_+(M^\Tt_\beta)$.

The comparison algorithm needs to be modified slightly. Suppose we are comparing models $\M,\N$, 
via padded $k$-maximal trees $\Tt,\Uu$, respectively, and we have produced $\Tt\rest\alpha+1$ 
and $\Uu\rest\alpha+1$. Let $\gamma$ be least such that 
$\M^\Tt_\alpha\wupto\gamma\neq\M^\Uu_\alpha\wupto\gamma$. 
If only one of these models is active, then we use that active extender next. Suppose both are 
active. If one active extender is type 3 and one is type 2, then we use only the type 3 extender 
next. Otherwise we use both extenders next. With this modification, and with the remarks in the 
preceding paragraph, the usual proof that comparison succeeds goes through.
\end{remark}

\begin{lemma}\label{lem:k-stack-max_pres_rpm}
Let $\M$ be a $k$-relevant opm and $\Tt$ a successor length $k$-stack-maximal 
tree on $\M$. Then $M^\Tt_\infty$ is a $\deg^\Tt(\infty)$-relevant 
opm.
\end{lemma}
\begin{proof}
Given the result for $k$-maximal trees $\Tt$, the generalization to $k$-stack-maximal is routine. 
But for $k$-maximal $\Tt$, the result follows from
\ref{lem:Ult_k_pres_fs}, by a straightforward induction on $\lh(\Tt)$.
\end{proof}

In \ref{lem:k-stack-max_pres_rpm}, it is important that $\Tt$ is $k$-stack-maximal;
the lemma can fail for trees produced by $\G^\M(k,\alpha,\theta)$.

\begin{definition} We say that $X$ is \textbf{explicitly swo'd (self-wellordered)} iff
$X=x\un\{x,<\}$ for some transitive set $x$, and wellorder $<$ of $x$. In this 
situation, $<_X$ denotes the wellorder of $X$ extending $<$, and with 
last two elements $x,<$. Clearly there are uniform methods of passing from an explicitly 
swo'd $X$ to a wellorder of $A={\hat{X}}$. Fix such a method, and for such $X,A$, let $<_A$ denote 
the resulting wellorder of $A$.
\end{definition}
\begin{definition}
 Let $\M$ be a Q-opm over some $A=\hat{X}$, where $X$ is swo'd. Let $\psi$ be an 
$\rSigma_1$ formula,
and suppose that every successor $\N\wins\M$ is $\psi$-stratified. We define the 
wellorder $<^\M_\psi$ of $\M$ by induction on $\wl(\M)$ as follows. Let $<^\M_\psi$ end-extend both 
$<_A$ and $<^\N_\psi$ for all $\N\wpins\M$. Suppose that $\M$ is a successor.
Let $\left<H_\alpha\right>_{\alpha<\gamma}$ be as in \ref{lem:local_hulls}. 
Using the definition of $H_\alpha$, let $\left<<_\alpha\right>_{\alpha<\gamma}$ be the natural 
increasing, continuous sequence of wellorders $<_\alpha$ of $H_\alpha$, end-extending 
$<^{\M^-}_\psi$ (or end-extending $<_A$ if $\xi=0$). Let
\[ <^\M_\psi=\bigcup_{\alpha<\gamma}<_\alpha. \]

Clearly $<_\psi^\M$ is $\Sigma_1^\M$, uniformly over all $\M$ as above.

When there is a natural choice of $\psi$ as above, let $<^\M=<^\M_\psi$.
For example, in \S\ref{StrategyPremice}, we will define strategy-premice $\M$, for which, if $\M$ 
is a successor, then the universe of $\M$ is just $\J_\lambda(\M^-)$, for some ordinal $\lambda$.
In this case, we can take our stratification $\Mtilde$ of $\M$ to be
\[ \Mtilde_\alpha=(\Ss_\alpha(\M^-),\emptyset,\Ss_\alpha(\M^-)\inter 
\hmP^\M,\ldots)\]
(Jensen's $\Ss$-hierarchy), and take $\psi$ to be 
the natural formula yielding $\Mtilde$.
\end{definition}

\section{$\Fop$-mice for operators $\Fop$}


\label{sec:operators}
We will be interested in opms $\M$ in which the successor steps are taken by some 
\emph{operator} 
$\Fop$; that is, in which $\N=\Fop(\N^-)$ for each successor $\N\wins\M$.
We call such an $\M$ an \emph{$\Fop$-opremouse}. As in 
\cite{cmi}, there are two main classes of operators we have in mind: 
\emph{mouse operators} and (iteration) \emph{strategy operators}. We will now give some 
abstract framework for this, and will discuss the specific types of operators 
in detail later.

\begin{definition}
We say that a set or class $\opbk$ is an \textbf{operator background} iff (i) $\opbk$ is 
transitive, rudimentarily closed and $\om\in\opbk$, (ii) for all $x\in\opbk$ and all $y,f$, if 
$f\maps x^{<\om}\to\trancl(y)$ is a surjection then $y\in\opbk$, and (iii) $\opbk\sats\DC$. (So 
$\OR(\opbk)=\rank(\opbk)$ is a cardinal; if $\om<\kappa\leq\Ord$ then $\her_\kappa$ is an operator 
background, and under $\ZFC$ these are the only operator backgrounds.) By 
(iii), every element of $\opbk$ has a countable elementary substructure.

Let $\opbk$ be an operator background. A set $C$ is a \textbf{cone of
$\opbk$} iff there is $a\in\opbk$ such that $C$ is the set of all 
$x\in\opbk$ such that $a\in\J_1(\hat{x})$. 
With $a,C$ as such, we say $C$ is \textbf{the cone above $a$}. If $b\in\J_1(a)$ 
we say $C$ is \textbf{above $b$}. A set $D$ 
is a \textbf{swo'd cone of $\opbk$} 
iff $D=C\inter S$, for some cone $C$ of $\opbk$, and where $S$ is the 
class of explicitly swo'd sets. Here $D$ is 
\textbf{(the swo'd cone) above $a$} iff $C$ is 
(the cone) above $a$. A \textbf{cone} is a 
cone of $\opbk$ for some operator background $\opbk$. Likewise for \textbf{swo'd cone}.
\end{definition}

\begin{definition}
An \emph{operatic argument} is a set $X$ such that either $X=\hat{Y}$ for some transitive $Y$,
or $X$ is an $\om$-sound opm. 
Given $C\sub\opbk$, let
\[ \witri{C}=\{\hat{Y}\st Y\in C\ \&\ Y\text{ is transitive}\}. \]
An \emph{operator domain over $\opbk$} is a set $D=\witri{C}\un P\sub\opbk$,
where $C$ is a possibly swo'd cone of $\opbk$, and $P$ is some class of $\om$-sound condensing 
opms, each over 
some $A\in \witri{C}$. (We do not make any closure requirements on $P$.) Write 
$C^D=C$ and $P^D=P$. Note that $\witri{C}\inter P=\emptyset$.

An \emph{operatic domain} is an operatic domain over some $\opbk$.
\end{definition}

\begin{definition}\label{dfn:operator}
Let $\opbk$ be an operator background. An \textbf{operator over $\opbk$ with 
domain $D$} is a function $\Fop:D\to\opbk$ such that (i) $D$ is an operatic 
domain over $\opbk$;
(ii) for all $X\in D$, $\M=\Fop(X)$ is a successor opm with $\M^-=X$ (so if $X\in\witri{C^D}$ then 
$\wl(\M)=1$ and $\hmb^\M=X$).
Write $C^\Fop=C^D$ and $P^\Fop=P^D$.
\end{definition}

\begin{remark}
The argument $X$ to an operator should be thought of as having one of two possible types.
It is a \emph{coarse object} if $X\in\witri{C^\Fop}$; it is an opm if $X\in P^\Fop$.
Some natural operators $\Fop$ have the 
property that, given
$\N\in P^\Fop$ (so $\widehat{\N}\in C^\Fop$), $\Fop(\widehat{\N})$ is inter-computable with 
$\Fop(\N)$. But 
strategy operators in 
the ``least tree'' hierarchy do not have this property.
\end{remark}

The simplest operator is essentially $\J$:

\begin{definition}
Let $\hmpv\in V$.
Let $C_\hmpv$ be the class of all $x$ such that $\hmpv\in\J_1(\hat{x})$.
Let $P_\hmpv$ be the class of all $\om$-sound condensing opms $\R$ over some $Y\in\witri{C_\hmpv}$,
with $\hmp^\R=\hmpv$.
Then $\J^\op_{\hmpv}$ denotes the operator over $V$
with domain $D=\witri{C_\hmpv}\un P_\hmpv$, where for $x\in D$, $\J^\op_\hmpv(x)$ is the passive 
successor opm $\M$ with universe $\J_1(x)$ and $\M^-=x$ and $\hmp^\M=\hmpv$.\footnote{It is easy to 
see that $\M$ is indeed an opm, so $\J^\op_\hmpv$ is an operator.} (So if $x\in\witri{C_\hmpv}$ 
then $\wl(\M)=1$ and $\hmb^\M=x$.)
Let $\J^\op=\J^\op_\emptyset$.
\end{definition}



\begin{definition}[$\Fop$-opremouse]\label{Fop-premouse}
For $\Fop$ an operator, an \textbf{$\Fop$-opremouse 
\tu{(}$\Fop$-opm\tu{)}}
is an opm $\M$
such that $\N=\Fop(\N^-)$ for every successor $\N\wins\M$.
\end{definition}

Let $\M$ be an $\Fop$-opremouse, where $\Fop$ is an operator over $\opbk$. Note that 
$\hmb^\M\in\witri{C^\Fop}$, as $\M\wupto1=\Fop(\M\wupto0)$ and $\M\wupto0=\hmb^\M=\hat{x}$ for some 
$x$, and 
$\hat{x}\notin P^\Fop$. Note also that
$\OR(\M)\leq\OR(\opbk)$.

We now define $\Fop$-iterability for $\Fop$-opremice $\M$.
The main point is that the iteration strategy should produce $\Fop$-opremice.
One needs to be a little careful, however,
because the background $\opbk$ for $\Fop$ might only be a set.
To simplify things, we restrict our attention to the case that $\M\in\opbk$.

\begin{definition}\label{dfn:F-iterability}
Let $\Fop$ be an operator over $\opbk$.
Let $\M$ be an opm and let $\Tt$ be a putative iteration tree on $\M$.
We say that $\Tt$ is a \textbf{putative $\Fop$-iteration tree} iff $M^\Tt_\alpha$ is an 
$\Fop$-opremouse for all $\alpha+1<\lh(\Tt)$.
We say that $\Tt$ is a \textbf{well-putative $\Fop$-iteration tree} iff $\Tt$ is an iteration 
tree and a putative $\Fop$-iteration tree (i.e. a putative $\Fop$-iteration tree whose models are 
all wellfounded).
We say that $\Tt$ is an \textbf{$\Fop$-iteration tree} 
iff $M^\Tt_\alpha$ is an $\Fop$-opremouse for all $\alpha+1\leq\lh(\Tt)$.
We may drop the ``$\Fop$-'' when it is clear from context.

Let $k<\om$ and let $\M\in\opbk$ be a $k$-sound $\Fop$-opremouse.
Let $\theta\leq\OR(\opbk)+1$.
The iteration game 
$\G^{\Fop,\M}(k,\theta)$ has the rules of $\G^\M(k,\theta)$, except for the following 
difference. Let $\Tt$ be the putative tree being produced.
For $\alpha+1\leq\theta$, if both players meet their requirements at all stages $<\alpha$, then,
in stage $\alpha$, player $\plII$ must first ensure that $\Tt\rest\alpha+1$ is a well-putative 
$\Fop$-iteration tree, and if $\alpha+1<\OR(\opbk)$, that $\Tt\rest\alpha+1$ is an 
$\Fop$-iteration tree. (Given this, if $\alpha+1<\theta$, player $\plI$ then selects 
$E^\Tt_\alpha$.)\footnote{
Thus, if we reach stage $\OR(\opbk)$, then after selecting a branch, player $\plII$ wins iff 
$M^\Tt_{\OR(\opbk)}$ is wellfounded. We cannot in general expect $M^\Tt_{\OR(\opbk)}$ to be an 
$\Fop$-opremouse in this situation. For example, suppose that $\opbk=\HC$ and $\theta=\om_1+1$ 
and $\lh(\Tt)=\om_1+1$. 
Then $M^\Tt_{\om_1}$ cannot be an $\Fop$-opremouse, since all $\Fop$-opremice have height 
$\leq\om_1$.
But in applications such as comparison, we only need to know that $M^\Tt_{\om_1}$ 
is wellfounded. So we still decide the game in favour of player $\plII$ in this situation.}

Let $\lambda,\alpha\leq\OR(\opbk)$, and suppose that either $\OR(\opbk)$ is regular or 
$\lambda<\OR(\opbk)$. Let $\theta\leq\lambda+1$.
The iteration game 
$\G^{\Fop,\M}(k,\alpha,\theta)$ is defined just as $\G^\M(k,\alpha,\theta)$,
with the differences that (i) the rounds are runs of $\G^{\Fop,\Q}(q,\theta)$ for some 
$\Q,q$,\footnote{By some straightforward calculations using the restrictions on $\alpha,\theta$, 
one can see that for any $\gamma<\alpha$,
if neither player has lost the game after the first $\gamma$ 
rounds,
and $\Ttvec\rest\gamma$ is the sequence of trees played thus far,
then $M^{\Ttvec\rest\gamma}_\infty\in\opbk$ and $M^{\Ttvec\rest\gamma}_\infty$ is an 
$\Fop$-opremouse, so $\G^{\Fop,\Q}(q,\theta)$ is defined for the relevant $(\Q,q)$. This uses the 
rule that if one of the rounds produces a tree of length $\theta$, then the game terminates.} and 
(ii) if $\alpha$ is a limit and neither player breaks 
any rule, and $\Ttvec$ is the sequence of trees played, then player $\plII$ wins iff
$M^{\Ttvec}_\infty$ is defined (that is, the trees eventually do not drop on their main branches, 
etc), wellfounded, and if $\alpha<\OR(\opbk)$ then $M^{\Ttvec}_\infty$ is an 
$\Fop$-opremouse.\footnote{It follows 
that if $\lambda=\OR(\opbk)$ then $M^{\Ttvec}_\infty\wupto\OR(\opbk)$ is an $\Fop$-opremouse.} 
Likewise, 
$\G_{\max}^{\Fop,\M}(k,\alpha,\theta)$ is analogous to $\G_{\max}^\M(k,\alpha,\theta)$.

An \textbf{$\Fop$-$(k,\theta)$-iteration strategy} for $\M$ is 
a winning strategy for player $\plII$ in $\G^{\Fop,\M}(k,\theta)$,
an \textbf{$\Fop$-$(k,\alpha,\theta)$-maximal iteration strategy} for $\M$ is likewise for 
$\G^{\Fop,\M}_{\max}(k,\alpha,\theta)$, and an 
\textbf{$\Fop$-$(k,\alpha,\theta)$-iteration strategy} is likewise for 
$\G^{\Fop,\M}(k,\alpha,\theta)$.

Now \textbf{$\Fop$-$(k,\theta)$-iterability}, etc, are defined in the obvious manner.
\end{definition}



In order to prove that $\Fop$-opremice built by background constructions are $\Fop$-iterable, we
will need to know that $\Fop$ has good \emph{condensation} properties.



\begin{definition}
 Let $\pi:\M\to\N$ be an embedding and $b$ be transitive. We say that $\pi$ is \emph{above $b$} iff 
$b\un\{b\}\sub\dom(\pi)$ and $\pi\rest b\un\{b\}=\id$.
\end{definition}


\begin{definition}\label{dfn:condenses_coarsely}
 Let $\Fop$ be an operator over $\opbk$ and $p\in\opbk$ be transitive.
We say that $\Fop$ \textbf{condenses coarsely above $p$} iff for
every successor $\Fop$-opm $\N$,
every set-generic extension $V[G]$ of $V$
and all $\M,\pi\in V[G]$,
if $\M^-\in V$ and
$\pi:\M\to\N$ is fully elementary and above $p$,
then $\M$ is an 
$\Fop$-opm (so in particular, $\M^-\in\dom(\Fop)$ and $\M=\Fop(\M^-)\in V$).

We say that $\Fop$ \textbf{almost condenses coarsely above $b$} iff the preceding holds for 
$G=\emptyset$.
\end{definition}


\begin{definition}
 An operator $\Fop$ over $\opbk$ is \emph{total} iff $P^\Fop$ includes all condensing $\om$-sound
$\Fop$-opms in $\opbk$.
\end{definition}

\begin{lemma}\label{lem:almost_redundancy_coarsely}
 Let $\Fop$ be a total operator which almost condenses coarsely above
 some $p\in\HC$.
 Then $\Fop$ condenses coarsely above $p$.
\end{lemma}
\begin{proof}[Proof Sketch]
Suppose the lemma fails and let $\PP$ be a poset, and 
$G\sub\PP$ be $V$-generic, such that in $V[G]$ there is a counterexample $\pi:\M\to\N$.
We may easily assume that $\M^-$ is an $\Fop$-opm, and therefore that $\M^-\in\dom(\Fop)$.
So $\M\neq\Fop(\M^-)$. By $\Sigma^1_1$-absoluteness, we may assume that 
$\PP=\Coll(\om,\Fop(\M^-)\un\N)$. Therefore there is a transitive, rud closed set $X\in\opbk$, 
where $\Fop$ is over $\opbk$, such that $\PP\in X$ and $X\sats$``It is forced by $\PP$ that there 
is an $\M$ and a fully elementary $\pi:\M\to\N$, with $\M\neq\Fop(\M^-)$.'' Because 
$\opbk\sats\DC$, we can take a countable elementary hull of $X$, such that letting 
$\sigma:\bar{X}\to X$ be the uncollapse, $\rg(\sigma)$ includes all relevant objects and all points 
in $p\un\{p\}\sub\rg(\sigma)$.
But we can find generics for $\bar{X}$, and because 
$\Fop$ almost condenses coarsely above $p$, this easily leads to contradiction.
\end{proof}

The notion of $(z_{k+1}^\M,\zeta_{k+1}^\M$) below is a direct adaptation from 
\cite[***where?]{extmax}. The facts proved there about this notion generalize readily to the 
present setting.

\begin{definition}
 Let $\M$ be a $k$-sound opm. Let $\Dd$ be the class of pairs 
$(z,\zeta)\in[\Ord]^{<\om}\cross\Ord$ such that $\zeta\leq\min(z)$. For $x\in[\Ord]^{<\om}$ let 
$f_x$ be the decreasing enumeration of $x$. For $x=(z,\zeta)\in\Dd$ let 
$f_x=f_z\conc\left<\zeta\right>$.
Order $\Dd$ by $x<^*y$ iff $f_x<_{\mathrm{lex}}f_y$. Then $(z_{k+1}^\M,\zeta_{k+1}^\M)$ denotes the 
$<^*$-least $(z,\zeta)\in\Dd$ such that
\[ \Th_{k+1}^\M(\hmb^\M\un z\un\zeta)\notin\M. \]
The \emph{$(k+1)$-solid-core} of $\M$ is
 \[ \mathfrak{S}_{k+1}(\M)=\cHull_{k+1}^\M(\hmb^\M\un z_{k+1}^\M\un\zeta_{k+1}^\M), \]
and the \emph{$(k+1)$-solid-core map} $\sigma_{k+1}^\M$ is the uncollapse map.
\end{definition}

If $\M$ is $(k+1)$-solid then $\mathfrak{S}_{k+1}(\M)=\core_{k+1}(\M)$ and 
$\sigma_{k+1}^\M$ is the core map. But we will need to consider the $(k+1)$-solid-core more 
generally, in the proof of $(k+1)$-solidity.

\begin{definition}
Let $k\leq\om$, let $\L,\M$ be $k$-sound opms and $\sigma:\L\to\M$. We say that $\sigma$ is 
\emph{$k$-tight} iff there is $\lambda\in\Ord$ and a sequence 
$\left<\L_\alpha\right>_{\alpha\leq\lambda}$ of opms such that $\L=\L_0$ and $\M=\L_\lambda$ and 
there is a sequence $\left<E_\alpha\right>_{\alpha<\lambda}$ of extenders such that each $E_\alpha$ 
is weakly amenable to $\L_\alpha$, with $\crit(E_\alpha)>\hmb^\L$,
\[ \L_{\alpha+1}=\Ult_k(\L_\alpha,E_\alpha), \]
and for limit $\eta$,
\[ \L_\eta=\dirlim_{\alpha<\beta<\eta}(\L_\alpha,\L_\beta;j_{\alpha\beta}) \]
where $j_{\alpha\beta}:\L_\alpha\to\L_\beta$ is the resulting ultrapower map,
and $\sigma=j_{0\lambda}$.
\end{definition}

\begin{definition}\label{dfn:k-factor}
Let $k\leq\om$ and $\M,\N$ be $k$-sound opms and $p$ be transitive.

We say that $\pi:\M\to\N$ is a \emph{$k$-factor above $p$}
iff $\pi$ is a weak $k$-embedding above $p$, and if $k<\om$ then there is a $k$-tight 
$\sigma:\L\to\M$ such that 
\[ \pi\com\sigma\com\sigma^\L_{k+1}:\mathfrak{S}_{k+1}(\L)\to\N \]
is a near $k$-embedding, $\sigma$ is above $p$,
and $\L$ is $k$-relevant.

For an operator $\Fop$, a $k$-factor is \emph{$\Fop$-rooted} iff either $k=\om$ or
we can take $\L$ to be an $\Fop$-opremouse.

A $k$-factor is \emph{good} iff $A\eqdef\hmb^\M=\hmb^\N$ and $\pi$ is above $A$.
\end{definition}

An $\om$-factor above $p$ is just an $\om$-embedding (i.e. fully elementary between 
$\om$-sound opms) above $p$. If $k<\om$, then both $\sigma$ and $\sigma_{k+1}^\L$, and 
therefore also $\sigma\com\sigma_{k+1}^\L$, are $k$-good. Any near $k$-embedding 
$\pi:\M\to\N$ between opms is a $k$-factor, and if $\M$ is an $\Fop$-opm, then $\pi$ is 
$\Fop$-rooted (if $k<\om$, use $\L=\M$ and $\sigma=\id$).


\begin{definition}
 Let $\C$ be a successor opm and $\M$ a successor Q-opm with $\C^-=\M^-$. We say that $\C$ is a 
\emph{universal hull} of $\M$
 iff there is an above $\C^-$, $0$-good embedding $\pi:\C\to\M$ and for every $x\in\M$,
$\Th_1^\M(\M^-\un\{x\})$ is $\bfrSigma_1^\C$ (after replacing $x$ with a constant symbol).
\end{definition}

We next define \emph{condenses finely}, a variant of the notion \emph{condenses well} (see 
\cite[***where?]{cmi_original},
\cite[2.1.10]{wilson2012contributions}).
There are a few differences. The first is that we weaken
the conclusion. 
The second is that we do not require that 
$\varphi\com\sigma\in V$. The third is that we make much stronger demands on $(\L,\sigma)$. In 
Appendix \ref{app:condenses}
we justify these modifications.

\begin{definition}\label{dfn:condenses_finely}
Let $\Fop$ be an operator over $\opbk$ and $b\in\opbk$ be transitive.
We say that $\Fop$ \textbf{condenses finely above $b$} iff (i) $\Fop$ condenses coarsely 
above $b$; and (ii) Let
$A,\Abar,\N,\L\in V$ and let $\M,\varphi,\sigma\in V[G]$ where $G$ is 
set-generic over $V$. Suppose that:
\begin{enumerate}[label=--]
 \item $b\in\J_1(\Abar)\inter\J_1(A)$,
 \item $\M$ is a Q-opm over $\Abar$, $\L$ is an opm over $\Abar$, and $\N$ is an 
opm over $A$, each of successor length,
\item $\L,\M^-,\N$ are $\Fop$-opremice,
\item $\varphi:\M\to\N$.
\end{enumerate}
Then:
\begin{enumerate}[label=--]
 \item If $\M$ is an opm and $k<\om$ and either
\begin{enumerate}[label=--]
 \item $\varphi$ is $k$-good, or
 \item $V[G]\sats$``$\varphi$ is a $k$-factor above $b$, as witnessed by 
$(\L,\sigma)$'' and $\M$ is $k$-relevant,
\end{enumerate}
then either $\M\in\Fop(\M^-)$ or $\M=\Fop(\M^-)$.
\item If $\rho_1^\M\leq\OR(\M^-)$ and $\varphi$ is $0$-good, then there is a universal hull $\Hh$ 
of $\M$ such that either $\Hh\in\Fop(\M^-)$ or $\Hh=\Fop(\M^-)$.
\end{enumerate}

We say $\Fop$ \textbf{almost condenses finely above $b$} iff $\Fop$ almost condenses 
coarsely above $b$ and condition (ii) above holds 
for $G=\emptyset$.
\end{definition}

As we will see later, there are natural examples of operators which condense finely, but 
do not condense well. 
We next observe that in certain key circumstances, we can actually conclude that
$\M=\Fop(\M^-)$.

\begin{lemma}\label{lem:strengthen_scf_conclusion}
 Let $k,\M,G,\N$, etc, be as in \ref{dfn:condenses_finely}.
Suppose that either $\M=\core_{k+1}(\N)$ or 
$\M$ is $k$-relevant. Then $\M\notin\Fop(\M^-)$, and if $k=0$ then there is no universal hull 
of $\M$ in $\Fop(\M^-)$.
\end{lemma}
\begin{proof}
Suppose otherwise. 
Then by projectum amenability for $\Fop(\M^-)$, $\M$ is not $k$-relevant. So 
$\M=\core_{k+1}(\N)\notin\N$; let $\varphi:\M\to\N$ be the core 
map. By \ref{lem:core_embedding}, $\varphi$ is $k$-good, so $\varphi(\M^-)=\N^-$.
Clearly $\M\neq\N$, so letting $\rho=\rho_{k+1}^{\N}$, we have $\rho<\rho_k^{\N}$, and by 
\ref{lem:non_k-rpm_sound}, $\N$ is $k$-relevant.
So $\rho<\rho_\om^{\N^-}$ and $\rho\leq\crit(\varphi)$.
We have $\varphi(\rho_\om^{\M^-})=\rho_\om^{\N^-}$, 
so $\rho\leq\rho_\om^{\M^-}$. 
Since $\varphi$ is $k$-good, $\rho<\rho_k^{\M}$.
Since $\M$ is not $k$-relevant, therefore $\rho=\rho_\om^{\M^-}=\crit(\varphi)$. So because 
$\N^-$ is condensing, and
$\rho$ is a cardinal of $\N^-$, we have $\M^-\wpins\N^-$, 
so $\Fop(\M^-)\wpins\N^-$, so either $\M\in\N$, 
or $k=0$ and there is a universal hull $\Hh$ of $\M$ in $\N$,
both of which contradict the fact that $\M=\core_{k+1}(\N)$.
\end{proof}

So under the circumstances of the lemma above, and if $\M$ is an opm, fine condensation (i.e. 
\emph{condenses finely})  
gives the stronger 
conclusion that $\M=\Fop(\M^-)$. However, we will need to apply fine 
condensation more generally, such as in the proof of solidity.

\begin{definition}
We say that $(\Fop,b,A)$ (or $(\Fop,b,A,B)$) is an \emph{\tu{(}almost\tu{)} fine ground}
iff $\Fop$ an operator which (almost) condenses finely above $b$ and
$A\in\witri{C_\Fop}$ and $b\in\J_1(A)$ (and $B\in\witri{C_\Fop}$ and $b\in\J_1(B)$).
\end{definition}

 Analogously to 
\ref{lem:almost_redundancy_coarsely}:

\begin{lemma}\label{lem:almost_redundancy_finely}
Let $\Fop$ be a total operator which almost condenses finely 
above some $p\in\HC$. Then $\Fop$ condenses finely above $p$.
\end{lemma}

We now show how fine condensation for $\Fop$ ensures that the copying construction proceeds 
smoothly for relevant $\Fop$-opremice.

\begin{definition}\label{dfn:uparrow}
 Let $\M$ be an opm.
 If $\M$ is not type 3 then $\M^\uparrow\eqdef\M$.
 If $\M$ is type 3 and $\kappa=\hmmu^\M$
then
 \[ \M^\uparrow\eqdef\Ult(\M\wupto(\kappa^+)^\M,\actext^\M). \]

  For $\pi:\M\to\N$, a $\Sigma_0$-elementary embedding between opms of the same type, we define 
$\pi^\uparrow:\M^\uparrow\to\N^\uparrow$ as follows.
 If $\M$ is not type 3 then $\pi^\uparrow=\pi$.
 If $\M$ is type 3 then $\pi^\uparrow$
 is the embedding induced by $\pi$.

 Let $\M,\N$ be opms.
 We write $\N\wins^\uparrow\M$ iff either $\N\wins\M$ 
or $\N\wpins\M^\uparrow$. We write $\N\wpins^\uparrow\M$ iff either $\N\wpins\M$ 
or $\N\wpins\M^\uparrow$.
Let $j,k\leq\om$ be such that $\M$ is $j$-sound and $\N$ is $k$-sound.
We write
\[ (\N,k)\wins(\M,j)\] 
iff either [$\N=\M$ and $k\leq j$] or $\N\wpins\M$.
We write
\[ (\N,k)\wins^\uparrow(\M,j)\]
iff 
either $(\N,k)\wins(\M,j)$ or $\N\wpins\M^\uparrow$.
\end{definition}

 The copying process is complicated by squashing of type 3 
structures; see \cite{?}. In order to reduce these complications, we will consider a trivial
\emph{reordering} of the tree order of lifted trees.
\begin{definition}
 Let $\Tt$ be a $k$-maximal iteration tree. An \emph{insert set} for $\Tt$ is a set $I\sub\lh(\Tt)$ 
be such that for all $\alpha\in I$, we have $\alpha+1<\lh(\Tt)$ and $M^\Tt_\alpha$ is type 3 and 
$E^\Tt_\alpha=F(M^\Tt_\alpha)$. Given such an $I$, the \emph{$I$-reordering} $<_{\Tt,I}$ of $<_\Tt$ 
is the iteration tree order defined as follows.
Let $\beta+1<\lh(\Tt)$ and $\gamma=\pred^\Tt(\beta+1)$. Then 
$\pred^{\Tt,I}(\beta+1)=\gamma$ unless $\beta+1\in D^\Tt$ and $\gamma=\alpha+1$ for some $\alpha\in 
I$ and $\crit(E^\Tt_\beta)<j(\kappa)$, where $j=i_{E^\Tt_\alpha}$ and $\kappa=\crit(E^\Tt_\alpha)$, 
in which case $\pred^{\Tt,I}(\beta+1)=\alpha$. For limits $\beta<\lh(\Tt)$, we set 
$[\gamma,\beta)_{\Tt,I}=[\gamma,\beta)_\Tt$ for all sufficiently large $\gamma<_\Tt\beta$.
\end{definition}

So if $\alpha=\pred^{\Tt,I}(\beta+1)\neq\pred^\Tt(\beta+1)$, then
$M^{*\Tt}_{\beta+1}\wpins M^\Tt_{\alpha+1}\wupto j(\kappa)$ (for $j,\kappa$ as above)
so $M^{*\Tt}_{\beta+1}\wpins^\uparrow 
M^\Tt_\alpha$,
but possibly $M^{*\Tt}_{\beta+1}\nwpins M^\Tt_\alpha$.


\begin{definition}\label{dfn:restricted_it_maps}
 Let $\Tt$ be a $k$-maximal tree on an opm $\M$, let $I$ be an insert set for $\Tt$, let 
$\N\wins\M$ and $\alpha<\lh(\Tt)$.
 Let $\left<\beta_1,\ldots,\beta_{n}\right>$ enumerate $D^\Tt\inter(0,\alpha]_{\Tt,I}$.
 Let $\beta_0=0$, let $\gamma_i=\pred^{\Tt,I}(\beta_{i+1})$ for $i<n$, and let 
$\gamma_n=\alpha$.
 Let $\pi_i=i^{*\Tt}_{\beta_i,\gamma_{i}}$, where $i^{*\Tt}_{0,\gamma_0}=i^\Tt_{0,\gamma_0}$.
 Let $\N_0=\N$ and $\N_{i+1}=\varrho_{\pi_i}(\N_i)$ if $\N_i\in\dom(\varrho_{\pi_i})$,
 let $\N_{i+1}=M^\Tt_{\gamma_{i}}$ if $M^{*\Tt}_{\beta_i}=\N_i$,
 and $\N_{i+1}$ is undefined otherwise (in the latter case, $\N_j$ is undefined for all $j>i$).
 
We say that $[0,\alpha]_{\Tt,I}$ \emph{drops below the image of $\N$} iff $\N_{n+1}$ is undefined.
If $[0,\alpha]_{\Tt,I}$ does not drop below the image of $\N$, we define 
$M^{\Tt,I}_{\N,\alpha}=\N'=\N_{n+1}$; and
\[ i^{\Tt,I}_{\N,0,\alpha}:\N\to\N' \] 
as follows. If $\N'=M^\Tt_\alpha$ then
\[ i^{\Tt,I}_{\N,0,\alpha}\eqdef 
i^{*\Tt}_{\beta_n,\alpha}\com\pi_{n-1}^\uparrow\com\pi_{n-2}^\uparrow
\com\ldots\com\pi_0^\uparrow\rest\core_0(\N) , \]
and if $\N'\wpins^\uparrow M^\Tt_\alpha$ then
\[ 
i^{\Tt,\N}_{0,\alpha}\eqdef\pi_n^\uparrow\com\pi_{n-1}^\uparrow
\com\ldots\com\pi_0^\uparrow\rest\core_0(\N).\]
Also for $\xi<_{\Tt,I}\alpha$, define
$i^{\Tt,I}_{\N,\xi,\alpha}:M^{\Tt,I}_{\N,\xi}\to M^{\Tt,I}_{\N,\alpha}$
to be the natural map $j$ such that
$j\com i^{\Tt,I}_{\N,0,\xi}=i^{\Tt,I}_{\N,0,\alpha}$
(so $j$ is given by composing restrictions of $\sigma^\uparrow$ for 
iteration maps $\sigma$ of $\Tt$ along segments of $[\xi,\alpha]_{\Tt,I}$).
\end{definition}

We now state the basic facts about the copying construction for $\Fop$-opremice. We begin with a 
simple lemma regarding type 3 $\Fop$-opremice.

\begin{lemma}\label{lem:type_3_F-pm_condensation}
Let $(\Fop,b,\Abar,A)$ be an almost fine ground. Let $\N$ be a type 3 $\Fop$-opm over $A$,
such that $\N^\uparrow$ is an $\Fop$-opm.
Let $\pi:\R\to\N^\sq$ be a weak $0$-embedding.
Then $\R=\M^\sq$ for some $\Fop$-opm $\M$.
\end{lemma}
\begin{proof}
Because $\pi$ is a weak $0$-embedding, $E=E^\R$ is an extender over $\R$.
So we can define $\R^\uparrow$ and $\pi^\uparrow:\R^\uparrow\to\N^\uparrow$ as in 
\ref{dfn:uparrow}.
By almost coarse condensation, $\R^\uparrow$ is an $\Fop$-opm, which yields the desired 
conclusion.
\end{proof}

Of course, in the preceding lemma we only actually needed almost \emph{coarse} condensation.
Below, the indexing function $\iota$ need not be the identity, because of the possibility of 
$\nu$-high copy embeddings; see \cite{copy_con}.

\begin{lemma}\label{lem:strategy_copying}
Let $(\Fop,b,\Abar,A)$ be an almost fine ground.
Let $j\leq\om$ and let $\Q$ be a $j$-sound $\Fop$-opremouse over $A$.
Let $(\N,k)\wins(\Q,j)$.
Let $\M$ be a $k$-relevant $\Fop$-opm over $\Abar$ and
$\pi:\M\to\N$ an $\Fop$-rooted $k$-factor above $b$.

Let $\Sigma_\Q$ be an $\Fop$-$(j,\om_1+1)$-strategy for $\Q$.
Then there is an $\Fop$-$(k,\om_1+1)$-strategy $\Sigma_\M$ for $\M$ such that trees $\Tt$ via 
$\Sigma_\M$ lift to trees $\Uu$ via $\Sigma_\Q$. In fact, there is an insert set $I$ for $\Uu$ and
$\iota:\lh(\Tt)\to\lh(\Uu)$ such that for each $\alpha<\lh(\Tt)$, letting $\alpha'=\iota(\alpha)$,
there is $N^\Uu_{\alpha}\wins^\uparrow M^\Uu_{\alpha'}$ such that 
\[ (N^\Uu_{\alpha},\deg^\Tt(\alpha))\wins^\uparrow (M^\Uu_{\alpha'},\deg^\Uu(\alpha')),\]
and there is an $\Fop$-rooted $\deg^\Tt(\alpha)$-factor above $b$
\[ \pi_\alpha:M^\Tt_\alpha\to N^\Uu_{\alpha}, \]
and if $\pi$ is good then 
$\pi_\alpha$ is good.
Moreover, $[0,\alpha]_\Tt\inter D^\Tt$ model-drops iff $[0,\alpha']_{\Uu,I}$ drops 
below the image 
of $\N$.
If $[0,\alpha]_\Tt\inter D^\Tt$ does not model-drop then
$N^\Uu_{\alpha}=M^{\Uu,I}_{\N,\alpha'}$ and
\begin{equation}\label{eqn:no_drop_comm} \pi_\alpha\com 
i^\Tt_{0,\alpha}=i^{\Uu,I}_{\N,0,\alpha'}\com\pi. \end{equation}
If either $[0,\alpha]_\Tt$ model-drops or \tu{[}$(\N,k)=(\Q,j)$ and $\pi$ is a near 
$j$-embedding\tu{]} then $N^\Uu_{\alpha}=M^{\Uu}_{\alpha'}$ and 
$\deg^\Tt(\alpha)=\deg^\Uu(\alpha')$ and $\pi_\alpha$ is a near $\deg^\Tt(\alpha)$-embedding.

The previous paragraph also holds with ``$(j,\om_1,\om_1+1)$-maximal'' replacing ``$(j,\om_1+1)$'' 
and ``$(k,\om_1,\om_1+1)$-maximal'' replacing ``$(k,\om_1+1)$''.
\end{lemma}

\begin{proof}
We just sketch the proof, for the $k$-maximal case. It is mostly the standard copying 
construction, augmented with propagation of near embeddings (see \cite{fine_tame}), and the 
standard extra details dealing 
with type 3 premice (see \cite{outline} and \cite{copy_con}). We put $\alpha'\in I$ iff either (i) 
$E^\Tt_\alpha=F(M^\Tt_\alpha)$ and $N^{\Uu}_{\alpha}\nwins M^{\Uu,I}_{\alpha'}$ (so 
$N^{\Uu}_{\alpha}\wpins^\uparrow M^{\Uu,I}_{\alpha'}$) or (ii) $E^\Tt_\alpha\neq F(M^\Tt_\alpha)$ 
and $\pi_\alpha^\uparrow(\lh(E^\Tt_\alpha))>\OR(M^{\Uu,I}_{\alpha'})$.
It follows that if $\alpha'\in I$ then $M^{\Uu}_{\alpha'}$ is type 3 and $[0,\alpha]_\Tt$ does not 
drop in model; the latter is by arguments in \cite{copy_con}. When $\alpha'\in I$, we set 
$E^{\Uu}_{\alpha'}=F(M^\Uu_{\alpha'})$, and then define $E^\Uu_{\alpha'+1}$ by copying
$E^\Tt_\alpha$ with $\pi_\alpha$ (and then $(\alpha+1)'=\alpha'+2$). We omit the remaining,
standard, details regarding the correspondence of tree structures and definition of 
$\iota,N^\Uu_\alpha,\pi_\alpha$.


Now the main thing is to observe that for each $\alpha$, $\pi_\alpha$ is 
an $\Fop$-rooted $\deg^\Tt(\alpha)$-factor (above $b$; for the rest of the proof we omit that 
phrase). For given this, 
fine condensation, together with \ref{lem:type_3_F-pm_condensation}, gives that $M^\Tt_\alpha$ is 
an 
$\Fop$-opm.
(If $M^\Tt_\alpha$ might be type 3 (i.e. $N^\Uu_{\alpha}$ is type 3), then 
\ref{lem:type_3_F-pm_condensation} applies, because $(N^\Uu_{\alpha})^\uparrow$ is an 
$\Fop$-opm, because we can extend $\Uu\rest(\alpha'+1)$ to a tree $\Uu'$, setting 
$E^{\Uu'}_{\alpha'}=F(N^\Uu_{\alpha})$.)
Fix $(\Ll_0,\sigma_0)$ 
witnessing the fact that $\pi$ is a (good) $\Fop$-rooted $k$-factor above $b$.

Suppose that $[0,\alpha]_\Tt$ does not drop in model.
Then it is routine that $[0,\alpha']_{\Uu,I}$ does not drop below the 
image of $\N$, $\pi_\alpha$ is a weak $\deg^\Tt(\alpha)$-embedding and line (\ref{eqn:no_drop_comm})
holds. If $\deg^\Tt(\alpha)=k$ then it follows that $(\Ll_0,\sigma)$ witnesses the fact that 
$\pi_\alpha$ is a (good) $\Fop$-rooted $k$-factor above $b$, where 
$\sigma=i^\Tt_{0,\alpha}\com\sigma_0$,
because $i^{\Uu,I}_{\N,0,\alpha'}$ and $\pi\com\sigma_0$ are both near $k$-embeddings,
and $\pi_\alpha\com i^\Tt_{0,\alpha}=i^{\Uu,I}_{\N,0,\alpha'}\com\pi$.

Suppose further that $[0,\alpha]_\Tt$ drops in degree and let $n=\deg^\Tt(\alpha)$. Then letting 
$\Ll=\core_{n+1}(M^\Tt_\alpha)$ and $\sigma:\Ll\to M^\Tt_\alpha$ be the core embedding, 
$(\Ll,\sigma)$ witnesses the fact that $\pi_\alpha$ is a (good) $\Fop$-rooted $n$-factor above $b$ 
(we have $\mathfrak{S}_{k+1}(\Ll)=\Ll$ and $\sigma_{k+1}^\Ll=\id$). The fact that 
$\Ll$ is $n$-relevant is verified as follows. There is $\beta+1\leq_\Tt\alpha$ such that 
$\Ll=M^{*\Tt}_{\beta+1}$ and $\sigma=i^{*\Tt}_{\beta+1,\alpha}$.
Suppose that $\Ll$ is a successor.
Then letting $\xi=\pred^\Tt(\beta+1)$, we have $\lh(E^\Tt_\xi)\leq\OR(\Ll^-)$.
So letting $\kappa=\crit(\sigma)$, $E^\Tt_\beta$ measures only 
$\pow(\kappa)\inter\Ll^-$. But since $\Ll^-\wpins M^{*\Tt}_{\beta+1}$,
therefore $\kappa<\rho_\om^{\Ll^-}$. But $\rho_{n+1}^\Ll\leq\kappa$, which suffices.
The fact that $\pi_\alpha\com\sigma$ is a near $n$-embedding is because
$\pi_\alpha\com\sigma=i^{\Uu,I}_{\N,\xi',\alpha'}\com\pi_\xi$ and $\pi_\xi$ is a weak 
$(n+1)$-embedding, and $i^{\Uu,I}_{\N,\xi',\alpha'}$ a near $n$-embedding.

Now suppose that $[0,\alpha]_\Tt$ drops in model. It is straightforward to see that 
$[0,\alpha']_{\Uu,I}$ drops below the image of $\N$ and that $N^\Uu_{\alpha}=M^\Uu_{\alpha'}$. The 
fact that $\pi_\alpha$ is an $\Fop$-rooted $\deg^\Tt(\alpha)$-factor is 
almost the same as in the dropping degree case above.
The fact that $\pi_\alpha$ is in fact a near $\deg^\Tt(\alpha)$-embedding  and 
$\deg^\Tt(\alpha)=\deg^\Uu(\alpha')$ follows from an examination of the proof
that near embeddings are propagated by the copying construction in
\cite{fine_tame}; similar arguments are given in \cite{copy_con}.
\end{proof}



We next consider constructions building $\Fop$-mice.

\begin{definition}
 Let $\N$ be an $\Fop$-opm and $k\leq\om$. Then $\N$ is 
\textbf{$\Fop$-$k$-fine} iff for each 
$j\leq k$:
\begin{enumerate}[label=--]
 \item $\core_j(\N)$ is a $j$-solid $\Fop$-opm,
 \item if $j<k$ then $\core_j(\N)$ is $(j+1)$-universal,
 \item if $k=\om$ then $\core_\om(\N)$ is condensing.\qedhere
\end{enumerate}
\end{definition}

\begin{definition}\label{dfn:Fop_con}
Let $\Fop$ be an operator over $\opbk$. Let $A\in\witri{C_\Fop}$ and $\chi\leq\OR(\opbk)+1$. An
\textbf{$L^\Fop[\es,A]$-construction (of length $\chi$)} is a 
sequence $\CC=\left<\N_\alpha\right>_{\alpha<\chi}$ such that for all $\alpha<\chi$:
\begin{enumerate}[label=--]
\item $\N_0=\Fop(A)$ and $\N_\alpha$ is an $\Fop$-opm over $A$.
\item If $\alpha$ is a limit then $\N_\alpha=\liminf_{\beta<\alpha}\N_\beta$.
\item If $\alpha+1<\chi$ then either (i) $\N_{\alpha+1}$ is $\hmE$-active and
$\N_{\alpha+1}\wdoubleupto\OR(\N_{\alpha+1})=\N_\alpha$, or (ii)
 $\N_\alpha$ is $\Fop$-$\om$-fine and $\N_{\alpha+1}=\Fop(\core_\om(\N_\alpha))$.
\end{enumerate}

We say that $\CC$ is $\Fop$-\emph{tenable} iff $\N^\uparrow$ is an 
$\Fop$-opm for each $\alpha<\chi$.
\end{definition}

We will now explain how condensation for $\Fop$ leads to the $\Fop$-iterability of 
substructures $\R$ of $\Fop$-opms built by background construction. The basic engine 
behind this is the realizability of iterates of $\R$ back into models of the 
construction.


\begin{definition}\label{dfn:pi_C_realizable}
Let $(\Fop,b,\Abar,A)$ be an almost fine ground 
$\CC=\left<\N_\alpha\right>_{\alpha\leq\lambda}$ be an
$L^\Fop[\es,A]$-construction. Let $k\leq\om$ and suppose that $\N_\lambda$ is 
$\Fop$-$k$-fine. Let $\R$ be a $k$-sound $\Fop$-opm over $\Abar$ 
and
$\pi:\R\to\core_k(\N_\lambda)$ be a weak $k$-embedding. Let 
$\Tt$ be a putative $\Fop$-iteration 
tree 
on $\R$, with $\deg^\Tt(0)=k$. We say that $\Tt$ 
is
\textbf{$(\pi,\CC)$-realizable above $b$} iff for every
$\alpha<\lh(\Tt)$, letting $\beta=\base^\Tt(\alpha)$ and $m=\deg^\Tt(\alpha)$,
there are $\zeta,\tau$ such that:
\begin{enumerate}[label=--]
 \item $(\zeta,m)\leq_\lex(\lambda,k)$,
 \item if $[0,\alpha]_\Tt$ does not drop in model or degree then 
$\zeta=\lambda$ and $\tau=\pi$,
 \item if $[0,\alpha]_\Tt$ drops in model or degree then
$\tau\colon M^{*\Tt}_\beta\to\core_m(\N_\zeta)$ is a near $m$-embedding above $b$,
 \item if $M^{*\Tt}_\beta$ is not type 3 then there is a weak $m$-embedding 
$\varphi:M^\Tt_\alpha\to\core_m(\N_\zeta)$ such that $\varphi\com 
i^{*\Tt}_{\beta,\alpha}=\tau$.
 \item if $M^{*\Tt}_\beta$ is type 3 then there is a weak $m$-embedding 
$\varphi:\Ss\to\core_m(N_\zeta)$ such that $\varphi\com i^{*\Tt}_{\beta,\alpha}=\tau$, where $\Ss$ 
is ``$(M^\Tt_\alpha)^\sq$''.\footnote{\label{ftn:squash}$(M^\Tt_\alpha)^\sq$ might not make literal 
sense, if say $M^\Tt_\alpha$ is not wellfounded. By ``$(M^\Tt_\alpha)^\sq$'' we mean that either 
$\alpha=\xi+1$ and $\Ss=\Ult_m((M^{*\Tt}_\alpha)^\sq,E^\Tt_\xi)$ (formed without unsquashing), or 
$\alpha$ is a limit and $\Ss$ is 
the direct limit of the structures $(M^\Tt_\xi)^\sq$ for $\xi\in[\beta,\alpha)_\Tt$, under 
the iteration maps.}
\end{enumerate}

We say that $\Tt$ is \textbf{weakly $(\pi,\CC)$-realizable} iff in some set-generic extension 
$V[G]$,
either $\Tt$ is $(\pi,\CC)$-realizable, or there is a limit $\lambda\leq\lh(\Tt)$
and a $(\Tt\rest\lambda)$-cofinal branch $b$ such that $(\Tt\rest\lambda)\conc b$ is 
$(\pi,\CC)$-realizable.
\end{definition}




\begin{definition}
A \textbf{putative $\Fop$-$(k,\theta)$-iteration strategy} for a $k$-sound $\Fop$-opm $\N$ is 
a function $\Sigma$ such that for every $k$-maximal $\Fop$-tree $\Tt$ on $\N$, 
with $\Tt$ via $\Sigma$ and $\lh(\Tt)<\theta$ a limit, $\Sigma(\Tt)$ is a $\Tt$-cofinal branch.
\end{definition}

\begin{lemma}\label{lem:L[E]_construction_iterability}
Let $(\Fop,b,\Abar,A)$ be an almost fine ground.
Let 
$\CC=\left<\N_\alpha\right>_{\alpha<\chi}$ be a tenable
$L^\Fop[\es,A]$-construction. Let $\lambda<\chi$ and $k\leq\om$ be such that $\N_\lambda$ is 
$\Fop$-$k$-fine, and let $\Ss=\core_k(\N_\lambda)$.
Let $\R$ be a $k$-relevant $\Fop$-opm over $\Abar$.
Let $\pi:\R\to\Ss$ be an $\Fop$-rooted $k$-factor above $b$.
Let $\Sigma$ be either:
\begin{enumerate}[label=--]
 \item a putative $\Fop$-$(k,\om_1+1)$-iteration strategy for $\R$, or
 \item a putative $\Fop$-$(k,\om_1,\om_1+1)$-maximal iteration strategy for $\R$.
 \end{enumerate}
Suppose that every putative $\Fop$-tree via $\Sigma$
is $(\pi,\CC)$-realizable above $b$. Then $\Sigma$ 
is an $\Fop$-$(k,\om_1+1)$, or $\Fop$-$(k,\om_1,\om_1+1)$-maximal, iteration strategy.
\end{lemma}

\begin{proof}
The argument is almost that used for \ref{lem:strategy_copying}, 
using the maps provided by $(\pi,\CC)$-realizability in place of copy maps. The tenability of 
$\CC$ is used to see that \ref{lem:type_3_F-pm_condensation} applies where needed.
\end{proof}

In practice, we will take $\R$ and $\pi:\R\to\Ss$ to be fully elementary, which will give that 
$\pi$ is an $\Fop$-rooted $k$-factor. The above proof does not work with 
\emph{$(k,\om_1,\om_1+1)$-maximal} replaced by $(k,\om_1,\om_1+1)$.

\begin{remark}
In this paper we will only make use of \emph{almost condenses finely}, as opposed to 
\emph{condenses finely}.\footnote{But \emph{condenses finely} is more analogous to \emph{condenses 
well} in this regard.} So we digress to mention a key application of 
the latter; this essentially comes from \cite{cmip}.
Adopt the assumptions and notation of the first paragraph of 
\ref{lem:L[E]_construction_iterability}.
Assume further that $(\Fop,b,\Abar,A)$ is a fine ground (not just almost),
$\opbk=V$, there is no $\Fop$-closed inner model with a Woodin,
and $\R\sats$``there is no Woodin''.
Let $\kappa$ be a cardinal.
Suppose that every $k$-maximal putative $\Fop$-tree $\Tt$ on $\R$ of length $\leq\kappa$ is 
weakly $(\pi,\CC)$-realizable.
Then $\R$ is $\Fop$-$(k,\kappa+1)$-iterable, via the strategy guided by Q-structures
of the form $\Fop^\alpha(M(\Tt))$ for some $\alpha\in\Ord$.\footnote{Here 
$\Fop^0(X)=X$ and $\Fop^{\alpha+1}(X)=\Fop(\Fop^\alpha(X))$, and we take unions at limit $\alpha$.
It might be that the Q-structure satisfies ``$\delta(\Tt)$ is not Woodin'',
but in this case, $\alpha=\beta+1$ for some $\beta$ and $\Fop^\beta(M(\Tt))$ 
satisfies ``$\delta(\Tt)$ is Woodin''.} This follows by a straightforward adaptation of the 
proof for standard premice (cf. \cite{cmip}). In the argument one needs to apply \emph{condenses 
finely} to embeddings $\varphi,\sigma$ when $\varphi\com\sigma\notin 
V$. We can only expect $\varphi\com\sigma\in V$ if the realized branch does not drop in model 
or degree (indeed, in the latter case, $\varphi\com\sigma=\pi$), or if all relevant objects are 
countable.
\end{remark}



We use the following variant of the weak Dodd Jensen property of \cite{wDJ}, extended to deal 
partially with good $k$-factors, analogously to how weak $k$-embeddings are dealt with in 
\cite[\S4.2]{copy_con}.

\begin{definition}
Let $k\leq\om$ and $\M$ be a countable $k$-relevant opm.

A $k$-factor $\pi:\M\to\N$ is \emph{simple} iff it is witnessed by $(\Ll,\sigma)=(\M,\id)$.

An iteration tree is \emph{relevant} iff it has countable, successor length.
We say that $(\Tt,\Q,\pi)$ is \emph{$(\M,k)$-simple} iff
$\Tt$ is a relevant $(k,\infty,\infty)$-maximal tree,
$\Q\wins M^\Tt_\infty$ and $\pi:\M\to\Q$ is a good simple $k$-factor.\footnote{
So $\Q$ is $k$-sound; the $(k,\infty,\infty)$-maximality of $\Tt$ then implies that if
$\Q=M^\Tt_\infty$ then $\deg^\Tt(\infty)\geq k$.
So we do not need to explicitly stipulate that $\deg^\Tt(\infty)\geq k$, unlike in \cite{copy_con}.}

Let $\Sigma$ be an iteration strategy 
for $\M$. Let $\alphavec=\left<\alpha_n\right>_{n<\om}$ enumerate $\OR(\M)$. We say that $\Sigma$ 
has the 
\emph{$k$-simple Dodd-Jensen \tu{(}DJ\tu{)} property for $\alphavec$} iff for all 
$(\M,k)$-simple $(\Tt,\Q,\pi)$ with $\Tt$ via 
$\Sigma$, we have $\Q=M^\Tt_\infty$ and $b^\Tt$ does not drop in model (or degree),
and if $\pi$ is also nearly $k$-good, then
\[ i^\Tt\rest\OR(\M)\leq^{\alphavec}_\lex\pi\rest\OR(\M) \]
(that is, either $i^\Tt\rest\OR(\M)=\pi\rest\OR(\M)$, or $i^\Tt(\alpha_n)<\pi(\alpha_n)$ where 
$n<\om$ is least such that $i^\Tt(\alpha_n)\neq\pi(\alpha_n)$).
\end{definition}

Note that in the context above, if 
$i^\Tt\rest\OR(\M)=\pi\rest\OR(\M)$, then $i^\Tt=\pi$, because $i^\Tt,\pi$ are both nearly $0$-good,
and $\M=\Hull_1^\M(\hmb^\M\un\OR(\M))$.

\begin{lemma}\label{lem:k-factor+weak_DJ}
 Let $(\Fop,b,A)$ be an almost fine ground with $A\in\HC$.
 Let $\M$ be a countable, $\Fop$-$(k,\om_1,\om_1+1)$-maximally iterable $k$-relevant $\Fop$-opm.
 Let $\alphavec=\left<\alpha_n\right>_{n<\om}$ enumerate $\OR(\M)$.
 Then there is an $\Fop$-$(k,\om_1,\om_1+1)$-maximal strategy for $\M$ with the 
$k$-simple 
DJ property for $\alphavec$.
\end{lemma}
\begin{proof}[Proof Sketch]
 The proof is mostly like the usual one (see \cite{wDJ}), with adaptations much as in 
\cite[***check ref: Lemma 4.6]{copy_con}.
 Let $\Sigma$ be an $\Fop$-$(k,\om_1,\om_1+1)$-maximal strategy for $\M$.
 Given a relevant tree $\Tt$ via $\Sigma$, $\P=M^\Tt_\infty$ and 
$m=\deg^\Tt(\infty)$, let $\Sigma^\Tt_\P$ be the $(m,\om_1,\om_1+1)$-maximal tail of $\Sigma$ for 
$\P$. If $(\Tt,\Q,\pi)$ is also $(\M,k)$-simple,
let $\Sigma^{\Tt,\Q,\pi}_\M$ be the $(k,\om_1,\om_1+1)$-maximal strategy for $\M$
given by $\pi$-pullback (as in \ref{lem:strategy_copying}).

Note that $(\Tt,\M,\id)$ is $(\M,k)$-simple where $\Tt$ is trivial on $\M$.
Let $(\Tt_0,\Q_0,\pi_0)$ be $(\M,k)$-simple, 
with $\Tt_0$ via $\Sigma$, and $\P_0=M^{\Tt_0}_\infty$,
such that for any $(\M,k)$-simple $(\Tt,\Q,\pi)$ via $\Sigma^{\Tt_0}_{\P_0}$, we have that 
$b^\Tt$ 
does not drop in model or degree,
if $\Q_0=\P_0$ then $\Q=M^\Tt_\infty$,
and if $\Q_0\wpins\P_0$ then $(i^\Tt)^\uparrow(\Q_0)\wins\Q$ (see \ref{dfn:uparrow}).

Let $\Sigma_1=\Sigma^{\Tt_0,\Q_0,\pi_0}_\M$. Working as in the standard proof (see \cite{wDJ}), let 
$\Tt_1$ be a relevant tree via $\Sigma_1$, with $b^{\Tt_1}$ not dropping in model or degree,
and let $\pi_1:\M\to\P_1= M^{\Tt_1}_\infty$ be nearly $k$-good,
such that for all relevant trees $\Tt$ via $\Sigma^{\Tt_1}_{\P_1}$,
if $b^{\Tt}$ does not drop in model or degree, then for any near $k$-embedding 
$\pi:\M\to\M^\Tt_\infty$, we have $i^\Tt\com\pi_1\leq^{\alphavec}_\lex\pi$.

Let $\Sigma_2=(\Sigma_1)^{\Tt_1,\P_1,\pi_1}_\M$. Then
$\Sigma_2$ is as desired; cf. \cite{copy_con}. 
(Use the propagation of near embeddings after drops in model given by 
\ref{lem:strategy_copying}, as in \cite{copy_con}.)
\end{proof}
\begin{definition}
 Let $\M$ be a $k$-sound opm and let $q=p_{k+1}^\M$. For $i<\lh(p_{k+1}^\M)$,
 $\Hh=\solwit_{k+1,i}(\M)$ denotes the corresponding solidity witness
 \[ \Hh=\cHull_{k+1}^\M(q_i\un\{q\rest i\}\un\pvec_k^\M), \]
 and $\varsigma_{k+1,i}(\M)$ denotes the uncollapse map $\Hh\to\M$.
\end{definition}

We can now state the central result of this section -- the fundamental fine structural facts for 
$\Fop$-opremice. The definitions \emph{$\Fop$-pseudo-premouse} and
\emph{$\Fop$-bicephalus}, and the \emph{$\Fop$-iterability} of such structures, are the obvious 
ones. Likewise the definition of \emph{$\Fop$-iterability} for phalanxes of $\Fop$-opms.

\begin{theorem}\label{lem:k+1-fineness}
Let $(\Fop,b,A)$ be an almost fine ground with $b\in\HC$.
Then:
\begin{enumerate}
\item\label{item:k+1-fine} For $k<\om$, every $k$-sound, $\Fop$-$(k,\om_1,\om_1+1)$-maximally 
iterable $\Fop$-opremouse over $A$ is 
$\Fop$-$(k+1)$-fine.
 \item\label{item:condensing} Every $\om$-sound, $\Fop$-$(\om,\om_1,\om_1+1)$-maximally iterable 
$\Fop$-opremouse over $A$ is condensing.
\item\label{item:pseudo-pm} Every $\Fop$-$(0,\om_1,\om_1+1)$-maximally iterable 
$\Fop$-pseudo-premouse over $A$ is an 
$\Fop$-opremouse.
\item\label{item:bicephalus} There is no $\Fop$-$(0,\om_1,\om_1+1)$-maximally iterable 
$\Fop$-bicephalus over $A$.
\end{enumerate}
\end{theorem}
\begin{proof}[Proof Sketch]
We sketch enough of the proof of parts \ref{item:k+1-fine} and \ref{item:condensing}, focusing 
on the new aspects, that by combining these sketches with the full proofs of these facts for 
standard premice, one obtains a complete proof. So one should have those proofs in mind (see 
\cite{fsit}, \cite{outline}, \cite{copy_con}). Part
\ref{item:pseudo-pm} involves similar modifications to the standard proof,
and part \ref{item:bicephalus} is an immediate transcription.
We begin with part \ref{item:k+1-fine}.

Let $\M$ be a $k$-sound, $\Fop$-$(k,\om_1,\om_1+1)$-maximally iterable $\Fop$-opremouse.
We may assume that $\rho_{k+1}^\M<\rho_k^\M$,
and by \ref{lem:non_k-rpm_sound}, that $\M$ is $k$-relevant.
We may assume that $\M$ is countable (otherwise we can replace $\M$ with a countable 
elementary substructure, because $\Fop$ almost condenses coarsely above $b\in\HC$ and 
$\opbk\sats\DC$).
Using \ref{lem:k-factor+weak_DJ}, let $\Sigma$ be an $\Fop$-$(k,\om_1+1)$ iteration strategy 
for $\M$ with the $k$-simple DJ property for some enumeration of $\OR(\M)$.
We assume that $\M$ is a successor, since the contrary case is simpler and closer to the 
standard proof.

We first establish $(k+1)$-universality and that $\Cc=\core_{k+1}(\M)$ is an $\Fop$-opm.
Let $\pi:\Cc\to\M$ be the core map.
We may assume that $\M$ is $k$-relevant, because otherwise $\Cc=\M$ and $\pi=\id$.

First suppose $k=0$, and consider $1$-universality.
Because $\pi$ is $0$-good and by \ref{lem:Qformula_pres_weak0}, $\Cc$ is a 
Q-opm, $\Cc$ is a successor and $\pi(\Cc^-)=\M^-$.
By fine condensation and \ref{lem:strengthen_scf_conclusion}, $\Hh=\Fop(\Cc^-)$ is a universal 
hull of $\Cc$, as witnessed by $\sigma:\Hh\to\Cc$.
Also, $\Cc$ is $0$-relevant. For otherwise, by the proof of \ref{lem:strengthen_scf_conclusion},
$\Hh\in\M$, but then $\Cc\in\M$, a contradiction. 
So
\[ \rho\eqdef\rho_1^\M=\rho_1^\Cc<\rho_\om^{\Cc^-}, \]
and since $\Hh^-=\Cc^-$, therefore $\Cc\wdoubleupto(\rho^+)^\Cc=\Hh\wdoubleupto(\rho^+)^\Hh$.
So it suffices to see that $\M\wdoubleupto(\rho^+)^\M=\Hh\wdoubleupto(\rho^+)^\Hh$.

Let $\rho=\rho_1^\M$. The phalanx
$\ph=((\M,{<\rho}),\Hh)$
is $\Fop$-$((0,0),\om_1+1)$-maximally iterable.\footnote{A $(k_0,k_1,\ldots,k)$-maximal tree on a 
phalanx $((M_0,\rho_0),(M_1,\rho_1),\ldots,H)$, is one formed according to the usual rules for 
$k$-maximal trees, except that an extender $E$ with $\rho_{i-1}\leq\crit(E)<\rho_i$ (where 
$\rho_{-1}=0$) is applied to $M_i$, at degree $k_i$.} Moreover, we get an 
$\Fop$-$((0,0),\om_1+1)$-iteration strategy for $\ph$ given by lifting to $k$-maximal 
trees on $\M$ via $\Sigma$.
This is proved as usual, using $\pi\com\sigma$ to lift $\Hh$ to $\M$, and using 
calculations as in
\ref{lem:strategy_copying} to see that the strategy is indeed an $\Fop$-strategy.
Since our strategies are $\Fop$-strategies, we can therefore compare $\ph$ with $\M$. 
The analysis of the comparison is mostly routine, using the $k$-simple DJ 
property. (Here all copy 
embeddings are near embeddings, so we only actually need the weak DJ property.)
The only, small, difference is when $b^\Tt$ is above $\Hh$ without drop and 
$M^\Tt_\infty\wins M^\Uu_\infty$. Because $\Hh$ is a universal hull of 
$\Cc=\core_1(\M)$, this implies that $b^\Uu$ does not drop and $M^\Tt_\infty=M^\Uu_\infty$;
now deduce that $\M\wdoubleupto(\rho^+)^\M=\Hh\wdoubleupto(\rho^+)^\Hh$ as usual, completing the 
proof.

We now show that $\Cc=\Hh$, and therefore that $\Cc$ is an $\Fop$-opm.
Because $\Hh$ is a universal hull of $\Cc$ and $\Cc$ is $0$-relevant, we have 
$\rho_1^\Hh=\rho<\rho_\om^{\Hh^-}$ (as $\Hh^-=\Cc^-$) and 
$p_1^\Cc\leq\sigma(p_1^{\Hh})$. But $\Hh$ is $(1,q^\Hh)$-solid,
so $\Cc$ is $(1,\sigma(q^\Hh))$-solid (using stratification), so $\sigma(q^\Hh)\wins p_1^\Cc$.
And since $\sigma$ is above $\Cc^-$, it follows that $\sigma(p_1^\Hh)=p_1^\Cc$. But by 
$1$-universality, $\pi(p_1^\Cc)=p_1^\M$, so $\Cc=\Hull_1^\Cc(A\un\rho\un p_1^\Cc)$,
so $\Hh=\Cc$ and $\sigma=\id$, completing the proof.

Now suppose $k>0$. Then $\Cc=\core_{k+1}(\M)$ is an 
opm by \ref{lem:Sigma_1_hull_reflects_opm}, and is $k$-relevant as 
$\rho_{k+1}^\Cc<\rho_k^\Cc\leq\rho_\om^{\Cc^-}$. So by fine condensation and 
\ref{lem:strengthen_scf_conclusion}, $\Cc=\Fop(\Cc^-)$ is an $\Fop$-opm. The rest is a 
simplification of the argument for $k=0$.

Now consider $(k+1)$-solidity. Let 
$q=p_{k+1}^\M$ and $i<\lh(q)$ and $\Ww=\solwit_{k+1,i}(\M)$ 
and $\pi=\varsigma_{k+1,i}$. We have
\[ \rho_{k+1}^\Ww\leq\mu\eqdef\crit(\pi)=q_i.\]
By \ref{lem:core_embedding} we may assume that $\pi$ is $k$-good, so $\Ww$ is a $k$-sound successor 
Q-opm and $\pi(\Ww^-)=\M^-$. By \ref{lem:succ_opm_top_param} we may assume that 
$\mu<\rho_\om^{\M^-}$, so $\mu\leq\rho_\om^{\Ww^-}$. Suppose $\mu=\rho_\om^{\Ww^-}$.
Then since $\M^-$ is condensing, $\Fop(\Ww^-)\in\M^-$. But by the fine condensation of 
$\Fop$, $\Ww$ is computable from $\Fop(\Ww^-)$, so $\Ww\in\M$, as required. So we may assume that 
$\mu<\rho_\om^{\Ww^-}$, so $\Ww$ is $k$-relevant, so $\Ww\notin\Fop(\Ww^-)$ and if $k=0$ then 
$\Ww$ has no universal hull in $\Fop(\Ww^-)$.

If $k=0$, let $\Hh=\Fop(\Ww^-)$; by fine condensation, $\Hh$ is an $\Fop$-opm, and is a 
universal hull of $\Ww$. If $k>0$ then $\Ww$ is an opm, so by fine condensation, $\Ww=\Fop(\Ww^-)$ 
is an $\Fop$-opm. If $k>0$, let $\Hh=\Ww$.

Let us assume that $\mu$ is not a cardinal of $\M$, since the contrary case is easier.
So $\mu=(\kappa^+)^\Hh=(\kappa^+)^\Ww$ for some $\M$-cardinal $\kappa$.
Let $\R\wpins\M$ be least such that $\mu\leq\OR(\R)$ and $\rho_\om^\R=\kappa$.
Let $\ph=((\M,<\kappa),(\R,<\mu),\Hh)$. Then $\ph$ is $(k,r,k)$-maximally iterable,
where $r$ is least such that $\rho_{r+1}^\R=\kappa$, by lifting to $k$-maximal trees $\Vv$ on $\M$
(possibly $r=-1$, i.e. $\R$ is active type 3 with $\mu=\OR(\R)$).
Let $I\sub\lh(\Vv)$ be the resulting insert set.
 Let $(\Tt,\Uu)$ be the successful comparison of $(\ph,\M)$. The analysis of the comparison is 
now routine except in the case that either (i) $k=0$ and $b^\Tt$ is above $\Hh$ without drop and 
$M^\Tt_\infty\wins M^\Uu_\infty$, or (ii)
$b^\Tt$ is above $\R$ and does not model-drop, $b^\Uu$ does not drop in model or degree and 
$M^\Tt_\infty=\Q=M^\Uu_\infty$. (As in \cite{copy_con}, when we are not in case (ii), the final 
copy map $\pi_\infty$ is a near $\deg^\Tt(\infty)$-embedding.)

We deal with case (i) much as in the proof of $1$-universality. Let $\Hh'=M^\Tt_\infty$.
Suppose that $b^\Uu$ does not drop and $\Hh'=M^\Uu_\infty$.
As usual, we have that $\rho\leq\crit(i^\Uu)$. So letting $t=\Th_1^\M(A\un\rho\un p_1^\M)$,
$t$ is $\bfSigma_1^{\Hh'}$, so is $\bfSigma_1^{\Hh}$, so is $\bfSigma_1^{\Ww}$, a 
contradiction as usual. So either $b^\Uu$ drops or $\Hh'\wpins M^\Uu_\infty$. But then as usual, 
$\Hh\in\M$, so $\Ww\in\M$, so we are done.

Now consider case (ii), under which $r\geq 0$.
So $k\leq l\eqdef\deg^\Tt(\infty)$, and the final copy map
$\pi_\infty:M^\Tt_\infty\to M^{\Vv,I}_{\R,\infty}$ is a weak $l$-embedding. If $k<l$ then 
$\pi_\infty$ is near $k$, which contradicts $k$-simple DJ (in fact weak DJ).
So suppose $k=l$. If $k=r$ then fairly standard arguments (such as in \cite{copy_con}) give a 
contradiction, so suppose $k<r$. Then
\[ \pi_\infty\com i^\Uu:\M\to M^{\Vv,I}_{\R,\infty} \]
is a good simple $k$-factor, as witnessed by $\L=\M$ and $\sigma=\id$; indeed,
\[ \pi_\infty\com i^\Uu\com\sigma_{k+1}^\M:\mathfrak{S}_{k+1}(\M)\to M^{\Vv,I}_{\R,\infty} \]
is nearly $k$-good, which is proved just as in \cite{copy_con}, which also implies that 
$\pi_\infty\com i^\Uu$ is weakly $k$-good, because $\sigma^\M_{k+1}$ is $k$-good. Since
$\R\wpins\M$, this contradicts $k$-simple DJ. (This is the only place we need $k$-simple DJ beyond 
weak DJ.)

Now consider part \ref{item:condensing}. Let $k<\om$ and 
let $\Hh$ be a $(k+1)$-sound potential opm which is soundly projecting. Let 
$\pi:\Hh\to\M$ be nearly $k$-good, with $\rho=\rho_{k+1}^\Hh<\rho_{k+1}^\M$. Then $\Hh$ is in fact 
an opm. Let us assume that $\Hh,\M$ are both successors, so $\pi(\Hh^-)=\M^-$. By fine condensation 
of $\Fop$, $\Hh^-$ is an $\Fop$-opm, and either $\Hh\in\Fop(\Hh^-)$ or $\Hh=\Fop(\Hh^-)$.
If $\Hh$ is not $k$-relevant then the result follows from the fact that $\M^-$ is condensing and 
$\Hh^-$ is an $\Fop$-opm. So assume $\Hh$ is $k$-relevant, so $\Hh=\Fop(\Hh^-)$.

Now use weak DJ (at degree $\om$) and the usual phalanx comparison argument to reach the desired 
conclusion.
Say $\ph=((\M,{<\rho}),\Hh)$ is the phalanx. Then $\ph$ is $\Fop$-$((\om,k),\om_1+1)$-iterable,
lifting to $\Fop$-$(\om,\om)$-maximal trees $\Vv$ on $\M$. (It could be that $\M$ is not 
$k$-relevant. So we want to keep the degrees of nodes of $\Vv$ at $\om$ where possible,
to ensure that each $M^\Vv_\alpha$ is an $\Fop$-opm.) Suppose $\Tt$ is non-trivial. Because 
$k<\om$, 
if $M^\Tt_\infty$ is above $\Hh$ without drop in model or degree, $\pi_\infty$ need only be a weak 
$k$-embedding.
But in this case, $M^\Tt_\infty$ is not $\om$-sound, which implies
$M^\Uu_\infty\wpins M^\Tt_\infty$, which contradicts weak DJ. The rest is routine.
\end{proof}



The operators we define in the paper will be extracted from $\J$-structures.

\begin{definition}[$\J$-structure]
Let $\alpha\in\Ord\cut\{0\}$, let $Y$ be an operatic argument, let
\[ D=\Lim\inter[\OR(Y)+\om,\OR(Y)+\om\alpha) \]
and let $\hmPvec=\left<\hmP_\beta\right>_{\beta\in D}$ be given.

We define $\J_\beta^{\hmPvec}(Y)$ for $\beta\in[1,\alpha]$, if possible, by recursion on 
$\beta$, as follows. We set
$\J_1^{\hmPvec}(Y)=\J(Y)$ and take unions at limit $\beta$.
For $\beta+1\in[2,\alpha]$, let $\R=\J_\beta^{\Pvec}(Y)$ and suppose that 
$\hmPvec_{\OR(\R)}=(\hmP_{0},\ldots,\hmP_{n-1})$ for some $n<\om$, and that for each $i<n$, 
$\hmP_i\sub\R$ and is amenable to $\R$. In this case we define
\[ 
\J_{\beta+1}^{\hmPvec}(Y)=\J(\R,\hmPvec\rest\R,\hmP_{0},\ldots,\hmP_{n-1}).
 \]
Note then that by induction, 
$\hmPvec\rest\R\sub\R$ and $\hmPvec\rest\R$ is amenable to 
$\R$.

For $m,n<\om$ let $\Ll_{\J,m,n}$ be the language with binary relation 
symbol 
$\dot{\in}$, 
predicate 
symbols $\dot{\hmPvec}$ and 
$\hmPdot_i$ for $i<m$, constant symbol $\hmbdot$ and constant 
symbols $\hmpdot_i$ for $i<n$.


Let $Y$ be an operatic argument, $m,n<\om$ and $q_0,\ldots,q_{n-1}\in\J(Y)$.
A \emph{$\J$-structure \tu{(}over $Y$, of signature 
$(m,n)$\tu{)}} is an amenable
$\Ll_{\J,m,n}$-structure
\[ \M=(\J_{\alpha}^\hmPvec(Y),\hmPvec,\hmP_0,\ldots,\hmP_{m-1},Y,q_0,\ldots,q_{n-1}), \]
where $\alpha\in\Ord\cut\{0\}$ and $\hmPvec=\left<\hmPvec_{\gamma}\right>_{\gamma\in D}$ 
with domain $D$ defined as above, 
$\univ{\M}=\J_\alpha^{\hmPvec}(Y)$ is defined, $\lh(\hmPvec_\gamma)=n$, $\dot{\hmPvec}^\M=\hmPvec$, 
$\hmPdot_i^\M=\hmP_i$, $\hmbdot^\M=Y$, 
$\hmpdot^\M_i=\hmpv_i$, and $\dot{\in}^\M={\in\inter\univ{\M}}$.

Let $\M$ be a $\J$-structure of signature $(m,n)$, and adopt the notation above. Let 
$\l(\M)$ denote $\alpha$. For 
$\beta\in[1,\alpha]$ and $\R=\J_\beta^{\hmPvec}(Y)$ and $\gamma=\OR(\R)$, let
\[ 
\M|\beta=(\R,\hmPvec\rest\R,\hmPvec_{\gamma,0},\ldots,\hmPvec_{\gamma,m-1},Y,\hmpv_0,\ldots,
\hmpv_{n-1}), \]
where $\hmPvec_{\OR(\M),i}=\hmP_i$.
We write $\N\ins\M$, and say that $\N$ is an \emph{initial segment} of $\M$, iff $\N=\M|\beta$ for 
some $\beta$. Clearly if $\N\ins\M$ then 
$\N$ is 
an $\J$-structure (over $Y$, of signature $(m,n)$).
We write $\N\pins\M$, and say that $\N$ is a \emph{proper segment} of $\M$, iff $\N\ins\M$ but 
$\N\neq\M$.

An $(m,n)$-$\J$\emph{-structure} is a $\J$-structure of signature $(m,n)$.
Let $\M$ be an $(m,n)$-$\J$-structure. The \emph{fine-structural notions} for 
$\M$ are those for $(\M,\Ll_{\J,m,n})$.
(Note that $\M$ is pre-fine.)
\end{definition}

\begin{definition}[Pre-operator]
Let $\opbk$ be an operator background.
A \emph{pre-operator over $\opbk$} is a function $G:D\to\opbk$, with $D$ an operatic 
domain over $\opbk$, such that for each $Y\in D$, $G(Y)$ is a $(1,1)$-$\J$-structure $\M$ 
over $Y$
such that (i) if $Y\in P^D$ then $\hmp^\M=\hmp^Y$,
(ii) every $\N\ins\M$ is $\om$-sound, and (iii) for some 
$n<\om$, 
$\rho_{n+1}^\M=\om$. Let $C^G=C^D$ and $P^G=P^D$.
\end{definition}

\begin{definition}[Operator $\Fop_G$]\label{dfn:operator_Fop_G}
Let $G$ be a pre-operator over $\opbk$, with domain $D$. We define
a corresponding operator $\Fop=\Fop_G$, also with domain $D$, as follows.

Let $X\in\witri{C^{D}}$ and 
$\N=G(X)=(\univ{\N},\hmPvec^\N,\hmP^\N,X,\hmpv)$.
Let $n<\om$ be such 
that $\rho_{n+1}^\N=\om$ and $\OR(X)<\rho_{n}^\N$.
If $n=0$ then let $\M=\N$.
If $n>0$ then let $\sigma=\rho_{n}^\N$ and $\Q=\N\Jupto\sigma$ and let $\M$ be the 
$(1,1)$-$\J$-structure
\[ \M=(\univ{\Q},\hmPvec^\N\rest\sigma,T,X,\hmpv),\]
where $T\sub\univ{\Q}$
codes
\[ \Th_{\rSigma_n}^\N(\univ{\Q}\un\pvec_{n}^\N) \]
in some uniform fashion, amenably to $\univ{\Q}$, such as with mastercodes.\footnote{For 
concreteness, we take $T$ to be the set of pairs $(\alpha,t')$ such that for some $t$,
$(\pvec_{n}^\M,\alpha,t)\in T_{n}^\M$, and $t'$ results from $t$
by replacing $\pvec_{n}^\M$ with $\R$ (the latter is not a parameter
of the theory $t$, so we can unambiguously use it as a constant symbol).}
Note that in either case, $\M=(\univ{\M},\hmPvec^\M,\hmP^\M,X,p)$ is an $\om$-sound 
$\J$-structure over $X$ and $\rho_{1}^{\M}=\om$.

Define $\Fop(X)$ as the hierarchical model $\K$ over $X$ with parameter $\hmpv$, of length $1$
(so $\hmS^{\K}=\emptyset$), with $\univ{\K}=\univ{\M}$,
$\hmE^{\K}=\emptyset$, and
\[ \hmP^{\K}=\{X\}\cross\left(\hmPvec^\M\oplus\hmP^\M\right).\]
(We use $\{X\}\cross\cdots$ to ensure that $\hmP^\K\sub\K\cut\K^-$.)

Now let $\R\in P^D$; we define $\Fop(\R)$.
Let
$A=\hmb^\R$ and $\rho=\rho_\om^\R$. 
Let $\P=G(\R)$. Let $\N\ins\P$ be largest such that for all $\alpha<\rho$, we have
\[ 
\pow(A^{<\om}\cross\alpha^{<\om})^\N=\pow(A^{<\om}\cross\alpha^{<\om}
)^\R. \]
Let $n<\om$ be such that
$\rho_{n+1}^\N=\om$ and $\OR(\R)<\rho_{n}^\N$. Now define $\M$ from $(\N,n)$ as in the 
definition of $\Fop(X)$ for $X\in 
\witri{C^{D}}$, but with $\hmb^\M=\R$ and $\hmp^\M=\hmp^\R$. 
Much as there, $\M=(\univ{\M},\hmPvec^\M,\hmP^\M,\R,\hmp^\R)$ is an $\om$-sound 
$\J$-structure over $\R$ and $\rho_{1}^{\M}=\om$.

Now set $\Fop(\R)$ to be the unique 
hierarchical model $\K$ of length $\wl(\R)+1$ with $\univ{\K}=\univ{\M}$,
$\R\wpins\K$ (so $\hmS^\K=\hmS^\R\conc\left<\R\right>$), $E^{\K}=\emptyset$, and
\[ \hmP^{\K}=\{\R\}\cross\left(\hmPvec^\M\oplus\hmP^\M\right). \]

This completes the definition.

Let $\R\in D$. We say that $\Fop(\R)$ \emph{projects early} iff $\R\in P^D$ and with $\N,\P$ as in 
the definition of $\Fop(\R)$ above, we have $\N\pins\P$. Note that if $\Fop(\R)$ does not project 
early, then $\Fop(\R)$ easily codes $G(\R)$.
\end{definition}

$\Fop_G$ is indeed an operator:

\begin{lemma}\label{lem:operator_Fop_G}
 Let $G$ be a pre-operator over $\opbk$ with domain $D$. Then
 $\Fop_G$ is an operator over $\opbk$. Moreover, for any $\Fop_G$-opremouse $\M$ of
length $\alpha+\om$, for all sufficiently large $n<\om$, 
$\Fop_G(\M\wupto(\alpha+n))$ 
does not project early.
\end{lemma}
\begin{proof}[Proof Sketch]
We first show that $\Fop_G$ is an operator.
Let $\Fop=\Fop_G$ and $X\in D=\dom(\Fop)$. We must verify that 
$\M=\Fop(X)$ is an opm. This follows from (i) the choice of $\univ{\Fop(X)}$ (i.e. the choice 
of $\N\ins G(X)$ in the definition of $\Fop(X)$, which gives, for example, projectum 
amenability 
for $\Fop(X)$), (ii) if $X\in P^{D}$ then $X$ is 
an $\om$-sound opm (acceptability follows from this and projectum amenability), (iii) standard 
properties of 
$\J$-structures (e.g. for stratification), and (iv) with $\P$ as in the definition 
$\Fop(X)$, the fact that $\P$ is $\om$-sound
and $\rho_{1}^\P=\om$ (for
sound projection).

Now let $\M$ be an $\Fop$-opremouse of limit length $\alpha+\om$. Then for all $m$,
\[ \rho_\om^{\M\wupto(\alpha+m+1)}\leq\rho_\om^{\M\wupto(\alpha+m)}, \]
because $\M\wupto(\alpha+m+1)$ 
is soundly projecting and $\M\wupto(\alpha+m)$ is $\om$-sound. So if $n<\om$ is such that 
$\rho_\om^{\M\wupto(\alpha+n)}$ is as small as possible, $n$ works.
\end{proof}

So any limit length $\Fop_G$-opremouse $\M$ is ``closed under $G$'' in the sense that for 
$\in$-cofinally many $X\in\M$, we have $G(X)\in\M$.

\begin{definition}
Let $\M$ be an opm and $\N\wins\M$. We say that $\N$ is an \textbf{cutpoint} of $\M$ 
iff for all $\P\wins\M$, if $\N\wpins\P$ and $\actext^\P\neq\emptyset$ then
$\OR(\N)\leq\crit(\actext^\P)$.
And $\N$ is a \textbf{strong cutpoint} of $\M$ iff likewise, but with the conclusion 
replaced with ``$\OR(\N)<\crit(\actext^\P)$''.
\end{definition}

\begin{definition}[$\Lp^\Fop$]
Let $\Fop$ be an operator over $\opbk$, with $C_\Fop$ the cone above some element of $\HC$.

Let $\M\in\opbk$ be an $\Fop$-opm and let $n\leq\om$ (and 
$\eta\leq\OR(\M)$). We say that 
$\M$ is \textbf{countably (above-$\eta$) $\Fop$-$(n,\om_1+1)$-iterable} iff
for every countable elementary substructure $\bar{\M}$ of $\M$, 
$\bar{\M}$ is 
an (above-$\bar{\eta}$) $\Fop$-$(n,\om_1+1)$-iterable $\Fop$-opm (where $\bar{\eta}$ is 
the collapse of $\eta$).

Let $x\in C_\Fop$ be transitive. Then 
$\Lp^\Fop(x)$ denotes the stack of all 
countably $\Fop$-$(\om,\om_1+1)$-iterable $\Fop$-opremice $\M$ over $\hat{x}$ such that $\M$ is 
fully sound 
and projects to $\om$.\footnote{This is indeed a stack because $\opbk\sats\DC$, which ensures that 
we can form countable elementary substructures.}
Assuming that 
$\RR\in\opbk$, for $X\sub\HC$, $\Lp^\Fop(\RR,X)$ 
denotes $\Lp^\Fop((\HC,X))$, and $\Lp^\Fop(\RR)$ denotes $\Lp^\Fop(\HC)$.\footnote{Since $\RR$ 
is not transitive, this is not an abuse of notation.}

Let $\N\in\opbk$ be an $\Fop$-opremouse. Then 
$\Lp^\Fop_+(\N)$ 
denotes the stack 
of all $\Fop$-opremice $\M$ such that either $\M=\N$, or $\N\wpins\M$, $\N$ is a strong cutpoint 
of 
$\M$,
$\M$ is $\OR(\N)$-sound, and there is $n<\om$ such that $\rho_{n+1}^\M\leq\OR(\N)<\rho_n^\M$ 
and $\M$ is countably above-$\OR(\N)$ 
$\Fop$-$(n,\om_1+1)$-iterable. Note that $\Lp_+^\Fop(\N)$ might have a largest element, which 
projects strictly across $\OR(\N)$ and is not $\om$-sound.

We write $\Lp,\Lp_+$ for the corresponding notions for standard premice.
So these are essentially equivalent to $\Lp^{\J^\op}$ and $\Lp^{\J^\op}_+$.
\end{definition}

\begin{example}
Let $\varphi\in\Ll_0$. Let $\opbk$ be an operator background. Suppose that for every transitive 
structure $x\in\opbk$ there is $\M\pins\Lp(x)$ such that $\M\sats\varphi$, and let $\M_x$ be the 
least such. Let $G:\opbk\partialto\opbk$ be the pre-operator 
where for $x$ as above, $G(\hat{x})$ is the $(1,1)$-$\J$-structure over $\hat{x}$ naturally 
coding $\M_x$.

The \emph{mouse operator} $\Fop_\varphi$ determined by $\varphi$ is $\Fop_{G_\varphi}$.
A straightforward argument shows that $\Fop_{\varphi}$ almost condenses finely.
We describe some of this argument, to provide some post-motivation for part of the definition of 
\emph{condenses finely}. Let $\Fop=\Fop_\varphi$, let $\N$ be a successor $\Fop$-opm.
Let $\M$ be a successor Q-opm with $\rho_1^\M\leq\OR(\M^-)$ and let $\pi:\M\to\N$ be a 
$0$-embedding, so $\pi(\M^-)=\N^-$. But $\M$ might not be an opm. Let 
$\N^*\pins\Lp(\N^-)$ be the premouse over $\widehat{\N^-}$ coded by $\N$. (So $\N^*$ has no proper 
segment satisfying $\varphi$, and either $\N^*\sats\varphi$ or $\N^*$ projects 
$<\rho_\om^{\N^-}$.) Let $n<\om$ be such that $\rho_{n+1}^{\N^*}\leq\OR(\N^-)<\rho_n^{\N^*}$. Then 
there is an $n$-sound premouse $\M^*$ over $\widehat{\M^-}$
and an $n$-embedding $\pi^*:\M^*\to\N^*$ with $\pi\sub\pi^*$. Because $\rho_1^\M\leq\OR(\M^-)$,
$\rho_{n+1}^{\M^*}\leq\OR(\M^-)$. So \emph{if} $\M^*$ is sound, then 
$\M^*\pins\Lp(\M^-)$, and it is easy to see that $\M^*\ins\M'$, where $\M'$ is the premouse 
coded by $\Fop(\M^-)$.
Suppose soundness fails, and let $\Hh^*=\core_{n+1}(\M^*)$. Then $\Hh^*\ins\M'$, and the 
$n^\nth$ master code $\Hh$ of $\Hh^*$ is a universal hull of $\M$, and either 
$\Hh\in\Fop(\M^-)$ or $\Hh=\Fop(\M^-)$, as required. Note that we made significant use of the fact 
that $\rho_1^\M\leq\OR(\M^-)$.
\end{example}

==> scales_J_premice_over_b.tex <==
We next work on defining g-organized $J$-premice. As mentioned in the 
introduction, the main point of this definition is due to Sargsyan:

\begin{definition}[Sargsyan, \cite{ATHM}]
Let $M$ be a transitive structure. Let $\dot{G}$ be the canonical
$Col(\omega,M)$-name
for the generic $G\subseteq Col(\omega,M)$ and $\dot{x}_{\dot{G}}$ be the
canonical name for the real coding $\{(n,m) \ | \ G(n) \in G(m)\}$, where we
identify $G$ with $\bigcup G$. Let $\Lambda$ be the strategy for $\MJsharp
=_{\textrm{def}} \M_1^{J,\sharp}$, where $J$ is a nice operator. The \emph{tree
$\Tt_M$ for making $M$
generically generic}, is the iteration tree $\Tt$ on $\MJsharp$ of maximal 
length such
that:
\begin{enumerate}
\item $\Tt$ is via $\Lambda$ and is everywhere non-dropping.
\item $\Tt\rest o^M$ is a linear iteration tree obtained by
iterating the first total measure of $\MJsharp$ and its images $\leq o^M$
times.
\item Suppose $\lh(\Tt)\geq o^M+2$ and let $\alpha+1\in(o^M,\lh(\Tt))$.
Let $\delta=\delta(\M^\Tt_\alpha)$ and let $\BB=\BB(M^\Tt_\alpha)$ be the 
extender algebra of
$M^\Tt_\alpha$ at $\delta$. Then $E^\mathcal{T}_\alpha$ is the extender $E$ with
least index in $M^\mathcal{T}_\alpha$ such that for some condition
$p\in\Coll(\omega,M)$, $p \Vdash$``There is a $\mathbb{B}$-axiom induced
by $E$ which fails for $\dot{x}_{\dot{G}}$''.
\end{enumerate}
Assuming that $\MJsharp$ is sufficiently iterable, then $\Tt_M$ exists, has 
successor length, and $\lh(\Tt_M) < |M|^+$.
\end{definition}

Sargsyan noticed that, in building a $J$-premouse $\N$, one can feed in $J$
indirectly, by instead feeding in the branches for $\Tt_\M$, for various 
$\M\ins\N$. The operator $F_J^*$, defined below, and used in building 
g-organized $J$-premice, feeds in 
branches for such $\Tt_\M$. We will also ensure that being such a structure is 
first-order - other than wellfoundedness and the correctness of the branches - 
by allowing sufficient spacing between these branches.

Before giving the definition we fix some notation. Let
$\varphi$ be a formula such that for some $\gamma>\delta^\MJsharp$,
$\MJsharp|\gamma\sats\varphi$. Given a tree $\Tt$ on $\MJsharp$ using only 
total extenders, let
$P^\varphi(\Tt)$
be the least $P\ins\N^\Tt$ such that for some cardinal $\delta'$ of
$\N^\Tt$, we have
$\delta'<\OR^P$ and $P\sats\varphi+$``$\delta'$ is Woodin''. Let
$\lambda=\lambda^\varphi(\Tt)$ be
least such that $P^\varphi(\Tt)\ins M^\Tt_\lambda$. Then $\delta'$ is a
cardinal of $M^\Tt_\lambda$. Let $I^\varphi=I^\varphi(\Tt)$ be
the set of limit ordinals $\leq\lambda$.

Fix a pair $(\varphi,\psi)$ that generically determines
$J$, for the remainder of the paper.

\begin{definition}[$F_J^*$]
\label{modelOpGenerala2}
Let $b$ be a transitive structure coding $\MJsharp$.
%footnote
\footnote{It seems we might have avoided identifying $\M_1^{J,\sharp}$
explicitly, by
proceeding as in the following sketch. Suppose we have $\M|\alpha$ for some
$\alpha$.
Let $\tilde{J}=J^{\M|\alpha}$ be the partial operator which has been defined so
far.
Let $\tilde{Q}$ be the function defined as follows: Let $H$ be a transitive
set. Suppose there is $\gamma\in\OR$ such that $Q=\J_\gamma^{\tilde{J}}(H)$ is
defined (i.e., $\tilde{J}$ is defined sufficiently for this), and $Q$ is a
Q-structure for $H$. Then set $\tilde{Q}(H)=Q$. Otherwise $\tilde{Q}(H)$ is
undefined. Then $\M|\alpha$ can define
``$\M_1^{\dot{J}\sharp}$-like, $\tilde{J}$-consistently $\tilde{J}$-short tree
iterable premouse'' using $\tilde{Q}$: this is a sound premouse $\N$ satisfying
``I am $\M_1^{\dot{J}\sharp}$ for some operator $\dot{J}$'', and for every
$\tilde{Q}$-guided tree $\Tt$ on $\N$: (a) every model of $\Tt$ is
consistent with $\tilde{J}$; (b) if $\Tt$ has successor length, then it is
normally extendible (to more wellfounded models), and if $b^\Tt$ does not drop,
then the active extender of $M^\Tt_b$ is iterable; (c) if $\Tt$ has limit
length, and if $Q=\tilde{Q}(M(\Tt))$ is defined, then there is a $\Tt$-cofinal
branch $b$ such that $Q\ins M^\Tt_b$ and $M^\Tt_b$ is wellfounded. Now,
$\M|\alpha$ can begin comparing all such premice. At limit stages of the
comparison, say with a common part model $\N'$, we feed in $\J_\gamma^J(\N')$,
until reaching $Q=\tilde{Q}(\N')$, if we ever do. After reaching the $Q$, the
comparison can continue. Meanwhile, levels $\M|\beta$ for $\beta>\alpha$ may
have seen more of $J$; i.e. we might have
$J^{\M|\alpha}\subsetneq\J^{\M|\beta}$. Then redefining
$\tilde{J}=J^{\M|\beta}$, we refine the collection of $\tilde{J}$-consistently
$\tilde{J}$-short tree iterable premice, and restart the comparison accordingly.
While comparing, we should also be making levels $\M|\beta$ generic over the
iterates. Thus, whenever we reach a limit stage $\N'$ and some
$\P\pins\tilde{Q}(\N')$ such that $\P\models\varphi$, we can certainly compute
more of $\tilde{J}$.}
%end footnote
We define $\M=F_J^*(b)$, a $\J$-model with parameter $b$, as follows.

For each $\alpha\leq\l(\M)$, $E^{\M|\alpha}=\emptyset$.

Let $\alpha_0$ be the least $\alpha$ such that $\J_\alpha(b)\sats\ZF$. Then 
$\M|\alpha_0=\Jop_{\alpha_0}(b)$.

Let $\Tt=\Tt_{\M|\alpha_0}$. Note that $\Tt\rest\alpha_0+1$ is just the linear 
iteration of $\MJsharp$ via its least total measure.
We use the notation $P^\varphi=P^\varphi(\Tt)$, 
$\lambda$, etc, described above.
The predicates
$B^{\M|\gamma}$ for $\alpha_0<\gamma\leq\l(\M)$ will be used to feed in branches
for $\Tt\rest\lambda+1$, and therefore $P^\varphi$ itself, into $\M$. Let 
$\left<\xi_\alpha\right>_{\alpha<\iota}$ enumerate 
$I^\varphi\un\{0\}\inter(\lambda+1)$.

There is a closed, increasing sequence of ordinals
$\left<\eta_\alpha\right>_{\alpha\leq\iota}$ and an increasing sequence of
ordinals $\left<\gamma_\alpha\right>_{\alpha\leq\iota}$ such that:

\begin{enumerate}
 \item $\eta_1=\gamma_0=\eta_0=\alpha_0$.
 \item For each $\alpha<\iota$, 
$\eta_\alpha\leq\gamma_\alpha\leq\eta_{\alpha+1}$, and if
$\alpha>0$ then $\gamma_\alpha<\eta_{\alpha+1}$.
 \item $\gamma_\iota=\l(\M)$, so $\M=\M|\gamma_\iota$.
 \item\label{item:gamma_alpha} Let $\alpha\in(0,\iota)$. Then $\gamma_\alpha$ 
is the least ordinal of
the form $\eta_\alpha+\tau$ such that
$\Tt\rest\xi_\alpha\in\J_\tau(\M|\eta_\alpha)$ and if 
$\alpha>\alpha_0$ then
$\delta(\Tt\rest\xi_\alpha)<\tau$. (We explain below why such $\tau$ 
exists.) And $\M|\gamma_\alpha= \Jop_\tau(\M|\eta_\alpha)\downarrow b$.
 \item Let $\alpha\in(0,\iota)$. Then
$\M|\eta_{\alpha+1}=\BBB(\M|\gamma_\alpha,\Tt\rest\xi_\alpha,
\Lambda(\Tt\rest\xi_\alpha))\downarrow b$.
 \item Let $\alpha<\iota$ be a limit. Then $\M|\eta_\alpha$ is passive.
 \item $\gamma_\iota$ is the least ordinal of the form $\eta_\iota+\tau$ such
that $\Tt\rest\lambda+1\in\J_{\eta_\iota+\tau}(\M|\eta_\iota)$ and
$\tau>\OR(M^\Tt_\lambda)$. And $\M=\Jop_\tau(\M|\eta_\iota)\downarrow 
b$.\qedhere
\end{enumerate}
\end{definition}

\begin{remark}\label{rem:local_def_P^varphi}
We have $P^\varphi\pins M^\Tt_\lambda\in \M=F_J^*(b)$. In fact, $\{P^\varphi\}$
is $\Sigma_1^{\M}(\{\MJsharp\})$, uniformly in $b$.\footnote{Since
$b=a^\M$, the $\Sigma_1^{\M}$
definition may use $b$ as a parameter.} We leave the proof of this to
the reader, but just note that this uses the fact that the relevant part of the
$\Coll(\om,\M|\alpha_0)$ forcing relation for $F_J^*(b)$ is sufficiently
locally definable. For given
$p\in\Coll(\om,\M|\alpha_0)$, and $\alpha\leq\lambda$, and an extender
$E\in\es(M^\Tt_\alpha)$ such that
$\nu(E)$ is inaccessible in $M^\Tt_\alpha$, the question of whether
$p\forces$``$E$
induces an extender algebra axiom not satisfied by $\dot{x}_{\dot{G}}$'' is 
computed over $\M|(\eta_\iota+\nu(E))$. (Such an axiom has form
\[
\bigvee_{\gamma<\crit(E)}\varphi_\gamma\iff\bigvee_{\gamma<\nu(E)}\varphi_\gamma
,
\]
where for each $\gamma<\nu(E)$, $\varphi_\gamma\in M^\Tt_\alpha|\nu(E)$, so the
forcing relation below $p$ regarding the truth of $\varphi_\gamma$ is computed
somewhere below $\M|(\eta_\iota+\nu(E))$.)

Likewise, in item \ref{item:gamma_alpha} of \ref{modelOpGenerala2}, $\tau$ 
exists. Also, for $\Mbar\ins\M=F_J^*(b)$, the sequences
$\left<\M|\eta_\alpha\right>_{\alpha\leq\iota}\inter\Mbar$ and
$\left<\M|\gamma_\alpha\right>_{\alpha\leq\iota}\inter\Mbar$ and
$\left<\Tt\rest\alpha\right>_{\alpha\leq\lambda+1}\inter\Mbar$ are
$\Sigma_1^{\Mbar}(\{\MJsharp\})$, uniformly in $b$ and $\Mbar$.
\end{remark}



\begin{definition}[g-organized potential $J$-premouse over $b$]
\label{PotJPremice2}
Let $b$ be a transitive structure coding $\MJsharp$.
We say that $\M$ is a \textbf{g-organized potential $J$-premouse over $b$}
iff $\M$ is an acceptable $\J$-model over $b\un\MJsharp\un\{(b,\MJsharp)\}$, 
and 
there is an
ordinal
$\iota$ and an
increasing, closed 
sequence $\left<\zeta_\alpha\right>_{\alpha\leq\iota}$ of ordinals,
such that for each $\alpha\leq\iota$, we have:
\begin{enumerate}
\item $0=\zeta_0\leq\zeta_\alpha\leq\zeta_\iota=l(\M)$ (so $\M|\zeta_0=b$ and
$\M|\zeta_\iota=\M$).
\item If $\alpha+1<\iota$, then
$\M|\zeta_{\alpha+1}=F^*_J(\M|\zeta_\alpha)\downarrow b$.
\item If $\alpha+1=\iota$, then $\M\ins
F^*_J(\M|\zeta_\alpha)\downarrow b$.
\item Let $\zeta=\zeta_\alpha$.
If $\dot{E}^{\M|\zeta}\neq\emptyset$ then $\dot{E}^{\M|\zeta}$ codes an
extender $E$ that coheres
$\M|\zeta$ and satisfies
the obvious modifications of the premouse axioms (in the sense of Definition
2.2.1 of \cite{wilson2012contributions}) and is
$b\times(\gamma+1)$-complete for all $\gamma < \crit(E)$.\footnote{$E$ is
$b\times(\gamma+1)$-complete iff
for all $c\in\lh(E)^{<\om}$ and all $\langle X_x \ | \ x\in b\times
\gamma\rangle\in \M|\zeta$, if $X_x\in E_c$ for each $x\in b\times \gamma$,
then $\cap_{x\in b}X_x \in E_c$.}\qedhere
\end{enumerate}
\end{definition}

\begin{definition}\label{dfn:whole_reorganized}
Let $\M$ be a g-organized potential $J$-premouse over $b$, and adopt the notation of
\ref{PotJPremice2}. We say $\M$ is \textbf{$J$-closed} iff $\iota$ is a limit.
We say $\M$ is \textbf{whole} iff either $\M$ is $J$-closed or $\iota=\alpha+1$
and $\M=F^*_J(\M|\zeta_\alpha)\downarrow b$.\footnote{This use of \emph{whole}
is somewhat different to that in \ref{dfn:whole_strategy}.}
\end{definition}

\begin{remark}\label{rem:sequence_whole_proper_segments}
With notation as above, if $\Mbar\ins\M$, then the sequence of whole proper
segments of $\Mbar$ is $\Sigma_1^{\Mbar}(\{\MJsharp\})$, uniformly in $b$ and 
$\Mbar$.
This follows from the observations in \ref{rem:local_def_P^varphi}.
\end{remark}

A key property of Definition \ref{PotJPremice2} is that it is
suitably preserved under taking hulls, and therefore, for example, a core of
a $J$-premouse over $b$ is a $J$-premouse over $b$:


\begin{lemma}\label{lem:weak_0_hull}
Let $\M$ be a (g-organized potential) $J$-premouse over $b$. Let $\Mbar$ be a
$\J$-model over $\bbar$, and suppose there is an $\MJsharp$-weak
$0$-embedding
$\pi:\Mbar\to\M$. Then $\Mbar$ is a (g-organized potential)
$J$-premouse over $\bbar$. Moreover, if $\M$ is whole then $\Mbar$ is
whole.\footnote{One can prove the same conclusion given instead that $\pi$ is a
weak $0$-embedding with respect to the full language $\Ll_0$ (i.e.,
$\Sigma_0$-elementary, and $\Sigma_1$-elementary on a cofinal set $X$, with
respect to $\Ll_0$). For it is easy enough to see
that every proper segment of $\Mbar$ is a $J$-premouse over $\bbar$. The main
issue is to see that $B^{\Mbar}$ is correct. The elementarity of $\pi$ with
respect to the symbol $\l$ gives that $\Mbar$ and $\M$ either (a) both have
successor length, or (b) both have limit length. Suppose (b) holds. Then $\M$
is not whole, so we just need to see that $\Mbar$ is a $J$-premouse over
$\bbar$. If $\Mbar$ is a limit of proper segments $\Mbar'$ such that
$B^{\Mbar'}=\emptyset$ then $B^{\Mbar}=\emptyset$, since $\pi``B^{\Mbar}\sub
B^\M$
and if $\gamma\in B^\M$ and $\M'\pins\M$ and $\gamma\in\M'$ then
$B^{\M'}\neq\emptyset$; this is just because $\M$ is a $J$-premouse over $b$. It
follows that $\Mbar$ is a $J$-premouse over $\bbar$, as required. Now suppose
(a) holds. Let $\Mbar'$ and $\M'$ be the largest proper segments of $\Mbar$
and $\M$ respectively. By the elementarity of $\pi$, $\pi(\Mbar')=\M'$, and
$\pi\rest\Mbar':\Mbar'\to\M'$ is fully elementary. Case (a) is easy enough
using \ref{lem:Bcondensation}.}
\end{lemma}
\begin{proof}[Proof Sketch]
This follows from \ref{lem:Bcondensation}, the observations in
\ref{rem:local_def_P^varphi} and \ref{rem:sequence_whole_proper_segments} and
the fact that the restriction of
$\Sigma_\MJsharp$ to nowhere-dropping trees has hull condensation (which uses 
the
fact that $J$ condenses well).
\end{proof}


\begin{comment}
The main issue is
whether $B^\Mbar$ is correct, since the $\Sigma_0$-elementarity of $\pi$ ensures
that for each $\Mbar'\pins\Mbar$,
\[ \pi\rest\Mbar':\Mbar'\to\pi(\Mbar') \]
is fully elementary, which gives easily enough that $\Mbar'$ is a
$J$-premouse over $\bbar$, and if $E^\Mbar\neq\emptyset$, then the standard
arguments for premice work.

Suppose $\l(\Mbar)$ is a limit, and $\Mbar$ is a limit of proper segments
$\Mbar'$ such that $B^{\Mbar'}\neq\emptyset$. If $\Mbar$ is also a limit of
proper segments $\Mbar'$ such that $B^{\Mbar'}=\emptyset$, then we just need to
see that $B^\Mbar=\emptyset$. But if not, then since $\pi``B^\Mbar\sub B^\M$,
then $B^\M\neq\emptyset$. Since $\M$ is a $J$-premouse over $b$, for every
$\gamma\in B^\M$, for every $\M'\pins\M$ such that $\gamma\in\M'$, we have
$B^{\M'}\neq\emptyset$. This is a contradiction. So assume that all
sufficiently large $\Mbar'\pins\Mbar$ are such that $B^{\Mbar'}\neq\emptyset$.
Since $\pi$ is a weak $0$-embedding, all sufficiently large
$\M'\pins\M$ are such that $B^{\M'}\neq\emptyset$. Therefore
\end{comment}


\begin{comment}
\begin{lemma}\label{lem:Qformula}
 Let $\M,\M'$ be $\J$-models over $b,b'$ respectively. Let
$\pi:\M'\to\M$
be such that $\pi(b')=b$ and either $\pi$ is $\Sigma_2$-elementary or cofinal
and $\Sigma_1$-elementary.

(a) If $\M$ is a (potential) $J$-premouse over $b$
then $\M'$ is a (potential) $J$-premouse over $b'$.

(b) If $\M'$ is a (potential) $J$-premouse over $b'$, and if there is $\M''$, a
(potential) $J$-premouse over $b''$, and a weak $0$-embedding
$\pi'':\M\to\M''$ such that $\pi''(b)=b''$, then $\M$ is a (potential)
$J$-premouse over $b$.
\end{lemma}

\begin{proof}
Consider part (a). The fact that $J$ is coded correctly over $\M'$ essentially
follows from the
fact that $J$ condenses well. So, modulo standard facts about Q-formulas, we
just need to see that the remaining
features of the $F^*_J$ operator are preserved by $\pi$. So let
$\lambda,\lambda'=\l(\M),\l(\M')$ respectively.
Let $\left<\zeta_\alpha\right>_{\alpha\leq\iota}$ be as in \ref{PotJPremice2}
with respect to $\M$; let $S$ be the set of all $\M|\zeta_\alpha$
for $\zeta_\alpha\leq\lambda$. Let $S'=\{\M'\}\un\pi^{-1}``S$ and let
$\left<\zeta'_\alpha\right>_{\alpha\leq\iota'}$ be such that
$\left<\M'|\zeta'_\alpha\right>_{\alpha\leq\iota'}$ enumerates $S'$ in
increasing order. Let $Z$ ($Z'$) be the set of all $\zeta_\alpha$
($\zeta_\alpha'$).

The following claim completes the proof.
\begin{claim} We have:
\begin{enumerate}
\item\label{i:1} $Z'$ is closed.
\item\label{i:2} For each
$\alpha'+1<\iota'$,
$\M'|\zeta_{\alpha'+1}'=F^*_J(\M'|\zeta_{\alpha'}')\downarrow b'$
and $\pi(\zeta_{\alpha'+1}')=\zeta_{\alpha+1}$ where
$\pi(\zeta_{\alpha'}')=\zeta_\alpha$.
\item\label{i:3} If $\alpha<\iota'$ is a limit then
$\pi(\zeta'_\alpha)=\zeta_\beta$ for a limit $\beta$.
\item\label{i:4} If $\iota'$ is a limit then $\zeta_{\iota'}'=\lambda'$ and
$\zeta_\iota=\lambda$ is also a limit.
\item\label{i:5} If $\iota'=\alpha'+1$ then $\M'\ins
F^*_J(\M'|\zeta_{\alpha'}')\downarrow b'$ and $\iota=\alpha+1$ where
$\pi(\zeta_{\alpha'}')=\zeta_\alpha$.
\end{enumerate}
\end{claim}

\begin{proof}[Proof Sketch]
Clauses \ref{i:1}-\ref{i:4} hold because $J$ condenses well and by
calculations like in \ref{rem:local_def_P^varphi}.

This
is because: (i) $\N$ is coded by $b$; (ii) the $\Coll(\om,\M|\zeta_\alpha)$
forcing relation, and so also, the choice of extenders used to form $\Tt$, are
locally definable; (iii) the codes for the structures $Q_\xi$ provided by
$F^*_J$ are locally convertible to the actual structures $Q_\xi$; (iv) the
correct branch $c=\Lambda(\Tt\rest\xi)$ is recognizable before we
feed in information regarding $M^\Tt_\xi$ beyond a Q-structure $Q_\xi$ (and so
that information can be confirmed by computing $M^\Tt_\xi$ from $\Tt\rest\xi$
and $c$); (v) the cardinals of the structures $Q_\xi$ are recognizable via
consulting $\Tt$; and (vi) the end of $F^*_J(\M|\zeta_\alpha)$ is recognizable
by (v) and the minimality of $Q^\varphi$. We leave the remaining details to the
reader.

Clause \ref{i:5} holds for similar reasons, combined with the following
observations. Suppose $\M'$ is active; the other case is simpler.
By the elementarity/cofinality of $\pi$, $\iota$ is also a successor $\alpha+1$
and $\pi(\zeta_{\alpha'}')=\zeta_\alpha$. So $E^{\M}=\emptyset=E^{\M'}$, so
$B^{\M'}=B'\neq\emptyset\neq B=B^\M$.

By the $1$-$J$-smallness of the Q-structures of $M_1^J$, $B$ codes
a piece of $J$ (i.e. $B$ codes $B^{Q|\gamma}$ for some $\gamma$ and
iterate $Q$ of $\N$). So $B'$ putatively does likewise (over some $\J$-model
$Q'$). But $Q|\gamma$ is sufficently simply definable over $\M$, and
$\pi$ sufficiently elementary/cofinal, that it induces a sufficient embedding
$(Q',B')\to Q|\gamma$ to ensure that $(Q',B')$ is a
$J$-premouse. But we have $\delta$ such that
$Q|\gamma\sats$``$\delta$ is Woodin'', so
$Q|\gamma=\J^J_{\gamma-\delta}(Q|\delta)$ by $1$-$J$-smallness. So
$Q'|\gamma'\sats$``$\delta'$ is Woodin'' and
$Q'|\gamma'=\J^J_{\gamma'-\delta'}(Q'|\delta')$, and $\pi(\delta')=\delta$.
Suppose we are in the case that $Q|\delta=M(\Tt\rest\xi)$ for some limit $\xi$.
The uniform definability of $\Tt\rest\xi$ and $M(\Tt\rest\xi)$ over the
appropriate $\M|\eta$ ensures its preservation under $\pi^{-1}$, so
$Q'|\delta'=M(\Tt'\rest\xi')$, for $\Tt'=\Tt_{\M'|\alpha'}$ and the appropriate
$\alpha',\xi'$. The other case is similar; the fact that $P^\varphi\npins
Q|\gamma$ reflects to $\M'$.

This completes our sketch of the proof of the claim.
\end{proof}

This completes the proof of part (a). Part (b) is similar.
\end{proof}
\end{comment}

\begin{comment}
\begin{definition}
Let $b$ be a transitive set coding $P$. A \emph{$P$-putative (potential)
$J$-premouse over $b$} is a structure satisfying
all first order axioms of (potential) $J$-premice over $b$, where $P$ is taken
in the role of $\N$.
\end{definition}

There is a
Q-formula describing $P$-putative potential $J$-premice. If $\M$ is an
$\N$-putative potential $J$-premouse, then $\M$ is a potential
$J$-premouse iff $\M$ is
wellfounded and for all $\alpha\leq\l(\M)$, if $B^{\M|\alpha}\neq\emptyset$
then $B^{\M|\alpha}$ correctly codes the $J$-predicate for the appropriate
initial segment of the appropriate iterate of $\N$.
\end{comment}

\begin{lemma}\label{lem:cores}
Suppose $N,P$ are g-organized $J$-premice over $b$, $P$ is sound and whole and $P\pins N\ins
F^*_J(P)$. Let $\pi:\core_\om(N)\to N$ be the uncollapse. Then $P\in\rg(\pi)$,
and letting $\pi(P')=P$, then $\core_\om(N)\ins F^*_J(P')$. Moreover, $N$ is
whole iff $\core_\om(N)$ is whole.
\end{lemma}
\begin{proof}
This follows from \ref{lem:weak_0_hull} (using the fact that the first core
embedding $\pi_{1,0}:\core_1(N)\to N$ is cofinal and
$\Sigma_1$-elementary to see that $P\in\rg(\pi)$), and using that if
$\core_\om(N)$ is whole then $\core_\om(N)=F^*_J(P')$, which easily gives that
$N=F^*_J(P)$.
\end{proof}

\begin{remark}
Lemma \ref{lem:weak_0_hull} ensures that in a g-organized $L^J[\es](b)$-construction, we
don't
get stuck at successor stages. For example, suppose we have produced a
sound, whole model $P_0$, and want to extend $P_0$. Let $N_0$ be the least $N$
such that $P_0\pins N\ins F^*_J(P_0)$ and either $N$ is unsound or
$N=F^*_J(P_0)$. Let $N'_0=\core_\om(N_0)$. So $N'_0$ is sound. If $N'_0$ is
whole, then we set $N'_0$ as our next model, and move on. Suppose otherwise. We
have $P_1\pins N'_0$ such that $\pi(P_1)=P_0$, where $\pi:N'_0\to N_0$ is the
core embedding. We set $P_1$ as our next model. Since $N'_0$ is sound but not
whole, defining $N_1\ins F_J^*(P_1)$ as before, we have $N'_0\pins N_1$. And so
on. One can show (even without using fine structural universality) that
defining $N_k$ in this manner for $k<\om$, if $N_{k+1}$ is not whole
then $\rho_\om(N_k)>\rho_\om(N_{k+1})$, and so there is $k$ such
that $N_k$ is whole.
\end{remark}

\begin{lemma}
\label{ClosedUnderJ}
Suppose $\M$ is a $J$-closed g-organized $J$-premouse over $b$, where $J$ is a nice operator. Then
$\M$ is closed under $J$;
furthermore, for any set generic extension $g$ of $\M$, $\M[g]$ is closed under
$J$ and in fact, $J$ is uniformly definable over $\M[g]$ (i.e. there is a
$\mathcal{L}_0$-formula $\phi$ that defines $J$ over any set generic extension
of
$\M$).
\end{lemma}
\begin{proof}[Proof sketch.]
We show that $\M$ is closed under $J$; the proof of the second clause of the
lemma is similar. Let $b\in |\M|$; we want to see that $J(b)\in |\M|$. Let
$\kappa<\l(\M)$ be such that $b\in\M|\kappa$ and $\M|\kappa$ is whole.
Let $P^\varphi=P^\varphi(\T_{\M|\kappa})$. Let $R=F^*_J(\M|\kappa)\lhd \M$. Let $\PP=\Coll(\om,\M|\kappa)$. Let $\dot{x}$ be the name for the
$\PP$-generic real coding $\M|\kappa$. It is forced by $\PP$,
over $R$, that $\dot{x}$ is extender algebra generic over $P^\varphi$.
Since $(\varphi,\psi)$ determines $J$, we have $b\in P^\varphi[\dot{x}]$ and
$\psi$ defines $J$ over $P^\varphi[\dot{x}]$. So by consulting the $\PP$-forcing
relation and by niceness of $J$ (in particular, $J(x)$ is canonically coded by $x$ and a set of ordinals), $J(b)\in R$ . The
definability follows this argument. This completes the proof sketch of the
lemma.
\end{proof}

\begin{definition}[$J$-mouse]
\label{JMouse}
Let $\MJsharp, b$ be as in Definition \ref{PotJPremice2}\footnote{If $J$ is a 
first order mouse operator that is defined on a cone above $a$, then we also 
assume $a\subseteq b$.}. We say that $\M$ is a \textbf{g-organized $J$-mouse}
(or a \textbf{g-organized $J$-mouse over $b$}) if $\rho_{\omega}(\M) =
b$ and whenever $\M^*$ is a countable
transitive g-organized $J$-premouse over some $b^*$ and there is an elementary embedding
$\pi: \M^*\rightarrow \M$ such that $\pi(b^*) = b$  and
$\pi(\MJsharp)=\MJsharp$, then $\M^*$ is
$(\om,\omega_1+1)$-iterable (as a g-organized $J$-mouse).
\end{definition}

\begin{definition}
Suppose $J$ is a nice operator and is an iteration strategy. We define $\Lp_*^J(\mathbb{R})$ as the stack of all g-organized $J$-mice $\N$ over  
$H_{\om_1}$. We also say (g-organized) $J$-premouse \textbf{over $\mathbb{R}$} to in fact
mean over $H_{\omega_1}$.\footnote{If $J$ is a mouse operator, Lp$^J(\mathbb{R})$ denote the usual stack of $J$-mice over $H_{\omega_1}$. If $J$ is a strategy $\Sigma$, then since $\mathbb{R}$ is not self-wellorderable, the usual definition Lp$^J(\mathbb{R})$ does not seem to make sense; it's not clear how to choose the ``next tree" without the branch branch information in the relevant model.}\end{definition}

In core model induction applications, we typically have a pair $(\P,\Sigma)$
where $\P$ is either a hod premouse and $\Sigma$ is $\P$'s strategy with branch
condensation and is fullness preserving (relative to mice in some pointclass) or
$\P$ is a sound (hybrid) premouse projecting to some countable set $a$ and
$\Sigma$ is the unique (normal) $\omega_1+1$-strategy for $\P$ ($\Sigma$ is typically known to be sufficiently iterable so that Lp$^\Sigma_*(\mathbb{R})$ makes sense). Lemma
\ref{GenericInt} shows that $\Sigma$
condenses well and determines itself on generic extensions in the sense defined
above. We then define $\Lp_*^\Sigma(\mathbb{R})$ as above and use a core model
induction to prove $\Lp_*^\Sigma(\mathbb{R})\vDash \textsf{AD}^+$. What's needed
to
prove this is the scales analysis of $\Lp_*^\Sigma(\mathbb{R})\vDash
\textsf{AD}^+$
from the optimal hypothesis similar to those used by Steel (see
\cite{ScalesK(R)} and \cite{Scalesendgap}) to analyze the
pattern of scales in $\rm{Lp}(\mathbb{R})$.\footnote{Suppose $\P=\M_1^\sharp$ and $\Sigma$ is $\P$'s unique iteration strategy. Suppose $\rm{Lp}_*^\Sigma(\mathbb{R})\vDash \sf{AD}^+ + \sf{MC}$. Then in fact $\rm{Lp}_*^\Sigma(\mathbb{R})\cap \powerset(\mathbb{R}) = \rm{Lp}(\mathbb{R})\cap \powerset(\mathbb{R})$. This is because in $L(\rm{Lp}_*^\Sigma(\mathbb{R}))$, $L(\powerset(\mathbb{R})) \vDash \sf{AD}^+ \ + \ $$\Theta = \theta_0 + \sf{MC}$ and hence by \cite{sargsyan2014Rmice}, in $L(\rm{Lp}_*^\Sigma(\mathbb{R}))$, $\powerset(\mathbb{R})\subseteq \rm{Lp}(\mathbb{R})$.  Therefore, even though the hierarchies $\rm{Lp}(\mathbb{R})$ and $\rm{Lp}_*^\Sigma(\mathbb{R})$ are different, as far as sets of reals are concerned, we don't lose any information by analyzing the scales pattern in $\rm{Lp}_*^\Sigma(\mathbb{R})$ instead of that in $\rm{Lp}(\mathbb{R})$.}


\begin{comment}
$\T_M^\varphi=\T_M\rest\lambda$, where $\lambda$ is least such that either
$\lambda=\lh(\T_M)$ or $\lambda$ is a limit ordinal and there is
$\P\ins Q(\T_M\rest\lambda)$ such that
$M(\T_M\rest\lambda)\ins\P$ and $\P\models\varphi$. Now suppose there is
$\P\pins\N$ such that $\N|\delta^\N\ins\P$ and $\P\models\varphi$. Let
$\lambda\leq\lh(\T_M^\varphi)$ be a limit. If
$\lambda<\lh(\T_M^\varphi)$ let
$Q^\varphi(\T_M\rest\lambda)=Q(M(\T_M\rest\lambda))$. Otherwise let
$Q^\varphi(\T_M\rest\lambda)=\P$, where $\P$ is least such that
$M(\T_M\rest\lambda)\ins\P\ins M^{\T_M}_{\Lambda(\T_M\rest\lambda)}$ and
$\P\models\varphi$.
\end{comment}


\begin{comment}Old...
\begin{definition}[Definition of $F_J^*$]
\label{modelOpGenerala2}
Suppose $b$ is a transitive structure coding $\M_1^{J,\sharp}$. Let $\Lambda$ be
the
strategy for $\M_1^{J,\sharp}$. 
%
\footnote{It seems we might have avoided identifying $\M_1^{J,\sharp}$
explicitly, by
proceeding as in the following sketch. Suppose we have $\M|\alpha$ for some
$\alpha$.
Let $\tilde{J}=J^{\M|\alpha}$ be the partial operator which has been defined so
far.
Let $\tilde{Q}$ be the function defined as follows: Let $H$ be a transitive
set. Suppose there is $\gamma\in\OR$ such that $Q=\J_\gamma^{\tilde{J}}(H)$ is
defined (i.e., $\tilde{J}$ is defined sufficiently for this), and $Q$ is a
Q-structure for $H$. Then set $\tilde{Q}(H)=Q$. Otherwise $\tilde{Q}(H)$ is
undefined. Then $\M|\alpha$ can define
``$\M_1^{\dot{J}\sharp}$-like, $\tilde{J}$-consistently $\tilde{J}$-short tree
iterable premouse'' using $\tilde{Q}$: this is a sound premouse $\N$ satisfying
``I am $\M_1^{\dot{J}\sharp}$ for some operator $\dot{J}$'', and for every
$\tilde{Q}$-guided tree $\Tt$ on $\N$: (a) every model of $\Tt$ is
consistent with $\tilde{J}$; (b) if $\Tt$ has successor length, then it is
normally extendible (to more wellfounded models), and if $b^\Tt$ does not drop,
then the active extender of $M^\Tt_b$ is iterable; (c) if $\Tt$ has limit
length, and if $Q=\tilde{Q}(M(\Tt))$ is defined, then there is a $\Tt$-cofinal
branch $b$ such that $Q\ins M^\Tt_b$ and $M^\Tt_b$ is wellfounded. Now,
$\M|\alpha$ can begin comparing all such premice. At limit stages of the
comparison, say with a common part model $\N'$, we feed in $\J_\gamma^J(\N')$,
until reaching $Q=\tilde{Q}(\N')$, if we ever do. After reaching the $Q$, the
comparison can continue. Meanwhile, levels $\M|\beta$ for $\beta>\alpha$ may
have seen more of $J$; i.e. we might have
$J^{\M|\alpha}\subsetneq\J^{\M|\beta}$. Then redefining
$\tilde{J}=J^{\M|\beta}$, we refine the collection of $\tilde{J}$-consistently
$\tilde{J}$-short tree iterable premice, and restart the comparison accordingly.
While comparing, we should also be making levels $\M|\beta$ generic over the
iterates. Thus, whenever we reach a limit stage $\N'$ and some
$\P\pins\tilde{Q}(\N')$ such that $\P\models\varphi$, we can certainly compute
more of $\tilde{J}$.}
%
Let $\M$ be the following $\J$-model over parameter $b$.
There is $\alpha < l(\M)$ such that $\M|\alpha\vDash \textsf{ZF}$ and letting
$\alpha$ be the least such, then $\M|\alpha = \J_\alpha(b)$. Let $\xi =
\rho_{\omega}(b)$. Let $\lambda\leq\lh(\Tt_{\M|\alpha}^\varphi)$ be a
limit. Let
\begin{center}
$\P_{\lambda}=Q^\varphi(\Tt_{\M|\alpha}\rest\lambda)$.
\end{center}
Let $B\sub o(\P_{\lambda})$ be the standard set
coding $\P_{\lambda}$. Let $\om\gamma=o(\P_{\lambda})$. Fix $\beta < l(\M)$. Let
\begin{center}
$A=\{o(\M|\beta)+\eta\st\eta\in B\}\times\{\lambda\}$. 
\end{center}
Let $F_{J,\lambda}(\M|\beta)=\mathfrak{R}(\J^A_\gamma(\M|\beta),
\M|\beta)$.\footnote {Technically, $F_{J,\lambda}(\M|\beta)$ is stratified as a
model over $b$ but we suppress the structure for brevity. See Definition
\ref{modelOpSoa} for the stratification.}. 

Let $b$ be a structure and let $M$ be a model with parameter $b$. Define
$\mathfrak{R}(c,b)$ to be $M|\alpha$, where $\alpha$ is least such that either
(i) $\alpha=\l(M)$ or (ii) $\rho(M|\alpha)<\rho(b)$ or (iii) $b\neq
M|\alpha$ and $M|\alpha$ is a Q-structure for $\rho(b)$.

We say that $\T^\varphi_{\M|\alpha}|\lambda$ is \textbf{taken care of in
$\M|\xi$} for some $\xi$ if there is a $\beta < l(\M|\xi)$ such that
$F_{J,\lambda}(\M|\beta)\lhd \M|\xi$ and  $F_{J,\lambda}(\M|\beta)\neq
\J(\M|\beta)$. Suppose $\M|\beta$ has been defined and there is a $\lambda$ such
that $\P_{\lambda}$ is defined, $\T^\varphi_{\M|\alpha}\rest\lambda\in
\M|\beta$, and $\T^\varphi_{\M|\alpha}|\lambda$ is not taken care of in
$\M|\beta$, we let then $\M|\xi^* = F_{J\lambda}(\M|\beta)$, where $\xi^* =
l(F_{J,\lambda}(\M|\beta))$ for the least such $\lambda$.

$\M$ is then the least such that for every limit $\lambda \leq
lh(\T^\varphi_{\M|\alpha})$, $\T^\varphi_{\M|\alpha}\rest \lambda$ is taken care
of in $\M$.

Finally, let $F_J^*(b) = \M$ if no level of $\M$ projects across $\xi$ or is a
$Q$-structure for $\xi$; in this case, we say that $F_J^*(b)$ is \textbf{defined
fully} or \textbf{how you like it}. Otherwise, let $F_J^*(b) = \M|\beta$, where
$\beta$ is the least such that $\rho_\omega(\M|\beta) < \xi$.

\end{definition}
\end{comment}

\begin{comment}
%Let $b$ be a structure and let $M$ be a model with parameter $b$. Define
%$\mathfrak{R}(c,b)$ to be $M|\alpha$, where $\alpha$ is least such that either
%(i) $\alpha=\l(M)$ or (ii) $\rho(M|\alpha)<\rho(b)$ or (iii) $b\neq
%M|\alpha$ and $M|\alpha$ is a Q-structure for $\rho(b)$.
\end{comment}

\begin{comment}
We say that $\T^\varphi_{\M|\alpha}|\lambda$ is \textbf{taken care of in
$\M|\xi$} for some $\xi$ if there is a $\beta < l(\M|\xi)$ such that
$F_{J,\lambda}(\M|\beta)\lhd \M|\xi$ and  $F_{J,\lambda}(\M|\beta)\neq
\J(\M|\beta)$. Suppose $\M|\beta$ has been defined and there is a $\lambda$ such
that $\P_{\lambda}$ is defined, $\T^\varphi_{\M|\alpha}\rest\lambda\in
\M|\beta$, and $\T^\varphi_{\M|\alpha}|\lambda$ is not taken care of in
$\M|\beta$, we let then $\M|\xi^* = F_{J\lambda}(\M|\beta)$, where $\xi^* =
l(F_{J,\lambda}(\M|\beta))$ for the least such $\lambda$.

$\M$ is then the least such that for every limit $\lambda \leq
lh(\T^\varphi_{\M|\alpha})$, $\T^\varphi_{\M|\alpha}\rest \lambda$ is taken care
of in $\M$.

Finally, let $F_J^*(b) = \M$ if no level of $\M$ projects across $\xi$ or is a
$Q$-structure for $\xi$; in this case, we say that $F_J^*(b)$ is \textbf{defined
fully} or \textbf{how you like it}. Otherwise, let $F_J^*(b) = \M|\beta$, where
$\beta$ is the least such that $\rho_\omega(\M|\beta) < \xi$.
\end{comment}

\begin{comment}
A \emph{pseudo-iteration tree $\Tt$ (on $M$)} is a structure satisfying all
requirements of an iteration tree $\Tt$ (on $M$), except for the wellfoundedness
of models. A pseudo-tree $\Tt$ is \emph{$\alpha$-wellfounded} iff
for all $\beta<\lh(\Tt)$, either $\alpha\sub\wfp(M^\Tt_\beta)$ or $M^\Tt_\beta$
is fully wellfounded. A pseudo-tree is \emph{reasonable}
iff for every $\beta<\lh(\Tt)$, $\Tt$ is $\lh(E^\Tt_\beta)+1$-wellfounded. For
a reasonable pseudo-tree, let $\delta(\Tt)$ denote
$\sup_{\alpha<\lh(\Tt)}\lh(E^\Tt_\alpha)$.

Let $M$ be a transitive structure. Let $\dot{G}$ be the canonical
$Col(\omega,M)$-name
for the generic $G\subseteq Col(\omega,M)$ and $\dot{x}_{\dot{G}}$ be the
canonical name for the real coding $\{(n,m) \ | \ G(n) \in G(m)\}$, where we
identify $G$ with $\bigcup G$. Using the
terminology of \cite{ATHM}, we say a reasonable psuedo-tree $\mathcal{T}$ on
$\N$ is a tree for making \textit{$M$ generically generic}
if the following holds:
%***Is \N=M_1^J^#?
\begin{enumerate}
\item $\mathcal{T}\rest\OR^M$ is a linear iteration tree obtained by
iterating the first total measure of $\N$ and its images $\leq\OR^M$
times.
\item $\mathcal{T}$ is everywhere non-dropping.
\item Suppose $\lh(\Tt)\geq\OR^M+2$ and let $\alpha+1\in(\OR^M,\lh(\Tt))$.
Let $\delta=\delta(\M^\Tt_\alpha)$ and let $\BB$ be the extender algebra of
$M^\Tt_\alpha$ at $\delta$. Then $E^\mathcal{T}_\alpha$ is the extender $E$ with
least index in $\M^\mathcal{T}_\alpha$ such that for some condition
$p\in\Col(\omega,M)$, $p \Vdash$``There is a $\mathbb{B}$-axiom induced
by $E$ which fails for $\dot{x}_{\dot{G}}$''.
\end{enumerate}
Note that even if the models of $\Tt$ are fully wellfounded, they might not
be $J$-premice. Also, $\Tt$ might not be a
successful genericity iteration.

Let $\Lambda$ be the strategy for
$\N=\M_1^{J,\sharp}$. We denote by $\T_{M}$ the unique successful such tree via
$\Lambda$. Note that $\T_M\in V$, $\T$ is nowhere
dropping, and $lh(\mathcal{T}_{M}) < |M|^+$. Also note that $\T_M$ does
not include the last branch.

Given such a tree $\Tt$ and a formula $\varphi$, we let $Q^\varphi(\Tt)$
be the least $Q\ins M(\Tt)$ such that for some cardinal $\delta'$ of
$M(\T_{M})$, we have
$\delta'<\OR^Q$ and $Q\sats\varphi+$``$\delta'$ is Woodin''.

We're almost ready to define $J$-premice over arbitrary transitive sets $b$
coding $\N$. We first define an operator $F_J^*$, to be used to feed $J$ into
such a structure. We now fix a pair $(\varphi,\psi)$ that generically determines
$J$.
\end{comment}
%For $\xi\in I^\varphi$, let
%$\delta_\xi=\delta(\Tt\rest\xi)$. If $\delta_\xi<\delta'$, let
%$Q^\varphi_\xi=Q(\Tt\rest\xi)$, and if $\delta_\xi=\delta'$, and
%therefore $\xi=\lambda$, let $Q^\varphi_\lambda=P^\varphi$ (in the latter case,
%$P^\varphi\ins Q(\Tt\rest\lambda)$).


\begin{comment}
We're almost ready to define $J$-premice $\M$  over arbitrary transitive sets
$b$
coding $\N$. The operator $F_J^*$, defined below, is used to feed $J$ into
$\M$. Given $\M|\beta$, the first step of extension of $\M|\beta$ in $\M$ is
through (initial segments of) $F_J^*(\M|\beta)$, which basically constructs
above $\M|\beta$ from the structure $P^\varphi$ defined as above, relative to
$\Tt=\Tt_{\M|\beta}$.
We must also ensure that suitable hulls $\M'$ of $\M$ will also be $J$-premice
over some $b'$. This will partly follow from the fact that $J$ condenses well,
but will
also depend on the precise manner in which we feed $P^\varphi$ into $\M$. The
intervals of $P^\varphi$ between $M(\Tt\rest\xi)$ and $Q^\varphi_\xi$ (for
limit $\xi$) simply involve $J$-construction, which is preserved by
condensation. We will only actually feed in these intervals. The remainder of
$P^\varphi$ can be computed over the resulting structure,
by computing enough of $\Tt$.
It seems we need to be a little careful to ensure that this makes sense, is
fairly local and that the coding of $J$ condenses properly. After feeding in a
given
$Q^\varphi_\xi$, given $\xi'>\xi$, the next element of $I^\varphi$, we will
insert enough ordinals that the branch $\Lambda(\Tt\rest\xi)$, and the next
piece of $\Tt_{\M|\beta}$, and $M(\Tt\rest\xi')$, can all be computed over
some $\M|\gamma$, before we feed in $Q^\varphi_{\xi'}$ beyond $\M|\gamma$.
\end{comment}

\begin{comment}
\begin{definition}[$F_J^*$]
\label{modelOpGenerala2}
Let $b$ be a transitive structure coding $\M_1^{J,\sharp}$.
%footnote
\footnote{It seems we might have avoided identifying $\M_1^{J,\sharp}$
explicitly, by
proceeding as in the following sketch. Suppose we have $\M|\alpha$ for some
$\alpha$.
Let $\tilde{J}=J^{\M|\alpha}$ be the partial operator which has been defined so
far.
Let $\tilde{Q}$ be the function defined as follows: Let $H$ be a transitive
set. Suppose there is $\gamma\in\OR$ such that $Q=\J_\gamma^{\tilde{J}}(H)$ is
defined (i.e., $\tilde{J}$ is defined sufficiently for this), and $Q$ is a
Q-structure for $H$. Then set $\tilde{Q}(H)=Q$. Otherwise $\tilde{Q}(H)$ is
undefined. Then $\M|\alpha$ can define
``$\M_1^{\dot{J}\sharp}$-like, $\tilde{J}$-consistently $\tilde{J}$-short tree
iterable premouse'' using $\tilde{Q}$: this is a sound premouse $\N$ satisfying
``I am $\M_1^{\dot{J}\sharp}$ for some operator $\dot{J}$'', and for every
$\tilde{Q}$-guided tree $\Tt$ on $\N$: (a) every model of $\Tt$ is
consistent with $\tilde{J}$; (b) if $\Tt$ has successor length, then it is
normally extendible (to more wellfounded models), and if $b^\Tt$ does not drop,
then the active extender of $M^\Tt_b$ is iterable; (c) if $\Tt$ has limit
length, and if $Q=\tilde{Q}(M(\Tt))$ is defined, then there is a $\Tt$-cofinal
branch $b$ such that $Q\ins M^\Tt_b$ and $M^\Tt_b$ is wellfounded. Now,
$\M|\alpha$ can begin comparing all such premice. At limit stages of the
comparison, say with a common part model $\N'$, we feed in $\J_\gamma^J(\N')$,
until reaching $Q=\tilde{Q}(\N')$, if we ever do. After reaching the $Q$, the
comparison can continue. Meanwhile, levels $\M|\beta$ for $\beta>\alpha$ may
have seen more of $J$; i.e. we might have
$J^{\M|\alpha}\subsetneq\J^{\M|\beta}$. Then redefining
$\tilde{J}=J^{\M|\beta}$, we refine the collection of $\tilde{J}$-consistently
$\tilde{J}$-short tree iterable premice, and restart the comparison accordingly.
While comparing, we should also be making levels $\M|\beta$ generic over the
iterates. Thus, whenever we reach a limit stage $\N'$ and some
$\P\pins\tilde{Q}(\N')$ such that $\P\models\varphi$, we can certainly compute
more of $\tilde{J}$.}
%end footnote
We define $\M=F_J^*(b)$, a $\J$-model with parameter $b$, as follows.

For each $\alpha\leq\l(\M)$, $E^{\M|\alpha}=\emptyset$.

There is $\alpha < \l(\M)$ such that $\M|\alpha=\J_\alpha(b)\sats\ZF$. Let
$\alpha$ be least such.

Let $\Tt=\Tt_{\M|\alpha}$. Let $\lambda$, $I^\varphi$, $P^\varphi$,
$Q_\xi$ be defined as above. Let
$\left<\xi_\alpha\right>_{\alpha\in[1,\zeta]}$ be an increasing enumeration of
$I^\varphi$ (if $I^\varphi=\emptyset$ then $\zeta=0$). By induction on
$\alpha$, we define sequences of
ordinals $\left<\gamma_\alpha\right>_{\alpha\leq\zeta}$ and
$\left<\eta_\alpha\right>_{\alpha\leq\zeta}$ such that
$\gamma_\alpha\leq\eta_\alpha\leq\gamma_\beta\leq\eta_\beta$ for
$\alpha<\beta\leq\zeta$. We
simultaneously define $\left<\M|\gamma_\alpha\right>_{\alpha\leq\zeta}$ and
$\left<\M|\eta_\alpha\right>_{\alpha\leq\zeta}$. We will also maintain that for
$\alpha<\zeta$, $\delta_{\xi_{\alpha+1}}\leq\eta_\alpha$, and that
$\Tt\rest\xi_{\alpha+1}$ and $M(\Tt\rest\xi_{\alpha+1})$ are definable over
$\M|\eta_\alpha$, and uniformly so.

Firstly, $\gamma_0=0$, so $\M|\gamma_0=a$. If $0<\zeta$, let
$\eta_0=\delta_{\xi_1}=\alpha+\delta_{\xi_1}$, and let
$\M|\eta_0=\J_{\delta_{\xi_1}}(\M|\alpha)$. We have $\xi_1=\om$, and
$\Tt\rest\om$ and $M(\Tt\rest\om)$ are definable over
$\J_{\delta_{\xi_1}}(\M|\alpha)$ by the local definability of forcing (cf.
\ref{rem:local_def_P^varphi}).

Suppose for some $\beta\leq\zeta$, $0<\beta$, we have defined
$\gamma_\eps,\eta_\eps$ and $\M|\eta_\eps$ for all
$\eps<\beta$. Let $\eta=\sup_{\eps<\beta} \eta_\eps$. By induction,
$\delta_\beta\leq\eta$ and $\Tt\rest\xi_\beta$ and $M(\Tt\rest\xi_\beta)$
are definable over $\M|\eta$. Set
$\gamma_\beta=\eta+(\OR(Q_{\xi_\beta})-\delta_\beta)$ (ordinal
subtraction)\footnote{I.e., $\OR_{\xi_\beta}-\delta$ is the unique ordinal
$\tau$ such that $\delta+\tau=\OR_{\xi_\beta}$}. Let
$A\sub\OR(Q_{\xi_\beta})^{<\om}$
be the natural set coding $Q_{\xi_\beta}$. Let
$\pi_1:\OR(Q_{\xi_\beta})\to\gamma_\beta$ be such that $\pi_1\rest\delta_\beta
=\idmap$
and for $\delta_\beta+\gamma\in[\delta_\beta,\OR(Q_{\xi_\beta}))$,
$\pi_1(\delta_\beta+\gamma)=\eta+\gamma$. Let
$\pi:\OR(Q_{\xi_\beta})^{<\om}\to\gamma_\beta^{<\om}$ be induced by
$\pi_1$. Let $A'=\pi``A$. To
define $\M|\gamma_\beta$, we must just specify $B^{\M|\eta+\eps}$ for each
$\eta+\eps\in[\eta,\gamma_\beta]$. We let these be specified by $A'$. So
for each such $\eps$, $B^{\M|\eta+\eps}\sub(\eta+\eps)^{<\om}$ and codes
$B^{Q_{\xi_\beta}|\delta_\beta+\eps}$ (note that
$E^{Q_{\xi_\beta}|\delta_\beta+\eps}=\emptyset$ by $1$-$J$-smallness).
Because $M(\Tt\rest\xi_\beta)$ is definable over $\M|\eta$, these predicates
are amenable (at each level $\eta+\eps$), and we get a $\J$-model.

Now suppose we have defined $\gamma_\beta$ and $\M|\gamma_\beta$ for some
$\beta\leq\zeta$. We must define $\eta_\beta$ and $\M|\eta_\beta$. Let
$\xi=\xi_\beta$. If $\beta<\zeta$ let $\delta=\delta_{\beta+1}$. Otherwise let
$\delta=\OR(P^\varphi)$.

Let $c=\Lambda(\Tt\rest\xi)$. Let $\eta_\beta=\gamma_\beta+\eta+\delta$
for the
least $\eta$ such that for some $\tau\in c$, we have
\[ Q_{\xi}\in\rg(i^\Tt_{\tau,\xi}) \]
and both $c$ and the sequence
\[ \left<i^\Tt_{\eps,\xi}\rest
(i^\Tt_{\eps,\xi})^{-1}(Q_{\xi})\right>_{\eps\in[\tau,\xi)} \]
are definable over $\J_\eta(\M|\gamma_\beta)$. With this $\eta$, set
$\M|\eta_\beta=\J_{\eta+\delta}(\M|\gamma_\beta)$. Then again using the
definability of forcing, we maintain the inductive hypotheses. (If
$\beta<\zeta$, then even if $\eta>\delta$, it seems that
$\Tt\rest\xi$ might not be definable over $\M|\gamma_\beta+\eta$.)

We finally require that $\M=\M|\eta_\zeta$. This completes the definition of
$F^*_J$.
\end{definition}
\end{comment}

==> scales_comments.tex <==
%scales_intro.tex

\begin{comment}For premice $\P,\Q$, we write
$\P\unlhd \Q$ ($\P\lhd \Q$) if there is some $\gamma\leq o(\Q)$ ($\gamma<o(\Q)$)
such that $\P=\Q|\gamma$. For $k\leq \omega$, ordinals $\alpha,\beta$, a $k$-
sound premouse $\M$ (in the sense of \cite{FSIT}) is
$(k,\alpha,\beta)$-iterable if player II (the good player) has a winning
strategy in the game $\mathcal{G}_k(\M,\alpha,\beta)$ (see
\cite[\S 4]{steel2010outline}). We customarily call a $k$-sound premouse
$\M$ that is $(k,1,\omega_1+1)$-iterable (or $(k,\omega_1,\omega_1+1)$-iterable)
a \textit{mouse}.
When the degree of soundness of $\M$ is clear from the
context, we will neglect to mention it in our notations. When $\M$ is
$(k,1,\beta)$-iterable, we just write $\M$ is $(k,\beta)$-iterable.
We write $\M^\T_\alpha$ for the $\alpha$-th model in the tree
$\T$ and if $b$ is a cofinal branch of $\T$, we write $\M^\T_b$ for the
corresponding branch model. 
If $\T$ is
an iteration tree on $\M$ with successor length, we write $M^\T_\infty$ for the last
model of $\T$. We also apply the preceding 
terminology and notation to $Y$-premice over $X$ for various $X,Y$; see
\end{comment}
% I removed the following paragraph because I think it is better dealt with
% following the definition of ``model with parameter a''.
\begin{comment}
We also consider in this paper $\J$-structures of the form $\M = (\J^A[E], \in,
E,A,F^\M)$ for some set of ordinals $A$. We define $\M|\gamma$ etc. in a similar
way, for instance $\M|\gamma = (\J^A[E]\rest \gamma, \in, E\rest\gamma,A\cap
\gamma, E(\gamma))$. Sometimes, we also write $\M_\gamma$ for $\M|\gamma$.
\end{comment}

\begin{comment}
We use $\Theta$ to denote the supremum of $\alpha$ such that there is a
surjection from $\mathbb{R}$ onto $\alpha$. Assuming $\textsf{AD}^+$, which
is a techincal strengthening of $\textsf{AD}$ (see \cite{DMT} or
\cite{steeltrang2010AD+reflection} for more on $\textsf{AD}^+$), the
\textit{Solovay sequence} is the sequence $\langle \theta_\alpha \ | \
\alpha\leq
\Omega \rangle$ such that: (i) $\theta_0$ is the supremum of ordinals $\alpha$
such that there is an $OD$ surjection from $\mathbb{R}$ onto $\alpha$; (ii) if
$\beta\leq\Omega$ is limit, then $\theta_\beta = \textrm{sup}_{\gamma<\beta}
\theta_\gamma$; (iii) if $\beta=\gamma+1\leq \Omega$, then letting $B\subseteq
\mathbb{R}$ have Wadge rank $\theta_\gamma$, $\theta_\beta$ is the supremum of
$\alpha$ such that there is an $OD(B)$ surjection from $\mathbb{R}$ onto
$\alpha$. We also write $\theta_X$ for the supremum of $\alpha$ such that there
is an $OD(X)$ surjection from $\mathbb{R}$ onto $\alpha$.
\end{comment}
\begin{comment}
 G-organized $J$-premice $\N$ are hybrid premice over a possibly 
non-selfwellordered
set $b$, where $b$ codes $\MFsharp=\M_1^{J,\#}$, and where the non-extender 
information fed into $\N$ is a certain fragment of the iteration strategy 
$\Sigma_\MFsharp$ for $\MFsharp$. In fact, we only feed in 
$\Sigma_\MFsharp(\Tt)$ for certain \emph{non-maximal} trees $\Tt$ on 
$\MFsharp$, so the fragment of $\Sigma_\MFsharp$ we feed in is equivalent to 
some fragment of $J$.\footnote{Why not just 
feed in those fragments of $J$ (enough to compute the Q-structures 
corresponding 
to the branches) directly? Because, by feeding in the branches directly, we can 
prove slightly stronger condensation properties for the resulting structures.}
\end{comment}
\begin{comment}
for many
instances of $\Fop$, under $\AD^+ + \MC(\Fop)$\footnote{$\MC(\Fop)$ is
the statement: for any $x,y\in\mathbb{R}$, if $x\in OD_\Fop(y)$, then $x$ is in 
a g-organized $\Fop$-mouse over $y$.}
\end{comment}
\begin{comment}
$\Lp^{J}(\mathbb{R})$ when $J$ is an
iteration strategy. For in this case, the models $\Lp^J_\alpha(\mathbb{R})$
fail to satisfy $\textsf{AC}$. Suppose we have $\Lp^J_\alpha(\RR)$, and wish to
define $\Lp^J_\beta(\RR)$ for some $\beta>\alpha$. In a typical such interval we
must feed in $J(\Tt)$ for certain iteration trees $\Tt$. But without
a wellorder of $\Lp^J_\alpha(\RR)$, there is no obvious choice for which tree
$\Tt$ to use next. It seems that one might overcome this by simultaneously
feeding in $J(\Tt)$ for all $\Tt\in\Lp^J_\alpha(\RR)$. However, it turns
out that there \emph{are} canonical choices of single trees $\Tt$ to use, and
moreover, making such choices helps the scales analysis.
\end{comment}

%scales_J_premice.tex below, and then somewhere starts scales_weak_gap.tex
\begin{comment}
\begin{definition}
Let $\opbk$ be an operator background. Let $\varphi\in\Ll_0$. Let $J_\varphi$
be the following partial function $J:\opbk\to\opbk$.
For $A\in\opbk'$,
$J(A)$ is the least $\M\wins\Lp(A)$ such that 
$\M\sats\varphi$, if there is such an $\M$; otherwise $J(A)$ is undefined.
For $\om$-sound op-premice $\R$ over some $A\in\opbk'$,
$J(\R)=J(\hat{\R})$.

A \emph{mouse pre-operator} is a pre-operator of the form $J_\varphi$,
for some formula $\varphi$.
\end{definition}

***could put the definition of mouse operator in here, as it was before

\begin{definition}
(***Maybe dont' need this definition for a while? And it's not correct, as it can project early.) 
For any $P$ and any ordinal $\alpha\geq 1$, the (pre-)operator $\Jop_\alpha(\ \cdot\ ;P)$ 
is defined as follows.\footnote{The ``$\mathsf{m}$'' is 
for 
``model''.} For $X$ such that $P\in\J_1(\hat{X})$, let
$\Jop_{\alpha}(X;P)$ be the $\J$-model $\M$ over $X$, with parameter $P$, such 
that
$\univ{\M}=\J_\alpha(\hat{X})$ and for each $\beta\in[1,\alpha]$, $\M_\beta$ is 
passive. Clearly $\Jop_\alpha(\ \cdot\ ;P)$ is basic and forgetful.
If $P=\emptyset$ or we wish to supress $P$, we just 
write $\Jop_\alpha(\ \cdot\ )$.
\end{definition}
\end{comment}
\begin{comment}
\begin{definition}
\label{model}
Let $a$ be transitive. Let $\varrho:a\to\rank(a)$ be the rank function. 
We write $A=\trancl(\{(a,\varrho)\})$. Let $\hmp\in\J_1(A)$.

A \textbf{$\J$-structure over $a$ (with parameter $\hmp$) (for $\Ll_0$)} 
is a structure $\M$ for $\Ll_0$ such that $a^\M=a$, ($\hmp^\M=\hmp$), and 
there is
$\lambda\in[1,\Ord)$ such that $\univ{\M}=\J_\lambda^{S^\M}(A)$.

Here we also let $\wl(\M)$ denote 
$\lambda$, the \textbf{length} of $\M$, and let $A^\M$ denote $A$.

For $\alpha\in[1,\lambda]$ let $\M_\alpha=\J_\alpha^{S^\M}(A)$.
We say that $\M$ is \textbf{acceptable} iff for each 
$\alpha<\lambda$ and $\tau<\OR(\M_\alpha)$, if 
\[ 
\pow(\tau^{<\om}\cross A^{<\om})\inter\M_\alpha\neq\pow(\tau^{<\om}
\cross A^{<\om})\inter\M_{\alpha+1},\]
then there is a surjection 
$\tau^{<\om}\cross A^{<\om}\to\M_\alpha$ in $\M_{\alpha+1}$.

A \textbf{$\J$-structure (for $\Ll_0$)} is a $\J$-structure over $a$, for some 
$a$.
\end{definition}

As all $\J$-structures we consider will be for $\Ll_0$, we will omit the 
phrase ``for $\Ll_0$''. We also often omit the phrase ``with parameter 
$\hmp$''. Note that if $\M$ is a $\J$-structure over $a$ then 
$\univ{\M}$ is transtive and rud-closed, $\hat{a}\in M$ and $\Ord\inter 
M=\rank(M)$. This last point is because we construct from $\hat{a}$ instead of 
$a$.

$\Fop$-premice will be $\J$-structures of the following form.

\begin{definition}
A \textbf{$\J$-model over $a$ (with parameter $\hmp$)} 
is an acceptable
$\J$-structure over $a$ (with parameter $\hmp$), of the form
\[ \M = (M; E, B, S, a, \hmp) \]
where $\hmEdot^\mathcal{M}=E$, etc, and letting $\lambda=\wl(\M)$, the following 
hold.
\begin{enumerate}
 \item $\M$ is amenable.
 \item $S = \langle S_\xi \ | \ \xi\in[1,\lambda) \rangle$
is a sequence of $\J$-models over $a$ (with parameter $\hmp$).
\item For each $\xi\in[1,\lambda)$, $\hmSdot^{S_\xi} = S\rest \xi$.
%\item If $\lambda$ is a successor ordinal then $\l=\lambda$; otherwise $\l=0$.
\item\label{item:extender} Suppose $E\neq\emptyset$. Then $B=\emptyset$ and 
there is an extender $F$ over $\M$ which is
$\hat{a}\times\gamma$-complete for all $\gamma < \crit(F)$ and such that 
the premouse axioms \cite[Definition 2.2.1]{wilson2012contributions} hold for $(\M,F)$, and
$E$ codes $\tilde{F}\un\{G\}$ where: (i) $\tilde{F}\sub M$ is the 
amenable code for $F$ (as in \cite{steel2010outline}); and (ii) if $F$ is not 
type 2 then $G=\emptyset$, and otherwise $G$ is the ``longest'' non-type Z 
proper segment of $F$ in $\M$.\footnote{We use $G$ explicitly, instead of the 
code $\gamma^\M$ used for $G$ in \cite[\S2]{FSIT}, because $G$ does not depend 
on which (if there is any) wellorder of $\M$ we use. This ensures that certain 
pure mouse operators are \emph{forgetful}.}
\qedhere
\end{enumerate}
\end{definition}

Note that with notation as above, if $\lambda$ is a successor ordinal then 
$M=\J(S^\M_{\lambda-1})$, and otherwise, 
$M=\bigcup_{\alpha<\lambda}\univ{S_\alpha}$.
The predicate $\hmPdot$ will be used to code extra information. Suppose $E^\M$ codes an extender 
$F$. Clearly $\rank(a)<\crit(F)$. Note that, in accordance with \cite[Definition 
2.2.1]{wilson2012contributions}, but as opposed 
to \cite[Definition 2.4]{steel2010outline}, \emph{we allow $F$ to be of superstrong type} (see 
below).\footnote{The main point of permitting superstrong type extenders is that it simplifies 
certain things. However, the cost is that it complicates others. If the reader prefers, one could 
instead require, as in \cite{steel2010outline}, that $F$ \emph{not} be of superstrong type, but 
various 
statements throughout the paper regarding condensation would need to be modified, along the lines 
of \cite[Lemma 3.3]{FSIT}.} Next, we describe some terminology and notation regarding the above 
definition.
\begin{definition}
\label{someNotations}
Let $\M$ be a $\J$-model with parameter $a$. Let $E^\M$ denote $\hmEdot^\M$, 
etc. Let $\lambda=\wl(\M)$, $S^\M_0=a$, $S^\M_\lambda=\M$, and
$\M|\xi=S^\M_\xi$ for all $\xi\leq\lambda$.
An \textbf{(initial) segment} of $\M$ is just a structure of 
the form $\M|\xi$ for some $\xi\in[1,\lambda]$. We write $\P\wins\M$ iff $\P$ is 
a segment of $\M$, and $\P\wpins\M$ iff $\P\wins\M$ and $\P\neq\M$.
Let $\M||\xi$ be the structure having the same universe
and predicates as $\M|\xi$, except that $E^{\M||\xi}=\emptyset$.
%***Is this definition of $\rho(\M)$ assuming that $\M$ is sound?***
We say that $\M$ is \textbf{$E$-active} iff
$E^\M\neq\emptyset$, and \textbf{$B$-active} iff
$B^\M\neq\emptyset$. \textbf{Active} means either
$E$-active or $B$-active; \textbf{$E$-passive} means not
$E$-active; \textbf{$B$-passive} means not $B$-active; and \textbf{passive}
means not active. Also, $\M$ is \textbf{type 0} iff $\M$ is passive, 
\textbf{type 4} iff $\M$ is $B$-active, and \textbf{type 1, 2} or \textbf{3} 
iff $\M$ is $E$-active, with the usual numerology.
If $\M$ is $E$-active with extender $F$, we say $\M$, or $F$, is \textbf{superstrong} iff 
$i_F(\crit(F))=\nu(F)$. We say that $\M$ is \textbf{super-small} iff $\M$ has no superstrong 
initial segment.

If $\M$ is not type 3, we define the fine-structural notions (i.e. 
projecta, parameters, solidity, soundness, cores) precisely as for passive 
premice
in \cite{FSIT}, using the language\footnote{So even if $E^\M\neq\emptyset$, we 
do not include constants analogous to those used in \cite{FSIT}. The 
interpretations of these constants are all encoded into $E^\M$.} 
$\Ll_0\un\hat{a}$, where $\hat{a}$ consists of constant 
symbols.\footnote{So 
$\core_0(\M)=\M$. We 
only define the $\rho_{k+1}$, $p_{k+1}$, etc, given that $\core_k(\M)$ is a 
$k$-sound model over $a$. In any case, it certainly makes sense to ask whether 
``$\M$ is $1$-solid'' or ``$\M$ is $1$-sound'', and to define $\core_1(\M)$, 
for 
example. We set $\rho_1$ to be the least ordinal $\rho$ such that 
$\rho\geq\rank(a)$ and $\rho\geq\om$ and there is some $A\sub\rho^{<\om}\cross 
\hat{a}^{<\om}$ 
which is $\Sigma_1^\M(\M)$, but $A\notin\M$. We say ``$\rho_1=a$'' to mean 
``$\rho_1=\max(\om,\rank(a))$''. Etc.} If $\M$ is type 3, we define the 
\textbf{squash} $\M^\sq$ of $\M$ as in \cite{FSIT}, and fine-structure is 
defined over $\M^\sq$, still using the same language as in 
the previous case.

The classes of \textbf{Q-formulas} and \textbf{P-formulas} in the language 
$\Ll_0$, are defined analogously to in \cite[\S\S2,3]{FSIT} (but 
with $\Sigma_1$ in place of the $\rSigma_1$ of \cite{FSIT}).

Let $\rho(\M)$ be the 
least $\rho\leq\lambda$ such that there
is some $A\subseteq\M$ such that $A$ is $\Sigma_\om^\M(\M)$ and
$A\cap\lpole\M|\rho\rpole\notin\M$.

An \textbf{$a$-cardinal} of $\M$ is an ordinal $\gamma<\OR(\M)$ such that in 
$\M$ there is no surjection $\hat{a}^{<\om}\cross\eta^{<\om}\to\gamma$ with 
$\eta<\gamma$. We write $\Theta^\M$ for the supremum of all $\gamma<\OR(\M)$ 
such that in $\M$ there is a surjection $\hat{a}^{<\om}\to\gamma$.

Let $\M$ be a $\J$-model and $\N\wins\M$. We say that $\N$ is a \textbf{(strong) cutpoint} of $\M$ 
iff for all $\P\wins\M$, if $\N\wpins\P$ and $E^\P\neq\emptyset$ then $\OR(\N)\leq\crit(E^\P)$ 
($\OR(\N)<\crit(E^\P)$).

Given a $\J$-model $\M_1$ over $b$ and a $\J$-model $\M_2$ over
$\M_1$, we write $\M_2\down b$ for the $\J$-model $\M$ over $b$,
such that $\M$ is ``$\M_1\conc\M_2$'', if this is well-defined. That is, $\M_2\down b$ is the 
unique $\J$-model $\M$ such that
$\univ{\M}=\univ{\M_2}$, $a^\M=b$, $E^\M=E^{\M_2}$, $B^\M=B^{\M_2}$,
and $\P\wpins\M$ iff $\P\wins\M_1$ or there is $\Q\wpins\M_2$ such that 
$\P=\Q\down b$, when such an $\M$ exists. (Existence depends only on whether the $\J$-structure 
$\M$ described here is acceptable.)

Inverting this, given a $\J$-model $\M$ over $b$ and $\M_1\wpins\M$ such that $\M_1$ is a strong 
cutpoint of $\M$, we write 
$\M\down\M_1$ for 
the $\J$-model $\M_2$ over $\M_1$ such that $\M_2\down b=\M$.
\end{definition}
\end{comment}

\begin{comment}
\begin{lemma}\label{lem:Qformula_pres}
The natural adaptations of Lemmas 2.4, 2.5, 3.2, 3.3 of \tu{\cite{FSIT}} 
hold,\footnote{Note that for type 1 or 2 $\J$-models, the 
$\mu^\M$ and $\nu^\M$ (with notation as in \cite[Lemma 2.5]{FSIT}) are in fact 
computable from any element of $E^\M$, and so we don't really need constant 
symbols for them.} and in fact, in adapting conclusion \tu{(}b\tu{)} of \tu{\cite[Lemma 
3.3]{FSIT}}, we can omit 
the clause ``or $\N$ is of superstrong type''.\footnote{Because we allow superstrong
extenders.}
\end{lemma}
\end{comment}
\begin{comment}
In fact, we can strengthen a little Lemmas 2.4 and 3.2 of \cite{FSIT}.

\begin{definition}\label{weak0}
Let $\N$ be a $\J$-structure with $E^\N\neq\emptyset$. If $E^\N$ is a set of 
partial extenders over $\N$, all with the same critical point $\mu$, then we 
define $\mu(E^\N)=\mu$.

Let $\M$ be a $\J$-model. Let $\R$ be an $\Ll_0$-structure (possibly illfounded). If $\M$ is 
type 3 then let $\pi:\R\to\M^\sq$, and otherwise let $\pi:\R\to\M$.

We say that $\pi$ is a \textbf{weak $0$-embedding} iff $\pi$ is 
$\Sigma_0$-elementary (therefore $\R$ is extensional and wellfounded, so we assume $\R$ is 
transitive) and there is an $\in$-cofinal set $X\sub\R$ such that 
$\pi$ is $\Sigma_1$-elementary on elements of $X$, and if $\M$ is type 1 or 2, 
then (by the proof of \ref{lem:Qformula_pres_weak0} it follows that 
$\mu=\mu(E^\R)$ is defined) there is an $\in\cross\in$-cofinal set 
$Y\sub\R|(\mu^+)^\R\cross\R$ such that $\pi$ is $\Sigma_1$-elementary on 
elements of $Y$.

More generally, we define \textbf{(weak, near) $k$-embedding} analogously to \cite{FSIT}. 
Let $\M$ be a $\J$-model of type 3. A (weak, near) $k$-embedding $\pi:\N\to\M$ 
literally has domain $\univ{\N^\sq}$ and codomain $\univ{\M^\sq}$ and the elementarity of $\pi$ is 
with regard to $\N^\sq,\M^\sq$. Here either $\N$ is a $\J$-model of type 3 (so $\N^\sq\neq\N$) or 
$\N$ is a $\J$-structure which we are already considering ``at the squashed level'' (for example, 
$\N=\Ult(\Q^\sq,E^\Q)$ for some $\J$-model $\Q$ of type 3), in which case $\N^\sq$ denotes $\N$ 
itself.
\end{definition}
\end{comment}
\begin{comment}
\begin{lemma}\label{lem:Qformula_pres_weak0}
Let $\pi,\R,\M$ be as in \ref{weak0}, with $\pi$ a 
weak $0$-embedding.\footnote{In case of any confusion in relation to the last paragraph of 
\ref{weak0}, let us clarify that here if $\M$ is type 3 then we are considering $\R$ 
``at the squashed level''.}
\begin{enumerate}[label=\tu{(}\arabic*\tu{)}]
\item\label{item:Jstructure} $\R$ is a $\J$-structure.
\item\label{item:nottype3} Suppose $\M$ is not type 3. Then for any Q-formula $\psi$ and
$z\in\R$, if $\M\sats\psi(\pi(z))$ then $\R\sats\psi(z)$.
Therefore $\R$ is a $\J$-model of the same type as $\M$.
\item Suppose $\M$ is type 3. Then for any P-formula $\psi$ and $z\in\R$,
if $\M^\sq\sats\psi(\pi(z))$ then $\R\sats\psi(z)$.
Let $\Uu=\Ult(\R,\actext^\R)$, $\gamma=\OR(\R)$ and $\lambda=(\gamma^+)^{\Uu}$. If 
$\Uu|\lambda$ is wellfounded then $\R=\N^\sq$ for some $\J$-model $\N$ of type 3.
\end{enumerate}
\end{lemma}
\begin{proof}
Let $X$, and $Y$ if $\M$ is type 1 or 2, witness that $\pi$ is a weak $0$-embedding.

We first prove \ref{item:Jstructure}. Given $x\in\R$, let $y\in X$ 
with $x\in y$. Since $\M\sats$``$\pi(y)\in\Ss^{S^\M}_\alpha(\hmb^\M)$ for some 
ordinal $\alpha$'', therefore $\R\sats$``$y\in\Ss^{S^\R}_\alpha(\hmb^\R)$ for 
some ordinal $\alpha$''. This suffices.

We now prove \ref{item:nottype3} assuming that $\M$ is type 1 or 2.
The function $f$ is $\Sigma_1^\R$, where $f:\R\to\R$ and
$f:y\mapsto\Ss_\alpha^{S^\R}(\hmb^\R)$
where $\alpha$ is least such that $y\in\Ss_\alpha^{S^\R}(\hmb^\R)$. Therefore 
we may and do assume that $X\sub\rg(f)$ and $Y\sub\rg(f)\cross\rg(f)$.

Now by $\Sigma_1$-elementarity without parameters, $E^\R\neq\emptyset$ and 
$\gamma^\R$ is defined, and since $\pi$ is $\Sigma_0$-elementary, 
$\pi``E^\R\sub E^\M$ and $\pi(\gamma^\R)=\gamma^\M$. Therefore
$\mu=\mu(E^\R)$ is defined.

Now for simplicity assume that $\psi$ has only $n=1$ free variable. Suppose 
\[ \psi(z)\ \iff\ \all x\all\theta<(\mu^+)\ex y\ex\nu[x\sub y\ \&\ 
\theta\leq\nu<(\mu^+)\ \&\ \varphi(z,y,\nu)] \]
where $\varphi$ is $\Sigma_1$. Let $z\in\R$ be such that $\M\sats\psi(\pi(z))$.
Let $x\in\R$ and $\theta<(\mu^+)^\R$. Let $x\in x'\in\R$ and $\theta\in 
t\in\R|(\mu^+)^\R$ be such that $(x',t)\in Y$. Let $\theta'=\OR(t)$. Then 
\[ \M\sats\ex y\ex\nu[\pi(x')\sub y\ \&\ \pi(\theta')\leq\nu\ \&\ 
\car(\theta')=\car(\nu)\ \&\ \varphi(\pi(z),y,\nu)], \]
and this statement pulls back under $\pi$, which completes the proof.

We leave the remaining cases to the reader.
\end{proof}



\begin{comment}
Suppose also that $\OR^{\P}$ is a strong cutpoint of $\N$. Then 
one might want to say that $\N|((\OR^\P)^+)^\N$ is $\Lp^\Sigma(\P)$. However, 
this is not likely to be true, for the trivial 
reason that these two structures are not even in the same hierarchy: in 
$\Lp^\Sigma(\P)$, $\P$ is treated as a coarse object, ignoring the history in 
$\P$, but in $\N|(\OR(\P)^+)^\N$, this history is respected. In the definition 
of \emph{operator}, When $i=2$ we respect two layers of history (given 
it exists). Having the latter respect gives us convenient terminology to define 
an analogue $\Lp^\Sigma_+(\P)$ of $\Lp^\Sigma_+(\P)$, which \emph{is} in the 
same hierarchy as $\N$.
\end{comment}

\begin{comment}
\begin{definition}\label{operatorWithParama}
Let $\opbk$ be an operator background. A \textbf{operator over $\opbk$ with 
domain $D$} is a function $\Fop:D\to\opbk$ where for some (maybe
swo'd) cone $C=C_\Fop$ of $\opbk$:
\begin{enumerate}[label=--]
 \item $D\sub\{0,1\}\cross C$,
 \item for all $X\in C$ we have $(0,X)\in D$,
 \item for all $(1,X)\in D$, $X$ is a $\J$-model over some $X_1\in C$,
\end{enumerate}
and for each $(i,X)\in D$, $\Fop_i(X)=\Fop(i,X)$ is a $\J$-model over $X$ 
such that for each $\P\wins \Fop_i(X)$, $\P$ is fully 
sound. (Note that $\P$ is a $\J$-model over $X$, so soundness is in this 
sense.)

Let $\Fop,D,\opbk$ be as above. For $a\in\opbk$ we say that $a$ is a \textbf{base for 
$\Fop$} iff $C_\Fop$ contains the (swo'd) cone above $a$. We say $\Fop$ is \textbf{forgetful} iff 
$\Fop_0(X)=\Fop_1(X)$ whenever $(0,X),(1,X)\in D$, and whenever $X$ is a 
$\J$-model over $X_1$, and $X_1$ is a $\J$-model over $X_2\in C_\Fop$ and $X\down X_2$ is 
acceptable, 
$\Fop_1(X)=\Fop_1(X\down X_2)$. 
Otherwise we say $\Fop$ is \textbf{historical}.
We say $\Fop$ is \textbf{basic} iff for all 
$(i,X)\in D$ and $\P\wins\Fop_i(X)$, we have $E^\P=\emptyset$.
We say $\Fop$ is \textbf{projecting} iff for all $(i,X)\in D$, we have 
$\rho_\om^{\Fop_i(X)}=X$.
\end{definition}

At times we write $\Fop(X)$ instead of $\Fop_i(X)$. Note that $\opbk,C_\Fop$ are determined 
by $\dom(\Fop)$.
Here are some examples of the above terminology. Strategy 
operators (to be explained in more detail later) are basic, and as usually 
defined, projecting and historical. The operator $\Fop(X)=X^\#$ is forgetful 
and projecting, and not basic.

\begin{definition}
For any $P$ and any ordinal $\alpha\geq 1$, the (pre-)operator $\Jop_\alpha(\ \cdot\ ;P)$ 
is defined as follows.\footnote{The ``$\mathsf{m}$'' is 
for 
``model''.} For $X$ such that $P\in\J_1(\hat{X})$, let
$\Jop_{\alpha}(X;P)$ be the $\J$-model $\M$ over $X$, with parameter $P$, such 
that
$\univ{\M}=\J_\alpha(\hat{X})$ and for each $\beta\in[1,\alpha]$, $\M|\beta$ is 
passive. Clearly $\Jop_\alpha(\ \cdot\ ;P)$ is basic and forgetful.
If $P=\emptyset$ or we wish to supress $P$, we just 
write $\Jop_\alpha(\ \cdot\ )$.
\end{definition}
\end{comment}
\begin{comment}
\begin{definition}[Potential $\Fop$-premouse]\label{potentialJpremouse}
Let $\Fop$ be an operator and $b\in C_\Fop$. A \textbf{potential
$\Fop$-premouse over $b$} is a $\J$-model $\M$ over $b$
such that there is an ordinal $\iota>0$ and an increasing, closed sequence
$\langle \zeta_\alpha \rangle_{\alpha\leq \iota}$ of ordinals such that for each
$\alpha\leq \iota$, we have:
\begin{enumerate}
\item $0=\zeta_0\leq\zeta_\alpha\leq\zeta_\iota=l(\M)$ (so $\M|\zeta_0=b$ and
$\M|\zeta_\iota=\M$).
\item If $1<\iota$ then $\M|\zeta_1=\Fop_0(b)$.
\item If $1=\iota$ then $\M\wins\Fop_0(b)$.
\item If $1<\alpha+1<\iota$ then
$\M|\zeta_{\alpha+1}=\Fop_1(\M|\zeta_\alpha)\down b$.
\item If $1<\alpha+1=\iota$, then $\M\wins
\Fop_1(\M|\zeta_\alpha)\down b$.
\item If $\alpha$ is a limit then $\M|\zeta_\alpha$ is $B$-passive.
\end{enumerate}
We say that $\M$ is \textbf{($\Fop$-)whole} iff, if
$\iota=\alpha+1$ then $\M = \Fop_1(\M|\zeta_\alpha)\down b$.

A \textbf{(potential) $\Fop$-premouse} is a (potential) $\Fop$-premouse over 
$b$, for some $b$.
\end{definition}
\end{comment}
\begin{comment}
Note that if $\Fop$ is over $\opbk$ and $\M$ is a potential $\Fop$-premouse then 
$\OR(\M)\leq\OR(\opbk)$.

\begin{definition}\label{dfn:pot_cont_pm}
Let $\Fop$ be an operator and $b\in C_\Fop$. Let $\N$ be a whole
$\Fop$-premouse over $b$. A \textbf{potential continuing $\Fop$-premouse over 
$\N$} is a $\J$-model $\M$ over $\N$ such that $\M\down b$ is a potential 
$\Fop$-premouse over $b$. (Therefore $\N$ is a whole strong cutpoint of $\M$.)

We say that $\M$ (as above) is \textbf{whole} iff $\M\down 
b$ is whole.

A \textbf{(potential) continuing $\Fop$-premouse} is a (potential) continuing 
$\Fop$-premouse over $b$, for some $b$.
\end{definition}


\begin{definition}
An \textbf{operator over $\opbk$} is an operator $\Fop$ over $\opbk$ such that  for 
every sound whole $\Fop$-premouse $\M\in\opbk$, $(1,\M)\in\dom(\Fop)$.

We say that an operator $\Fop$ is
\textbf{uniformly $\Sigma_1$} iff there are $\Sigma_1$ formulas $\varphi_1$ and 
$\varphi_2$ in $\Ll_0^-$ such that for all (continuing) 
$\Fop$-premice $\M$, 
then
the set of whole proper segments of $\M$ is defined over $\M$ by $\varphi_1$ 
($\varphi_2$). For 
such an operator $\Fop$, let $\varphi^\Fop_\wh$ denote the least such 
$\varphi_1$.

 Given a $\J$-model $\R$ and $\varphi$ in $\Ll_0^-\mhyphen\Sigma_1$ and $\P\wpins\R$, 
we say that $\P$ is \textbf{$\varphi$-putatively whole (for $\R$)} iff 
$\R\sats\varphi(\P)$.
\end{definition}


\begin{lemma}\label{lem:critFext}
Let $\Fop$ be a projecting, uniformly $\Sigma_1$ operator and let 
$b\in C_\Fop$. Let $\M$ be an $\Fop$-premouse.
Let $0<\eta<\wl(\M)$ be such that $\M|\eta$ is whole and let 
$\gamma\in[\Theta^\M,\OR(\M|\eta)]$ be a cardinal of $\M$. Then 
$\gamma\leq\eta$ and $\OR(\M|\gamma)=\gamma$ and $\M|\gamma$ is a limit of whole 
proper segments of $\M$.
\end{lemma}
\end{comment}
\begin{comment}
For (b),
suppose $\kappa=\crit(E)\leq\OR(\N)$. Let $\varphi$ be a $\Sigma_1$ formula of 
$\Ll_0^-$ such that 
$\{x\in\M\st\M\sats\varphi(x)\}$ is precisely the set of whole proper 
segments of $\M$. Then by (a), $\M\sats$``For every cardinal 
$\gamma\geq\Theta$, there are unboundedly many $\P\wpins\M|\gamma$ such that 
$\varphi(\P)$''. Also, because every proper segment of an $\Fop$-premouse is an 
$\Fop$-premouse, $\M\sats$``For all $\gamma<\wl(\M)$, if $\varphi(\M|\gamma)$ 
then $\M|(\gamma+1)\sats\varphi(\M|\gamma)$''. Therefore $\Ult(\M,E)$ 
satisfies both of these statements. But $\Theta^{\Ult(\M,E)}=\Theta^\M<\lh(E)$ 
and $\lh(E)$ is a cardinal in $\Ult(\M,E)$. But then $\M|\lh(E)\sats$``I am a 
limit of segments $\P$ such that $\varphi(\P)$''. But $\M|\lh(E)$ is an 
$\Fop$-premouse, so each such $\P$ is whole. This contradicts the choice of 
$\N$.
\end{comment}

\begin{comment}
\begin{lemma}
Let $\Fop$ be a projecting, uniformly $\Sigma_1$ operator and let 
$b\in\C_\Fop$. 
Then $\Lp^\Fop(b)$ is a countably iterable $\Fop$-premouse over $b$, is a limit 
of 
whole proper segments projecting to $b$, and satisfies $\ZFmin$.

Let $\N$ be an $\Fop$-premouse over $b$. Then either the analogous statement 
holds regarding $\Lp^\Fop_+(\N)$, or else $\M=\Lp^\Fop_+(\N)$ is a 
countably iterable, sound, continuing $\Fop$-premouse over $\N$ which 
projects to $\N$, and $\M\down b$ is not sound.
\end{lemma}
\begin{proof}
We just discuss $\Lp^\Fop(b)$. We omit the phrase ``over $b$''.

\begin{claim}
Let $\M$ be a
sound $\Fop$-premouse projecting to $b$. Let $\M|\zeta$ be the largest whole 
segment of $\M$. Then $\M|\zeta\in\dom(\Fop)$ and $\Fop(\M|\zeta)\down b$ 
is a 
sound $\Fop$-premouse projecting to $b$. Moreover, if $\M$ is countably 
iterable, 
then so is $\Fop(\M|\zeta)\down b$.
\end{claim}
\begin{proof}
Let $\R=\Fop(\M|\zeta)$. Note that $\M\wins\R\down b$.
The iterability and the fact that $\R\down b$ projects to $b$ 
is because $\M$ is sound and projects to $b$ and $\R$ is sound and 
projects to $\M|\zeta$.

So let $P\wins\R$ with $\M\in P$; we just need to see 
that $P\down b$ is sound.
If $\rho_\om^P\neq\M|\zeta$ then this follows 
easily because $P$ is sound. Suppose $\rho_\om^P=\M|\zeta$, and let $k<\om$ be 
least such that $\rho_{k+1}^P=\M|\zeta$. In fact, for simplicity, suppose 
$k=0$; the general argument is similar. Then $\rho_1^{P\down b}=b$, since 
$\M$ projects to $b$ and is sound.

Now we may and do assume that $\M$ is minimal in that there 
is no $\M'$ such that $\M|\zeta\wins\M'\wpins\M$ and $\M'$ projects 
to $b$.

Let $p=p_1^P$. We consider two cases.

\begin{case}
 $p\neq\emptyset$.

We claim that $p_1^{P\down b}=p$ and $P\down b$ is $1$-sound.

For note that $\OR(\M|\zeta)<\min(p)$. Letting\footnote{The hulls here are 
formed in the relevant fine-structural language, so for example, we trivially 
have $b\un\{b\}\sub\Hull_1^{P\down b}(\emptyset)$.} $H=\Hull_1^{P\down 
b}(p)$, this gives that $\M|\zeta\in H$ (because $\Fop$ is uniformly 
$\Sigma_1$), 
and therefore that $\M\in H$ (by the minimality of $\M$). Since $\M$ projects 
to $b$ and is sound, therefore $\M\sub H$, so $\M|\zeta\un\{\M|\zeta\}\sub H$. 
But then since $P$ is $1$-sound, we have $P=H$. And the $1$-solidity of $p$ for 
$P$ easily implies it for $P\down b$.
\end{case}

\begin{case}
$p=\emptyset$.
 
Let $q\in\Ord^{<\om}$ be least such that $\M|\zeta\in\Hull_1^{P\down 
b}(q)$. We claim that $p_1^{P\down b}=q$ and $P\down b$ is $1$-sound.

For as in the previous case, $\Hull_1^{P\down b}(q)=P$, so it suffices to 
see that $q$ is $1$-solid for $P\down b$. Suppose for simplicity that 
$q=\{\gamma\}$ for some ordinal $\gamma$. We just need to see that 
$\Th_1^{P\down b}(\gamma)\in P$. But
\[ \Hull_1^{P\down b}(\gamma)\sub\M|\zeta, \]
by choice of $q$ and because $\Fop$ is uniformly $\Sigma_1$. Since also $P$ is 
amenable, we get $\Th_1^{P\down b}(\gamma)\in P$, as required.
\end{case}

This completes the proof of the claim.
\end{proof}

The fact that $\N=\Lp^\Fop(b)$ is a limit of whole proper segments which 
project 
to $b$, and is therefore an $\Fop$-premouse, follows immediately from the claim.
Therefore $\N$ is also countably iterable, since it is a limit of countably 
iterable segments which project to $b$.

Now suppose that $\N\not\sats\ZFmin$. It is then easy to see that $\N$ projects 
to $b$ (using the fact that cofinally many segments of $\N$ project to $b$), 
and also therefore $\N\in\dom(\Fop)$. We claim that $\N$ is sound. Since it is 
also countably iterable, the claim gives that $\Fop(\N)\down 
b\wins\Lp^\Fop(b)$, 
a contradiction. So let $\tau=\max(\om,\rank(b))$. Let $k<\om$ be such that 
$\rho_{k+1}^\N=b$ and $\rho_k^\N=\OR^\N$. Assume $k=0$ for simplicity. Let 
$p=p_{1}^\N$. It is easy to see that there is an $\rSigma_{1}^\N(p)$ partial map 
from $b^{<\om}\cross\tau^{<\om}$ cofinal into $\OR(\N)$, and therefore that 
$\Hull_1^\N(p)=\N$. For the $1$-solidity of $P$, assume for simplicity that 
$p=\gamma\in\Ord$. Then $(b\un\gamma)\sub\Hull_1^\N(\gamma)$, so 
$\Hull_1^\N(\gamma)$ is transitive, but $\gamma\notin\Hull_1^\N(\gamma)$, so
this $\Hull_1^\N(\gamma)=\N|\gamma$, which gives $1$-solidity, 
as required. This completes the proof.
\end{proof}

We remark that $\N=\Lp^\Fop(b)$ has a little more closure than just
$\ZFmin$. For let $\kappa$ be such that $\C_\Fop$ is a cone of 
$\opbk_\kappa$. If $\OR(\N)<\kappa$ then $\N\in\dom(\Fop)$, and we can 
define $\M=L^\Fop_\kappa(\N)$ in the natural manner; otherwise let $\M=\N$. It 
is 
easy to show that $\M$ has no level projecting $<\OR(\N)$ (after $\OR(\N)$), 
and that $L(\M)$ has no level projecting $<\kappa$. Also, by the preceding 
proof, every level of $L(\M)$ is fully sound.
\end{comment}

\begin{comment}
\begin{definition}
Let $x$ be transitive. We say that \textbf{countable $x$-based hulls are club} iff for 
all $a\sub\hat{x}^{<\om}$, there are club many 
countable elementary substructures of $(\hat{x}^{<\om},a)$.

Let $\Fop$ be an operator over $\opbk$ with a base in $\HC$. (Therefore 
if $x\in C_\Fop$ then for club many countable hulls $\bar{x}$ of $x$, $\bar{x}\in C_\Fop$.)

Let $\M$ be an $\Fop$-premouse over $a$ and let $n\leq\om$ (and $\eta\leq\OR(\M)$). We say that 
$\M$ is \textbf{countably (above-$\eta$) $n$-$\Fop$-iterable} iff
for club many countable substructures $\bar{\M}$ of $\M$, $\bar{\M}$ is 
an (above-$\bar{\eta}$) $(n,\om_1+1)$-$\Fop$-iterable $\Fop$-premouse (where $\bar{\eta}$ is the 
collapse of $\eta$).

Let $x\in C_\Fop$ and assume that countable $x$-based hulls are club. Then 
$\Lp^\Fop(x)$ denotes the stack of all 
countably $\om$-$\Fop$-iterable $\Fop$-premice $\M$ over $x$ such that $\M$ is fully sound 
and projects to $x$.\footnote{Our 
assumptions ensure that $\Lp^\Fop(x)$ is indeed a 
stack. For assume that $x$ is infinite and let $\M_1,\M_2$ be $\J$-models meeting the criteria. 
We can code $\M_1\oplus\M_2$ with some structure $(\hat{x}^{<\om},a)$ with $a\sub\hat{x}^{<\om}$. 
Taking a countable hull, we get $\Mbar_1,\Mbar_2$ over $\bar{x}$, which we can compare, to deduce 
that $\Mbar_1=\Mbar_2$, as usual; for the latter we just need iterability, the ISC and 
fine structure. (Because all models which appear during the comparison are 
$\Fop$-premice, all extenders used are non-$\Fop$.) If $x$ is finite, it is easier.} Assuming that 
$\RR\in\opbk$, for $X\sub\HC$, $\Lp^\Fop(\RR,X)$ 
denotes $\Lp^\Fop((\HC,X))$.\footnote{Since $\RR$ is 
not transitive, this is not an abuse of notation.}

Let $\N$ be a whole $\Fop$-premouse in $\opbk$. Then $\Lp^\Fop_+(\N)$ 
denotes the stack 
of all continuing $\Fop$-premice $\M$ over $\N$ such that $\M$ is fully sound, 
$\rho_\om^\M=\N$ and $\M\down a^\N$ is countably above-$\OR(\N)$ $(\om,\om_1+1)$-$\Fop$-iterable,
if there is any such $\M$; otherwise $\Lp^\Fop_+(\N)=\N$.
\end{definition}
\end{comment}

\begin{comment}
From now on, whenever we refer (implicitly) to $\Lp^\Fop$ or $\Lp^\Fop_+$, we are making the 
assumptions above. Note that if $x$ is countable then countable $x$-based hulls are club.
We can now describe the kinds of non-basic operators we will be interested in:
\end{comment}

\begin{comment}
\begin{definition}[Mouse operator]\label{MouseOperator}
Let $Y$ be a basic, projecting, uniformly $\Sigma_1$ operator, over $\opbk$.

A \textbf{lower $Y$-mouse operator $\Fop$}
is an operator over $\opbk$ such that for each $(i,X)$ in its domain, 
$\Fop_i(X)\wins\Lp^Y(X)$.

A \textbf{continuing $Y$-mouse operator $\Fop$} is an operator over $\opbk$ with domain $D$ 
such that for each 
$(0,X)\in D$, $\Fop_0(X)\wins\Lp^Y(X)$, and for each $(1,X)\in 
D$, $X$ is a sound whole $Y$-premouse and $X\wpins\Fop_1(X)\wins\Lp^Y_+(X)$.

Let $\Fop$ be a continuing $Y$-mouse operator. We say that $\Fop$ is \textbf{whole} iff for all 
$(0,X)\in D$, $\Fop_0(X)$ is $Y$-whole, and for all $(1,X)\in D$, either $\Fop_1(X)$ is $Y$-whole, 
or $\Fop_1(X)\down \hmb^X$ is not sound (and therefore $\Fop_1(X)=\Lp^Y_+(X)$).

Let $\Fop$ be a $Y$-mouse operator with domain $D$. Let $a$ be a set such that 
$a\in\J_1(X)$ for all $X\in D$. Then $\Fop$ is 
\textbf{first-order in $a$} iff there is an $\Ll_0$ formula $\varphi$ such 
that for
all $X\in D$, if $\Fop(X)$ is the least 
$Z\wpins\Lp^Y(X)$ such that $Z\sats\varphi(X,a)$.
\end{definition}
\end{comment}

\begin{comment}
\begin{lemma}
Let $\Fop$ be a whole continuing $Y$-mouse operator. Then every $\Fop$-premouse is a 
$Y$-premouse.
\end{lemma}
\end{comment}

\begin{comment}
We now describe background extender constructions to build $\Fop$-mice.

\begin{definition}
 Let $\N$ be an $\Fop$-premouse and $k\leq\om$. Then $\N$ is 
\textbf{$k$-$\Fop$-solid} iff $\N$ is $k$-solid, and for each 
$i\leq k$, $\core_{k}(\N)$ is an $\Fop$-premouse.
\end{definition}
\end{comment}

\begin{comment}
\begin{definition}
Given a $\J$-model $\N$ over $a$, and $\M\wpins\N$ such that $\M$ is fully 
sound, the 
\textbf{$\M$-drop-down sequence} of $\N$ is the sequence of
pairs $\left<(\Q_n,m_n)\right>_{n<k}$ of maximal length such that $\Q_0=\M$ and 
$m_0=\om$ and for each $n+1<k$:
\begin{enumerate}
 \item $\M\wpins\Q_{n+1}\wins\N$ and $\Q_n\wins\Q_{n+1}$,
 \item every proper segment of $\Q_{n+1}$ is fully sound,
 \item $\rho_{m_n}(\Q_n)$ is an $a$-cardinal of $\Q_{n+1}$,
 \item $0<m_{n+1}<\om$,
 \item $\Q_{n+1}$ is $(m_{n+1}-1)$-sound,
 \item 
$\rho_{m_{n+1}}(\Q_{n+1})<\rho_{m_n}(\Q_n)\leq\rho_{m_{n+1}-1}(\Q_{n+1})$. 
 \qedhere
\end{enumerate}
\end{definition}

\begin{comment}
\begin{definition}\label{dfn:Fop_con}
Let $\Fop$ be an operator over $\opbk$ and let $C$ be some class of $E$-active 
$\Fop$-premice. Let $b\in C_\Fop$ and $\chi\leq\OR(\opbk)+1$. A \textbf{($C$-certified) 
$L^\Fop[\es,b]$-construction (of length $\chi$)} is a 
sequence $\left<\N_\alpha\right>_{\alpha<\chi}$ with the 
following properties.

We have $\N_0=b$ and $\N_1=\Fop(0,b)$.

Let $0<\alpha<\chi$. Then $\N_\alpha$ is an $\Fop$-premouse over $b$. If 
$\alpha$ is a limit then $\N_\alpha=\liminf_{\beta<\alpha}\N_\beta$. Now suppose 
that $\alpha+1<\chi$.
Then either:
\begin{enumerate}[label=(\roman*)]
\item $\N_\alpha$ is a passive limit of whole proper segments and
$\N_{\alpha+1}=(\N_\alpha,G)$ for some extender $G$ (with $\N_{\alpha+1}\in 
C$); or
\item\label{item:apply_Fop} $\N_\alpha$ is $\om$-$\Fop$-solid. Let $\M_\alpha=\core_\om(\N_\alpha)$.
Let $\M$ be the largest whole segment of $\M_\alpha$. So either $\M_\alpha=\M$ or 
$\M_\alpha\down\M\wpins\Fop_1(\M)$.
Let $\N\wins\Fop_1(\M)$ be least such that either $\N=\Fop_1(\M)$ or for some $k<\om$, 
$(\N\down b,k+1)$ is 
on the $\M_\alpha$-drop-down sequence of $\N\down b$. Then $\N_{\alpha+1}=\N\down b$. Note 
that $\M_\alpha\wpins\N_{\alpha+1}$.\qedhere
\end{enumerate}
\end{definition}

We now proceed to describe some 
consendation properties for operators $\Fop$ under which together whether sufficient iterability 
ensure that $L^\Fop[\es]$-constructions do not break down.

\begin{definition}\label{dfn:condenses_coarsely}
 Let $Y$ be an operator. We say that $Y$ 
\textbf{condenses coarsely} iff 
for all $i\in\{0,1\}$ and $(i,\Xbar),(i,X)\in\dom(Y)$, and all $\J$-models 
$\M^+$ over $\Xbar$, if $\pi:\M^+\to Y_i(X)$ is fully elementary, then 
\begin{enumerate}[label=--]
 \item if $i=0$ then $\M^+\wins Y_0(\Xbar)$; and
 \item if $i=1$ and $X$ is a sound whole $Y$-premouse, then $\M^+\wins 
Y_1(\Xbar)$.\qedhere
\end{enumerate}
\end{definition}

\begin{lemma}\label{lem:whole_Y_pm_elem_hull}
 Let $Y$ be a uniformly $\Sigma_1$ operator which condenses coarsely and let $\M$ be an $E$-passive 
whole $Y$-premouse. Let $\pi:\N\to\M$ be fully elementary, where $\hmb^\N\in C_Y$. Then 
\tu{(}a\tu{)} $\N$ is a 
$Y$-premouse and for all 
$\P\wpins\N$, $\P$ is whole iff $\pi(\P)$ is whole. Moreover, \tu{(}b\tu{)} if $\M$ is sound or a 
limit of 
whole proper segments then $\N$ is whole.
\end{lemma}
\begin{proof}
If $\M=Y_0(\hmb^\M)$ then a slight variant of the argument to 
follow shows that $\N=Y_0(\hmb^\N)$, which suffices. So assume that $Y_0(\hmb^\M)\wpins\M$.
We claim then that for all $\P\wpins\N$, $\N\sats\varphi_Y(\P)$ iff $\P$ is a whole $Y$-premouse. 
This can be proved by induction on $\P$. We again skip the argument 
as it is similar to the one to follow.

It now follows easily that if $\Q\wins\N$ and $\Q$ is a 
limit of whole proper segments $\P$, then $B^\Q=\emptyset$ and so $\Q$ is a (whole) $Y$-premouse.
In particular, if $\M$ is a limit of whole proper segments then $\N$ is 
likewise and the lemma follows easily. So suppose instead that $\M$ has a largest whole 
proper segment; then this is $\pi(\P)$ where $\P$ is the largest whole proper segment of $\N$. 
Now $\M=Y_1(\pi(\P))\down \hmb^\M$. So by coarse 
condensation, $\N\down\P\wins Y_1(\P)$, so $\N$ is a $Y$-premouse, giving (a). 
Now suppose that $\M$ is sound but $\N\down\P\wpins Y_1(\P)$. Then there
is a $Y$-premouse $\M'$ such that $\M\wpins\M'$ and $\wl(\M')=\wl(\M)+1$. Because $Y$ is 
uniformly $\Sigma_1$, $\M'\sats\varphi_Y(\M)$. But $\varphi_Y\in\Ll_0^-$, so by elementarity, $\N$ 
is sound and $(\Jop_1(\N;\hmp^\N)\down \hmb^\N)\sats\varphi_Y(\N)$ and there is a 
$Y$-premouse $\N'$ such that $\N\wpins\N'$ and $\univ{\N'}=\J_1(\N)$. But then 
$\N'\sats\varphi_Y(\N)$, so $\N$ 
is whole, contradiction. This proves (b).
\end{proof}
\end{comment}

\begin{comment}
\begin{lemma}\label{lem:E_active_Y_pm_elem_hull}
Let $Y$ be a uniformly $\Sigma_1$ operator which condenses coarsely and let $\M$ be an $E$-active
$Y$-premouse. Let $\pi:\N\to\M$ be a weak $0$-embedding, where $a^\N\in C_Y$. If $\M$ is type 3, 
suppose also that 
$\Ult(\M^\sq,E^\M)$ is a $Y$-premouse. Then $\N$ is a $Y$-premouse.
\end{lemma}
\begin{proof}
Consider the case that $\M$ is type 3. Let 
$\psi:\Ult(\N^\sq,E^\N)\to\R=\Ult(\M^\sq,E^\M)$
be the map induced by $\pi$. Let $\psi'=\psi\rest(\N||\OR(\N))$. 
Then $\psi':\N||\OR(\N)\to\R|\psi(\OR(\N))$ is fully elementary. Now 
apply \ref{lem:whole_Y_pm_elem_hull} and \ref{lem:Qformula_pres_weak0}.
\end{proof}
\end{comment}

\begin{comment}
\begin{definition}
Let $\M,\N$ be $k$-sound $\J$-models over $a,b$ and 
$\pi:\M\to\N$. Then $\pi$
is \textbf{(weakly, nearly) $k$-good} iff $\pi\rest a\un\{a\}=\id$ and $\pi$ is 
a (weak, near)
$k$-embedding.

If $\pi\colon\M\to\N$ is a weak $0$-embedding then $\pi$ is 
\textbf{$\nu$-preserving} iff, if $\M,\N$ are type 3 (so literally 
$\pi\colon\M^\sq\to\N^\sq$) and $a,f\in\M^\sq$ are such that 
$\nu(E^{\M})=[a,f]^{\M}_{E^{\M}}$, then $\nu(E^{\N})=[\pi(a),\pi(f)]^{\N}_{E^{\N}}$. 
\end{definition}
\begin{remark}
We use the following in place of the notion of \emph{condenses well} (see 
\cite[2.1.10]{wilson2012contributions}). We explain why we made this 
replacement in Appendix \ref{app:condenses}.
\end{remark}
\end{comment}
\begin{comment}
\begin{definition}\label{dfn:condenses_finely}
Let $Y$ be a projecting, uniformly $\Sigma_1$ operator. We say that $Y$ 
\textbf{condenses finely} iff $Y$ condenses 
coarsely and we have the following. Let $k<\om$. Let $\M^*$ 
be a $Y$-premouse over $a$, with a largest whole proper segment $\M$, 
such that $\M^+=\M^*\down\M$ is sound and $\rho_{k+1}(\M^+)=\M$. Let 
$\P^*,\abar,\P,\P^+$ be likewise. Let $\N$ be a sound whole $Y$-premouse over 
$\abar$. Let
$G\sub\Coll(\om,\P\un\N)$ be $V$-generic. Let $\N^+,\pi,\sigma\in V[G]$,
with $\N^+$ a sound $\J$-model over $\N$ such that
$\N^*=\N^+\down\abar$ is defined (i.e. acceptable). Suppose $\pi:\N^*\to\M^*$ is such that
$\pi(\N)=\M$ and
either:
\begin{enumerate}
 \item $\M^*$ is $k$-sound and $\N^*=\core_{k+1}(\M^*)$; or
 \item $(\N^*,k+1)$ is in the 
$\N$-dropdown sequence of $\N^*$, and likewise $(\P^*,k+1),\P$, and 
either:
\begin{enumerate}
\item\label{item:condense_k-good} $\pi$ is $k$-good, or

\item\label{item:condense_fully} $\pi$ is fully elementary, or

\item\label{item:condense_realize} $\pi$ is a weak $k$-embedding, 
$\sigma:\P^*\to\N^*$ is 
$k$-good, $\sigma(\P)=\N$ and $\pi\com\sigma\in V$ is a near $k$-embedding.
\end{enumerate}
\end{enumerate}
Then $\N^+\wins Y_1(\N)$.

We say that $Y$ \textbf{almost condenses finely} iff $\N^+\wins Y_1(\N)$ whenever the hypotheses 
above hold with $\N^+,\pi,\sigma\in V$.
\end{definition}

In the preceding definition, if $\N^*,\M^*$ are type 3, and so 
$\dom(\pi)=(\N^*)^\sq$, then by \ref{lem:critFext}, 
$\OR(\M)<\crit(E^{\M^*})<\nu(E^{\M^*})$, so it is reasonable to say 
that $\pi(\N)=\M$, for instance.
\end{comment}

\begin{comment}
\begin{lemma}\label{lem:almost_condenses_finely}
Let $Y$ be an operator over $\opbk$ with base in $\HC$. Suppose that $Y$ almost condenses 
finely. Then $Y$ condenses finely.
\end{lemma}
\begin{proof}
Suppose not. Let $\M^*,\P^*,\N^+$, etc, as in \ref{dfn:condenses_finely}, constitute a 
counterexample. Let $\M^\$=Y_1(\M)$ and $\P^\$,\N^\$$ likewise. Since $\M^*$ has a 
largest whole proper segment, $\M^*$ and all other
relevant objects are in $\opbk$. Note that $\N^\$\not\wins\N^+$. For if 
$\N^\$\wpins\N^+$ then $\N^\$\down a^\N$ is a sound $Y$-premouse and there is a $Y$-premouse 
$\N'$ such that $\univ{\N'}=\J_1(\N^\$)$. But then because $Y$ is uniformly $\Sigma_1$ and using 
$\pi$, $Y_1(\M)\wpins\M^+$, contradiction.

Let $\PP=\Coll(\om,\P\un\N)$. Let $X\in\opbk$ be transitive, containing all relevant 
objects, and such that $X\sats(\ZFmin)^{-\eps}$. (For any $A\in\opbk$ there is 
$\gamma$ such that $L_\gamma(A)\sats(\ZFmin)^{-\eps}$, so there is such a $\gamma<\OR(\opbk)$.) In 
particular, in $X$ we have $\M,\N,\P$, 
etc, and have $p\in\PP$ and $\PP$-names $\tilde{{\N}}^+,\tilde{\pi},\tilde{\sigma}$ for 
$\N^+,\pi,\sigma$, and in $X$, $p$ forces that
\begin{equation}\label{eqn:force_counterex} \text{``}\M^*,\tilde{\N}^+,\N^\$\text{, etc, 
satisfy the hypotheses of \ref{dfn:condenses_finely} and 
}\tilde{\N}^+\not\wins\N^\$\ \&\ \N^\$\not\wins\tilde{\N}^+\text{''.}\end{equation}
Let $\pi:Z\to X$ be 
elementary with $Z$ countable, and everything 
relevant in $\rg(\pi)$. Let $\pi(\N^Z)=\N$, etc. Let $G\sub\Coll(\om,\P^Z\un\N^Z)$ be 
$Z$-generic with $p^Z\in G$. Then because $Y$ condenses coarsely and by 
\ref{lem:whole_Y_pm_elem_hull} and \ref{lem:E_active_Y_pm_elem_hull}, 
$(\M^*)^Z,(\tilde{\N}^+)^Z_G$, etc, satisfy the hypotheses of 
\ref{dfn:condenses_finely}, and $(\N^\$)^Z\wins Y_1(\N^Z)$. But then because $Y$ 
almost condenses finely, $(\tilde{\N}^+)^Z_G\wins Y_1(\N^Z)$. Therefore either 
$(\N^\$)^Z\wins(\tilde{\N}^+)^Z_G$ or $(\tilde{\N}^+)^Z_G\wins(\N^\$)^Z$, contradicting line 
\ref{eqn:force_counterex}.\end{proof}

\begin{definition}
An \textbf{$\Fop$-putative iteration tree} is a putative $\Fop$-iteration tree. (That is, 
every model of $\Tt$ except the last, if there is one, is an $\Fop$-premouse, and every extender 
used in $\Tt$ is non-$\Fop$).

An \textbf{$\Fop$-putative iteration strategy} for a $\J$-model
$\N$ is 
a function $\Sigma$ such that for each limit length $\Fop$-tree $\Tt$ on $\N$, 
via 
$\Sigma$, $\Sigma(\Tt)$ is a $\Tt$-cofinal branch $b$. (Thus, player $\plII$ 
\emph{wins} any round of the iteration game which has a last model 
which is not an $\Fop$-premouse, and in particular, wins by default if $\N$ is 
not an $\Fop$-premouse.)
\end{definition}
\end{comment}

\begin{comment}
\begin{lemma}\label{lem:strong_condenses_coarsely}
Let $Y,\Fop$ be uniformly $\Sigma_1$ operators with bases in $\HC$. Suppose that $Y$ 
condenses finely. Suppose that $\Fop$ is a whole continuing $Y$-mouse operator. Then \tu{(}a\tu{)} 
$\Fop$ 
condenses finely. Moreover, \tu{(}b\tu{)} let 
$\M$ be an $\Fop$-whole $\Fop$-premouse. Let $\pi\maps\N\to\M$ be fully elementary with $\hmb^\N\in 
C_\Fop$. Then $\N$ is an 
$\Fop$-whole 
$\Fop$-premouse. So regarding $\Fop$, the conclusion of \ref{dfn:condenses_coarsely} may be 
modified by 
replacing ``$\wins$'' with ``$=$''.
\end{lemma}
\begin{proof}[Proof Sketch]
Let $\Fop,Y$ be over $\opbk$. Consider (a). By \ref{lem:almost_condenses_finely} it 
suffices to see that $\Fop$ almost condenses finely. We just 
consider the case of this proof when (\ref{item:condense_realize}) of \ref{dfn:condenses_finely} 
holds (omitting the proof that $\Fop$ condenses coarsely), since this illustrates the main points. 
So suppose that $\M^*$, etc, are as in (\ref{item:condense_realize}) of \ref{dfn:condenses_finely}.

Let us first observe that $\N^*$ is a $Y$-premouse. This is easy if $\P^*$ has no largest $Y$-whole 
proper segment, so suppose otherwise, and let $\P_Y$ be the largest. Since $\P$ is $\Fop$-whole 
and $\Fop$ is whole, therefore $\P\wins\P_Y\wpins\P^*$. Then $\M_Y=\pi(\sigma(\P_Y))$ is the 
largest 
$Y$-whole proper segment of $\M^*$, so by \ref{lem:whole_Y_pm_elem_hull} and 
\ref{lem:E_active_Y_pm_elem_hull} and using $\pi$, $\N_Y=\sigma(\P_Y)$ is a sound $Y$-whole
$Y$-premouse. Also,  $(\P^*,k+1)$ is on the $\P_\Fop$-dropdown sequence of $\P^*$, and so on 
the $\P_Y$-dropdown sequence of $\P^*$. Likewise $\N^*,\N_Y$. Since $Y$ 
condenses finely, this implies that $\N^+\wins Y_1(\N_Y)$, so $\N^*$ is a $Y$-premouse.

So $\N^+$ is a sound continuing $Y$-premouse (over $\N$) and
$\rho_{k+1}(\N^+)=\N$. We claim that $\N^+$ is countably $k$-$Y$-iterable. Given this, 
$\N^+\wins\Lp_+^Y(\N)$, so either $\N^+\wins\Fop_1(\N)$ or $\Fop_1(\N)\wins\N^+$. But then 
$\N^+\wins\Fop_1(\N)$ because if $\Fop_1(\N)\wpins\N^+$ then the usual argument shows that 
$\Fop_1(\M)\wpins\M^+$, a contradiction. So it suffices to prove this claim.

Let $X\in\opbk$ be transitive and containing all relevant objects. Let $\tau:Z\to X$ be 
elementary, with $Z$ countable, and such that $\tau^{-1}(\M^*,\P^*,\N)$ are 
$Y$-premice and $\tau^{-1}(\M^+)$ is $k$-$Y$-iterable. Using $\tau^{-1}(\pi)$ we can lift 
(above-$\tau^{-1}(\N)$) $Y$-putative trees on $\tau^{-1}(\N^+)$ to $Y$-trees on $\tau^{-1}(\M^+)$. 
Let $\Tt$ on $\tau^{-1}(\N^+)$ be via this strategy, of length $\alpha+1$. Then using that $Y$ 
condenses finely and standard fine structure, one can show that $M^\Tt_\alpha$ is 
a $Y$-premouse. (One extra point here is the following. Suppose $M^{\pi\Tt}_\alpha$ is type 3. Then 
literally the copy map $\pi_\alpha:(M^\Tt_\alpha)^\sq\to(M^{\pi\Tt}_\alpha)^\sq$, so it is not 
immediate that $M^\Tt_\alpha$ is a $Y$-premouse. Let
\[ \psi:\Ult(M^\Tt_\alpha,E(M^\Tt_\alpha))\to\Ult(M^{\pi\Tt}_\alpha,E(M^{\pi\Tt}_\alpha))\]
be the map induced by $\pi_\alpha$. Then using $\psi$ and $\pi_\alpha$ together one can show that 
$M^\Tt_\alpha$ is wellfounded and is a $Y$-premouse.)

Part (b) follows from \ref{lem:whole_Y_pm_elem_hull} and \ref{lem:E_active_Y_pm_elem_hull}, and the 
observation that if $\N$ has a largest $\Fop$-whole proper segment $\N_\Fop$ and $\N$ is unsound 
then $\N\down\N_\Fop=\Lp_+^Y(\N_\Fop)$, and so $\N\down\N_\Fop=\Fop_1(\N_\Fop)$.

This completes the sketch of the proof.
\end{proof}
\end{comment}
\begin{comment}
We first show that $\Fop$ condenses coarsely. Let $X$ be a sound whole $\Fop$-premouse and let 
$\M^+$ be a $\J$-model over $\Xbar$ and $\pi:M^+\to\Fop_1(X)$ be elementary.
Now $\M^*=\Fop_1(X)\down a^X$ is a $Y$-premouse (because it is an $\Fop$-premouse). If $\M^*$ is 
$Y$-whole it is easier (we can make do with the fact that $Y$ condenses coarsely, instead of 
finely), so assume otherwise. Since $\M^*$ is $\Fop$-whole but not $Y$-whole, $\M^*$ is not 
sound (by \ref{dfn:continuing_mop}). Let $X^*$ be the largest $Y$-whole proper segment of $\M^*$. 
Then $X\wins X^*$ ($X$ is sound, and therefore $Y$-whole). So $X^*$ is sound, but $\M^*$ is not, 
which implies that for some $k<\om$, $(\M^*,k+1)$ is on the $X^*$-dropdown sequence of $\M^*$ (see 
\ref{...}). Because $Y$ condenses finely and by \ref{...}, it follows that $\M^+$ is a 
$Y$-premouse, and note that $\pi(X^+)=X^*$ for some $X^+$, and that $\M^+\wins Y_1(X^+)\down 
a^\Xbar$. Also by elementarity, $\M^+$ is not sound. Now arguing as in \ref{...} and \ref{...} we 
get that $\M^+$ is an $\Fop$-premouse, and $\M^+\wins\Fop_1(\Xbar)$, as required. 
(For example, given $\P\wpins\Q\wpins\M^+$ such that $\P$ is $\Fop$-whole, and therefore $Y$-whole, 
and $\P$ is $\varphi_\Fop$-putatively whole, show that $\Q$ is $Y$-iterable above $\P$, by using 
$\pi$ to lift to $\pi(\Q)$, and that $Y$ condenses finely.)  
Since every $\Fop$-premouse is a $Y$-premouse, by \ref{lem:...}, $\N$ is a $Y$-premouse.

Now let $\pi:\N\to\M$ be fully elementary, where $\M$ is an $\Fop$-whole $\Fop$-premouse. By 
\ref{...}, we now know that $\N$ is an $\Fop$-premouse; we want to see that $\N$ is $\Fop$-whole. 
If $\M$ is sound or a limit of $\Fop$-whole segments then this is by \ref{...}, so assume 
otherwise. Let $\P\wpins\M$ be the largest $\Fop$-whole proper segment of $\M$; so $\pi(\Q)=\P$ for 
some $\Q\wpins\N$. Then because $\M$ is not sound, one can show that $\M=\Lp_+(\P)\down a^\M$, and 
conclude that $\N=\Lp_+(\Q)\down a^\N$.
\end{comment}

\begin{comment}
\begin{definition}\label{dfn:condenses_basically}
Let $Y$ be a projecting, uniformly $\Sigma_1$ operator. We say that 
$Y$ \textbf{condenses basically} iff $Y$ condenses 
coarsely, and we have the following. Let $k<\om$. Let $\Mbar,\M$ be 
whole $Y$-premice over $a$. Let $\M^+\wins Y(1,\M)$ and let $\Mbar^+$ be a 
$\J$-model over $\Mbar$. Suppose that all proper segments of 
$\Mbar^*=\Mbar^+\down a$ and of $\M^*=\M^+\down a$ are fully 
sound. Suppose that $(\M^*,k+1)$ is on the $\M$-drop-down sequence of 
$\M^*$, and likewise $(\Mbar^*,k+1),\Mbar$. Suppose there is a nearly 
$k$-good $\pi:\Mbar^*\to\M^*$ with 
$\pi(\Mbar)=\M$ and $p_{k+1}\cut\theta\in\rg(\pi)$, where 
$\theta=\car^{\M^*}(\OR(\M))$. Then $\Mbar^*\wins Y(1,\Mbar)$.\end{definition}

Note that in the previous definition, we do not assume that $\Mbar^+$ is sound, 
but the conclusion implies that $\Mbar^+$ is indeed sound.
This means that one cannot expect that mouse operators will condense basically 
in general. However, it is reasonable to expect a strategy operator to condense 
basically.
\end{comment}

\begin{comment}
\begin{lemma}
 Let $Y$ be a basic, projecting, uniformly $\Sigma_1$ operator. Let $\Fop$ be a 
projecting, uniformly $\Sigma_1$, $Y$-mouse operator. Suppose that $Y$ 
condenses basically and finely. Then $\Fop$ condenses finely.
\end{lemma}
\begin{proof}
 Because $\Fop$ is uniformly $\Sigma_1$ and because of the existence of $\pi$, 
it suffices to show that $\Mbar^+\wins\Lp^Y(\Mbar)$. But $\Mbar^+$ is sound and 
projects to $\Mbar$ by hypothesis. So it suffices to see that $\Mbar^+$ is a
$Y$-premouse and is iterable (above $\Mbar$).

Let $\psi=\varphi^Y_\wh$. Suppose that $\Mbar^*$ has a largest proper 
$\psi$-whole segment $\Nbar$, as the contrary case is simpler. Now because $Y$ 
condenses coarsely and using $\psi$ and $\pi$, we get that $\pi(\Nbar)$ is 
$Y$-whole and $\Nbar$ is a whole $Y$-premouse. Because $(\Mbar^*,k+1)$ is on 
the $\Mbar$-drop-down sequence of $\Mbar^*$, it is easy to see that 
$(\Mbar^*,k+1)$ is also on the $\Nbar$-drop-down sequence of $\Mbar^*$. 
Likewise for $(\M^*,k+1)$ and $\pi(\Nbar)$. Because $\pi$ is $\Sigma_1$ 
elementary, $\pi(\Nbar)$ is the largest whole proper segment of $\M^*$. 

Now suppose that $\pi$ is $k$-good. Consider using $\pi$ to lift a 
$k$-maximal tree $\Tt$ on $\Mbar^+$ to a tree $\Uu$ on $\M^+$. We claim that 
every model on $\Tt$ is a $Y$-premouse. For let $\pi_\alpha$ be the 
$\alpha^\nth$ copy map. The $\psi$-whole proper segments of $M^\Tt_\alpha$ are 
in fact whole $Y$-premice by coarse condensation. So we may assume that 
$M^\Tt_\alpha$ has a largest whole proper segment $N^\Tt_\alpha$. Since $\pi$ is 
(nearly) $k$-good, $\pi_\alpha$ is also nearly $\deg^\Tt(\alpha)$-good, and in 
particular, $\pi_\alpha(N^\Tt_\alpha)$ is the largest whole proper 
segment of $\M^{\Uu}_\alpha$. Suppose now that $[0,\alpha]_\Tt$ does not 
drop in model or degree. Then $\pi_\alpha$ is in fact $k$-good. 
Moreover, letting $(M^\Tt_\alpha)'$ be the $\J$-model with parameter 
$N^\Tt_\alpha$ such that $M^\Tt_\alpha=(M^\Tt_\alpha)'\down a$, 
then $(M^\Tt_\alpha)'$ is sound. (This is because if $\beta<_\Tt\alpha$ 
then $\crit(i^\Tt_{\alpha,\beta})<\OR(N^\Tt_\beta)$.) Likewise for 
$(M^\Uu_\alpha)'$. But $\pi_\alpha:(M^\Tt_\alpha)'\to(M^\Uu_\alpha)'$ is 
$k$-good and $Y$ condenses finely. So $(M^\Tt_\alpha)'$ is indeed a 
$Y$-premouse. Consider this lSo in the latter case, since $Y$ condenses finely, 

Therefore since $Y$ condenses finely and $\pi$ is $k$-good, we have 
$\Mbar^*\wins Y(\Nbar)\down a$, so $\Mbar^*$ is a $Y$-premouse.

\end{proof}
\end{comment}




\begin{comment}
\begin{definition}
For $\Tt$ an iteration tree and $\alpha<\lh(\Tt)$ let $\base^\Tt(\alpha)$ 
denote the least $\beta\leq_\Tt\alpha$ such that $(\beta,\alpha]_\Tt$ does not 
drop in model or degree. (Therefore either $\beta=0$ or $\beta$ is a 
successor.) Also let $M^{*\Tt}_0=M^\Tt_0$ and $i^{*\Tt}_0=\id$.
\end{definition}


\begin{definition}\label{dfn:pi_C_realizable}
Let $\CC=\left<\N_\alpha\right>_{\alpha\leq\lambda}$ be an
$L^\Fop[\es,b]$-construction. Let $k\leq\om$ and suppose that $\N_\lambda$ is 
$k$-$\Fop$-solid. Let $\R$ be a $k$-sound $\Fop$-premouse over $b$ 
and let
$\pi:\R\to\core_k(\N_\lambda)$ be fully elementary. Let $\Tt$ be an
$\Fop$-putative iteration tree on $\R$, with $\deg^\Tt(0)=k$. We say that $\Tt$ 
is
\textbf{$(\pi,\CC)$-realizable} iff for every
$\alpha<\lh(\Tt)$, letting $\beta=\base^\Tt(\alpha)$ and $m=\deg^\Tt(\alpha)$,
there is $\zeta\leq\lambda$ such that:
\begin{enumerate}[label=--]
 \item if $[0,\alpha]_\Tt$ does not drop in model or degree then 
$\zeta=\lambda$, and let $\tau=\pi$,
 \item if $\zeta=\lambda$ then $m\leq k$,
 \item if $[0,\alpha]_\Tt$ drops in model or degree then there is a $\nu$-preserving near
$m$-embedding $\tau\colon M^{*\Tt}_\beta\to\core_m(\N_\zeta)$, and
 \item if $M^{*\Tt}_\beta$ is not type 3 then there is a weak $m$-embedding 
$\sigma:M^\Tt_\alpha\to\core_m(\N_\zeta)$ such that $\sigma\com 
i^{*\Tt}_{\beta,\alpha}=\tau$.
 \item if $M^{*\Tt}_\beta$ is type 3 then there is a weak $m$-embedding 
$\sigma:\R\to\core_m(N_\zeta)$ such that $i^{*\Tt}_{\beta,\alpha}=\tau$, where $\R$ 
is ``$(M^\Tt_\alpha)^\sq$''.\footnote{\label{ftn:squash}$(M^\Tt_\alpha)^\sq$ might not make literal 
sense, if say $M^\Tt_\alpha$ is not wellfounded. By ``$(M^\Tt_\alpha)^\sq$'' we mean that either 
$\alpha=\xi+1$ and $\R=\Ult_m((M^{*\Tt}_\alpha)^\sq,E^\Tt_\xi)$, or $\alpha$ is a limit and $\R$ is 
the direct limit of the structures $(M^\Tt_\xi)^\sq$ for $\xi\in[\beta,\alpha)_\Tt$, under 
the iteration maps.}\qedhere
\end{enumerate}
\end{definition}
\end{comment}
\begin{comment}
\begin{lemma}\label{lem:L[E]_construction}
Let $\Fop$ be a projecting, uniformly $\Sigma_1$ operator over $\opbk$, with a base in $\HC$, 
and which condenses finely.
Let $\CC=\left<\N_\alpha\right>_{\alpha<\chi}$ be an
$L^\Fop[\es,b]$-construction.
Suppose that for all $\alpha<\chi$ and all $\R$, if $\N_\alpha,\R$ are $\Fop$-premice of type 
3, $\R$ is $(0,\om_1+1)$-iterable and $\pi:\R^\sq\to\N_\alpha^\sq$ is $\Sigma_0$-elementary, 
then $\R$ is not 
superstrong. Then:

\begin{enumerate}[label=\tu{(}\arabic*\tu{)}]
 \item\label{item:chi_limit} If $\chi$ is a limit there is a unique
$\N_\chi$ such that $\CC\conc\left<\N_\chi\right>$ is an $L^\Fop[\es,b]$-construction.

\item\label{item:om_solid} Suppose $\chi=\lambda+1$, $\N_\lambda$ is $\om$-$\Fop$-solid and 
$\lambda\in\opbk$. Then there is a unique $\N_{\chi}$ such that 
$\CC\conc\left<\N_{\chi}\right>$ is an $L^\Fop[\es,b]$-construction and 
$\core_\om(\N_\lambda)\wpins\N_{\chi}$.

\item\label{item:k_solid} Suppose $\chi=\lambda+1$ and $k<\om$ is such that $\N_\lambda$ is 
$k$-$\Fop$-solid and for a club of countable 
elementary $\pi:\M\to\core_k(\N_\lambda)$, 
there is a $Y$-putative, $(k,\om_1,\om_1+1)$-iteration 
strategy $\Sigma$ for $\M$, such that every $\Tt$ via 
$\Sigma$ is $(\pi,\CC)$-realizable.
Then $\N_\lambda$ is $(k+1)$-$\Fop$-solid.
\end{enumerate}
\end{lemma}

\begin{proof} 
We will use \ref{lem:whole_Y_pm_elem_hull} without explicit mention. Consider
\ref{item:chi_limit}. Let $\N_\chi=\liminf_{\alpha<\lambda}\N_\alpha$. Then
$\N_\chi$ is a passive limit of sound whole proper segments, so $\N_\chi$ is an 
$\Fop$-premouse.

Now consider \ref{item:om_solid}. Let 
$\M_\lambda=\core_\om(\N_\lambda)$ and let $\M$ be the largest 
$\Fop$-whole segment of $\M_\lambda$. We must verify that $\N_{\lambda+1}$, defined as in 
\ref{dfn:Fop_con}\ref{item:apply_Fop} (with $\alpha=\lambda$), is well-defined (i.e. acceptable) 
and is an $\Fop$-premouse. Let $\N$ also be as there. Since every segment of $\M_\lambda$ is 
sound, it suffices to see that for every $\R'\wpins\N$, letting $\R=\R'\down b$, $\R$ is sound (by 
induction, we may assume that $\R$ is acceptable). We may assume that 
$\M_\lambda\wpins\R$.
\begin{comment}
We claim that for some $j\leq\om$, $(\M_\alpha,j)$ is in the $\M$-dropdown 
sequence of $\N_\lambda$. If $\M=\M_\alpha$ this is trivial, so suppose that 
$\M\wpins\M_\alpha$.

Suppose for a moment that $\M\wpins\M_\alpha$. Then there is 
Note that if $\N_\alpha$ is a limit of $\Fop$-whole proper segments then so is 
$\M_\alpha$, since $\Fop$ is uniformly $\Sigma_1$. If $k<\om$ and
$\core_k(\N_\alpha)$ has a largest 
$\Fop$-whole proper segment $\M$ then, letting 
$\sigma:\core_{k+1}(\N_\alpha)\to\core_k(\N_\alpha)$ be the core map, there is 
$\Mbar$ such that $\sigma(\Mbar)=\M$, $\Mbar$ is the largest $\Fop$-whole 
proper segment of $\core_{k+1}(\N_\alpha)$, and moreover, if 
$j\leq k$ and $(\core_k(\N_\alpha),j+1)$ is in the $\M$-dropdown sequence of 
$\core_k(\N_\alpha)$, then $(\core_{k+1}(\N_\alpha),j+1)$ is in the 
$\Mbar$-dropdown sequence of $\core_{k+1}(\M_\alpha$.
\end{comment}
\begin{comment}
We have $\rho=\rho_\om(\M_\lambda)\leq\rho_\om^\P$, 
for each
$(\P,j+1)$ in the $\M$-dropdown sequence of $\M_\lambda$. 
Therefore $\rho\leq\rho_\om(\R)$. If 
$\rho<\rho_\om(\R)$ then the soundness of $\R'$ implies that of 
$\R$. So suppose $\rho_\om(\R)=\rho$. Let $k<\om$ be such that 
$\rho_{k+1}(\R)=\rho<\rho_k(\R)$. Then as before, $\R$ is $k$-sound. Let 
$p=p_{k+1}(\R)$. Then $\M\in H=\Hull_{k+1}^\R(\rho\un p)$ because $\Fop$ is 
uniformly $\Sigma_1$, and because $H$ is cofinal in $\R$ if $k=0$. Therefore 
$H$ has every element of $\R$ which is in the $\M$-drop-down sequence of 
$\R$. It follows that $\M\un\{\M\}\sub H$. 
Since $\rho_{k+1}(\R)\leq\OR(\M)$, $\rho_{k+1}(\R')=\M$. Also, 
$p_{k+1}(\R')=p_{k+1}(\R)\cut(\OR(\M)+1)$ because $\R'$ is $(k+1)$-sound 
(including $(k+1)$-solid). Therefore $H=\R$.

So it remains to verify that $\R$ 
is $(k+1)$-solid. If $k>0$ or $p_{k+1}(\R')\neq\emptyset$, we have 
$p_{k+1}(\R)=p_{k+1}(\R')$ as before,
so we are done. Suppose $k=0$ and $p_1(\R')=\emptyset$. Let
let $q$ be $<_\lex$-least such that $\M\in H_q=\Hull_1^\R(\rho\un q)$. 
Then $H_q=\R$, as before. But we claim that $q$ is $1$-solid for $\R$. For 
let us assume that $q=\{\gamma\}$ for some ordinal $\gamma$, for simplicity. 
Then $\M\notin H_\gamma=\Hull_1^\R(\gamma)$, and therefore $H_\gamma$ is 
bounded in $\R$, and therefore $\Th_1^\R(\gamma)\in\R$, as required. But 
then $p_1^\R=q$, so we are done.

Now consider \ref{item:k_solid}. We may assume that $\lambda>1$, as the only extenders of $\N_1$ 
are $\Fop$-extenders, so there are no non-trivial iteration trees on it.
Let us also assume that $\N_\lambda$ has a largest $\Fop$-whole proper segment, 
since the contrary case is similar but easier. Then $\M^*$ has a largest 
$\Fop$-whole proper segment $\M_\Fop$; so $\M^+=\M^*\down\M_\Fop\wins\Fop_1(\M_\Fop)$. If 
$(\M^*,k+1)$ is not on 
the $\M_\Fop$-drop-down sequence of $\M^*$, then the proof of (a) shows that 
$\M^*$ 
is $(k+1)$-sound, and therefore $(k+1)$-$\Fop$-solid (the ``$\Fop$'' since 
$\core_{k+1}(\M^*)=\M^*$ in this case). So assume otherwise.

If $\M^*$ is whole let $\M'=\Fop_1(\M^*)$; otherwise let $\M'=\Fop_1(\M_\Fop)$. So $\M^*\in\M'$.
Let $\pi':\Mbar'\to\M'$ be elementary, with $\Mbar'$ countable and 
$\pi'(\Mbar)=\M^*$ for some $\Mbar$ and also such that 
$\pi=\pi'\rest\Mbar$ is in the hypothesized club and $\abar=a^{\Mbar}\in C_\Fop$. Because $\Fop$ 
condenses coarsely (and using 
\ref{lem:whole_Y_pm_elem_hull} or \ref{lem:E_active_Y_pm_elem_hull}), $\Mbar$ is an $\Fop$-premouse.
Now let $\Sigma$ be an $\Fop$-putative strategy for $\Mbar$ as hypothesized.

\begin{claim}\label{clm:Sigma_is_F_strat}
$\Sigma$ is an $\Fop$-$(k,\om_1,\om_1+1)$-strategy for $\Mbar$.
\end{claim}
\begin{proof}[Proof Sketch]
This is basically as in the proof of \ref{lem:strong_condenses_coarsely} (though here it is more 
important that \emph{condenses finely} works with respect to weak embeddings as in 
(\ref{item:condense_realize}) of \ref{dfn:condenses_finely}). One further point arises, 
however, in verifying that various models are in the right dropdown sequences in order to apply 
\ref{dfn:condenses_finely}. For let $\Tt$ be via $\Sigma$, with last model $M^\Tt_\alpha$; say 
we want to apply \ref{dfn:condenses_finely} in order to deduce that $\Q=M^\Tt_\alpha$ is an 
$\Fop$-premouse. Let $m=\deg^\Tt(\alpha)$. Then by \cite[Corollary 2.20]{extmax}, 
$\rho_{m+1}^\Q<\rho_m^\Q$; this 
helps to ensure that \ref{dfn:condenses_finely} applies. (Note that possibly
$[0,\alpha]_\Tt$ does not drop in model or degree, so $m=k$, and 
$\crit(i^\Tt_{0,\alpha})<\rho_{k+1}^{\Mbar}$. In this case, by \cite{extmax}, $\rho_{k+1}^\Q=\sup 
i^\Tt_{0,\alpha}``\rho_{k+1}^{\Mbar}$. We also need this observation in other places, because $\Tt$ 
need not be normal.)
\begin{comment}
We can now deduce that $M^\Tt_\alpha$ is an $\Fop$-premouse. Part of the proof is like that of 
\ref{lem:whole_Y_pm_elem_hull}, and part is as follows.
Suppose that we have determined that $\R=M^\Tt_\alpha|\gamma$ is an 
$\Fop$-premouse, and that this is the largest $\varphi_\Fop$-putatively whole proper 
segment of $M^\Tt_\alpha$. So we want to know that
$M^\Tt_\alpha\wins\Fop_1(\R)\down\abar$. Now $M^\Tt_\alpha\down\R$ projects to $\R$
and is sound (the latter because $\Tt$ uses 
only non-$\Fop$ extenders). We already know that $M^\Tt_\alpha$ is a 
$Y$-premouse. Thus, it suffices to see that $M^\Tt_\alpha\down\R$ 
is $Y$-iterable (above $\R$, as a continuing $Y$-premouse). But the realization map $\pi_\alpha$ 
allows us to lift trees $\Uu$ on $M^\Tt_\alpha\down\R$ to a countably 
iterable continuing $Y$-premouse which appeared somewhere in $\CC$. This 
provides a $Y$-putative strategy for $M^\Tt_\alpha\down\R$, and 
we can then use the fact that $Y$ condenses finely to see that this is in fact a 
$Y$-strategy. So $M^\Tt_\alpha\wins\Lp_+^Y(\R)$. But then since $\Fop$ 
is uniformly $\Sigma_1$, this implies that 
$M^\Tt_\alpha\wins\Fop_1(\R)\down\abar$.

We remark that, now that we know $M^\Tt_\alpha$ is an $\Fop$-premouse, the fact 
that $\Tt$ is $(\pi,\CC)$-realizable and $\Fop$ is uniformly $\Sigma_1$, 
ensures that if we want to extend $\Tt$ with some non-$\Fop$ extender $E$, then 
the realization map $\pi_\alpha$ will lift $M^\Tt_\alpha|\lh(E)$ to some 
certified model, and so it is reasonable that $\Tt\conc\left<E\right>$ will 
be $(\pi,\CC)$-realizable.\footnote{However, one of course expects to need 
more hypotheses on agreement between realization embeddings to ensure that 
$\Tt\conc\left<E\right>$ will indeed by $(\pi,\CC)$-realizable.}

Note that $\Sigma$ extends uniquely to a
$Y$-$(k,\om_1,\om_1+1)$-strategy for $\Mbar$. Thus, we take $\Sigma$ to be 
this strategy from now on, and in the proof of the following claim, we think of 
$\Mbar$ purely as a $Y$-premouse.

Let us assume from now on that $\M^*_Y\wpins\M^*$ and let $\pi(\Mbar_Y)=\M^*_Y$; the contrary case 
is easier. As $\Fop$ is whole, $\Mbar_\Fop\wins\Mbar_Y$, so
$(\Mbar,k+1)$ is 
on the $\Mbar_Y$-dropdown sequence of $\Mbar$.

Let 
$\sigma:\N^*\to\M^*$ be the core map. Let $\sigma(\N_\Fop)=\M_\Fop$ and let 
$\N^+=\N^*\down\N_\Fop$. Then $\rho_{k+1}(\N^+)=\N_\Fop$ and it easy to see 
that $\N^+$ is $(k+1)$-sound. Since $\sigma$ exists, we therefore have 
$\N^+\wpins\Lp_+^\Fop(\N_\Fop)$, so $\N^+$ is an $\Fop$-premouse. 
\end{comment}
\begin{comment}
\end{proof}


Let $\Nbar=\core_{k+1}(\Mbar)$ and let $\tau:\Nbar\to\Mbar$ be the 
core map. Then there is $\Nbar_\Fop$ such that $\tau(\Nbar_\Fop)=\Mbar_\Fop$.
Then $\Nbar_\Fop$ is a whole $\Fop$-premouse, and is the largest $\varphi_\Fop$-putatively whole 
proper segment of $\Nbar$. And $\Nbar$ is a $\Fop$-premouse because 
$\Fop$ condenses finely.

\begin{claim}\label{clm:dropdown}
$(\Nbar,k+1)$ is on the $\Nbar_\Fop$-dropdown sequence of $\Nbar$.
\end{claim}
\begin{proof}

Suppose not.
We will show that $\Nbar_\Fop\wpins\Mbar_\Fop$. But then 
$(\Fop(\Nbar_\Fop)\down 
\abar)\wins\Mbar_\Fop$, so $\Nbar\in\Mbar$, a contradiction.

Let $\rho=\rho_{k+1}(\Mbar)$. Let $(\R,j)$ be the last element of the 
$\Mbar_\Fop$-dropdown sequence of $\Mbar$ with $\R\wpins\Mbar$. 
So
\[ \rho<\rho_{j'}^\R=\rho_\om^\R=\car^{\Mbar}(\Mbar_\Fop)\in\rg(\tau).\]
The negation of the claim implies that 
$\rg(\tau)\inter\rho_\om^\R=\rho$, so $\crit(\tau)=\rho$ and
$\tau(\rho)=\rho_\om^\R$. Let $\tau(\Ss)=\R$, so
$\tau\rest\Ss:\Ss\to\R$ is fully 
elementary and $\crit(\tau)=\rho_\om^\Ss$. Therefore since $\Fop$ condenses 
finely, $\Ss$ is a $\Fop$-premouse.
We will show that $\Ss\wpins\Mbar|\tau(\rho)$, which suffices since 
$\Nbar_\Fop\wins\Ss$.

Let $\xi\leq\wl(\Ss)$ be the supremum of $\rho$ and all $\alpha\leq\wl(\Ss)$ such 
that $\Ss|\alpha$ is $E$-active. Then $\rho\leq\xi\leq\wl(\Mbar_\Fop)$. Let 
$(\Q,l')$ be the last element of the 
$\Ss|\xi$-dropdown sequence of $\Ss$; so $\Ss|\rho\wins\Q\wins\Ss$ and 
$\rho_\om^\Q=\rho$. We claim that $\Q\wpins\Mbar$.

For let $\P=\tau(\Q)$. We may assume that $\rho<\rho_0^\Q$ (by the ISC).
So let $l<\om$ be such that $\rho_{l+1}^\Q=\rho<\rho_l^\Q$. 
Then $\P$ is $(l,\om_1,\om_1+1)$-$\Fop$-iterable, since $l$-bounded trees $\Tt$ on $\P$ 
can be lifted to $k$-bounded trees $\Uu$ on $\Mbar$, using that $\Fop$ condenses 
finely.

Now arguing as in \cite{wDJ} and \cite{copy_con}, we obtain a strategy 
$\Sigma'$ for $\Mbar$ 
with the variant of the $\mm$-weak Dodd-Jensen property (see \cite{copy_con}) 
given by replacing all uses of near $j$-embeddings with nearly 
$j$-good embeddings. Then using $\Sigma'$, the usual proof of condensation
works, giving that $\Q\wpins\P$, so $\Q\wpins\Mbar|\tau(\rho)$.

Now $\Ss\wins \Fop^\alpha(\Q)$ for 
some $\alpha\in\Ord$, and $\Ss\in\R$, and $\rho_\om^\Ss=\rho$, and $\tau(\rho)$ 
is a cardinal of $\Mbar$. So $\OR(\Ss)<\tau(\rho)$, and because $\Mbar$ is 
$\Fop$-iterable, therefore $\Ss\wpins\Mbar|\tau(\rho)$.

This completes the proof of the claim.
\end{proof}

\begin{claim}
$\Mbar$ is $(k+1)$-universal.
\end{claim}
\begin{proof}
Since $\Fop$ condenses 
finely, and using Claim \ref{clm:dropdown}, the phalanx 
$(\Mbar,\Nbar,\rho_{k+1}(\Mbar))$ is $\Fop$-iterable,
via lifting to $\Mbar$ using the maps $(\id,\tau)$.

Now we can adapt the usual proof of universality in the same manner 
that we adapted the proof of condensation above.
\end{proof}

\begin{claim}
 $\Nbar=\core_{k+1}(\Mbar)$ is $(k+1)$-solid.
\end{claim}
\begin{proof}

This is proved similarly to the previous claim, given a couple of observations. 
Let $p=p_{k+1}(\Nbar)$. Let 
$\alpha\in p$ and 
$q=p\cut(\alpha+1)$. Let $H$ be the transitive collapse of 
$\Hull_{k+1}^{\Nbar}(\alpha\un q)$; we need to see that $H\in\Nbar$. As 
in the proof of (a), we may assume that $\alpha<\car^{\Nbar}(\Nbar_\Fop)$. 
Now let $\sigma:H\to\Nbar$ be the uncollapse. So $\sigma$ is a near 
$k$-embedding. If $\sigma$ fails to be a $k$-embedding, i.e., if $\rg(\sigma)$ 
is 
bounded in $\rho_k(\Nbar)$, then we easily have $H\in\Nbar$. So assume 
$\sigma$ is a $k$-embedding. Also as in the proof of (a), we may 
assume that $\Nbar_\Fop\in\rg(\sigma)$. Then
$\rho_{k+1}^H\leq\alpha<\car^{\Nbar}(\Nbar_\Fop)$, and so $(\Nbar,k+1)$ is on 
the $\Nbar_\Fop$-dropdown sequence of $\Nbar$.

Now since $\Fop$ condenses finely, $H$ is a 
$\Fop$-premouse, and moreover, the phalanx $(\Nbar,H,\alpha)$ is $\Fop$-iterable, 
via lifting to $\Nbar$ (which is $\Fop$-iterable via lifting to $\Mbar$). Now 
we can adapt the proof of solidity just as for universality.
\end{proof}

By elementarity, it follows that $\M^*$ is $(k+1)$-universal and 
$\N^*=\core_{k+1}(\M^*)$ is $(k+1)$-solid. Therefore $\N^*$ is 
$(k+1)$-sound. Because $\Fop$ condenses finely, $\N^*$ is an $\Fop$-premouse. This completes the 
proof.
\end{proof}
\end{comment}

\begin{comment}
We can now deduce that $M^\Tt_\alpha$ is an $\Fop$-premouse. Part of the proof is like that of 
\ref{lem:whole_Y_pm_elem_hull}, and part is as follows.
Suppose that we have determined that $\R=M^\Tt_\alpha|\gamma$ is an 
$\Fop$-premouse, and that this is the largest $\varphi_\Fop$-putatively whole proper 
segment of $M^\Tt_\alpha$. So we want to know that
$M^\Tt_\alpha\wins\Fop_1(\R)\down\abar$. Now $M^\Tt_\alpha\down\R$ projects to $\R$
and is sound (the latter because $\Tt$ uses 
only non-$\Fop$ extenders). We already know that $M^\Tt_\alpha$ is a 
$Y$-premouse. Thus, it suffices to see that $M^\Tt_\alpha\down\R$ 
is $Y$-iterable (above $\R$, as a continuing $Y$-premouse). But the realization map $\pi_\alpha$ 
allows us to lift trees $\Uu$ on $M^\Tt_\alpha\down\R$ to a countably 
iterable continuing $Y$-premouse which appeared somewhere in $\CC$. This 
provides a $Y$-putative strategy for $M^\Tt_\alpha\down\R$, and 
we can then use the fact that $Y$ condenses finely to see that this is in fact a 
$Y$-strategy. So $M^\Tt_\alpha\wins\Lp_+^Y(\R)$. But then since $\Fop$ 
is uniformly $\Sigma_1$, this implies that 
$M^\Tt_\alpha\wins\Fop_1(\R)\down\abar$.

We remark that, now that we know $M^\Tt_\alpha$ is an $\Fop$-premouse, the fact 
that $\Tt$ is $(\pi,\CC)$-realizable and $\Fop$ is uniformly $\Sigma_1$, 
ensures that if we want to extend $\Tt$ with some non-$\Fop$ extender $E$, then 
the realization map $\pi_\alpha$ will lift $M^\Tt_\alpha|\lh(E)$ to some 
certified model, and so it is reasonable that $\Tt\conc\left<E\right>$ will 
be $(\pi,\CC)$-realizable.\footnote{However, one of course expects to need 
more hypotheses on agreement between realization embeddings to ensure that 
$\Tt\conc\left<E\right>$ will indeed by $(\pi,\CC)$-realizable.}

Note that $\Sigma$ extends uniquely to a
$Y$-$(k,\om_1,\om_1+1)$-strategy for $\Mbar$. Thus, we take $\Sigma$ to be 
this strategy from now on, and in the proof of the following claim, we think of 
$\Mbar$ purely as a $Y$-premouse.

Let us assume from now on that $\M^*_Y\wpins\M^*$ and let $\pi(\Mbar_Y)=\M^*_Y$; the contrary case 
is easier. As $\Fop$ is whole, $\Mbar_\Fop\wins\Mbar_Y$, so
$(\Mbar,k+1)$ is 
on the $\Mbar_Y$-dropdown sequence of $\Mbar$.

Let 
$\sigma:\N^*\to\M^*$ be the core map. Let $\sigma(\N_\Fop)=\M_\Fop$ and let 
$\N^+=\N^*\down\N_\Fop$. Then $\rho_{k+1}(\N^+)=\N_\Fop$ and it easy to see 
that $\N^+$ is $(k+1)$-sound. Since $\sigma$ exists, we therefore have 
$\N^+\wpins\Lp_+^\Fop(\N_\Fop)$, so $\N^+$ is an $\Fop$-premouse. 
\end{comment}
\begin{comment}
We will use \ref{lem:whole_Y_pm_elem_hull} without explicit mention. Consider
\ref{item:chi_limit}. Let $\N_\chi=\liminf_{\alpha<\lambda}\N_\alpha$. Then
$\N_\chi$ is a passive limit of sound whole proper segments, so $\N_\chi$ is an 
$\Fop$-premouse.

Now consider \ref{item:om_solid}. Let 
$\M_\lambda=\core_\om(\N_\lambda)$ and let $\M$ be the largest 
$\Fop$-whole segment of $\M_\lambda$. We must verify that $\N_{\lambda+1}$, defined as in 
\ref{dfn:Fop_con}\ref{item:apply_Fop} (with $\alpha=\lambda$), is well-defined (i.e. acceptable) 
and is an $\Fop$-premouse. Let $\N$ also be as there. Since every segment of $\M_\lambda$ is 
sound, it suffices to see that for every $\R'\wpins\N$, letting $\R=\R'\down b$, $\R$ is sound (by 
induction, we may assume that $\R$ is acceptable). We may assume that 
$\M_\lambda\wpins\R$.
\end{comment}
\begin{comment}
We claim that for some $j\leq\om$, $(\M_\alpha,j)$ is in the $\M$-dropdown 
sequence of $\N_\lambda$. If $\M=\M_\alpha$ this is trivial, so suppose that 
$\M\wpins\M_\alpha$.

Suppose for a moment that $\M\wpins\M_\alpha$. Then there is 
Note that if $\N_\alpha$ is a limit of $\Fop$-whole proper segments then so is 
$\M_\alpha$, since $\Fop$ is uniformly $\Sigma_1$. If $k<\om$ and
$\core_k(\N_\alpha)$ has a largest 
$\Fop$-whole proper segment $\M$ then, letting 
$\sigma:\core_{k+1}(\N_\alpha)\to\core_k(\N_\alpha)$ be the core map, there is 
$\Mbar$ such that $\sigma(\Mbar)=\M$, $\Mbar$ is the largest $\Fop$-whole 
proper segment of $\core_{k+1}(\N_\alpha)$, and moreover, if 
$j\leq k$ and $(\core_k(\N_\alpha),j+1)$ is in the $\M$-dropdown sequence of 
$\core_k(\N_\alpha)$, then $(\core_{k+1}(\N_\alpha),j+1)$ is in the 
$\Mbar$-dropdown sequence of $\core_{k+1}(\M_\alpha$.
\end{comment}
\begin{comment}
We have $\rho=\rho_\om(\M_\lambda)\leq\rho_\om^\P$, 
for each
$(\P,j+1)$ in the $\M$-dropdown sequence of $\M_\lambda$. 
Therefore $\rho\leq\rho_\om(\R)$. If 
$\rho<\rho_\om(\R)$ then the soundness of $\R'$ implies that of 
$\R$. So suppose $\rho_\om(\R)=\rho$. Let $k<\om$ be such that 
$\rho_{k+1}(\R)=\rho<\rho_k(\R)$. Then as before, $\R$ is $k$-sound. Let 
$p=p_{k+1}(\R)$. Then $\M\in H=\Hull_{k+1}^\R(\rho\un p)$ because $\Fop$ is 
uniformly $\Sigma_1$, and because $H$ is cofinal in $\R$ if $k=0$. Therefore 
$H$ has every element of $\R$ which is in the $\M$-drop-down sequence of 
$\R$. It follows that $\M\un\{\M\}\sub H$. 
Since $\rho_{k+1}(\R)\leq\OR(\M)$, $\rho_{k+1}(\R')=\M$. Also, 
$p_{k+1}(\R')=p_{k+1}(\R)\cut(\OR(\M)+1)$ because $\R'$ is $(k+1)$-sound 
(including $(k+1)$-solid). Therefore $H=\R$.

So it remains to verify that $\R$ 
is $(k+1)$-solid. If $k>0$ or $p_{k+1}(\R')\neq\emptyset$, we have 
$p_{k+1}(\R)=p_{k+1}(\R')$ as before,
so we are done. Suppose $k=0$ and $p_1(\R')=\emptyset$. Let
let $q$ be $<_\lex$-least such that $\M\in H_q=\Hull_1^\R(\rho\un q)$. 
Then $H_q=\R$, as before. But we claim that $q$ is $1$-solid for $\R$. For 
let us assume that $q=\{\gamma\}$ for some ordinal $\gamma$, for simplicity. 
Then $\M\notin H_\gamma=\Hull_1^\R(\gamma)$, and therefore $H_\gamma$ is 
bounded in $\R$, and therefore $\Th_1^\R(\gamma)\in\R$, as required. But 
then $p_1^\R=q$, so we are done.
\end{comment}
\begin{comment}
%\begin{enumerate}[label=\tu{(}\arabic*\tu{)}]
\item\label{item:chi_limit} If $\chi$ is a limit there is a unique
$\N_\chi$ such that $\CC\conc\left<\N_\chi\right>$ is an $L^\Fop[\es,A]$-construction.

\item\label{item:om_solid} Suppose $\chi=\lambda+1$, $\N_\lambda$ is $\om$-$\Fop$-fine and 
$\lambda\in\opbk$. Then $\Fop(\Nthere is a unique $\N_{\chi}$ such that 
$\CC\conc\left<\N_{\chi}\right>$ is an $L^\Fop[\es,b]$-construction and 
$\core_\om(\N_\lambda)\wpins\N_{\chi}$.
\item\label{item:k_solid}
\end{enumerate}
\end{comment}
\begin{comment}
Let $\Fop,D,\opbk$ be as above. For $a\in\opbk$ we say that $a$ is a \textbf{base for 
$\Fop$} iff $C_\Fop$ contains the (swo'd) cone above $a$. We say that $\Fop$ 
is \textbf{forgetful} iff for allpms $\N\in D$, we have 
$\Fop(\hat{\N})\down a^\N=\Fop(\N)$. We say that $\Fop$ is \textbf{historical} iff $\Fop$ 
is not forgetful.
\end{comment}
\begin{comment}
We say $\Fop$ is \textbf{basic} iff for all 
$(i,X)\in D$ and $\P\wins\Fop_i(X)$, we have $E^\P=\emptyset$.
We say $\Fop$ is \textbf{projecting} iff for all $(i,X)\in D$, we have 
$\rho_\om^{\Fop_i(X)}=X$.
\end{comment}
\begin{comment}
Considering the definitions \emph{forgetful} and \emph{historical}, the intuition is that, in 
computing $\Fop(\N)$,
we are considering $\N$ as a premouse over $a^\N$, with its history $S^\N$,
whereas in computing $\Fop(\hat{\N})$, we are just considering $\hat{\N}$ (and so $\N$) as a coarse 
object. For certain operators, this distinction may affect the output of the computation.
(***This paragraph isn't correct now***) At times we write $\Fop(X)$ instead of $\Fop_i(X)$. Note 
that $\opbk,C_\Fop$ are determined 
by $\dom(\Fop)$.
Strategy operators (to be explained in more detail later), defined by adjoining the correct branch 
for the least tree for which the branch has not yet been adjoined, are historical. The operator 
$\Fop(X)=X^\#$ is forgetful.
\end{comment}
\begin{comment}
\begin{proof}
Suppose not. Let $k,\M,\M^*,G$, etc, constitute a 
counterexample. All relevant objects are in $\opbk$. Let $\N^\$=\Fop(\N)$; so $\N^\$\neq\N^*$. Note 
that $\N^\$\not\wins\N^*$. For if 
$\N^\$\wpins\N^*$ then $\N^\$\down a^\N$ is a sound $\Fop$-premouse and there is a $\Fop$-premouse 
$\N'$ such that $\univ{\N'}=\J_1(\N^\$)$. But then because $\Fop$ is uniformly $\Sigma_1$ and using 
$\pi$, $\Fop_1(\M)\wpins\M^+$, contradiction.

Let $\PP=\Coll(\om,\P\un\N)$. Let $X\in\opbk$ be transitive, containing all relevant 
objects, and such that $X\sats(\ZFmin)^{-\eps}$. (For any $A\in\opbk$ there is 
$\gamma$ such that $L_\gamma(A)\sats(\ZFmin)^{-\eps}$, so there is such a $\gamma<\OR(\opbk)$.) In 
particular, in $X$ we have $\M,\N,\P$, 
etc, and have $p\in\PP$ and $\PP$-names $\tilde{{\N}}^+,\tilde{\pi},\tilde{\sigma}$ for 
$\N^+,\pi,\sigma$, and in $X$, $p$ forces that
\begin{equation}\label{eqn:force_counterex} \text{``}\M^*,\tilde{\N}^+,\N^\$\text{, etc, 
satisfy the hypotheses of \ref{dfn:condenses_finely} and 
}\tilde{\N}^+\not\wins\N^\$\ \&\ \N^\$\not\wins\tilde{\N}^+\text{''.}\end{equation}
Let $\pi:Z\to X$ be 
elementary with $Z$ countable, and everything 
relevant in $\rg(\pi)$. Let $\pi(\N^Z)=\N$, etc. Let $G\sub\Coll(\om,\P^Z\un\N^Z)$ be 
$Z$-generic with $p^Z\in G$. Then because $\Fop$ condenses coarsely and by 
\ref{lem:whole_Y_pm_elem_hull} and \ref{lem:E_active_Y_pm_elem_hull}, 
$(\M^*)^Z,(\tilde{\N}^+)^Z_G$, etc, satisfy the hypotheses of 
\ref{dfn:condenses_finely}, and $(\N^\$)^Z\wins \Fop_1(\N^Z)$. But then because $\Fop$ 
almost condenses finely, $(\tilde{\N}^+)^Z_G\wins \Fop_1(\N^Z)$. Therefore either 
$(\N^\$)^Z\wins(\tilde{\N}^+)^Z_G$ or $(\tilde{\N}^+)^Z_G\wins(\N^\$)^Z$, contradicting line 
\ref{eqn:force_counterex}.\end{proof}
\end{comment}
\begin{comment}
Let $\M_\alpha=\core_\om(\N_\alpha)$.
Let $\M$ be the largest whole segment of $\M_\alpha$. So either $\M_\alpha=\M$ or 
$\M_\alpha\down\M\wpins\Fop_1(\M)$.
Let $\N\wins\Fop_1(\M)$ be least such that either $\N=\Fop_1(\M)$ or for some $k<\om$, 
$(\N\down b,k+1)$ is 
on the $\M_\alpha$-drop-down sequence of $\N\down b$. Then $\N_{\alpha+1}=\N\down b$. Note 
that $\M_\alpha\wpins\N_{\alpha+1}$.
\end{comment}

\begin{comment}
\begin{definition}
 Let $\Fop$ be an operator (what is that?). We say that $\Fop$ \dfnemph{condenses well} iff 
for all transitive $P,\Mbar,\Mbar^+,M,M^+,\abar,a$ (in the relevant domain?) with $\abar\in P$ and 
$\abar\in\Mbar$ and $a\in M$, 
\end{definition}
\end{comment}


\begin{comment}
Suppose also that $\OR^{\P}$ is a strong cutpoint of $\N$. Then 
one might want to say that $\N|((\OR^\P)^+)^\N$ is $\Lp^\Sigma(\P)$. However, 
this is not likely to be true, for the trivial 
reason that these two structures are not even in the same hierarchy: in 
$\Lp^\Sigma(\P)$, $\P$ is treated as a coarse object, ignoring the history in 
$\P$, but in $\N|(\OR(\P)^+)^\N$, this history is respected. In the definition 
of \emph{operator}, When $i=2$ we respect two layers of history (given 
it exists). Having the latter respect gives us convenient terminology to define 
an analogue $\Lp^\Sigma_+(\P)$ of $\Lp^\Sigma_+(\P)$, which \emph{is} in the 
same hierarchy as $\N$.
\end{comment}

\begin{comment}
\begin{definition}
 Let $\M$ be an adequate model over an explicitly swo'd set $a$.
 Then $<^\M$ denotes the wellorder of $\M$ end-extending $<_a$,
 and such that for all $\xi\in[1,\wl(\M))$, $<^{\M|\xi}$ is end-extened by $<^\M$,
 and if $\wl(\M)=\xi+1$ then $<^\M$ is determined in a standard manner from the fact that 
$\M=\Hull^\M(x\un\{x\}\un\OR(\M))$
 Also, first define $<^{\M|0}=<^a=<_a$.
 Now if $\wl(\M)=\xi+1$ for some $\xi$ then $<^\M$ is the end-extension of $<^{\M|\xi}$,
 defined in the usual manner (as for the standard wellorder of $L$ using the $\J$-hierarchy).
 And if $\wl(\M)$
\end{definition}
\end{comment}

\begin{comment}(i) 
$\N=\Hull_{\Sigma_1}^\N(A^{<\om}\cross\OR(\N)^{<\om})$ and (ii) there is $n<\om$ such 
that
$\N=\Hull_{\Sigma_{n+1}}^\N(A^{<\om}\un S_{\xi}\un\{S_\xi\})$.
\end{comment}
\begin{comment}
 \item There is $n<\om$ such that $\M$ is $n$-sound and $\rho_{n+1}^\M\leq\max(\xi,\om)$, and 
letting $n$ be least such, $\M=\Hull_{n+1}^\M(Y^{<\om}\un\{Y\}\un\pvec_{n+1}^\M)$.
\end{comment}
\begin{comment}
\begin{proof}
Consider \ref{item:Q-pres_not_type_3}. It is easy to see $\R\sats\varphi_{\mathrm{pair}}$, and if 
$\varphi$ is an $\Ll_0$-simple-Q-formula, then the proof $\R\sats\varphi$ given
$\M\sats\varphi$ is standard. So we may assume that $\M$ is active type 1 or 2.
By $\Sigma_1$-elementarity without parameters, $\hmE^\R\neq\emptyset$ and 
$\gamma^\R$ is defined, and since $\pi$ is $\Sigma_0$-elementary, 
$\pi``\hmE^\R\sub \hmE^\M$ and $\pi(\gamma^\R)=\gamma^\M$. Therefore
$\mu=\mu(\hmE^\R)$ is defined and $\pi((\mu^+)^\R)=(\kappa^+)^\M$ where $\kappa=\crit(\actext^\M)$.

Let $X,Y$ witness that $\pi$ is a weak $0$-embedding.
Let $f^\M:\M\to\M$ be
$f(y)=\M_\alpha$
where $\alpha$ is least such that $y\in\M_\alpha$. So $f^\M$ is total
and $\Sigma_1^\M$. Defining $f=f^\R:\R\to\R$ likewise, easily $f$ is also total (and 
$\Sigma_1^\R$). Moreover, $\pi(f(y))=f^\M(\pi(y))$.
So we may and do assume that $X\sub\rg(f)$ and $Y\sub\rg(f)\cross\rg(f)$.


For simplicity assume that $\varphi$ has only 1 free variable. Suppose 
\[ \varphi(z)\ \iff\ \all x\all\theta<\mu^+\ex y\ex\nu[x\sub y\ \&\ 
\theta\leq\nu<(\mu^+)\ \&\ \psi(z,y,\nu)] \]
where $\psi$ is $\Sigma_1$. Let $z\in\R$ be such that $\M\sats\varphi(\pi(z))$.
Let $x\in\R$ and $\theta<(\mu^+)^\R$. Let $x\in x'\in\R$ and $\theta\in 
t\in\R_{(\mu^+)^\R}$ be such that $(x',t)\in Y$. Let $\theta'=\OR(t)$. Then 
\[ \M\sats\ex y\ex\nu[\pi(x')\sub y\ \&\ \pi(\theta')\leq\nu\ \&\ 
\car(\theta')=\car(\nu)\ \&\ \psi(\pi(z),y,\nu)], \]
and this statement pulls back under $\pi$, which completes the proof.

We leave the rest to the reader.
\end{proof}
\end{comment}

\begin{comment}
***The remaining things to be moved later or deleted:

***Do we still use the following definition?

\begin{definition}
 Let $\M$ be an adequate model over $A$ and $\Hh\wpins\M$ and let $\xi=\wl(\Hh)$ and
$\xi+\eta=\wl(\M)$.
 Then we define $\M\down\Hh$ as the adequate model over $\Hh$ (literally, over 
$\widehat{\Hh}$) such that $\hmp^\N=\hmp^\M$, $\wl(\N)=\eta$, and for each 
$\gamma\in[1,\eta]$, letting $\N'=\N_\gamma$ and $\M'=\M_{\xi+\gamma}$, we have 
$\univ{\N'}=\univ{\M'}$, $\hmP^{\N'}=\hmP^{\M'}$ and $\hmE^{\N'}=\hmE^{\M'}$.
We also write $\N\down A=\M$.

Given an adequate model $\Hh$ and an adequate model $\N$ over $\Hh$, let $\N\down \hmb^\Hh$
be the natural candidate $\M$ for an adequate model over $\hmb^\Hh$ such that $\Hh\wpins\M$ and
$\M\down\Hh=\N$. So $\M$ is an adequate model iff $\M$ is acceptable.
\end{definition}

***Do we need the following remark?

\begin{remark}
 Let $\M$ be a potential opm over $A$ and $\N\wpins\M$.
 Then $\M\down\N$ is a potential opm over $\N$ iff $\N$ is a strong $\hmSdot$-cutpoint of $\M$.
\end{remark}

A \textbf{putative $(k,\theta)$-iteration strategy} for $\M$
is a function $\Sigma$ such that for every $k$-maximal tree $\Tt$ on $\N$, 
with $\Tt$ via $\Sigma$ and $\lh(\Tt)<\theta$ a limit, $\Sigma(\Tt)$ is a $\Tt$-cofinal branch.
(***? This is inconsistent with chapter 4.)
\end{comment}
\begin{comment}
\begin{definition} (***move this forward or to introduction)
For operator-premice $\M,\N$ and $\pi:\M\to\N$,
we say that $\pi$ is \textbf{$\nu$-preserving} iff $\pi$ is $\Sigma_0$-elementary
and, if $\M,\N$ are type 3 and $a,f\in\M^\sq$ are such 
that $\nu(\actext^{\M})=[a,f]^{\M}_{\actext^{\M}}$, then 
$\nu(\actext^{\N})=[\pi(a),\pi(f)]^{\N}_{\actext^{\N}}$.
(The latter does not follow from $\Sigma_0$-elementarity in the case that $\M,\N$ 
are type 3 and, literally, $\dom(\pi)=\M^\sq$.)
\end{definition}
\end{comment}

\begin{comment}
\begin{definition}\label{dfn:pot_cont_pm}
(***Need this?) Let $\Fop$ be an operator and $b\in C_\Fop$. Let $\N$ be an
$\Fop$-premouse over $b$. A \textbf{continuing $\Fop$-premouse over 
$\N$} is an adequate model $\M$ over $\N$ such that $\M\down b$ is an 
$\Fop$-premouse over $b$. (Therefore $\N$ is a strong cutpoint of $\M$.)

A \textbf{continuing $\Fop$-premouse} is a continuing 
$\Fop$-premouse over $b$, for some $b$.
\end{definition}
\end{comment}

\begin{comment}
In the definition of \emph{operator} below, the reason 
we incorporate the variable $i$ is as follows. Suppose we want to build a 
\emph{strategy premouse} $\N$, i.e. an opm in which the $B$-predicates are used to code some 
fradequate modelent of an iteration strategy $\Sigma$ (see \ref{dfn:pot_Sigma_pm} for a precise 
definition). 
Suppose we feed $\Sigma$ into 
$\N$ by always providing $b=\Sigma(\Tt)$, for the $<^\N$-least tree $\Tt$ for 
which this information is required. (Assume here that $\N$ is a $\J$-structure over $A=\hat{X}$, 
where $X$ is swo'd.) So given a reasonably closed 
level 
$\P\wpins\N$, the choice of which tree $\Tt$ should be processed next 
will usually depend on the information regarding $\Sigma$ already encoded in 
$\P$ (its \emph{history}). Using an operator $\Fop$ to build $\N$, then $\Fop(i,\P)$ will be a 
structure extending $\P$ and over which $b=\Sigma(\Tt)$ is encoded. The variable 
$i$ should be interpreted as 
follows. When $i=1$, we respect the history of $\P$ when selecting $\Tt$. When $i=0$ we 
ignore history when selecting $\Tt$.
\end{comment}

\begin{comment}
\begin{definition}
Let $m<\om$ and let $\M$ be an opm of successor length $\xi+1$. We say that $\M$ 
is \emph{$(m+1)$-soundly-projecting} iff $\M$ is $m$-sound, $\rho_{m+1}^\M\leq\OR(\M_\xi)$ and $\M$ 
is $\OR(\M_\xi)$-sound. We say that $\M$ is \emph{soundly-projecting} iff $\M$ is 
$(m+1)$-soundly-projecting for some $m<\om$.
\end{definition}
\end{comment}

\begin{comment}
\begin{definition} (***Is this too demanding?)
An \textbf{operator over $\opbk$} is an operator $\Fop$ over $\opbk$ such that 
$\dom(\Fop)\cut 
C'_\Fop$ is the set of all $\om$-sound $\Fop$-premice in $\opbk$ ($C'_\Fop$ as in 
\ref{dfn:operator}).
\end{definition}

From now on we will deal exclusively with operators (as opposed to the more general 
operators).
\end{comment}
\begin{comment}
These considerations also indicate that the burden, on player $\plII$,
to ensure that $M^\Tt_\alpha$ is an $\Fop$-opm when $\alpha+1<\theta$,
might be too demanding in the context of forming iteration trees on $\Fop$-opms $\Ww$ of height 
$\OR(\opbk)$. For example, if $\opbk=\her_{\kappa^+}$, $\kappa$ singular, then there could be 
$E\in\es^\Ww$ such that $\Ult(\Ww,E)$ has height $>\OR(\opbk)$, and is therefore not an $\Fop$-opm.
\end{comment}
\begin{comment}
We say that $\Fop$ \textbf{condenses $*$-well above $b$} iff the preceding holds, after making the 
following modifications. Replace ``$\varphi$ is a $k$-factor'' with ``$\varphi$ is a potential 
$k$-factor'', remove the phrase ``and $\M$ is $k$-relevant'', and strengthen 
the 
conclusion to ``$\M=\Fop(\M^-)$''.\footnote{This notion is almost that of \emph{condenses 
well}.}
\end{comment}

\begin{comment}
\begin{definition}
Given an opm $\N$ over $A$ and $\M\wpins\N$, the 
\textbf{$\M$-drop-down sequence} of $\N$ is the sequence of
pairs $\left<(\Q_n,m_n)\right>_{n<k}$ of maximal length such that $\Q_0=\M$ and 
$m_0=\om$ and for each $n+1<k$:
\begin{enumerate}[label=--]
 \item $\M\wpins\Q_{n+1}\wins\N$ and $\Q_n\wins\Q_{n+1}$ and $\rho_\om(\Q_n)$ is a cardinal of 
$\Q_{n+1}$,
 \item $0<m_{n+1}<\om$ and $\Q_{n+1}$ is $(m_{n+1}-1)$-sound,
 \item $\rho_{m_{n+1}}^{\Q_{n+1}}<\rho_{m_n}^{\Q_n}\leq\rho_{m_{n+1}-1}^{\Q_{n+1}}$.\qedhere
\end{enumerate}
\end{definition}
\end{comment}
\begin{comment}
\begin{remark}\label{rem:weakly_condenses_finely}
We could have made do with the following notion, which by 
\ref{lem:strengthen_scf_conclusion}, follows from fine condensation. (We will not make use of this 
notion, however.)
Let $\Fop$ be an operator over $\opbk$ and $b\in\opbk$ be transitive. Say that $\Fop$ 
\emph{weakly condenses finely above $b$} iff (i) $\Fop$ condenses 
coarsely above $b$ and (ii) we have the following.
Let $k,A,\M,G$, etc, be as in \ref{dfn:strongly_condenses_finely} (we maintain all hypotheses 
there, so $\varphi:\M\to\N$, etc). Suppose also that $\N^-$ satisfies 
$\om$-condensation. Then:
\begin{enumerate}[label=--]
\item If $\M$ is a $k$-relevant operator-premouse then $\M=\Fop(\M^-)$.
\item If $k=0$ and $\M=\core_1(\N)$ then $\M=\Fop(\M^-)$.
\item If $k=0$ and for some $i$, $\M=\solwit_{1,i}(\N)$ and 
$\varphi=\varsigma_{1,i}(\N)$ is $0$-good
then either $\M=\Fop(\M^-)$ or $\M\in\Fop(\M^-)$.
\end{enumerate}
\end{remark}
\end{comment}
\begin{comment}
***This statement no longer correct: In \ref{dfn:condenses_finely}, we
could have dropped the requirement 
``$\mathfrak{S}_{k+1}(\L)$ is an $\Fop$-pm'':

\begin{lemma}\label{lem:S_k+1_F_condensation}
***This lemma no longer correct: Let $(\Fop,b,\Abar,A)$ be an almost fine ground.
Let $k\leq\om$ and let $\M,\N$ be $\Fop$-premice over $\Abar,A$ respectively, not of type 3. Let 
$\pi:\M\to\N$ be a 
$k$-factor above $b$, as witnessed by $(\L,\sigma)$. Then
$\L$ is a $k$-sound $\Fop$-premouse, and if $k<\om$ then $\L$ and $\mathfrak{S}_{k+1}(\L)$ are both
$k$-relevant $\Fop$-premice.
\end{lemma}
\begin{proof}
If $k=\om$ this is immediate by almost coarse condensation. Suppose $k<\om$.
It is easy unless $\M,\N$ are successors, so assume this. So $\L$ is a $k$-relevant successor opm, 
and since $\sigma$ is $k$-good, almost fine condensation gives that either $\L=\Fop(\L^-)$ or 
$\L\in\Fop(\L^-)$. But $\L\notin\Fop(\L^-)$ as $\L$ is $k$-relevant. So $\L$ is an $\Fop$-pm. Let 
$\Ss=\mathfrak{S}_{k+1}(\L)$ and $\sigma=\sigma_{k+1}^\L$ and $\zeta=\zeta_{k+1}^\L$.
So $\sigma$ is $k$-good. It follows that $\Ss$ is a
successor opm and either $\Ss=\Fop(\Ss^-)$ or $\Ss\in\Fop(\Ss^-)$,
and $\zeta_{k+1}^\L\leq\rho_\om^{\L^-}$. If $\zeta=\rho_\om^{L^-}$ 
then $\Ss=\Ll$, in which case we are done, so suppose $\zeta<\rho_\om^{\L^-}$.
Clearly $\rho_{k+1}^\Ss\leq\zeta$. But then one can argue as in \ref{lem:strengthen_scf_conclusion} 
to show that $\Ss$ is $k$-relevant, and so also $\Ss\notin\Fop(\Ss^-)$, so $\Ss=\Fop(\Ss^-)$.
\end{proof}
\end{comment}
\begin{comment}
\begin{definition}
Let $\M,\N$ be type 3 opms. Let $a,f\in\M^\sq$ be such that
\[ \nu(E^\M)=[a,f]^\M_{E^\M}.\]
Let $\pi:\N^\sq\to\M^\sq$ be $\Sigma_0$-elementary.
Following \cite{something}, we say that $\pi$ is
\begin{enumerate}[label=--]
\item \emph{$\nu$-preserving} iff $\nu(E^\N)=[\pi(a),\pi(f)]^\N_{E^\N}$,
\item \emph{$\nu$-high} iff $\nu(E^\N)<[\pi(a),\pi(f)]^\N_{E^\N}$,
\item \emph{$\nu$-low} iff $\nu(E^\N)>[\pi(a),\pi(f)]^\N_{E^\N}$.
\end{enumerate}

For $\Sigma_0$-elementary embeddings $\pi:\R\to\Ss$ between opms $\R,\Ss$ not of type $3$,
we say that $\pi$ is \emph{$\nu$-preserving}.
\end{definition}

The results in \cite{something} on $\nu$-preservation, etc, generalize immediately to opms.
A weak $0$-embedding can be $\nu$-high or $\nu$-low, and a near $0$-embedding can be 
$\nu$-high. But it is easy to see that:

\begin{lemma}
 Let $\Q,\R,\Ss$ be $k$-sound type $3$ opms and let $\pi:\R\to\Ss$ be a weak $k$-embedding
 and $\sigma:\Q\to\R$ a near $k$-embedding, such that $\pi\com\sigma$ is a $\nu$-preserving near 
$k$-embedding. Then $\pi$ is not $\nu$-high.
\end{lemma}
\begin{proof}
Because $\sigma$ is a near $0$-embedding, $\sigma$ is not $\nu$-low.
If $\sigma$ is $\nu$-preserving then clearly so is $\pi$.
If $\sigma$ is $\nu$-high then $\pi$ is $\nu$-low.
\end{proof}
\end{comment}

\begin{comment}Now consider \ref{item:k_solid}. We may assume that $\lambda>1$, as the only 
extenders of $\N_1$ 
are $\Fop$-extenders, so there are no non-trivial iteration trees on it.
Let us also assume that $\N_\lambda$ has a largest $\Fop$-whole proper segment, 
since the contrary case is similar but easier. Then $\M^*$ has a largest 
$\Fop$-whole proper segment $\M_\Fop$; so $\M^+=\M^*\down\M_\Fop\wins\Fop_1(\M_\Fop)$. If 
$(\M^*,k+1)$ is not on 
the $\M_\Fop$-drop-down sequence of $\M^*$, then the proof of (a) shows that 
$\M^*$ 
is $(k+1)$-sound, and therefore $(k+1)$-$\Fop$-solid (the ``$\Fop$'' since 
$\core_{k+1}(\M^*)=\M^*$ in this case). So assume otherwise.

If $\M^*$ is whole let $\M'=\Fop_1(\M^*)$; otherwise let $\M'=\Fop_1(\M_\Fop)$. So $\M^*\in\M'$.
Let $\pi':\Mbar'\to\M'$ be elementary, with $\Mbar'$ countable and 
$\pi'(\Mbar)=\M^*$ for some $\Mbar$ and also such that 
$\pi=\pi'\rest\Mbar$ is in the hypothesized club and $\abar=a^{\Mbar}\in C_\Fop$. Because $\Fop$ 
condenses coarsely (and using 
\ref{lem:whole_Y_pm_elem_hull} or \ref{lem:E_active_Y_pm_elem_hull}), $\Mbar$ is an $\Fop$-premouse.
Now let $\Sigma$ be an $\Fop$-putative strategy for $\Mbar$ as hypothesized.
\end{comment}
\begin{comment}
Suppose first that $k<\om$. We just consider the case that $\Q,\R$ are $k$-relevant, as this is the 
important case,
and if $\Fop$ condenses $*$-well it is easier. Let $\Tt$ be a putative 
$\Fop$-tree via $\Sigma$ (so $k$-maximal), of successor length $\alpha+1$. We must show that 
$M^\Tt_\alpha$ is an $\Fop$-premouse. Let $\beta=\base^\Tt(\alpha)$, let $\M=M^\Tt_\alpha$ and 
$\varphi,\tau$ 
be the embeddings provided by the $(\pi,\CC)$-realizability of $\Tt$. The 
existence of $\varphi,i^{*\Tt}_{\beta,\alpha}$, together with almost coarse condensation and the 
fact 
that $\CC$ is tenable, ensure that $\M$ is an opm whose proper segments are all 
$\Fop$-premice.

So we may assume that $\wl(\M)$ is a successor. Suppose $[0,\alpha]_\Tt$ does not drop in 
model or degree. Then letting $\L=\Q$, $\N=\Ss$, $\sigma=i^\Tt_{0,\alpha}\com\psi$, (and 
$\M,\varphi$ have already been defined), the hypotheses of \emph{almost condenses finely} attain. 
Indeed, 
$\varphi\com\sigma=\pi\com\psi$, a near $k$-embedding,
and $\M$ is $k$-relevant because $\R$ is $k$-relevant and by \ref{lem:k-stack-max_pres_rpm}.
If $[0,\alpha]_\Tt$ drops in model or degree, it is similar.

The case that $k=\om$ is similar, just noting that if $\R$ has successor length 
and $[0,\alpha]_\Tt$ does not drop in model or degree, then the realizing map $\varphi$ is fully 
elementary, so almost coarse condensation ensures that $M^\Tt_\alpha$ is an 
$\Fop$-premouse.
\end{comment}

\begin{comment}
\begin{definition}[Weak fine structure]
Let $\N$ be a pre-fine $\Ll$-structure.

 We say $\M$ is \emph{$0$-weakly-sound}, and let $\rho_{\wk,0}^\M=\OR(\M)$ and
 $\rSigma_1^\M=\Sigma_1^\M$ (using $\Ll$).

 Let $n<\om$ and suppose that $\M$ is $n$-weakly-sound and $\om<\rho_{\wk,n}^\M$.
 Then $\rho_{\wk,n+1}^\M$ is the least $\rho\geq\om$ such that there is a $\bfwSigma_{n+1}^\M$
 set $X\sub Y^{<\om}\cross\rho^{<\om}$ with $X\notin\M$.
 We say that $\M$ is \emph{$(n+1)$-weakly-sound} iff there is $p\in\OR(\M)^{<\om}$ such that
 \begin{equation}\label{eqn:weakly_sound_witness} 
\M=\Hull_{\rSigma_{n+1}}^\M(Y\un\rho_{\wk,n+1}^\M\un\{p\}). \end{equation}
 Now suppose that $\M$ is $(n+1)$-weakly-sound and $\om<\rho_{\wk,n+1}^\M$. Then $T_{\wk,n+1}^\M$ 
denotes the set of all $(q,\alpha,t)\in\M$ such that $q\in\M$,
 $\alpha<\rho_{\wk,n+1}^\M$ and
 \[ t=\Th_{\rSigma_{n+1}}^\M(Y\un\alpha\un\{q\}). \]
 And $\rSigma_{n+2}^\M$ is the class of formulas of the form
 \[ \varphi(x_0,\ldots,x_{n-1})\ \iff\ \ex y\left[T_{\wk,n+1}^\M(y)\ \&\ 
\psi(y,x_0,\ldots,x_{n-1})\right], \]
where $\psi$ is $\rSigma_1$.

Let $p_{\wk,0}^\M=\emptyset$. Suppose $\M$ is $n$-weakly-sound and let
$\pvec_{\wk,n}^\M=(p_{\wk,0}^\M,\ldots,p_{\wk,n}^\M)$.
If $\M$ is $(n+1)$-weakly-sound, let $p_{\wk,n+1}^\M$ denote the least $q$
such that $p=\pvec_{\wk,n}^\M\conc q$ witnesses line (\ref{eqn:weakly_sound_witness}) (such a $q$ 
exists by $\Sigma_1$-ordinal-generation).

If $n$ is least such that $\rho_{\wk,n+1}^\M=\om$,
then for $m>n+1$, we say that $\M$ is \emph{$m$-weakly-sound} iff $\M$ is $(n+1)$-weakly-sound.

We say $\M$ is \emph{$\om$-weakly-sound} iff $\M$ is $n$-weakly-sound for all $n<\om$.
\end{definition}
\end{comment}
\begin{comment}
 \begin{definition}[Operator $\Fop_G$]\label{dfn:operator_Fop_G}
Let $G$ be a pre-operator over $\opbk$, with domain $D$. We define
a corresponding operator $\Fop=\Fop_G$, with domain $D'$, as follows.

We set $C^{D'}=C^D$. Let $X\in\witri{C^{D'}}$ and 
\[ \N=G(X)=(\univ{\N},\hmPvec^\N,\hmP^\N,X,\hmpv). \]
Let $n<\om$ be least such 
that $\rho_{\wk,n+1}^\N=\om$.
If $n=0$ then let $\M=\N$.
If $n>0$ then let $\sigma=\rho_{\wk,n}^\N$ and $\Q=\N|^\J\sigma$ and let $\M$ be the $\J$-structure
\[ \M=(\univ{\Q},\hmPvec^\N\rest\sigma,T,X,\hmpv),\]
where $T\sub\univ{\Q}$
codes
\[ \Th_{\rSigma_n}^\N(\univ{\Q}\un\pvec_{\wk,n}^\N) \]
in some uniform fashion, amenably to $\univ{\Q}$, such as with mastercodes.\footnote{For 
concreteness, we take $T$ to be the set of pairs $(\alpha,t')$ such that for some $t$,
$(\pvec_{\wk,n}^\M,\alpha,t)\in T_{\wk,n}^\M$, and $t'$ results from $t$
by replacing $\pvec_{\wk,n}^\M$ with $\R$ (the latter is not a parameter
of the theory $t$, so we can unambiguously use it as a constant symbol).}
Note that in either case, $\M=(\univ{\M},\hmPvec^\M,\hmP^\M,X,p)$ is an $\om$-weakly-sound 
$\J$-structure over $X$ and $\rho_{\wk,1}^{\M}=\om$.

Define $\Fop(X)$ as the hierarchical model $\K$ over $X$ with parameter $\hmpv$, of length $1$
(so $\hmS^{\K}=\emptyset$), with $\univ{\K}=\univ{\M}$, $\wl(\K)=1$,
$\hmE^{\K}=\emptyset$, and
\[ \hmP^{\K}=\{X\}\cross\left(\hmPvec^\M\oplus\hmP^\M\oplus\{p_{\wk,1}^\M\}\right).\]
(We use $\{X\}\cross\cdots$ to ensure that $\hmP^\K\sub\K\cut\K^-$.)

We next define $P^{D'}$ and $\Fop\rest P^{D'}$; in the end, every element of $P^{D'}$ will be an 
$\Fop$-premouse (and $\om$-sound). We define the relation ``$\R\in P^{D'}$'' and the value 
of $\Fop(\R)$ (for $\R\in 
P^{D'}$) by induction on $\wl(\R)$. More precisely, by 
induction on $\alpha\in\Ord\cut\{0\}$, we simultaneously define:
\begin{enumerate}
 \item $P^\Fop_{\alpha}$, which is the class of all 
$\Fop$-premice $\R$ such that $\wl(\R)\leq\alpha$,
 \item $P^G_{\alpha}$, which is the class of all \emph{$G$-whole} $\R\in P^\Fop_{\alpha}$.
 \item $P^{D'}_{\alpha}=D'\inter P^\Fop_{\alpha}$, and $\Fop\rest P^{D'}_{\alpha}$.
\end{enumerate}
Moreover, we will maintain that whenever $\R\in P^\Fop_{\alpha}$ and $\wl(\R)$ is a 
limit, then $\R$ is $G$-whole. We will also set 
$P^\G_1=P^\Fop_1$. Therefore, for every $\R\in P^\Fop_{\alpha}$ there is a largest 
$G$-whole $\Q\wins\R$.

We have already defined $C^{D'}$ and $\Fop\rest C^{D'}$, and this determines $P^\Fop_1$.
Set $P^G_1=P^\Fop_1$. (Note that every $\R\in P^\Fop_1$ is equivalent to 
$G(\hmb^\R)$; it is not equivalent to some $\R'\wpins^\J G(\hmb^\R)$; in this sense, $\R$ is 
\emph{$G$-whole}.)

Now let $1\leq\alpha<\OR(\opbk)$ and suppose we have defined $P^\Fop_{\alpha}$ and $P^G_{\alpha}$, 
maintaining the inductive hypotheses. Let $\R\in P^\Fop_{\alpha}$ be $\om$-sound, with 
$\wl(\R)=\alpha$, and let 
$\Q\wins\R$ be the largest $G$-whole segment of $\R$. Then we put $\R\in D'$ iff $\Q\in D$.
(This defines $P^{D'}_\alpha$.) Now suppose $\R\in D'$; we define $\Fop(\R)$.

Let
$A=\hmb^\R$ and $\rho=\rho_\om^\R$. 
Let $\P=G(\Q)$. Let $\N\wins^\J\P$ be largest such that for all $\alpha<\rho$, we have
\[ 
\pow(A^{<\om}\cross\alpha^{<\om})^\N=\pow(A^{<\om}\cross\alpha^{<\om}
)^\Q. \]
Let $n<\om$ be least such that
$\rho_{\wk,n+1}^\N=\om$. Now define $\M$ from $(\N,n)$ as in the definition of $\Fop(X)$ for $X\in 
\witri{C^{D'}}$, but with $Y^\M=\Q$ and $p^\M=\hmp^\Q$. 
Much as there, $\M=(\univ{\M},\hmPvec^\M,\hmP^\M,\Q,\hmp^\Q)$ is an $\om$-weakly-sound 
$\J$-structure over $\Q$ and $\rho_{\wk,1}^{\M}=\om$.

We claim that ($*$) $\R\in\M$; see \ref{?} below. We therefore (can) set $\Fop(\R)$ to be the 
unique 
hierarchical model $\K$ of length $\wl(\R)+1$ with $\univ{\K}=\univ{\M}$,
$\R\wpins\K$ (so $\hmS^\K=\hmS^\R\conc\left<\R\right>$), $E^{\K}=\emptyset$, and
\[ \hmP^{\K}=\{\R\}\cross\left(\hmPvec^\M\oplus\hmP^\M\oplus\{p_{\wk,1}^\M\}\right). \]

We set $\Fop(\R)=\K$.

This completes the definition of $\Fop\rest P^{D'}_\alpha$,
which also determines $P^\Fop_{\alpha+1}$. Now given $\K\in P^\Fop_{\alpha+1}\cut P^\Fop_\alpha$,
we put $\K\in P^G_{\alpha+1}$ iff $\N=\P$, where letting $\R=\K^-=\K|\alpha$, then $\N,\P$ are as 
in the definition of $\K=\Fop(\R)$. This completes the successor stage of the recursion.

Now let $\alpha<\OR(\opbk)$ be a limit. Then $P^\Fop_\alpha$ is determined by 
$\left<P^\Fop_\beta\right>_{\beta<\alpha}$. Given $\R\in P^\Fop_\alpha$ with 
$\wl(\R)=\alpha$, we put $\R\in P^G_\alpha$ (cf. \ref{?} below).
This completes the definition.
\end{definition}
\end{comment}
\begin{comment}
Adopt the notation of \ref{dfn:operator_Fop_G}($*$). If 
$\Q=\R$ then it is 
trivial,
so suppose $\Q\wpins\R$. Note then that for each $\Q'\wpins\R$ such that $\Q\wins\Q'$, $\Q$ is 
the largest $G$-whole proper segment of $\Q'$. So when defining $\Fop(\Q')$, we use the same 
$\P=G(\Q)$. It follows that $\rho_\om^{\Fop(\Q')}<\rho_\om^{\Q'}$. Therefore there are only 
finitely many such $\Q'$. Let these be $\left<\Q_i\right>_{i<m}$, enumerated in increasing 
order, and let $\Q_m=\R$; so $\Q_0=\Q$ and $\Q_{i+1}=\Fop(\Q_i)$, and in particular, 
$\R=\Fop(\Q_{m-1})$. Let $\N_i$ be the ``$\N$'' used in the definition of $\Fop(\Q_i)$.
Then if $i<j$ then $\N_i\wpins^\J\N_j$. But $\R$ is definable over $\N_{m-1}$,
and so $\R\in\N=\N_m$ and $\OR(\R)<\rho_{\wk,n}^\N$, which implies $\R\in\M$, as required.

Part \ref{item:limit_of_G-whole} also follows from the observations above.
Part \ref{item:dom_Fop_G} is easy.
\end{comment}

\begin{comment}
 \section{Operator condensation}\label{app:condenses}

Our use of \ref{dfn:condenses_finely} (i.e., \emph{condenses finely}) overcomes a problem which 
arises with the notion of \emph{condenses well} from 
\cite[2.1.10]{wilson2012contributions} when it is used in concert with 
other 
definitions 
in \cite{wilson2012contributions}. (\emph{Condenses well} 
also appeared in early 
versions of \cite{cmi}, in the same form.) In this appendix we illustrate this problem. All 
definitions and notation here are following 
\cite[\S2]{wilson2012contributions}.

Let $J$ be the function $x\mapsto\J_2(x)$. Clearly $J$ is a mouse operator (see 
\cite[2.1.7]{wilson2012contributions}). Let $F=F_J$ 
(see \cite[2.1.8]{wilson2012contributions}). Then we claim that $F$ does not 
condense well 
(contrary to \cite[2.1.12]{wilson2012contributions}). We verify this.

Clearly regular premice $\M$ whose ordinals are closed under ``$+\om$'' can be 
arranged as models $\tilde{\M}$ with parameter $\emptyset$ (see 
\cite[2.1.1]{wilson2012contributions}), such that for each 
$\alpha<\l(\tilde{\M})$, 
$\tilde{\M}|\alpha+1=F(\tilde{\M}|\alpha)$.

Now let $\M$ be a premouse such that for some 
$\kappa<\OR(\M)$, $\kappa$ is measurable in $\M$, via some measure on 
$\es=\es^\M$, and $\M\sats$``$\lambda=\kappa^{+\kappa}$ exists'', 
$\rho_\om^\M=\lambda$, and $\M=\J_1(\M_0)$ where $\M_0=\J^\es_\lambda$. 
Let $\M^*=\J_1(\tilde{\M_0})$, arranged as a model with parameter 
$\emptyset$ extending $\tilde{\M_0}$. Note that because 
$\rho_\om^\M=\lambda=\rho(\M_0)$, we have $\tilde{\M_0}\in\M^*\in 
F(\tilde{\M_0})$. Also,
$\l(\M^*)=\lambda+1$ and $(\M^*)^-=\tilde{\M_0}$ (see 
\cite[2.1.3]{wilson2012contributions}). 
(Thus, we can't say 
$\M^*=\tilde{\M}$, because $\tilde{\M}$ is not defined.)

Let $E\in\es^\M$ be $\M$-total with $\crit(E)=\kappa$. Let $\N=\Ult_0(\M,E)$ 
and $\pi=i_E$. Then 
$\rho_1^\N=\sup\pi``\lambda<\pi(\lambda)$. Let $\N_0=\pi(\M_0)$ and 
$\N^*=\J_1(\tilde{\N_0})$, arranged as a model with parameter $\emptyset$ 
extending $\tilde{\N_0}$. Then $\rho_1(\N^*)<\pi(\lambda)=\rho(\tilde{\N_0})$, 
and therefore $\N^*=F(\tilde{\N_0})$. But $\pi:\M^*\to\N^*$ is a $0$-embedding 
(and $\pi(\tilde{\M_0})=\tilde{\N_0}$). Since $\M^*\neq F(\tilde{\M_0})$, $F$ 
does not condense well (see \cite[2.1.10(1)]{wilson2012contributions}). 
(Note also that by using $\Ult_1(\M,E)$ in place of 
$\Ult_0(\M,E)$, we would get that $\pi$ is \emph{both} a 
$0$-embedding and $\Sigma_2$-elementary, so even this hypothesis 
is consistent with having $\M^*\neq F(\tilde{\M_0})$.)

Here is a second example, and one in which the embedding is the kind that can arise in the proof of 
solidity of the standard parameter. Certainly in this context we want to make 
use of \emph{condenses well}. We claim there are (consistently) mice $M$, containing large 
cardinals, and $\rho,\alpha\in\Ord^M$ such that:
\begin{enumerate}[label=--]
 \item $M=\J(N)$ where $N=M|(\rho^+)^M$,
 \item $M$ is $1$-sound,
 \item $\rho_1^M=\rho<\alpha<(\rho^+)^M$,
 \item $p_1^M=\{(\rho^+)^M,\alpha\}$, and
 \item letting $H=\cHull_1^M(\alpha\un\{(\rho^+)^M\})$ (here $\cHull$ denotes the transitive 
collapse of the hull), we have $\rho_\om^H=\alpha$.
\end{enumerate}
Given such $M$, note that $\alpha=(\rho^+)^H$ and $H=\J(M||\alpha)$.
Then $H$ is a $1$-solidity witness for $M$, and the $0$-embedding $\pi:H\to M$ is the one that 
would be used in the proof of the $1$-solidity of $M$.
Moreover, with $F$ as before, ``$M=\J(N)=F(N)$'' (since $M$ projects below $\Ord^N$) but 
``$H\neq F(M||\alpha)=\J(\J(M||\alpha))$''. So we have a failure of \emph{condenses well}, and one 
which is arising in the context of the proof of solidity. (Of course, in the example we are already 
assuming $1$-solidity, but the example seems to indicate that we cannot really expect to use
\emph{condenses well} in the proof of solidity for $F$-mice.)

Now let us verify that such an $M$ exists. Let $P$ be any mouse (with large cardinals) and $\rho$ a 
cardinal of $P$ such that $(\rho^{++})^P<\Ord^P$. Let $\gamma=(\rho^+)^P+1$. For 
$\alpha<(\rho^+)^P$ 
let
\[ H_\alpha=\cHull_1^{P|\gamma}(\alpha\un\{(\rho^+)^P\}). \]
Because $\rho_\om^{P|\gamma}=(\rho^+)^P$, it is easy to find $\alpha$ with 
$\rho<\alpha<(\rho^+)^P$ and such that the 
uncollapse map $H_\alpha\to P|\gamma$ is fully 
elementary, and so $\rho_\om(H_\alpha)=\alpha=(\rho^+)^{H_\alpha}$.
Fix such an $\alpha$. Then let $H=H_\alpha$ and let
\[ M=\cHull_1^{P|\gamma}(\rho\un\{(\rho^+)^P,\alpha\}). \]
We claim that $M,\rho,\alpha$ are as required. For $M\in 
P$, which easily gives that $\rho_1^M=\rho$. Clearly $M=\J(N)$ where $N=M|(\rho^+)^M$. The 
$1$-solidity witness associated to $(\rho^+)^M$ is
\[ \cHull_1^M((\rho^+)^M), \]
which is just $M|(\rho^+)^M$, because the latter satisfies $\ZFmin$, and therefore 
$M|(\rho^+)^M\elem_1 M$.
And the $1$-solidity witness assoicated to $\alpha$ is
\[ \cHull_1^M(\alpha\un\{(\rho^+)^M\}), \]
which is just $H$, and $H\in M$ because $H=\J(P||\alpha)$. All of the required properties follow.

The preceding examples seem to extend to any (first-order) mouse operator $J$ 
such that for all $x$, $\J_1(x)\in J(x)$.
\end{comment}
 \begin{comment}
\begin{definition}
 Let $t\in\RR$ and let $\N$ be an $\Fop$-premouse over $t$. We define
$\Lp^{\Fop,\Gamma}_+(\N)$ to be the stack of all $\Fop$-premice such that 
$\N\ins\Q$, $\Q$ projects
$\leq\OR^\N$, and $\Q$ is $(\om,\om_1)$-iterable above $\N$ via a $\Gamma$
strategy.
\end{definition}

Note that in the case that $\N$ above is a strategy premouse,
$\Lp^{\Fop,\Gamma}_+(\N)$ is usually not $\Lp^{\Fop,\Gamma}(\N)$, because
$\Fop^\N\neq\emptyset$ from the perspective of the former, but
$\Fop^\N=\emptyset$ from the perspective of the latter; and also because the
canonical wellorders of mice in the former hierarchy differ from those in the
latter.
\end{comment}

\begin{comment}
\begin{lemma} \label{UniquenessOfQStructures}Let
$\P$ be $k$-suitable and let $\Tt$ be a
normal
iteration tree of limit length on $\P$. Suppose $b_0,b_1$ are $\Tt$-cofinal branches and 
$\Q_0,\Q_1$ are such that for each
each $i$, $M(\Tt)\ins \Q_i\ins M^\Tt_{b_i}$, $\rho_\om(\Q_i)\leq\delta=\delta(\Tt)$, 
$\Q_i\sats$``$\delta$ is Woodin'' and
$\Phi(\Tt)\conc Q_i$ is
$(\om,\om_1)$-iterable. Then
either $\Q_0\ins \Q_1$ or $\Q_1\ins \Q_0$.\end{lemma}
\begin{proof}
Suppose not. Compare $\Phi(\Tt\conc b_0)$ with $\Phi(\Tt\conc b_1)$, and use the fact that 
$\P$ has only $\om$-many Woodins, to reach a contradiction.

Let $\Q=\Q_0$. We may 
assume $\delta$ is not a cutpoint of $\Q$. But then the comparis Let
$E\in\es_+(\Q)$ be least such that $\kappa=\crit(E)<\delta$. Let
$\alpha<\lh(\Tt)$ be least such that $\kappa<\nu(E^\Tt_\alpha)$. Let
$\gamma\leq\OR(M^\Tt_\alpha)$ be largest such that $\pow(\kappa)\inter
M^\Tt_\alpha|\gamma=\pow(\kappa)\inter \Q|\lh(E)$. Then:
\begin{enumerate}
 \item Either $[0,\alpha]_\Tt$ drops or $\gamma<\OR(M^\Tt_\alpha)$.
\item $\rho_\om(M^\Tt_\alpha|\gamma)\leq\kappa$ and $M^\Tt_\alpha|\gamma$ is
$\kappa$-sound.
\item $M^\Tt_\alpha|\gamma\sats$``$\kappa$ is a limit of Woodin cardinals and a limit
of cutpoints''.
\item Therefore, $\Tt\rest[\alpha,\lh(\Tt))$ can be considered a normal tree
on $M^\Tt_\alpha|\gamma$, above $\kappa$.
\end{enumerate}
These properties follow from the $k$-suitability of $\P$ and the fact that since
$E$ overlaps $\delta$, $\Q|\lh(E)\sats$``$\kappa$ is a limit of Woodins''.

Let $\Tt'=\Tt\rest[\alpha,\lh(\Tt))$, with
$M^{\Tt'}_\alpha=M^\Tt_\alpha|\gamma$. It follows that a normal tree on
$\Phi(\Tt)\conc\left<\Q_0,\delta\right>$ can be considered a normal tree on
$\Phi(\Tt')\conc\left<\Q_0,\delta\right>$. Likewise for $\Q_1$. The
lemma then follows from comparison and fine structural arguments. Here though,
there is one thing to mention. Because we have not required that
$\Q_0\ins M^\Tt_b$ for some $\Tt$-cofinal branch $b$, we don't know that all
extenders used in $\Uu$ are close to the model to which they apply. Therefore
the theory of \cite{FSIT} doesn't quite give us sufficient fine structural
preservation for this argument. However, we do in fact get enough preservation
in the present context, by \cite{?}.
\end{comment}
\begin{comment}
Note that by Lemma \ref{UniquenessOfQStructures}, if $\T$ is short, then there
is at most one ``good" branch for $\T$ (according to $\M|\beta$). The good
branch is the branch $b$ such
that there is a $\Q\unlhd \M^\T_b$ such that $\Q$ is a $Q$-structure for
$\delta(\T)$ and the phalanx $\Phi(\T)^\smallfrown \langle \Q,\delta(\T) \rangle$
is $(\omega,\omega_1)$-iterable in $\Gamma$. This motivates our next definition.
\end{comment}
\begin{comment}
Let $\Sigma$ and $\Lambda$ be normal $A$-iteration
strategies of $\P$ and $\Q$ respectively. The restriction of $\Sigma$
($\Lambda$) to short trees witnesses that $\P$ ($\Q$) is short tree iterable.
Also, nondropping $\Sigma$ ($\Lambda$) iterates of $\P$ ($\Q$) are $k$-suitable.
Since we will successively compare
$\P$ and $\Q$ on windows of consecutive Woodin cardinals, we assume $k=1$
without loss of generality. This is just a standard comparison. Let $\T$ and
$\U$ be the comparison trees according to $\Sigma$ and $\Lambda$ respectively.
The only point worth noticing is that there are no drops on the main branches of
$\T$ and $\U$; this follows from the definition of suitability and short-tree
iterability since otherwise, supposing $\T$ drops on the main branch then there
is a dropping iterate of $\P$ (namely the final model $\N^\T$ of $\T$) that
contains a strict initial segment (namely $\N^\U$) which is $1$-suitable; this
contradicts short tree iterability. Also, for each limit $\lambda < $ lh$(\T)$
(similarly for
$\lambda < $ lh$(\U)$), the $Q$-structure $\Q([0,\lambda]_\T,\T\rest \lambda)$
does not have any extender $E$ such that crit$(E) < \delta(\T\rest\lambda) \leq
$ lh$(E)$ since otherwise, the tree $\T$ drops in such a way that we can't undo
the drop; that is, there is some $\alpha<\textrm{lh}(\T)$ and some $\gamma <
o^{\M^\T_\alpha}$ such that $\T\rest [\alpha,\textrm{lh}(\T))$ is a tree based
on $\M^\T_\alpha\rest \gamma$ (this is described in more details in the proof of
Lemma \ref{UniquenessOfQStructures}). But this implies that any cofinal branch
$b$ of $\T$ drops. This contradicts the previous point.
\end{comment}
\begin{comment}We remark that in the comparison of, for example, 
$\R|0$ with $\N|0$ above, The discussion in the proof of Lemma \ref{Comparisons} also shows that if 
$\T$
is a genericity iteration tree on a $k$-suitable premouse $\P$ then for no limit
$\lambda\leq \textrm{lh}(\T)$, there is a $Q$-structure $\Q\unlhd \M^\T_\lambda$ for
$\delta(\T\rest\lambda)$ such that there is some $F \in \mathbb{E}_+(\Q)$ such
that crit$(F) < \delta(\T\rest \lambda) \leq $ lh$(F)$ as this would imply that $\T$ drops while 
genericity iteration trees are nowhere dropping.
\end{comment}
\begin{comment}
Since $\M|\alphabar$ is admissible, arguments in \cite{twms} give:

\begin{fact}\label{clm:norm_iter_stacks}
 If $Q$ is a $k+1$-sound g-organized $\Fop$-premouse such that $\rho_{k+1}^Q=\om$, and $Q$ is
$(k,\om_1+1)$-iterable in $\M|\alphabar$, then $Q$ is $(k,\om_1,\om_1+1)$-iterable 
in $\M|\alphabar$.
\end{fact}
\end{comment}
\begin{comment}Suppose that 
$\Q||(\delta^+)^\Q\in\LpGbgF_+(M_\Tt)$. 
Let $\Q'\pins\LpGbgF_+(M_\Tt)$ be such that 
$\Q'||(\delta^+)^{\Q'}=\Q||(\delta^+)^\Q$ and $\Q'$ projects to $\delta$. Now $\Q'$ is 
$\delta$-sound. For let $n<\om$ be such that $\rho_{n+1}^{\Q'}=M_\Tt\neq\rho_n^{\Q'}$. 
Then 
$\Q'\down z_1$ is $n$-sound, and $p_{n+1}^{\Q'}$ is $(n+1)$-solid for $\Q'\down z_1$, and 
\begin{equation}\label{eqn:Q'=Hull} Q'=\Hull_{n+1}^{Q'}(p_{n+1}^{Q'}),\end{equation}
and so it suffices to see that $\Q'=\K$ where
\[ \K= \Hull_{n+1}^{\Q'\down z_1}(\delta\un p_{n+1}^{\Q'}). \]
By line (\ref{eqn:Q'=Hull}), it suffices to see that $\delta\in\K$. But if not then 
$\delta=\crit(\pi)$ where $\pi$ is the uncollapse embedding, but since $\delta$ is Woodin in 
$\Q$, this implies that $\delta$ is not a cutpoint of $\Q$, a contradiction. 
So comparing $\Q$ with $\Q'\down z_1$, we get $\Q=\Q'\down z_1$. So $\Q$ is 
$(\Gammabar,\delta)$-iterable, a contradiction.
\end{comment}
\begin{comment}
there is a countable g-organized-$\Fop$-premouse 
$\R$ over $s$ and $\nu<\OR^\R$ such that $\nu$ is a strong cutpoint of $\R$, 
$\R$ is $\nu$-sound, $\rho_{m+1}^\R\leq\nu<\rho_m^\R$, and there is a weak 
$m$-embedding $\pi:\R\to\core_m(N_{\gamma'})$, but $\R$ is not above-$\nu$, 
$(m,\om_1)$-iterable in $\M|\alphabar$. (Thus, $\gamma$ exists 
because $\gamma_1$ is such a $\gamma'$.) Fix $\R,\nu,\pi$ witnessing this.
Also let $\chi$ be large and such that $(V_\chi,\delta)$ is a coarse premouse 
and let $W$ be countable and $\tau:W\to (V_\chi,\delta)$ be elementary, with 
everything relevant in $\rg(\tau)$. Let $\Sigma_W$ be the realization 
strategy for $W$. Let $\Sigma$ be the above-$\nu$,
$(m,\om_1,\om_1)$-strategy for $\R$ given by copying/resurrection to $\Sigma_W$.

Say a countable $m$-maximal stack $\Ttvec$ of countable trees on $\R$ is 
\emph{good} iff every tree $\Tt$ in $\Ttvec$ is above $\nu$, has a last model 
and $b^\Tt$ does not drop in model or degree.
\end{comment}
\begin{comment}
  \item If $\Uu$ is of limit length, via $\Sigma_N$, and is $\Gammabar$-short, then 
$\Sigma_N(\Uu)$ $k<\om$ then $P$ has 
a $k$-suitable segment iff 
``$i^\Tt(\gamma)$'' makes sense, where $\gamma=((\delta_k^N)^+)^N$; that is, letting 
$\alpha_0+1,\ldots,\alpha_j+1$ enumerate the elements of $b^\Tt$ at which $\Tt$ drops in model, in 
increasing order, and $\beta_i=\pred^\Tt(\alpha_i+1)$, and $\alpha_{-1}=-1$, then 
$\gamma\in\dom(\pi)$ where \[ \pi=i^{*\Tt}_{{\alpha_j}+1}\com 
i^{*\Tt}_{\alpha_{j-1}+1,\beta_j}\com\ldots\com 
i^{*\Tt}_{\alpha_0+1,\beta_1}\com i^\Tt_{0,\beta_0}, \]
and in this case, $\pi(N|\gamma)$ is the unique $k$-suitable segment of $P$.
 \item If $b^\Tt$ drops, then letting $k$ be largest such that $P$ has a $k$-suitable segment, the 
tail of $\Sigma_N$ for trees on $P$, above $\delta_k^P$, is the $\Gammabar$-short 
strategy.
 \item If $P$ has a $k$-suitable segment, and $j<k$, and $\alpha<\delta_{j+1}^P$, then the tail of 
$\Sigma_N$ for trees on $P$, based on the interval $[\delta_j^P,\alpha]$, is the $\Gammabar$-short 
strategy.
\end{comment}
\begin{comment}
Suppose now we are in Case \ref{case:M_relevant}. Let the notations be as above. The case 
$\dot{B}^\M=\emptyset$ and $\dot{E}^\M\neq \emptyset$ is proved exactly as in \cite[Lemma 
1.16.2]{Scalesweakgap}. Suppose $\dot{B}^\M\neq \emptyset$. The key point is 
that we can define a map $\pi^*\maps\OR(\M^*) \rightarrow \OR(\M)$ which is 
cofinal and 
$\Sigma_1$ elementary with respect to $\Sigma_1$ truth about ordinals and $z^*$ 
in $\M^*$ and about ordinals and $z$ in $\M$. This suffices to give us $\M^*$ 
is 
a $\Theta$-g-organized $\Fop$-premouse (and in this case, soundness of $\M^*$ is automatic because 
$p_1^\M = \emptyset$). The embedding $\pi^*$ can be extended to 
$\Hh^{\dot{\M}_i^{\M^*}}$ if this is defined and gives $0$-iterability 
of $\dot{\M}_i^{\M^*}$; otherwise, $\pi^*$ gives wellfoundedness of 
$\dot{\M}_i^{\M^*}$. We then get $\M^* = \bar{\M}$ as before. 

Otherwise, $\M = \Jop_\gamma(\M|\theta)$ for 
some $\gamma$ and no $\theta < \gamma^* \leq \gamma$ is such that $\M|\gamma^* 
\vDash \textsf{ZF}$. The map $\pi^*$ as in the previous paragraph guarantees 
iterability of $\M^*$ below $\theta^*$. This easily implies $\M^* = \bar{\M}$.

Case \ref{case:M_not_relevant} is dealt with as in the proof of \cite[Lemma 
1.16.2]{Scalesweakgap}.
\end{comment}
\begin{comment}
Using the above discussion, we get (see 
\cite[Definition 1.17 ]{Scalesweakgap} for \emph{$k$-stability}):
\begin{lemma}
For some $k<\omega$, there is an $k$-stable $\N$
which is $S_i$-iterable for all $i<\omega$.
\end{lemma}

Now armed with a $k$-stable $\N$,}
\end{comment}
\begin{comment}
Suppose for simplicity that $\Tt$ is based on $\Q|\delta_0^\Q$. Let $\alpha<\lh(\Tt)$ be such that 
$[0,\alpha]_\Tt$ drops and suppose that $M^\Tt_\alpha|\gamma$ is $1$-suitable, with Woodin 
$\delta$. 
Assume that $\alpha$ is least possible. Then all generators used in $[0,\alpha]_\Tt$ are $<\delta$. 
Therefore there is $\R\ins M^\Tt_\alpha$ which is a Q-structure for $\delta$. Since $\delta$ is the 
least Woodin of $\R$, $\delta$ is a cutpoint of $\R$. Let $\sigma:M^\Tt_\alpha\to 
M^{\pi\Tt}_\alpha$ 
be the copy map; assume for simplicity that $M^\Tt_\alpha$ is not type 3. Then $\sigma(\R)$ is the 
Q-structure for $\sigma(\delta)$, and $\sigma(\delta)$ is a cutpoint of $\sigma(\R)$. Since 
$\Psishort_\N$ is suitability strict, therefore $\sigma(\R)$ is above-$\sigma(\delta)$ iterable in 
$\M|\alpha$. But therefore $\R$ is above-$\delta$ iterable in $\M|\alpha$, a 
contradiction.\end{comment}


\begin{comment}
For let $\Tt$ be on 
$\Q$ and via both the short tree strategy and $\Psi^\pi_\N$, of limit length, suitability 
strict, and suppose that $\pi\Tt$ is short. To simplify notation assume that $\Tt$ is based on 
$\Q|\delta_0^\Q$. Let $b=\Psi^\pi_\N(\Tt)$. Let $\sigma:M^\Tt_b\to M^{\pi\Tt}_b$ be the copy map. 
We 
want to see that $\Tt$ is short and $\Tt\conc b$ via the short tree strategy. If 
$\sigma(\delta(\Tt))=\delta(\pi\Tt)$ this is easy so suppose $\sigma(\delta(\Tt))>\delta(\pi\Tt)$. 
Since $\Hull_1^\N(\{\tau^\N_{i,j}\}_{i,j<\om})$ is cofinal in $\delta_0^\N$, note that if $b$ does 
not drop then $\sigma(\delta(\Tt))<\delta_0^{M^{\pi\Tt}_b}$. So in any case, $\R=\Q(\Tt,b)$ exists 
and $\sigma(\R)=\Q(\pi\Tt,b)$. If $\delta$ is a cutpoint of $\R$ then $\sigma(\delta)$ is a 
cutpoint 
of $\sigma(\R)$ and because $\Psi_\N$ is suitability strict, therefore $\sigma(\R)$ is 
above-$\sigma(\delta)$ iterable in $\M|\alpha$, and so likewise $\R$ above $\delta$, which 
suffices. 
If $\delta$ is not a cutpoint of $\R$ use the proof of
\ref{lem:short_tree_strat_tracks} and the fact that $\Tt$ is suitability strict to see that $\Tt$ 
passes through a fatal drop, to a projecting mouse which is iterable in $\M|\alpha$, which 
suffices. If instead, $\pi\Tt$ is maximal, then it is easy to see that $\Tt$ 
is maximal.
\end{comment}


\begin{comment}
 Note then that since $\N\sats\AD$ and $\Fop$ is very nice, for every 
$X\in\pow(\RR)\inter\N|\alpha$, we have $X<_W\Fop\rest\RR$. 

As mentioned above, Theorem \ref{gapInTheMouse} is typically used when $\Fop\rest \textrm{HC}\notin 
\N$, where $\N$ ends a nontrivial weak gap in $\textrm{Lp}^{\gamma\Fop}(\mathbb{R})$. In this case, 
we do need to assume $\Jop_{1}(\N)\vDash \textsf{AD}$. In practice (e.g. in core model induction 
applications), we have $\J_1(\mathbb{R},\Fop\rest \textrm{HC}) \vDash \textsf{AD}$ and it's easy to 
see that every $A\in \powerset(\mathbb{R})\cap \Jop_1(\N)$ belongs to $\J_1(\mathbb{R},\Fop\rest 
\textrm{HC})$; therefore, our determinacy assumption is not unreasonable.
\end{comment}



\begin{comment}
Suppose there is no $E\in\es_+(\N|\eta)$ such that $\crit(E)\leq\xi<\lh(E)$ and
$E$ is total over $\N|\eta$. It follows that $\N|\gamma$ is
passive, that for eventually all $\eta'<\gamma$, $(\N|\eta')^*$ is already
defined, and for all $E\in\es_+(\N|\eta)$ with $\gamma\leq\lh(E)$, we have
$\gamma<\crit(E)$. Suppose $\gamma=\eta'+\om$ for some $\eta'$. Then
$\gamma=\eta$. Then $(\N|\eta')^*$ has already been defined. Moreover,
$\N|\eta'$ needs $J$-information at the next stage iff $(\N|\eta')^*$ does, and
if they do, then letting $\alpha=\alpha(\N|\eta')$, then
$\alpha=\alpha((\N|\eta')^*)$, and letting $\beta=\beta(\N|\eta')$ and
$\beta^*=\beta((\N|\eta')^*)$, then $(\N|\beta)^*=(\N|\eta')^*|\beta^*$ (so
since $\N|\beta$ is interdefinable with $(\N|\beta)^*$, we get
$\alpha(\N|\eta')=\alpha((\N|\eta')^*)$), and
$(\N|\alpha)^*=(\N|\eta')^*|\alpha$, so they're interdefinable, which implies
that $\Tt_{\N|\alpha}=\Tt_{(\N|\eta')^*|\alpha}$. The latter is just because
$\N|\alpha$ and $(\N|\eta')^*|\alpha$ have the same universe, and $\Tt_\M$ only
depends on the universe of $\M$. So by induction,
$(\N|\eta')^*=F_J^{+,\eta'-\alpha}((\N|\alpha)^*)$. So we can set
$(\N|\eta)^*=F_J^{+,\eta-\alpha}((\N|\alpha)^*)$ (which has height $\eta$).

, and
$\eta''\in(\alpha,\eta']$, we can just define $(\N|\eta)$
$\alpha(\N|\eta')=\alpha(\N$
and we set $(\N|\eta)^*=\J_\om((\N|\eta')^*)$.
Suppose $\gamma$ is a limit of limits. If $\gamma=\eta$ let
$(\N|\eta)^*=\sup_{\alpha<\gamma}(\N|\alpha)^*$. Suppose $\gamma<\eta$; so
$(\N|\gamma)^*$ is already defined. Let $(\N|\eta)^*$ be the
$(J,\N|\xi)$-premouse $\M$ of height $\eta$, such that $\M|\gamma=(\N|\gamma)^*$
and above $\gamma$, the extenders on $\es_+(\M)$ are exactly those on
$\es_+(\N|\eta)$.

Now suppose there is $E\in\es_+(\N|\eta)$ such that $\crit(E)\leq\xi<\lh(E)$
and $E$ is total over $\N|\eta$. Let $E$ be such with $\lh(E)$ minimal. Then by
hypothesis, $\rho_\om(\N|\eta)\leq\crit(E)$. Let $k<\om$ be such that
$\rho_{k+1}^{\N|\eta}\leq\crit(E)<\rho_k^{\N|\eta}$. Let $U=\Ult_k(\N|\eta,E)$.
Note that $\lh(E)$ is a strong cutpoint of $U$. Also, either (i)
$\car^U(\xi)=\crit(E)$, $E$ is type 1, and $(\car^U(\xi)^+)^U$ is a strong
cutpoint of $U$; or (ii) $\crit(E)<\car^U(\xi)$ and $\lh(E)=(\car^U(\xi)^+)^U$. 
In either case, let $\zeta$ be least such that $\zeta\geq\xi$ and
$\rho_\om(\N|\zeta)=\car^U(\xi)$. Then for all
$\eta'\in[\zeta,(\car^U(\xi)^+)^U)$ such that $\rho_\om(\N|\eta')=\car^U(\xi)$,
$(\N|\eta')^*$ is already defined.
Let $(\N|\eta)^*$ be the $(J,\N|\xi)$-premouse $\M$ such that
$\M|\lh(E)=\sup_{\eta'<\lh(E)}(\N|\eta')^*$, and above $\lh(E)$, the extenders
on $\es_+(\M)$ are exactly those on $\es_+(U)$.
\end{comment}

%Suppose $\gamma$ is a cutpoint of $\N|\eta$.
%Then $(\N|\eta)^*$ is
%the $(J,\N|\xi)$-premouse $\M$ where (i) $\M|\gamma=(\N|\gamma)^*$; (ii) above
%$\gamma$, the extenders on $\es_+(\M)$ are exactly those on $\es_+(\N|\eta)$.
%This makes sense because $\N|\gamma$ and $(\N|\gamma)^*$ are interdefinable.

%Now suppose $\gamma=\eta$. If $\gamma$ is a limit of limits, this has been
%dealt with by 

%(c) Let $\alpha\in[\gamma,\eta]$ be minimal such that
%$\N|\alpha$ is active and $\crit(F^{\N|\alpha})<\gamma\leq\lh(F^{\N|\alpha})$.
%Let $E=F^{\N|\alpha}$. So $\rho_\om(\N|\eta)\leq\theta\leq\crit(E)$ (in
%fact, $\crit(E)$ is a cutpoint of $\N|\eta$). Let $k<\om$ be such that
%$\rho_{k+1}^{\N|\eta}\leq\crit(E)<\rho_k^{\N|\eta}$. Let $U=\Ult_k(\N|\eta,E)$.
%Note that $\gamma=(\xi^+)^U$ and $U|\gamma$ is passive and is a cutpoint of
%$U$. Let $(\N|\eta,\N|\xi)^*$ be the $(J,\N|\xi)$-premouse $\M$ such that
%$\M|\gamma=(\N|\gamma)^*$ and above $\gamma$, the extenders on $\es_+(\M)$ are
%exactly those on $\es_+(U)$.

%(d) Let $(\N|\eta,\N|\xi)^*=\sup_{\alpha<\eta}(\N|\alpha,\N|\xi)^*$.


%If $\xi$ is a strong cutpoint of $\N|\eta$ then $\N|\eta\approx Q$. (That is,
%that are equal except for the fact that $Q$ is literally an
%$\N|\xi$-$J$-premouse.)

%Suppose $\xi$ is not a cutpoint of $\N|\eta$. Let $E\in\es^{\N|\eta}$ be least
%such that $\kappa=_{\mathrm{def}}\crit(E)<\xi<\lh(E)$. Then
%$\N|\eta\vDash$``$\kappa$ is a limit of Woodins''. Since $\N$ is suitable,
%therefore $\car^\N(\eta)<\kappa$. Let $\gamma\geq\eta$ be least such that
%$\rho_\om(\N|\gamma)\leq\kappa$, and let $n<\om$ be such that
%$\rho_{n+1}(\N|\gamma)=\kappa<\rho_n(\N|\gamma)$. Then
%$\mathrm{Ult}_n(\N|\gamma,E)\approx Q$. So from $(\N|\gamma,\xi)$ we compute
%$Q$.
%Conversely, given $Q$, we can compute $\N|\gamma=\mathcal{C}_\om(Q)$, and $Q$
%specifies $\xi$.

%Finally suppose $\xi$ is a cutpoint, but not a strong cutpoint, of $\N|\eta$.
%Then we translate from $\N|\eta$ to $Q$ by taking ultrapowers by all
%type 1 extenders on \end{comment}
%$\es(\N|\eta)$ having critical point $\xi$.
%We translate in reverse by undoing this process. That is, call a $J$-premouse
%$R$ \emph{relevant} iff $\N|\xi\ins R\ins\N|\eta$ and
%either $\rho_\om(R)\leq\xi$ or $R\sats$``$\kappa$ is the largest cardinal''. We
%define the \emph{$*$-translation} $R^*$ of relevant $J$-premice $R$, by
%induction on $\OR(R)$. The $*$-translation will be a fully sound $J$-premouse
%over $\N|\xi$. We will maintain by induction that if $\N|\xi\ins R\ins\N|\eta$
%and $R\sats$``$\kappa^+$ exists'' then $(R|(\kappa^+)^R)^*$ is
%$\Sigma_1(\{\xi\})$ over $R|(\kappa^+)^R$, and $R|(\kappa^+)^R$ is
%$\Sigma_1(\emptyset)$ over $(R|(\kappa^+)^R)^*$. So let $R$ be relevant.

%If $R\sats$``$\kappa$ is the largest cardinal'' then define
%$R^*=\sup_{\N|\xi\ins S\pins R}S^*$. (Note that $R$ is passive in this case,
%since $\xi$ is a cutpoint.)

%Now suppose $R\sats$``$\kappa^+$ exists''.

%Suppose $(\kappa^+)^R$ is a cutpoint of $R$.
%We define $R^*$ to be the $J$-premouse $R'$ such that
%$\OR(R')=\OR(R)$, $R'|(\kappa^+)^R=(R|(\kappa^+)^R)^*$, and above
%$(\kappa^+)^R$, $\es(R')_+$ consists of exactly the same extenders as does
%$\es(R)_+$. Because $(R|(\kappa^+)^R)$ is interdefinable
%with $(R|(\kappa^+)^R)^*$, this makes sense, and above $(\kappa^+)^R$, the fine
%structure of $R$ corresponds exactly to the fine structure of $R^*$ (though if
%$(\kappa^+)^R<\gamma\leq\OR(R)$ then
%$p_n^{R^*|\gamma}=p_n^{R|\gamma}\cut\{\kappa\}$), so $R^*$ is a sound
%$J$-premouse over $\N|\xi$.

%Now suppose $(\kappa^+)^R$ is not a cutpoint of $R$. Let $E$ be the
%least extender on $\es(R)_+$ witnessing this; so
%$\kappa=\crit(E)$ and $(\kappa^+)^R<\lh(E)$. Let
%$n<\om$ be such that $\rho_{n+1}^R=\kappa<\rho_n^R$. Let $Q=\Ult_n(R,E)$.
%Define $R^*$ from $Q$ just as we defined $R^*$ from $R$ in the previous case.
%Since $E$ is type 1, $R^*$ is sound. To undo the $*$-translation, we just
%compute $Q$ from $R^*$, and find $R=\core_\om(Q)$.

\begin{comment}
\begin{definition}[$*$-translation](***Didn't mention I'd also define
*-translation of $\N||\alpha$ when $\N|\alpha$ is active.***]
Let $\N$ be a $J$-mouse and $\xi<\OR^\N$. Let $\eta\in[\xi,\OR(\N))$, such that
for every $E\in\es_+(\N|\eta)$, if
$\crit(E)\leq\xi<\lh(E)$ and $E$ is total over $\N|\eta$, then
$\rho_\om(\N|\eta)\leq\crit(E)$.
%either (a) $\eta=\xi$; or (b)
%$(\xi^+)^{\N|\eta}$ is a passive level and is a cutpoint of $\N|\eta$; or (c)
%$(\xi^+)^{\N|\eta}$ is either (i) active or (ii) fails to be a cutpoint of
%$\N\|\eta$; and $\rho_\om(\N|\eta)\leq\theta\leq\xi$ for some cutpoint $\theta$
%of $\N|\eta$; or (d)
%$\N|\eta$ is a limit of such levels.
We define the \emph{$*$-translation}
$(\N|\eta,\N|\xi)^*$ (or just $(\N|\eta)^*$ if $\xi$ is understood). The
definition proceeds by recursion on $\eta$. We will maintain that
$(\N|\eta)^*\pins\Lp^J(\N|\xi)$ and
$(\N|\eta,\N|\xi)$ is definably equivalent to $((\N|\eta)^*,\N|\xi)$ (over the
least admissible
structure containing either of these), uniformly in $\eta$. We now
give the definition.

We set $(\N|\xi)^*=\N|\xi$. Similarly, for $\eta>\xi$ such that
$\xi$ is a
strong cutpoint of $\N|\eta$, we similarly set $(\N|\eta)^*\approx\N|\eta$;
that is, $(\N|\eta)^*$ is the 

Suppose $\alpha_0=\alpha>\xi$ is least such that $\N|\alpha$ is active and $\xi$
is not a strong cutpoint of $\N|\alpha$. Let $F=F^{\N|\alpha}$ and
$\kappa_0=\crit(F)$. Let $\eta=\eta_0$ be least such that
$\eta\geq\alpha$ and $\rho_\om(\N|\eta)\leq\kappa_0$, so we must define
$(\N|\eta)^*$. (We need not define $(\N|\gamma)^*$ for
$\gamma\in[\alpha,\eta)$.)

Let $\rho_{k+1}^{\N|\eta}\leq\kappa_0<\rho_k^{\N|\eta}$. Let
$P=\Ult_k(\N|\eta,F)$. We claim that $\lh(F)$ is a cutpoint of $P$. It follows
that $\xi$ is a strong cutpoint of $P$, and so we set $(\N|\eta)^*\approx
P$. (Clearly $P$ can be computed from $(\N|\eta,\N|\xi)$, as just described. To
recover $\N|\eta$ from $P$, we just take the core.) So suppose $\lh(F)$ is not a
cutpoint of $P$. Then by the initial segment condition and the minimality of
$F$, $\nu(F)$ is a limit cardinal and $\nu(F)=\crit(E)$ for any $E\in\es^P$
overlapping $\lh(F)$. Let $E$ be the least. Then $\kappa_0$ is strong below
$\nu(F)$ in $\N|\lh(E)$ (as witnessed by $\es^\N$). But then by applying $E$,
and the initial segment condition, $\kappa_0$ is strong below $\lh(E)$,
contradiction.

For $\eta>\eta_0$ such that $\N|\eta=\J_{\eta-\eta_0}(\N|\eta_0)$, just set
$(\N|\eta)^*=\J_{\eta-\eta_0}((\N|\eta_0)^*)$. Then for $\eta$ least such that
$\N|\eta$ is admissible, $\N|\eta$ has the same universe as $(\N|\eta)^*$ (and
$(\N|\eta)^*$ is the least admissible structure containing $(\N|\eta_0)^*$).

So for $\eta>\eta_0$ such that $\xi$ is a strong cutpoint of $\N|\eta$
(equivalently, $\kappa_0$ is a strong cutpoint, or $\eta_0$ is a strong
cutpoint), we can literally copy extenders across to define $(\N|\eta)^*$.
Let $\alpha_1>\eta_0$ be least such that $\kappa_0$ is not a strong cutpoint of
$\N|\alpha_1$. Let $F=F^{\N|\alpha_1}$.

Suppose $\kappa_0$ is a cardinal of
$\N|\alpha_1$. Then $\kappa_0=\crit(F)$, because otherwise $\crit(F)$ would be
strong below $\kappa_0$ in $\N|\kappa_0$, and we would get a contradiction like
before. Therefore, since $\N|\eta_0$ projects to $\kappa_0$, also $F$ is type 1.
Now choose $\eta_1\geq\alpha_1$ least such that $\N|\eta_1$ projects to
$\kappa_0$ and define $(\N|\eta_1)^*$ by:
$(\N|\eta_1)^*||\alpha_1=(\N||\alpha_1)^*$, and above $\alpha_1$, the extender
sequence of $(\N|\eta_1)^*$ is given by copying extenders from
$\Ult_k(\N|\eta_1,F)$, where $k$ is chosen as before.

We carry on in this way, defining pairs $\alpha_\gamma,\eta_\gamma$,
until reaching the lea\end{enumerate}
st $\gamma$ such that $\kappa_0$ is not a cardinal of
$\N|\alpha_\gamma$, and we have defined $(\N||\alpha_\gamma)^*$. Let
$\kappa'=\crit(F^{\N|\alpha_\gamma})$.

For $\eta\geq\eta_\gamma$, define $(\N|\eta)^*$ (when required) by:
$(\N|\eta)^*|\alpha_\gamma=(\N||\alpha_\gamma)^*$, and the extender sequence
above $\alpha_\gamma$ is given by copying $(\N|\eta,\N|\kappa')^*$. (Note that
$(\N||\alpha_\gamma,\N|\kappa)^*\approx\N||\alpha_\gamma$, so is
inter-computable with $(\N||\alpha_\gamma,\N|\xi)^*$. Moreover, for
$\eta\geq\alpha_\gamma$, $(\N|\eta)^*=(\N|\eta,\N|\xi)^*$ is defined iff
$(\N|\eta,\N|\kappa')^*$ is defined.)\end{definition}
\end{comment}

\begin{comment}
\begin{theorem}
\label{gapInTheMouse}
Let $\M$ be a $J$-mouse over $\mathbb{R}^\M$. Suppose $\M \vDash \textsf{AD}^+$
and $[\alpha,\beta]$ is a weak gap in $\M$ and $\omega\beta < o(\M)$. Let $n$ be
the least such that $\rho_n(\M|\beta) = \mathbb{R}^\M$. Then $\M \vDash
``r\utilde{\Sigma}^{\M|\beta}_n$ has the scale property".
\end{theorem}
\begin{proof}[Proof Sketch]
Since the proof is almost the same as that of \cite[Theorem 4.16]{ScalesK(R)},
we only sketch it here, focusing on a new case. There are three main cases:
\begin{enumerate}
\item $\M|\beta$ is passive;
\item $\M|\beta$ is active with $\dot{E}^{\M|\beta}\neq \emptyset$;
\item\label{passive_active_cases_3} $\M|\beta$ is active with
$\dot{B}^{\M|\beta}\neq \emptyset$.
\end{enumerate}
Case \ref{passive_active_cases_3} is new here so we'll focus on it. The other
cases are handled just like
in the proof of Theor\end{enumerate}
em 4.16 in \cite{ScalesK(R)}. To simplify the notation, we
assume $n=1$. Note that $\beta$ is a successor ordinal. Suppose $\Sigma = 
\Sigma_a^{1,\M}$ is a
non-reflecting type, where $a=\langle G, w_1\rangle$ for some real $w_1$ and a
finite set of ordinals $G$. We take $G$ to be $<_{\textrm{lex}}$-least. 

Let $\eta<\beta$ be largest such that $\M|\eta$ is whole. So
$\M|\beta\ins\BBB(\M|\eta,\Tt,b)$ for some $\Tt,b$.
Suppose $\M|\beta = (\lpole\M|\beta\rpole,\in,\emptyset,B,S,\l,\RR^\M)$ for some
$B,S,\l$. We define a sequence $(\beta_i \ | \ i<\omega)$ as in the proof of
\cite[Theorem 4.16]{ScalesK(R)}. Let $\beta_0 = \max\{\eta,
\max\{G\}\}$.\end{enumerate}

Suppose $\beta_i<\beta$ is defined. For $\gamma<\beta$ let
\[
\R_{\gamma}=(\lpole\M|\gamma\rpole,\in,\emptyset,B\inter\gamma,S^{\M|\gamma}
,\l^{\M|\gamma},a). \]
Let
\[
Y_i = \{ a \ | \ a \textrm{ is definable over } \R_{\beta_i} \textrm{ from }
\mathbb{R}^\M\cup\{G, \beta_0,\dots,\beta_{i-1}\}\}.
\]
Let $\psi_i$ be the least $\psi\in \Sigma$ such that $\R_{\beta_i} \vDash \neg
\psi[\langle G,w_1\rangle]$. Let 
\begin{center}
$\beta_{i+1}$ = least $\gamma$ such that $\R_\gamma \vDash \psi_i[\langle
G,w_1\rangle]$.
\end{center}
\noindent \textbf{Claim:} $\cup_{i<\omega} Y_i = \M|\beta$. In particular, the
$\beta_i$'s are cofinal in $\beta$.
\begin{proof}
Let $N$ be the transitive collapse of $\cup_{i<\omega} Y_i$ and let $\pi: N
\rightarrow \cup_{i\end{enumerate}
<\omega} Y_i$. Then $N = \mathcal{C}_0(\N)$ for some
$J$-premouse $\N$ over $\mathbb{R}^\M$. This uses that $J$ condenses well. Since
trees on $\N$ can be lifted to trees on $\M$ via $\pi$, $\N$ is $0$-countably
iterable. This implies $\N\lhd \M$. Since $\N$ realizes $\Sigma$, $\N = \M$.
This proves the claim.
\end{proof}
The rest of the proof is just as in the proof of
\cite[Theorem 4.16]{ScalesK(R)}. This completes our sketch of the theorem.
\end{proof}
A corollary of the proof of Theorem \ref{gapInTheMouse} is the following
theorem.
\begin{theorem}\end{enumerate}

\label{GapPassiveMouse}
Let $\M$ be a $J$-mouse over $\mathbb{R}^\M$ and $[\alpha,\beta]$ is a weak gap
in $\M$. Suppose either $\Theta^\M$ doesn't exist or sup$\{ \gamma < l(\M) \ | \
\M|\gamma \textrm{ is active}\} < l(\M)$. Letting $n$ be least such that
$\rho_n(\M|\beta)=\mathbb{R}^\M$, then $\M \vDash
``\utilde{\Sigma}^{\M|\beta}_n$ has the scale property". 
\end{theorem}
\begin{proof}[Sketch]
Note that $\beta$ could be $l(\M)$. The proof of this theorem follows from that
of Theorem \ref{gapInTheMouse} without significant changes. The point worth
mentioning is the following. Using the notation of the proof of Theorem 4.16 in
\cite{ScalesK(R)}, the condition (v) in the definition of $x$-honest becomes
\\
\noindent (v') \inde\end{enumerate}
nt if $\sigma_0,\dots, \sigma_n$ enumerates those
$B_0$-formulae $\sigma$ of one free variable such that $n(\sigma)\in
\textrm{dom}(u)$ and 
\begin{center}
$(|\M|\beta|,\in,I_u) \vDash i v \sigma(v) \in \textrm{OR}$,
\end{center}  
and if $\delta_m < o(\M|\beta)$ is such that 
\begin{center}
$(|\M|\beta|,\in,I_u) \vDash i v \sigma_m(v) = \delta_m$,
\end{center}  
for all $m\leq n$, then the map $\pi(\delta_m)= \eta_{n(\sigma_m)}$ for $m\leq
n$ is well-defined and for each $k<\omega$, $\pi$ is extendable to an
order-preserving map $\pi_k:o(\M|\beta_k)\rightarrow o(\M|\beta_k)$ such that
\begin{center}
$\M|\beta_k \vDash \theta[\gamma,w_1,w_2] \Leftrightarrow
\theta[\pi_k(\gamma),w_1,w_2]$.
\end{center}
\end{enumerate}

Note then that determinacy of $\M|\beta$ is enough to compute this aspect of
honesty. The rest of the proof is the same as before. 
\end{proof}
\end{comment}
\begin{comment}
 \item\label{item:local_cutpoint} Let $\eta<\xi<\OR^\N$ be such that $\eta$ is 
a strong cutpoint of
$\N|\xi$ and $\rho_\om(\N|\xi)\leq\eta$. Then
$\N|\xi\ins\Lp^{J,\Gamma}_+(\N|\eta)$.
\end{comment}
\begin{comment}
 \begin{definition}
  Let $t\in\RR$ and $1\leq k\leq\om$. A $J$-premouse $\N$ over $t$ is
\emph{$k$-suitable\end{enumerate}
} iff there is a strictly increasing sequence
$\left<\delta_i\right>_{i<k}$ such that \cite[1.2(a),(b),(d)]{Scalesweakgap}
hold (call these conditions (a),(b),(d)), along with: (c) Let $\xi\in\OR(\N)$
and let $\xibar=\car^\N(\xi)$. Among those extenders $E\in\es(\N)$ such that
$\xi<\lh(E)$, let $E$ be the extender for which $(\crit(E),\lh(E))$ is
$<_\lex$-minimal. Let $\kappa=\crit(E)$. 
 \begin{enumerate}
  \item Suppose $\kappa<\car^\N(\xi)$ (so $E$ is total over $\N$). Then
$\Lp^{J,\Gamma}(\N|\xi)=\N||\lh(E)$.
\item Suppose $\car^\N(\xi)\leq\kappa$. Then
$\Lp^{J,\Gamma}(\N|\xi)=(\N|(\xi^+)^\N,\N|\xi)^*$.
 \end{enumerate}
\end{definition}
For each $i\leq k$, we will write $\delta^\N_i$ for the $\delta_i$ in the above
definition. In the context of $k$-suitability, we omit the phrase ``over
$t$'', but all relevant premice will implicitly be over $t$ for some fixed $t$.
\end{comment}
\begin{comment}
Consider comparing $M^\Tt_b$ with the least
$\P\pins\Lp^{J,\Gamma}_+(M(\Tt))$ such that $\P$ projects to
$\delta(\Tt)$ and $\P\notin M^\Tt_b$, producing trees $\Uu,\Vv$ on
$M^\Tt_b,\P$. 

 Since $\P$ projects to $\delta(\Tt)$, $b^\Uu$ does
not drop. But then $\N$ is $\Gamma$-iterable, since the last model of $\Vv$ is
$\Gamma$-iterable (here we use that $\Lp^{J,\Gamma}_+(M(\Tt))$ is iterable for
finite stacks of normal trees). This is a contradiction. So if $i$ is least
such that $\Tt$ is based on $\N|\delta_i^\N$, then
$i^\Tt_b(\delta_i^\N)>\delta(\Tt)$. Therefore there is a Q-structure
$Q(\Tt,b)\ins M^\Tt_b$. If $Q(\Tt,b)$ does not overlap $\delta(\Tt)$ then we
can compare $Q(\Tt,b)$ with the Q-structure $Q\pins\Lp^{J,\Gamma}_+(M(\Tt))$,
as before, and therefore $Q(\Tt,b)=Q$, and we are done. Suppose $Q(\Tt,b)$
overlaps $\delta(\T\end{enumerate}
t)$.
\end{comment}

\begin{comment}
 Wfd'ness of $Q_\infty$ is not clear without $\RR=\RR^\M$. We do have wellfoundedness through 
$\Theta^\M$ tho. Regarding Lemma 2.1.2, it's okay as the linear chain gets in $\M_\DC$, so those 
iterates can all be compared inside $\M_\DC$.
\end{comment}

\begin{comment}
 Let $\Fop$ be an operator. We say that $\Fop$ is \textbf{extremely nice} iff there is a sequence 
of 
sets 
of reals 
$\left<A_i\right>_{i<\om\beta}$ for some $\beta$ such that:
\begin{enumerate}[label=(\arabic*)]
 \item $\Fop$ is very nice;
 \item for each $i<\beta$, $\left<A_{\omega i+n}\right>_{n<\om}$ is a self-justifying system;
 \item for each $i<\beta$, $n,m<\omega$, there is no scale on $A_{\om i + n}$ which is Wadge below 
$A_{\omega i + m}$, and $A_{\omega i + n}<_W 
A_{\omega i + k}$ for some $k<\om$;
\item for $i<j<\beta$, $A_{\omega i + n} <_W A_{\omega j}$ for all $n<\omega$;
 \item \label{item:ProjEqui}$\Fop\rest\HC$ is projectively equivalent to a set of 
Wadge rank sup$_{i<\beta}w(A_{\om i})$; and
 \item For every $\AD$-pointclass $\utilde{\Gamma}$, $\utilde{\Gamma},\Fop\rest\HC$ are Wadge 
compatible.
\begin{comment}and every $i<\beta$, $\utilde{\Gamma},A_{\omega 
i}$ are 
Wadge compatible.
\qedhere\end{enumerate}

\end{enumerate}
\end{definition}

\begin{remark}\label{rem:application}
Let $\Fop$ be an extremely nice operator.
We want to see that the scales analysis in 
$\Lp^{^\gTheta\Fop}(\RR)$ proceeds from optimal determinacy assumptions. Let 
$\N\pins\Lp^{^\gThe
ta\Fop}(\RR)$ be such that $\N\sats\AD$ and 
$\N$ ends a gap 
$[\alpha,\beta]$ of $\Lp^{^\gTheta\Fop}(\RR)$, such that $[\alpha,\beta]$ is not strong. Suppose 
that 
if $[\alpha,\beta]$ is weak and $\Fop\rest\HC\in\N|\alpha$ then super-small mouse capturing 
for $\Gamma=\Sigma_1^{\N|\alpha}$ holds on a cone. We claim that one of the scale existence 
theorems 
\ref{passiveGameScale}, 
\ref{gapInTheMou\end{enumerate}
se}, or \ref{weak gap from MC} applies.

For by \ref{rem:non_adm_gap_dealt_with} and the mouse capturing hypothesis, we may assume that the 
gap is admissible, and so weak, and that $\Fop\rest\HC\notin\N|\alpha$. We claim that then 
$\J_1(\N)\sats\AD$, so \ref{gapInTheMouse} applies. If every set of reals in $\J_1(\N)$ is Wadge 
below $A_{\om i}$ for some $i<\beta$, then this follows immediately because 
$\J_1(\HC,\Fop\rest\HC)\sats\AD$. So suppose otherwise. Let $\P\ins\N$ be least such that there is 
a 
set $X\in\J_1(\P)$ with $X$ not Wadge below any $A_{\om i}$. If $\P\pins\N$ then 
$\J_1(\P)\sats\AD$, 
so by 
Wadge compatibility (i.e. \ref{dfn:extremely}\ref{item:ProjEqui}), we have 
$\Fop\rest\HC\in\J_1(\P)$, so 
$\alpha\leq\l(\P)$. Now we claim that $\Fop\rest\HC\notin\N|\beta$. Because $\Fop$ is very nice 
and by 
\ref{InsideGap}, this is clear if $\Th_{\rPi_1}^{\N|\alpha}\leq_W
\Fop\rest\HC$ or $\Th_{\rSigma_1}^{\N|\alpha}\leq_W\Fop\rest\HC$. Otherwise, by Wadge 
compatibility, 
$\Fop\rest\HC<_W\Th_{\rSigma_1}^{\N|\alpha}$. But then because $\N|\alpha$ is 
admissible, 
$\Fop\rest\HC\in\N|\alpha$, contradiction. So $\P=\N$. 
Since $\N$ ends a 
weak gap, there are sets $X_i\in\pow(\RR)\inter\N$ such that $\pow(\RR)\inter\J_1(\N)$ is exactly 
the sets which are projective in $\oplus_{i<\om}X_i$. It follows that
$\pow(\RR)\inter\J_1(\N)=\pow(\RR)\inter\J_1(\HC,\Fop\rest\HC)$, so $\J_1(\N)\sats\AD$, as required.

%Let $T=\Th_{\rPi_1}^{\N|\alpha}(\RR)$; so $T\in\N$, so by Wadge compatibility, 
%either $T<_W A_{\om i}$ for some $i<\beta$ or $A_{\omega i}\leq_W T$ for all $i<\beta$. But if 
$T<_W A_{\omega i}$ then because $\Fop$ 
%is very nice, there is a scale on $T$ in $\J_1(\P)$, contradicting \ref{InsideGap}. So 
%$A_{\om i}\leq_W T$ for all $i<\beta$, and so $A_{\omega i} \leq_W\neg T$ for all $i<\beta$.


%Therefore $A_0<_W\neg T$, which 
%implies $A_0\in\N|\alpha$ because $\N|\alpha$ is admissible. But then there is a scale $S$ for 
$A_0$ 
%in $\N|\alpha$, so $S$ is not Wadge below any $A_i$, contradiction. 
\end{remark}

\end{comment}

% scales_local_HOD_J.tex below:

\begin{comment}
Note that $\mathcal{H}_{\alpha+1} =
(|\mathcal{J}(\mathcal{H}_\alpha)[A]|; \in, \emptyset,
A\cap|\mathcal{J}(\mathcal{H}_\alpha)[A]|,\dot{S}^\smallfrown
\mathcal{H}_\alpha, l(\mathcal{H}_\alpha) + 1, a)$ for some $A$, where
$\dot{S}=\dot{S}^{\mathcal{H}_\alpha}$ and it's easy using the local
definability of $\mathbb{P}$ over the structure $\mathcal{H}_{\alpha+1}$ and the
proof of Theorem 3.9 in \cite{ScalesK(R)} to show that $\M_{\alpha+1} =
(|\mathcal{J}(\mathcal{M}_\alpha)[A]|; \in, \emptyset,
A\cap|\mathcal{J}(\M_\alpha)[A]|,\dot{S}^\smallfrown \mathcal{M}_\alpha,
l(\mathcal{M}_\alpha) + 1, a)$, where $\dot{S} = \dot{S}^{\M_\alpha}$ and that
$\M_{\alpha+1}$ and $\mathcal{H}_{\alpha+1}$ are fine structurally equivalent.
\end{comment}

% scales_strategy_premice.tex

\begin{comment}
For certain $\Sigma$-premice, we will need to be able to cut off an application 
of the $\BBB$ operator mid-way. We use the following definition to facilitate 
this.

\begin{definition}\label{dfn:B_psi}
 Let $\psi\in\Ll_0^-$ be $\Sigma_1$ and let $a,\Tt,b$ be as in 
\ref{dfn:B(M,T,b)}. Let $\N=\BBB(a,\Tt,b)$. Then $\BBB_\psi(a,\Tt,b)$ is the 
unique $\J$-model $\R$ over $a$ such that either:
\begin{enumerate}
 \item $\N\sats\neg\psi$ and $\R=\N$; or
 \item $\N\sats\psi$, and $\R=\N||\alpha$, where $\alpha$ 
is least such that $\N||\alpha\sats\psi$.\qedhere
\end{enumerate}
\end{definition}

Clearly $\BBB=\BBB_\psi$ for some $\psi$, so we can just talk about 
$\BBB_\psi$, without loss of generality.
\end{comment}
\begin{comment}
\begin{definition}
A class $C$ is \textbf{admissibly $\Sigma_1$} iff there is a $\Sigma_1$ formula 
$\psi_C$ in the language of set theory, such that for all 
transitive admissible sets $X$ and $x\in X$, we have $x\in C$ iff 
$X\sats\psi_C(x)$.

Let $C$ be a class of limit length iteration trees, 
closed under limit initial segment, admissibly $\Sigma_1$, as witnessed by 
$\psi_C$. For a $\J$-model $\M$ over $a$, where $a$ is self-wellordered 
(implicitly or explicitly), define $\Tt=\Tt^C(\M)$ recursively by: if there is a 
limit length iteration tree $\Uu$ on $\hmp$ such that $\M\sats\psi_C(\Uu)$, 
and for each limit $\eta\leq\lh(\Uu)$, $\Uu\rest\eta=\Tt^C_{\M|\alpha}$ for 
some $\alpha\in[1,\l(\M))$ iff $\eta<\lh(\Uu)$, then $\Tt$ is the $<_\M$-least 
such $\Uu$; otherwise $\Tt=\emptyset$. Clearly there 
is a formula $\varphi_C$ in $\Ll_0^-$ such that for all $\M,a$ as above, we 
have $\Tt=\Tt^C(\M)$ iff $\Tt\in\M$ and $\M\sats\varphi_C(\Tt)$. Then, a 
\textbf{potential $\hmp$-strategy premouse of type $C$} is a potential 
$\hmp$-strategy premouse of type $\varphi_C$.
Fix $C,\varphi_C$ as above. Then 
$\hist_C$ is the 
$\Ll_0^-$-formula, in one free variable $\Tt$, asserting ``Either
\begin{enumerate}
\item There is no $\alpha\in\dom(\dot{S})$ such that $\dot{S}_\alpha$ is 
admissible, and $\varphi_C(\Tt)$; or
\item Let $\xi\in\dom(\dot{S})$ be least such that $\dot{S}_\xi$ is 
admissible. Then $\dot{S}_\xi$ is a $\hmp$-strategy premouse of type 
$\varphi_C$; let $\Sigma=\Sigma^{\dot{S}_\xi}$. Then there is $n<\om$ an a 
sequence $\left<\M_i\right>_{i\leq n}$, and with $\M_n=\dot{S}_\xi$, and for 
each $i\in(0,n]$, $\M_i$ is a $\J$-model over $\M_{i-1}$ with parameter 
$\hmpdot$, and there is a passive $\J$-model $\N$ over $\M_0$, with 
parameter $\hmpdot$, such that $\univ{\N}=\univ\{\M_n\}$, and $\N$ is 
$\Sigma_1^{\M_n}(\M_n)$, and $\M_n$ is $\Sigma_1^{\N}(\N)$, and $\M_0\ins\N$, 
and $\N$ is a potential $\hmp$-strategy premouse of type $\varphi_C$, and 
$\Sigma^\N=\Sigma$, and for each $i\in(0,n]$, and each $\alpha\leq\l(\M_i)$, 
either:
\begin{enumerate}
 \item there is no $\beta<\alpha$ such that $\M_i|\beta$ is 
admissible, and $\M_i|\alpha$ is a $\hmp$-strategy premouse of type 
$\varphi_C$; or
 \item there is some $\zeta<\alpha$ such that $\M_i|\zeta$ is 
admissible, and letting $\gamma$ be such that 
$\OR(\N|\gamma)=\OR(\M_i|\alpha)$, we have $E^{\N|\gamma}=E^{\M_i|\alpha}$ and 
$B^{\N|\gamma}=B^{\M_i|\alpha}$.
\end{enumerate}
Moreover, there is no such sequence of length $>n$. Now let $\N^*$ be the 
proper class $\J$-model such that $E^{\N^*}=\dot{E}$ and $B^{\N^*}=\dot{B}$ 
and for all $\alpha\in(\xi,\dom(\dot{S}))$, 
$E^{\N^*|\alpha}=E^{\dot{S}_\alpha}$ and $B^{\N^*|\alpha}=B^{\dot{S}_\alpha}$. 
Then $\N^*\sats\varphi_C(\Tt)$.''
\end{enumerate}

Then a \textbf{potential continuable $(\hmp,C)$-strategy premouse} is a 
potential $\hmp$-strategy premouse of type $\hist_C$.
\end{definition}
\end{comment}
\begin{comment}
\begin{definition}\label{dfn:strategy_op}
Let $\P$ be transitive and $\Sigma$ a partial iteration strategy for $\P$.
Let $\varphi\in\Ll_0$. Let $\Fop=\Fop_{\Sigma,\varphi}$ be 
the operator such that:
\begin{enumerate}
 \item $\Fop_0(a)=\Jop_1(a;\P)$, for all transitive 
$a$ such that $\P\in\J_1(\ahat)$;
 \item Let $\M$ be a sound branch-whole $\Sigma$-premouse of 
type $\varphi$. Let $\lambda=\l(\M)$ and with notation as in \ref{PotStrPremouse}, let 
$\Tt=\Tt_\lambda$. If $\Tt=\emptyset$ then $\Fop_1(\M)=\Jop_1(\M;\P)$. If 
$\Tt\neq\emptyset$ then $\Fop_1(\M)=\BBB(\M,\Tt,b)$ where $b=\Sigma(\Tt)$.
\end{enumerate}
We say that $\Fop$ is a \textbf{strategy operator}.
\end{definition}

Clearly, with the notation above, if $\Sigma$ is a strategy for $\P$ which is sufficiently total 
over an operator background $\opbk$ and $\M\in\opbk$, then $\M$ is an 
$\Fop_{\Sigma,\varphi}$-premouse iff 
$\M$ is a $\Sigma$-premouse of type $\varphi$.
\end{comment}

\begin{comment}
\begin{enumerate}[label=--]
 \item $\hmb$ is swo'd, with ordering $\prec_{\hmb}$, and $\hmp$ is transitive.
Let $\prec$ be the canonical wellorder of the universe extending $\prec_{\hmb}$.
 \item For $\alpha\leq\l(V)$, define $\Sigma_\alpha$ (a putative iteration strategy for 
$\hmp$, to be definable over $V|\alpha$), and $\Tt_\alpha\in V|\alpha$, by 
recursion on $\alpha$, as follows. Let $\Sigma_0=\Sigma_1=\Tt_0=\emptyset$. 
Fix $\alpha$ and suppose we have defined
$\Sigma_\alpha$ and $\Tt_\beta$ for all $\beta<\alpha)$. If there is $\beta<\alpha$ such that 
$\Tt_{\beta}\neq\emptyset$ but $\Tt_{\beta}\notin\dom(\Sigma_\alpha)$, then let
$\beta$ be least such and let $\Tt_\alpha=\Tt_{\beta}$. Otherwise, $\Tt_\alpha$ is the 
$\prec$-least $\Tt\in V|\alpha$ such that $V|\alpha\sats\psi(\Tt)$, $\Tt$ is a limit length 
iteration tree on $\hmp$, $\Tt$ is via $\Sigma_\alpha$, and $\Tt\notin\dom(\Sigma_\alpha)$, if such 
a $\Tt$ exists, and otherwise $\Tt_\alpha=\emptyset$. Now fix $\alpha'\leq\lh(V)$ and suppose we 
have defined $\Sigma_\beta,\Tt_\beta$ for all $\beta<\alpha'$. Suppose that (i) there is 
$\beta_0<\alpha$ such that $\Tt_{\beta_0}\neq\emptyset$ and for all $\beta\in[\beta_0,\alpha)$, 
$\Tt_\beta=\Tt_{\beta_0}$. Let $\beta_0$ be least such. Suppose also that (ii)
$\om\beta_0+\lh(\Tt)=\om\alpha$. Then
\[ 
\Sigma_{\alpha}=\Sigma_{\beta_0}\un\{(\Tt_{\beta_0},b^{V|\alpha})\}. \]
If instead either (i) or (ii) fail, then
$\Sigma_\alpha=\bigcup_{\beta<\alpha}\Sigma_\beta$.
\item $\Tt_{\l(V)}$ is defined and $x=\Tt_{\l(V)}$.\qedhere
\end{enumerate}
\end{comment}



\begin{comment}
\begin{definition}\label{dfn:suitable}
We say that $(\Fop,\Sigma,\varphi,D,X)$ is 
\textbf{suitable} iff $X\in\HC$ is transitive and 
$\M_1^{\Fop,\#}(X)$ exists (so $X\in\witri{C_\Fop}$), where either
\begin{enumerate}[label=(\roman*)]
 \item\label{item:mouse_op} $\Fop$ is an operator which condenses 
finely, $D$ is the set of pairs $(i,X)\in\dom(\Fop)$ such 
that either $i=0$ or $X$ is a sound whole $\Fop$-premouse,  and 
$\Sigma=\varphi=0$, or
 \item $\P,\Sigma,\varphi,D_\varphi$ are as in \ref{lem:FSigma_condenses}, 
$Y=\Sigma$, $\Fop=\Fop_{\Sigma,\varphi}$, $D_\varphi\sub D$, $D$ is a class of limit length 
iteration trees on $\P$, via $\Sigma$, $\Sigma(\Tt)$ is defined for 
all $\Tt\in D$, $(\Sigma,D)$ is suitably condensing and $\P\in\J_1(\ahat)$.
\end{enumerate}
We write 
$\Omega_\Fop$ for the function 
with domain $C$, such that $x\mapsto\Sigma(x)$ in case (ii), and in case (i), 
$\Omega_\Fop(0,X)=\Fop(0,X)$ and $\Omega_\Fop(1,X)=\R\down a^X$ for the least $\R\ins\Fop_1(X)$ 
such that 
either $\R=\Fop_1(X)$ or $\R\down a^X$ is unsound.
\begin{comment}
The objects $a,\Fop,C,\MFsharp,\Omega_\Fop$ are now fixed for the remainder of the 
paper.
\end{definition}
\end{comment}

\begin{comment} For example, the fact that 
\ref{rem:M_1^Jsharp}(ii) gives hull
condensation, is because of the following. Let $\P$ be the
structure for which
$\Fop$ is an iteration strategy. If $\Tt,\Uu$ are trees on $\MFsharp$, and
``$\pi:\Tt\to\Uu$'' is a hull embedding, and $\Tt$ has length $\lambda+1$ for a
limit $\lambda$, and $[0,\lambda]_\Tt$ drops, then $\pi$ induces a weak
$0$-embedding $M^\Tt_\lambda\to M^\Uu_{\gamma}$, where
``$\gamma=\pi(\lambda)$''. So by \ref{StrategyCondensation}, $M^\Tt_\lambda$ 
is a
$\Fop$-premouse over $a$. But since $[0,\lambda]_\Tt$ drops, it 
follows
that $[0,\lambda]_\Tt=\Sigma(\Tt\rest\lambda)$.
\end{comment}
\begin{comment}
\begin{definition}[Whole]\label{dfn:whole_strategy}
Let $\M$ be a $\P$-strategy-premouse of type $\varphi$. We say 
$\M$
is \textbf{$\varphi$-branch-whole} (or just \textbf{branch-whole} if $\varphi$ 
is fixed) iff
for every $\eta<\l(\M)$, if
$\Tt_{\eta}\neq\emptyset$ and $\Tt_\eta\neq\Tt_{\eta'}$ for all
$\eta'<\eta$, then for some $b$,
$\BBB(\M|\eta,\Tt_{\eta},b)\ins\M$.\footnote{\emph{$\varphi$-whole} depends on
$\varphi$ as the definition of $\Tt_\eta$ does.}
\end{definition}

\begin{definition}[Potential $\Sigma$-premouse]\label{dfn:pot_Sigma_pm}
Let $\Sigma$ be a (partial) iteration strategy for a transitive
structure $\P$.
A \textbf{potential $\Sigma$-premouse (over $a$, of type $\varphi$)}
is a
potential
$\P$-strategy premouse $\M$ (over $a$, of type $\varphi$) such that
$\Sigma^\M\sub\Sigma$.\footnote{If $\M$ is a model all of whose proper segments
are potential $\Sigma$-premice, and the rules for potential $\P$-strategy
premice
require that $B^\M$ code a $\Tt$-cofinal branch, but $\Sigma(\Tt)$ is not
defined,
then $\M$ is not a potential $\Sigma$-premouse, whatever its predicates are.}
\end{definition}
\end{comment}

% scales_g_organized.tex

\begin{comment}
\begin{lemma}
 Let $\N,\delta$, etc, be as in \ref{dfn:determines}, except that we allow
$\N$ to be the last model of a tree $\Tt$ on $\MFsharp$ via $\Sigma_\MFsharp$, 
with $\Tt$
of any length. Then $(\N|\gamma)[g]$ is closed under $\Omega_\Fop$ 
and letting $\Omega'$ be the interpretation of $\Psi$ over $(\N|\gamma)[g]$,
$\Omega'\rest C=\Omega_\Fop\rest(\N|\gamma)[g]$.\end{lemma}

\begin{proof}
Suppose not. Let $x\in(\N|\gamma)[g]$ be a counterexample to the claimed
agreement between $\Omega_\Fop,\Omega'$. Let
$\alpha$ be large and let $X\elem V_\alpha$ be countable, with
$x,\Sigma_\MFsharp$, etc, in $X$. Let $\pi:M\to X$ be the uncollapse. Write
$\pi(\Ttbar)=\Tt$, etc. By \ref{lem:Sigma_N_condensation}, $\Ttbar$ is via
$\Sigma_\MFsharp$. We have $x\in C$ by hypothesis, and therefore $\xbar\in C$ 
(by suitability), so by 
\ref{dfn:determines}, $\xbar\in\dom(\Omega_\Fop)$ and
$\Omega_\Fop(\xbar)=\overline{\Omega'}(\xbar)\in\overline{(\N|\gamma)[g]}$. So 
$x\in\dom(\Omega')$,
and so $\Omega'(x)\neq\G_\Fop(x)$, by choice of $x$. 
Therefore $\overline{\G'(x)}\neq\overline{\G_\Fop(x)}$, 
contradicting 
the fact that $\overline{\G_\Fop(x)}=\G_\Fop(\xbar)$, which holds by 
suitability.\end{proof}
\end{comment}
\begin{comment}
By suitability, 
$G(x)$ is determined by its theory $t$ over parameters in $\hat{x}$, and
$G'(x)$ is determined by its theory $t'$ in such 
parameters (the latter is forced). So let $\varphi$ be some formula and 
$z\in\hat{x}^{<\om}$ such that $\varphi(z)\in t$ but $\neg\varphi(z)\in t'$. 
Fixing a $\PP$-name $\dot{t'}$ for $t'$, we may assume that 
$z,\dot{t'}\in\rg(\pi)$ and that $\PP$ forces that 
$\neg\varphi(\check{z})\in\dot{t'}$. So with $H^*$, etc, as above, 
$G^*(\xbar)\neq\overline{G(x)}$.
Therefore by line (\ref{eqn:agmt_G}), $\overline{G(x)}\neq G(\xbar)$. This easily 
implies that we are in the first case of suitability (so in particular $G=\Fop$). 
\end{comment}
\begin{comment}
Therefore $\PP$ forces that $G'(x)\down y \sats$``I have an element $\R$ such 
that $x\in\R$ and Th$^\R(x) = t$ and $\varphi(\hat{z})\in t$". Reflecting this to $M$, 
$G^*(\xbar)\in G(\xbar)$, contradiction.
\end{comment}

\begin{comment}
Below, for an operator $\Fop$, an ordinal $\alpha$, an $x\in \dom(\Fop)$, $\Fop_\alpha(x)$ is the 
opm defined inductively as follows: $\Fop_1(x) = \Fop(x)$; if $\Fop_{\beta}(x)$ has been defined 
for 
$\beta<\alpha$, then $\Fop_{\beta+1}(x) = \Fop(\Fop_\beta(x))$; if $\beta\leq \alpha$ is limit and 
$\Fop_\gamma(x)$ has been defined for all $\gamma<\beta$ then $\Fop_\beta(x)$ is the unique opm 
$\M$ 
such that $l(\M)=\beta$, $\dot{E}^\M=\dot{P}^\M=\emptyset$ and $\N\pins \M$ iff $\N=\Fop_\gamma(x)$ 
for some $\gamma<\beta$. 
\end{comment}
\begin{comment}
as witnessed by $\W_\N, \Yy_\N$. Let 
$\T=\T_\N$, 
$\lambda^\Tt_{\Phi_0}$ 
etc. (cf. Definition \ref{dfn:P^Phi}) and for each initial segment $\U$ of $\T$ of limit length, 
let 
$\R_\U,\mathcal{S}_\U,\gamma_\U$ be defined as above. We have $\MFsharp^\Tt_{\Phi_0}\pins 
M^\Tt_\lambda\in 
\mathcal{Y}_\N$. In fact, $\{\MFsharp^\Tt_{\Phi_0}\}$
is $\Sigma_1^{\mathcal{Y}_\N}(\Ll^-;\{\N\})$, uniformly in $\N$.
\end{comment}
\begin{comment}
Likewise, in item \ref{item_2} of the definition of $\varphi_{\rm{g}}$, $\tau$ 
exists. Also, for $\Mbar\ins\mathcal{Y}_\N$ such that $\N\ins\Mbar$, the sequences
$\left<\R_{\T\rest\alpha}\right>_{\alpha\in I_{\Phi_0}^\Tt}\inter\Mbar$ and
$\left<\mathcal{S}_{\T\rest\alpha}\right>_{\alpha\in I_{\Phi_0}^\Tt}\inter\Mbar$ and
$\left<\Tt\rest\alpha\right>_{\alpha\leq\lambda+1}\inter\Mbar$ are
$\Sigma_1^{\Mbar}(\Ll^-;\{\N\})$, uniformly in $\N$ and $\Mbar$.

$^{g,*}\Fop$ is a pre-operator. To see this, it suffices to see that every initial 
segment of ${^{\g,*}\Fop}(b)$ is (weakly $\omega$-)sound; the other clauses are easier. By the 
above 
remarks, 
there is a $\Sigma_1$ formula $\psi$ of 
$\Ll_\J\backslash \{\dot{P}\}$, such that ${^{\g,*}\Fop}(b)\sats\neg\psi$, and for any 
$\J$-structure 
$\N$ such that whenever $\alpha<\iota$, $\M|\gamma_\alpha\ins \N$ ($\M|\eta_\alpha\ins \N$) then 
either $\M|\eta_{\alpha+1}\ins\N$ or $\N\ins \M|\eta_{\alpha+1}$ ($\N\ins \M|\gamma_{\alpha+1}$ or 
$\M|\gamma_{\alpha+1}\ins \N$), $\N$ is an acceptable initial segment of ${^{\g,*}\Fop}(b)$ iff 
$\N\sats\neg\psi$. 
(Here $\psi$ asserts that ``some proper segment has the form of 
${^{\g,*}\Fop}(b)$''.) But therefore if 
$\N$ is such, then $\N$ is sound, by \ref{lem:Sigma_N_condensation} and 
\ref{StrategyCondensation} and the proof that initial segments of $\N$ are 
sound.
\end{comment}
\begin{comment}for some $\M'\pins 
\M$, letting $\T=\T_\N$, $\lambda=\lambda_{\Phi_0}^{\T}$, $\lambda'$ be the least limit ordinal 
$\leq \lambda$, $\M'=\mathcal{S}_{\T\rest{\lambda'}}$ 
and 
$\J^{\hpm}_\tau(\M')\ins\M$ where $\tau$ is the least such that 
$\T\rest(\lambda+1)\in\J_{l(\M')+\tau}(\M')$ and $\tau>\OR(M^\Tt_\lambda)$. 

We let $\W_\N = \M'$ and $\mathcal{Y}_{\N}=\J^{\hpm}_\tau(\M')$. Also let $\mathcal{Y}^*_\N$ be the 
least $\N\ins \mathcal{Y}\ins \mathcal{Y}_\N$ such that $\mathcal{Y} \vDash ``\Theta$ does not 
exist" if such a $\mathcal{Y}$ exists; otherwise, $\mathcal{Y}^*_\N = \mathcal{Y}_\N$.
\end{comment}
\begin{comment}
$\M_\alpha\pins \P\pins\M$ such that $\P\vDash \sf{ZF}^-$ and letting $\T=\T_{\N_{\alpha+1}}, 
\lambda$ be the least limit ordinal $\leq \lambda^\T_{\Phi_0}$, 
$\M_{\alpha+1}=\J_\tau^{\hpm}(\mathcal{S}_{\T\rest\lambda})$ where for some $\eta_\alpha$, 
$\mathcal{S}_{\T\rest\lambda}=\BBB(\M|\eta_\alpha,\T\rest\lambda,\Sigma^\M(\T\rest\lambda)) = 
\M|(\eta_{\alpha+1})$,  
$\tau$ is least such that $\delta(\T\rest (\lambda+1))<\tau$ and $\T\rest (\lambda^\T_{\Phi_0}+1) 
\in 
\J_\tau(\mathcal{S}_{\T\rest\lambda})$. $\N$ is the least $\P\pins \M$ such that $\P\vDash 
\sf{ZF}^-$ and $\forall \alpha<\gamma \ \M_\alpha \ins \P$.\qedhere
\end{comment}
\begin{comment}
\begin{enumerate}[label=\tu{(}\alph*\tu{)}]
\item \label{item_a} For every strict initial segment $\U$ of $\T$ of limit length, there are 
$\R,\Ss$ such that $\N \pins \R\pins\Ss\pins \M$ and
$\Ss=\BBB(\R,\U,b)$ for $b=\Lambda_\MFsharp(\U)$. We write
$\R_\Uu=\R$, $\gamma_\Uu=\OR(\R)$ and $\Ss_\Uu=\Ss$.
 

\item\label{item_b} For $\U,\W$ initial segments of $\T$ of limit length such that lh$(\W) = 
\rm{lh}(\U)+\omega$, letting $\R_\U,\gamma_\U,\mathcal{S}_\U$ be defined for $\U$ as in the 
previous 
line, then we define $\tau_\W$ to be the least $\tau$ such that $\W\in \J_\tau(\mathcal{S}_\U)$, 
$\J^{\hpm}_\tau(\mathcal{S}_\U) \ins \M$, and if lh$(\W)>o(\N)$, then 
$\delta(\W)<\tau$.\footnote{The existence of $\tau$ is explained in Remark 
\ref{rem:local_def_P^varphi}.} Letting $\xi$ be such that $\M|\xi=  
\J^{\hpm}_\tau(\mathcal{S}_\U)$, 
then either $\M|\xi = \M$ (in which case $\W=\T$ and $\R_\W=\M$), or else $\R_\W=\M|\xi\pins \M$ 
and 
either $\mathcal{S}_\W=\BBB(\R_\W,\W,\Lambda_{\MFsharp}(\W))\ins \M$ (in which case lh$(\W) < 
$lh$(\T)$) or $\M\pins  \BBB(\R_\W,\W,\Lambda_{\MFsharp}(\W))$ (in which case $\W = \T$).


%\begin{comment}
%or there is $0<k\in\omega$ such that for every $i < k$, $\M|(\xi+i+1)$ is the least strict initial 
segment $\mathcal{S}$ of $\BBB(\M|(\xi+i), \W, \Lambda_{\MFsharp}(\W))$\footnote{Similarly to the 
previous footnote, $\mathcal{S}$ is an opm coding the appropriate $\J$-initial segment of 
$\BBB(\M|(\xi+1), \W, \Lambda_{\MFsharp}(\W))$.} such that 
$\rho_\omega(\mathcal{S})<\rho_\omega(\M|(\xi+i))$, and either $\R_\W=\M|(\xi+k)\pins \M$ (so 
$\mathcal{S}_\W=\M|(\xi+k+1)\ins\M$) or $\M=\M|(\xi+k)$ (in which case $\W=\T$). 


\item \label{item_c} Letting $\lambda' = \sup_{\xi<\rm{lh}(\T)} \gamma_{\T\rest\xi}$, then 
$\lambda' 
< l(\M)$ and $\J^{\hpm}_\tau(\M|\lambda')\ins \M \ins \BBB(\J^{\hpm}_\tau(\M|\lambda'), \T, 
\Lambda_\MFsharp(\T))$ where $\tau$ is least such that $\T\in \J_\tau(\M|\lambda)$ and if 
lh$(\T)>o(\N)$ then $\delta(\T)<\tau$.
\end{enumerate}

 
 
%\begin{comment}
%or else, letting $\M|\xi = \J^{\hpm}_\tau(\M|\lambda)$ and let $k$ be defined as above but for 
$\M|\xi, \T$, then $\M = \M|(\xi+k)$.


%footnote
\footnote{G-organized premice identify 
$\MFsharp$ explicitly. For our intended application, i.e. the analysis of scales in 
$\Lp^{^\gTheta\Fop}(\RR,\Fop\rest\HC)$, this is not of importance, because anyway, $\M_1^{\Fop,\#}$ 
is analytical in $\Fop\rest\HC$. However, it seems that one might want to consider a 
hierarchy of premice $\M$ over $\RR$, similar to $\Lp^{^\g\Fop}(\RR)$, but in which $\MFsharp$ is 
not identified explicitly. It seems we might have achieved this by, in some initial segment of 
$\M$, feeding in $\Fop(X)$ for enough sets $X\in\hod^\M$, until $\MFsharp$ can be identified, as 
in the following sketch. Suppose we have defined $\M|\alpha$; let 
$\tilde{\Fop}=\Fop^{\M|\alpha}$ be the 
partial operator which is computed naturally from the fragment of $\Fop$ already fed in to 
$\M|\alpha$. Working in $\M|\alpha$,
let $\tilde{Q}$ be the function defined as follows. Let $H$ be a transitive
set. Suppose there is $\gamma\in\Ord$ such that $Q=\J_\gamma^{\tilde{\Fop}}(H)$ 
is defined (i.e., $\tilde{\Fop}$ computes this), and $Q$ is a
Q-structure for $H$. Then set $\tilde{Q}(H)=Q$. Otherwise $\tilde{Q}(H)$ is
undefined. Over $\M|\alpha$, consider the set $\MFsharp^{\M_\alpha}$ of countable 
\emph{$\M_1^{\Fop,\#}$-like} $\J$-models $\N$ which are \emph{$\tilde{\Fop}$-consistently 
$\tilde{Q}$-short tree iterable}; we omit any precise definitions of these notions. Then 
$\MFsharp\in\MFsharp^{\M|\alpha}$, and $\tilde{Q}$-guided trees on $\MFsharp$ will be via 
$\Lambda_\MFsharp$. Over $\M|\beta$ for $\beta\geq\alpha$, attempt to compare all such $\N$, and 
simultaneously iterate to make $\M|\alpha$ generically generic. If at some stage the least 
disagreement, between say $\N_1$ and $\N_2$, is due to the fact that say 
$\Fop^{\N_1}(x)\neq\Fop^{\N_2}(x)$, then we can feed in $\Fop(x)$ over some later $\M|\gamma$. Then 
if $\N_i$ is an iterate of $\M_i$, we will have $\{\M_1,\M_2\}\not\sub\MFsharp^{\M|\gamma}$, and 
we start over with $\gamma$ replacing $\alpha$. If we reach a $\tilde{Q}$-maximal stage 
of the comparison, which is in fact not maximal (for $\MFsharp$) then we can feed in the 
corresponding Q-structure. This process will eventually produce an iterate of $\MFsharp$ over which 
$\RR$ is generic, and therefore, over which $\Fop\rest\HC$ and $\MFsharp$ are definable.}
%end footnote


First let $\mathcal{G} = \J^{\op}_{\MFsharp}$.

For each $\alpha\leq\l(\M)$, $E^{\M|\alpha}=\emptyset$.

Let $\alpha_0$ be the least $\alpha$ such that $\J_\alpha(b)\sats\ZF$. Then 
$\M|\alpha_0=\mathcal{G}_{\alpha_0}(b)$.

Let $\Tt=\Tt_{\M|\alpha_0}$.
We use the notation $P^\Phi=P^\Phi(\Tt)$, $\lambda=\lambda^\Phi(\Tt)$, etc, 
as in \ref{dfn:P^Phi}.
The predicates
$P^{\M|\gamma}$ for $\alpha_0<\gamma\leq\l(\M)$ will be used to feed in branches
for $\Tt\rest\lambda+1$, and therefore $P^\Phi$ itself, into $\M$. Let 
$\left<\xi_\alpha\right>_{\alpha<\iota}$ enumerate 
$I^\Phi\un\{0\}$.

There is a closed, increasing sequence of ordinals
$\left<\eta_\alpha\right>_{\alpha\leq\iota}$ and an increasing sequence of
ordinals $\left<\gamma_\alpha\right>_{\alpha\leq\iota}$ such that:

\begin{enumerate}
 \item $\eta_1=\gamma_0=\eta_0=\alpha_0$.
 \item For each $\alpha<\iota$, 
$\eta_\alpha\leq\gamma_\alpha\leq\eta_{\alpha+1}$, and if
$\alpha>0$ then $\gamma_\alpha<\eta_{\alpha+1}$.
 \item $\gamma_\iota=\l(\M)$, so $\M=\M|\gamma_\iota$.
 \item\label{item:gamma_alpha} Let $\alpha\in(0,\iota)$. Then $\gamma_\alpha$ 
is the least ordinal of
the form $\eta_\alpha+\tau$ such that
$\Tt\rest\xi_\alpha\in\J_\tau(\M|\eta_\alpha)$ and if 
$\alpha>\alpha_0$ then
$\delta(\Tt\rest\xi_\alpha)<\tau$. (We explain in the remark below why such $\tau$ 
exists.) And $\M|\gamma_\alpha= \mathcal{G}_\tau(\M|\eta_\alpha)$.
 \item Let $\alpha\in(0,\iota)$. Then
$\M|\eta_{\alpha+1}=\BBB_+(\M|\gamma_\alpha,\Tt\rest\xi_\alpha,
\Lambda(\Tt\rest\xi_\alpha))$.
 \item Let $\alpha<\iota$ be a limit. Then $\M|\eta_\alpha$ is passive.
 \item $\gamma_\iota$ is the least ordinal of the form $\eta_\iota+\tau$ such
that $\Tt\rest\lambda+1\in\J_{\eta_\iota+\tau}(\M|\eta_\iota)$ and
$\tau>\OR(M^\Tt_\lambda)$; with this $\tau$, $\M=\mathcal{G}_\tau(\M|\eta_\iota)$.
\end{enumerate}
%Finally, we let $^\g\Fop = \Fop_{^{\g,*}\Fop}$.
\end{comment}

\begin{comment}
\begin{definition}[${^\g\Omega}$]\label{dfn:gF}
\label{modelOpGenerala2}
We define $^\g\Omega$ to be the operator $\F_G$ where $G = G_{\Lambda_\MFsharp,\varphi_{\rm{g}}}$.
\qedhere\end{definition}
\end{comment}
\begin{comment}
\begin{definition}
\label{PotJPremice2}
Let $b$ be transitive with $\MFsharp\in\J_1(\hat{b})$.
A \textbf{potential g-organized $\Fop$-premouse over $b$}
is a potential ${^\g\Fop}$-premouse over 
$b$, with parameter $\MFsharp$.
\end{definition}

Note that because we only feed in branches for non-maximal trees on 
$\MFsharp$, the only non-extender information being fed into a g-organized 
$\Fop$-premouse can be computed by $\Fop$-construction. The following lemma is an easy corollary to 
\ref{rem:local_def_P^varphi}.

\begin{lemma}\label{lem:varphi_g}
There is a formula 
$\varphi_\g$ in $\Ll_0$, such that for any transitive $b$ with 
$\MFsharp\in\J_1(\hat{b})$, and any
$\J$-structure $\M$ over $b$, $\M$ is a potential 
g-organized $\Fop$-premouse over $b$ iff $\M$ is a potential 
$\Lambda_\MFsharp$-premouse over $b$, of type $\varphi_\g$.
\end{lemma}
\end{comment}
\begin{comment}
 \footnote{***Correct this footnote (uses old 
language): One can prove the 
same conclusion given instead that $\pi$ is a
weak $0$-embedding with respect to the full language $\Ll_0$ (i.e.,
$\Sigma_0$-elementary, and $\Sigma_1$-elementary on a cofinal set $X$, with
respect to $\Ll_0$). For it is easy enough to see
that every proper segment of $\Mbar$ is an $\Fop$-premouse over $\bbar$. The 
main
issue is to see that $B^{\Mbar}$ is correct. The elementarity of $\pi$ with
respect to the symbol $\l$ gives that $\Mbar$ and $\M$ either (a) both have
successor length, or (b) both have limit length. Suppose (b) holds. Then $\M$
is not whole, so we just need to see that $\Mbar$ is an $\Fop$-premouse over
$\bbar$. If $\Mbar$ is a limit of proper segments $\Mbar'$ such that
$B^{\Mbar'}=\emptyset$ then $B^{\Mbar}=\emptyset$, since $\pi``B^{\Mbar}\sub
B^\M$
and if $\gamma\in B^\M$ and $\M'\pins\M$ and $\gamma\in\M'$ then
$B^{\M'}\neq\emptyset$; this is just because $\M$ is an $\Fop$-premouse over 
$b$. It
follows that $\Mbar$ is an $\Fop$-premouse over $\bbar$, as required. Now 
suppose
(a) holds. Let $\Mbar'$ and $\M'$ be the largest proper segments of $\Mbar$
and $\M$ respectively. By the elementarity of $\pi$, $\pi(\Mbar')=\M'$, and
$\pi\rest\Mbar':\Mbar'\to\M'$ is fully elementary. Case (a) is easy enough
using \ref{lem:Bcondensation}.}


\begin{definition}\label{dfn:whole_reorganized}
Let $\M$ be a g-organized $\Fop$-premouse over $b$. We say $\M$ is 
\textbf{$\Fop$-closed} iff $\M$ is a limit 
of ${^\g\Fop}$-whole proper segments.
\end{definition}
\end{comment}
\begin{comment}
***Don't need this definition here; move it later. Recall that $(\Omega,a)$ is nice.
We write $\Omega^*$ for the coding of $\Omega\rest\HC$ over 
$\RR$, in the above codes.\footnote{In 
particular, $\Omega^*$ is a partial function $\RR\to\RR$.}
 We say that $(\Omega,a)$ is \textbf{extra nice} iff 
there are scales on $\Omega^*$ and 
$\RR\cut\Omega^*$ which are projective 
in $\Omega^*$.
\end{comment}
\begin{comment}
\begin{definition}[$\varphi_{\mathrm{G}}$]\label{dfn:varphi_G}
Let $\M$ be an aspm. Let $x\in \M$.
$\M\vDash \varphi_{\rm{G}}(x)$ iff the following hold 
\begin{itemize}[label=--]
\item There is $\N\pins \M$ such that $\N\vDash \sf{ZF}^-$ and $x$ is a limit length initial segment 
$\Tt$ of 
$\T_\N\rest(\lambda^{\T_\N}_{\Phi_0}+1)$ according to $\Sigma^\M$. 
\item $\Theta$ exists.
\item Using the notation of Definition \ref{dfn:g_whole}, let $(\N_\alpha:\alpha<\gamma)$ and 
$(\M_\alpha: \alpha<\gamma)$ be sequences 
of strict segments of $\N$ defined (inductively) as follows. Let $\M_{-1}=\M|1$. $\N_0$ is the least 
$\P\pins\M$ such 
that $\P\vDash \sf{ZF}^-$; suppose $\alpha+1<\gamma$ ($\alpha\geq -1$), then $\N_{\alpha+1}$ is the 
least 
$\M_\alpha\pins \P\pins\M$ such that $\P\vDash \sf{ZF}^-$ and $\M_{\alpha+1} = 
\mathcal{Y}^*_{\N_{\alpha+1}}$. $\N$ is the least $\P\pins \M$ such that $\P\vDash 
\sf{ZF}^-$ and $\forall \alpha<\gamma \ \M_\alpha \ins \P$.

\qedhere
\end{itemize}
\end{definition}
\begin{remark}
With the notation as in \ref{dfn:varphi_g} and \ref{dfn:varphi_G}, $\varphi_{\mathrm{G}}$ is, for 
the most part $\varphi_\g$, except that it terminates the process of feeding in branches of initial 
segments of $\T_\N\rest (\lambda+1)$ at $\mathcal{Y}^*_\N$. The next tree activation level of $\M$ 
if exists, is the least $\R$ such that $\mathcal{Y}^*_\N\pins \R\pins\M$ and $\R\vDash 
\ZF^-$.

\end{remark}
\end{comment}
\begin{comment}
We prove the ``moreover'' clause, using the equivalence of (i) and (iii) in 
\ref{lem:charac_Tg-org}. Let 
$\pi:\R\to\M$ be a very weak $0$-embedding as in Definition \ref{dfn:very_condensing} where $\M$ is 
a $\Theta$-g-organized 
$\Fop$-premouse. Because of the elementarity of $\pi$ with respect to $\dot{cb}$, $\R|1$ is a 
$\Theta$-g-organized premouse. If $\R$ is active then $\M$ is active, so $\M\sats$``$\Theta$ 
exists'' and $(\dot{P}^\M\cup \dot{E}^\M)\inter\M|\Theta^\M=\emptyset$, so $\Theta^\M\in\rg(\pi)$ 
and 
$\pi(\Theta^\R)=\Theta^\M$. So if $\R\sats$``$\Theta$ does not exist'' then $\R$ is passive. 
If $\R\sats$``$\Theta$ exists'' then $\M\sats$``$\Theta$ exists'' and 
$\pi(\Theta^\R)=\Theta^\M$, and letting $X$ witness that $\pi$ is a very weak 
$0$-embedding, we may assume that $\R|\Theta^\R\in X$. Therefore $\pi:\R'\to\M'$ 
is a very weak $0$-embedding, where $\R'=\R\down(\R|\Theta^\R)$ and 
$\M'=\M\down(\M|\Theta^\M)$. So by \ref{lem:gF_props}, 
$\R'$ is a g-organized $\Fop$-premouse.
\end{comment}
\begin{comment}
\begin{corollary}\label{cor:Tg_pullback}
 Let $\M$ be an $n$-sound $\Theta$-g-organized $\Fop$-premouse and let $\pi:\R\to\M$ be a weak 
$n$-embedding. If $\M$ is ${^\gTheta\Fop}$-iterable then so is $\R$.
\end{corollary}
\begin{definition}[$\Fop$-mouse]
\label{JMouse}
Let $\MFsharp, b$ be as in Definition \ref{PotJPremice2}\footnote{If $\Fop$ is 
a 
first order mouse operator that is defined on a cone above $a$, then we also 
assume $a\subseteq b$.}. We say that $\M$ is a \textbf{g-organized $\Fop$-mouse}
(or a \textbf{g-organized $\Fop$-mouse over $b$}) if $\rho_{\omega}(\M) =
b$ and whenever $\M^*$ is a countable
transitive g-organized $\Fop$-premouse over some $b^*$ and there is an 
elementary embedding
$\pi: \M^*\rightarrow \M$ such that $\pi(b^*) = b$  and
$\pi(\MFsharp)=\MFsharp$, then $\M^*$ is
$(\om,\omega_1+1)$-iterable (as a g-organized $\Fop$-mouse).
\end{definition}

\begin{definition}
Suppose $\Fop$ is a nice operator and is an iteration strategy. We define 
$\Lp^{^\g\Fop}(\mathbb{R})$ as the stack of all g-organized $\Fop$-mice $\N$ 
over  
$H_{\om_1}$. We also say (g-organized) $\Fop$-premouse \textbf{over 
$\mathbb{R}$} to in fact
mean over $H_{\omega_1}$.\end{definition}
\end{comment}

% scales_weak_gap_below.tex
\begin{comment}
In Case \ref{case:M_not_relevant}, argue as in \cite{Scalesendgap}.
Let $\theta^\N=\Theta^\N$ if $\N\sats$``$\Theta$ exists'', and otherwise let 
$\theta^\N=\l(\N)$. Note that 
$\N|\theta^\N\ins\M$, because of iterability and the soundness of all proper 
segments of $\N|\theta^\N$. But either $\N=\N|\theta^\N$ or 
$\N=\Jop_\lambda(\N|\theta^\N)\down\HC^\M$ for some $\lambda$. Since $\N$ 
is minimal realizing $\Sigma$, it follows that $\N=\M$, and now the usual 
argument gives that $\pi=\id$.
\end{comment}
\begin{comment}
A corollary of the proof of Theorem \ref{gapInTheMouse} is the following
theorem.***I think there's a problem with this theorem, in the case that there is some extender on 
the $\M$-sequence which is $\M$-total***
\begin{theorem}
\label{GapPassiveMouse}
Let $\M$ be a $\Theta$-g-organized $\Fop$-mouse and let $[\alpha,\beta]$ be a weak gap
of $\M$. Suppose $\M\sats\AD$. Suppose either $\Theta^\M$ doesn't exist in $\M$ or 
$\sup\{ \gamma < l(\M) \ 
| \
\M|\gamma \textrm{ is active}\} < l(\M)$. Letting $n$ be least such that
$\rho_n(\M|\beta)=\mathbb{R}^\M$, then $\M \vDash
``\bfrSigma_n^{\M|\beta}$ has the scale property". 
\end{theorem}
\begin{proof}[Sketch]
Note that $\beta$ could be $l(\M)$; we assume this. The proof of this theorem follows from that
of Theorem \ref{gapInTheMouse} without significant changes. The point worth
mentioning is the following. Using the notation of the proof of \cite[Theorem 4.16]{ScalesK(R)} and 
Theorem \ref{gapInTheMouse}, the condition (v) in the definition of $x$-honest becomes
\\
\noindent (v') \indent if $\sigma_0,\dots, \sigma_n$ enumerates those
$B_0$-formulae $\sigma$ of one free variable such that $n(\sigma)\in
\textrm{dom}(u)$ and 
\begin{center}
$(\M,I_u) \vDash i v \sigma(v) \in \textrm{OR}$,
\end{center}  
and if $\delta_m < l(\M)$ is such that 
\begin{center}
$(\M,I_u) \vDash i v \sigma_m(v) = \delta_m$,
\end{center}  
for all $m\leq n$, then the map $\pi(\delta_m)= \eta_{n(\sigma_m)}$ for $m\leq
n$ is well-defined and for each $k<\omega$, $\pi$ is extendable to an
order-preserving map $\pi_k:o(\M^\restpred_{\beta_k}) \rightarrow o(\M^\restpred_{\beta_k})$ such 
that
\begin{center}
$\M^\restpred_{\beta_k} \vDash \theta[\gamma,w_1,w_2] \Leftrightarrow
\M^\restpred_{\beta_k} \vDash \theta[\pi_k(\gamma),w_1,w_2]$.
\end{center}

Note then that determinacy of $\M$ is enough to compute this aspect of
honesty. The rest of the proof is the same as before. 
\end{proof}
\end{comment}

\begin{comment}
Now suppose $\dot{B}^\M\neq \emptyset$. Let $\eta<\beta$
be largest such that $\M|\eta$ is whole. Then 
$\M|\beta\unlhd\mathfrak{B}(\M|\eta,\T,b)$ for some $\T,b$.
Suppose $\M|\beta = 
(\left\lfloor\M|\beta\right\rfloor,\in,\emptyset,B,S,\mathbb{R}^\M)$ for some
$B,S$. We define a sequence $(\beta_i \ | \ i<\omega)$ as in the proof of
\cite[Theorem 4.16]{ScalesK(R)}. Let $\beta_0 = \max\{\eta,
\max\{G\}\}$.
Suppose $\beta_i<\beta$ is defined. For $\gamma<\beta$ let
\[
\R_{\gamma}=(\left\lfloor\M|\gamma\right\rfloor,\in,\emptyset,B\cap\gamma,S^{
\M|\gamma}
,a). \]
Let
\[
Y_i = \{ a \ | \ a \textrm{ is definable over } \R_{\beta_i} \textrm{ from }
\mathbb{R}^\M\cup\{G, \beta_0,\dots,\beta_{i-1}\}\}.
\]
Let $\psi_i$ be the least $\psi\in \Sigma$ such that $\R_{\beta_i} \vDash \neg
\psi[\langle G,w_1\rangle]$. Let 
\begin{center}
$\beta_{i+1}$ = least $\gamma$ such that $\R_\gamma \vDash \psi_i[\langle
G,w_1\rangle]$.
\end{center}
\end{comment}
\begin{comment}
Let $\Sigma = \Sigma_a^{1,\M}$ be a
non-reflecting type, where $a=\langle G, w_1\rangle$ for some real $w_1$ and a
finite set of ordinals $G$. We take $G$ to be $<_\lex$-least.
\end{comment}
\begin{comment}
\begin{proof}[Proof Sketch]
Since the proof is almost the same as that of \cite[Theorem 4.16]{ScalesK(R)},
we only sketch it here, focusing on a new case. There are three main cases:
\begin{enumerate}
\item $\M|\beta$ is passive;
\item $\M|\beta$ is active with $\dot{E}^{\M|\beta}\neq \emptyset$;
\item\label{passive_active_cases_3} $\M|\beta$ is active with
$\dot{B}^{\M|\beta}\neq \emptyset$.
\end{enumerate}
Case \ref{passive_active_cases_3} is new here so we'll focus on it. The other
cases are handled just like
in the proof of \cite[4.16]{ScalesK(R)}. To simplify the notation, we
assume $n=1$. Let $\Sigma = 
\Sigma_a^{1,\M}$ be a
non-reflecting type, where $a=\langle G, w_1\rangle$ for some real $w_1$ and a
finite set of ordinals $G$. We take $G$ to be $<_\lex$-least.

Since $\M|\beta$ is active, $\M|\beta\sats$``$\Theta$ exists''. Let 
$\eta\in[\Theta^{\M|\beta},\beta)$ be largest such that $\M|\eta$ is 
branch-whole. So
$\M|\beta\ins\BBB(\M|\eta,\Tt,b)$ for some $\Tt,b$.
Suppose $\M|\beta = (\lpole\M|\beta\rpole,\in,\emptyset,B,S,\HC^\M,\MFsharp)$ 
for some
$B,S$. We define a sequence $(\beta_i \ | \ i<\omega)$ as in the proof of
\cite[4.16]{ScalesK(R)}. Let $\beta_0 = \max\{\eta,
\max\{G\}\}$.
Suppose $\beta_i<\beta$ is defined. For $\gamma<\beta$ let
\[
\R_{\gamma}=(\lpole\M|\gamma\rpole,\in,\emptyset,B\inter\gamma,S^{\M|\gamma}
,\l^{\M|\gamma},a). \]
Let
\[
Y_i = \{ a \ | \ a \textrm{ is definable over } \R_{\beta_i} \textrm{ from }
\mathbb{R}^\M\cup\{G, \beta_0,\dots,\beta_{i-1}\}\}.
\]
Let $\psi_i$ be the least $\psi\in \Sigma$ such that $\R_{\beta_i} \vDash \neg
\psi[\langle G,w_1\rangle]$. Let 
\begin{center}
$\beta_{i+1}$ = least $\gamma$ such that $\R_\gamma \vDash \psi_i[\langle
G,w_1\rangle]$.
\end{center}
\noindent \textbf{Claim:} $\cup_{i<\omega} Y_i = \M|\beta$. In particular, the
$\beta_i$'s are cofinal in $\beta$.
\begin{proof}
Let $N$ be the transitive collapse of $\cup_{i<\omega} Y_i$ and let $\pi: N
\rightarrow \cup_{i<\omega} Y_i$. Then $N = \mathcal{C}_0(\N)$ for some
$J$-premouse $\N$ over $\mathbb{R}^\M$. This uses that $J$ condenses well. Since
trees on $\N$ can be lifted to trees on $\M$ via $\pi$, $\N$ is $0$-countably
iterable. This implies $\N\lhd \M$. Since $\N$ realizes $\Sigma$, $\N = \M$.
This proves the claim.
\end{proof}
The rest of the proof is just as in the proof of
\cite[Theorem 4.16]{ScalesK(R)}. This completes our sketch of the theorem.
\end{proof}
\end{comment}
\begin{comment}%except for the 
following.
%\begin{IEEEeqnarray*}{ll}
%(7a) & \ \ \text{if } (\iota v \phi(v) < \dot{\beta}_0)\in 
%T_k 
%\text{ then }  \\ 
%& \ \ ``\text{max}(\dot{p})\geq\iota v \phi(v) \vee \ \dot{W}\notin H_1^{\dot{\M}_0}(\iota v 
%\phi(v),\dot{x}_1)"\in T_{m_k}   \\
%(7a) & \ \  \text{If } \psi_i = \exists u \psi'_i \text{ then there is some } \phi \text{ such 
that 
%} ``\psi_i'(\iota v \phi(v), \langle \dot{G},\dot{x}_1 \rangle)^{\dot{\M}_{i+1}}"\in T_{i+1} ;\\ 
%& \ \ \text{ and if } ``\dot{E}^{\dot{\M}_{i+1}}\neq \emptyset" \in T_{i+1} \text{ then } (\dot{E} 
\text{ is total over } H_\omega^{\dot{\M}_i}(\mathbb{R}\cup \{\dot{G},\dot{\beta}_0,\ldots, 
\dot{\beta}_{i-1}\}))^{\dot{\M}_{i+1}} \in T_{i+1};\\
%(7b) & \ \ \text{For any } i, \text{ if } ``\iota v \phi(v) < \dot{\beta}_{i+1}"\in T_k \text{ 
then 
for no } l, (\M^\restpred_{\iota v \phi(v)} \vDash \psi_i[\dot{G},\dot{x}_1])^{\dot{\M}_l}\in 
T_{l+1};\\
%(8) & \ \ \text{Suppose } (\iota v \phi(v) <_b \dot{p})\in T_k \text{. Then } \forall n, ``\iota v 
\phi(v)\in \dot{\M}_n \Rightarrow H_1^{\dot{\M}_n}(\iota v \phi(v),\mathbb{R}^{\dot{\M}_n})\in 
\dot{\M}_{m_k}"\in T_{m_{n}}.
%& \ \ \text{Furthermore, either there is a }\Pi_1\text{ formula }\varphi\in \Sigma\text{ such that 
}(\neg \varphi(\iota v \phi(v), \dot{x_1}))^{\dot{\M}_{m_k}}) \\
%& \ \ \text{or there is a }\Sigma_1\text{ formula } \varphi\text{ which is one of the first } m_k 
\text{ elements of } \Sigma \text{such that}\\
%& \ \  \text{for all } j\text{ and } l, (\varphi(\iota v \phi(v), \dot{x}_1))^{\dot{\M}_l}\notin 
T_j.  
%(2) &\text{``I am a }\J\text{-model''}\\
%(3)_i &\ \dot{x_i} \in \RR\\
%(4)&\ \Phi(\dot{x}_0)
%\wedge \forall \gamma>0\left[\dot{S}_\gamma\nvDash 
%\Phi(\dot{x}_0)\right]\\
%(5)&\ \forall u,v,y,z\left[\sigma_0(u,v,y)\wedge
%\sigma_0(u,v,z) \Rightarrow y = z\right]\\
%(6)_{\varphi} &\ \exists v \varphi(v) \Rightarrow \exists v\exists
%F\in \Ord^{<\omega}\left[\varphi(v) \wedge
%\sigma_0(F,\dot{x}_{m(\varphi)},v)\right]\\
%(7)_\varphi &\ \exists v\left[\varphi(v) \wedge v\in\RR\right]
%\Rightarrow \varphi(\dot{x}_{n(\varphi)}).
%\end{IEEEeqnarray*}
%(7a) and (7b) fix the meaning of $\langle \beta_i \ | \ 1\leq i <\omega\rangle$ and (7a), (7b), 
and 
(8) fix the meaning of $\dot{p}$. 
\end{comment}


==> scales_weak_gap_a_bkp.tex <==
We now proceed to the generalization of \cite[Theorem 0.1]{Scalesweakgap}, the final scale 
construction of the paper. While it uses only the weaker 
determinacy 
assumption, it requires a mouse capturing hypothesis, as in \cite{Scalesweakgap}.

\begin{definition}
Suppose $V$ is an hpm and $\HC$ exists. Let $\Gamma$ be a pointclass of the form 
$\rSigma_1^{V|\alpha}\inter\pow(\RR)$ 
for some $\alpha<\l(V)$. In this setting, for $x\in\RR$, we write $C_\Gamma(x)$ for the set 
of all $y\in\RR$ such that for some ordinal $\gamma<\om_1$, $y$ (as a subset of $\om$) is 
$\Delta_\Gamma(\{\gamma,x\})$.
Let $x\in\HC$ be such that $x$ is transitive and $f:\om\onto x$. Then $c_f\in\RR$ 
denotes the code for $(x,\in)$ determined by $f$.
And $C_\Gamma(x)$ denotes the set of all 
$y\in\pow(x)$ such that for all $f:\om\onto x$ we have $f^{-1}(y)\in 
C_\Gamma(c_f)$.
\end{definition}

\begin{lemma}\label{lem:C_Gamma_characterize} Let $\P$ be a $\Theta$-g-organized $\Omega$-pm 
satisfying $\AD$.
Let $\Q\pins\P$ be such that $\Q$ is passive and admissible. Work in $\P$. Let $\Gamma$ be the 
pointclass $\rSigma_1^\Q\inter\pow(\RR)$. Let $x\in\HC$ with $x$ transitive and infinite. Then 
for all $y\in\HC$, the following are equivalent:
\begin{enumerate}[label=\tu{(}\arabic*\tu{)}]
 \item\label{item:y_in_C_G(x)} $y\in C_\Gamma(x)$,
 \item\label{item:y_OD^alpha(x)} there is $\R\pins\Q$ such that $y$ is definable over 
$\R$ from parameters in $\Ord\un x\un\{x\}$,
 \item\label{item:comeager} for comeager many bijections $f:\om\to x$, $f^{-1}(y)\in 
C_\Gamma(c_f)$.
\end{enumerate}
\end{lemma}
\begin{proof}
 The proof is mostly like that of \cite[Theorem 3.4]{twms}; we just mention a couple of points. 
For $x\in\RR$, the equivalence of \ref{item:y_in_C_G(x)} and \ref{item:y_OD^alpha(x)} follows 
because $\Q\sats\AD+\KP$. Now consider the proof 
that \ref{item:comeager} implies \ref{item:y_OD^alpha(x)}. If $\P$ satisfies 
\ref{item:comeager}, then we may take the witnessing comeager set $C$ to be a 
countable intersection of dense sets, and then $C\in\Q$. So by 
$\KP$ there is $\R\pins\Q$ such that for every $f\in C$, $f^{-1}(y)$ is definable over $\R$ 
from parameters in $\Ord\un\{c_f\}$. As in \cite{twms}, there is then some $\alpha<\om_1^\P$ and 
$n<\om$ and injection $\sigma:n\to x$ such that for comeager many bijections $f:\om\to x$ extending 
$\sigma$, $f^{-1}(y)$ is the $\alpha^\nth$ real which is definable over $\R$ from parameters in 
$\Ord\un\{c_f\}$, in the natural ordering. Letting $\delta=\l(\R)$, this defines $y$ over 
$\Q|(\delta+2)$ from parameters in $\{\delta,x\}\un\rg(\sigma)$.
\end{proof}

\begin{definition}
Let $\P,\Q,\Gamma,x$ be as in \ref{lem:C_Gamma_characterize}.
Suppose that $\MFsharp\in\J(\hat{x})$ and $\Omega^*\in\Q$ where 
$\Omega^*=\Omega\rest\HC^\P$.
Work in $\P$. Then
$\Lp^{\Gamma,{\gOmega^*}}(x)$ denotes 
$(\Lp^{\gOmega^*}(x))^\Q$.\footnote{So $\Q\sats$``$\N$ is $\gOmega^*$-$(\om,\om_1+1)$-iterable''
for all $\N\pins\Lp^{\Gamma,\gOmega^*}(x)$. Note here that $\Q\sats$``$\pow(\om_1)$ exists'' 
because $\Q\sats\AD$.} Similarly for $\Lp_+^{\Gamma,\gOmega^*}(x)$.
We say that \textbf{super-small $\Gamma$-${\gOmega^*}$-mouse capturing
holds on a cone} 
iff there is $z\in\RR$ such that for all transitive $x\in\HC$, if
$\MFsharp,z\in\J(\hat{x})$ then $\Lp^{\Gamma,{\gOmega^*}}(x)$ is 
super-small and
\[ C_\Gamma(x)=\Lp^{\Gamma,{^\g\Omega^*}}(x)\inter\pow(x).\qedhere \]
\end{definition}

\begin{theorem}
\label{weak gap from MC}
Let $\M$ be a $\Theta$-$\g$-organized $\Omega$-pm
satisfying $\AD$. Suppose $[\alpha_0,\l(\M)]$ is a weak gap of $\M$ and $\M$ is countably 
$\gOmega$-$(n,\om_1+1)$-iterable where $n<\om$ is least such that $\rho_{n+1}^\M=\om$. Suppose 
there is a transitive rud-closed 
set $\M_\DC$ such 
that $\M\in\M_\DC$ and $\RR^\M=\RR^{\M_\DC}$ and $\M_\DC\sats\DC_{\RR}$.\footnote{$\M_\DC$
provides a universe in which we can execute certain arguments in the proof of \cite[Theorem 
0.1]{Scalesweakgap} without introducing new reals. The authors believe that \cite[Theorem 
0.1]{Scalesweakgap} should also have adopted a hypothesis along these lines.}
Suppose that $\Omega^*\in\M|\alpha_0$ where $\Omega^*=\Omega\rest\HC^\M$.
In $\M$, let $\Gamma$ be the 
pointclass $\rSigma_1^{\M|\alpha}\inter\pow(\RR)$, and assume that super-small 
$\Gamma$-${\gOmega^*}$-mouse 
capturing holds on a cone. Then
$\M\sats$``$\bfrSigma_{n+1}^\M$ has the scale property''.
\end{theorem}

\begin{proof}
 We follow the proof of \cite{Scalesweakgap}, making some modifications.
 By \ref{thm:self_anal_coded} we may assume that 
$\M\sats$``$\Theta$ exists'' and there is some $\xi+1\in(\Theta^\M,\l(\M))$ such that $\M|\xi\vDash 
\ZF^-$. Therefore $\pow(\RR)\inter\M\in\M|\xi$ and $\M|\xi\sats\ZF^-+\AD$.
We work mostly inside $\M$ or $\M_\DC$, and so we write $\RR=\RR^\M$, $\HC=\HC^\M$, etc.
We have $\Omega^*\in\M|\alpha_0$. Let $z_0\in\RR$ be in the mouse capturing cone, with 
$z_0\geq_T (a_0,t)$ where $t$ codes $\Th_1^{\MFsharp}$ relative to $a_0$, and such that 
$\{\Omega^*\}$ is $\rSigma_1^{\M|\alpha_0}(z_0)$.
Say that $x$ is \emph{high} iff $x\in\HC$, $x$ is transitive and 
$z_0,\MFsharp\in\J(\hat{x})$.
For this proof, except context dictates otherwise, \emph{premouse} 
abbreviates \emph{$\g$-organized $\Omega^*$-pm over $\hat{x}$ for some high $x$}; likewise all 
related 
terminology (such as \emph{iteration tree}, \emph{iterability}, $\Lp$, etc).

Because $[\alpha_0,\l(\M)]$ is a $\Sigma_1$ gap of $\M$,  for high $x$ we have (with terminology as 
just described above)
\[ \Lp^\Gamma(x)=\Lp(x)^{\M|\alpha_0}=\Lp(x)^{\M}.\]
Likewise for $\Lp_+^\Gamma(x)$.

\begin{remark}
Let $\N$ be a $\g$-whole premouse and $\N\pins\Q\ins\Lp^\Gamma_+(\N)$ with $\Q$ projecting to $\N$.
Then $\Q$ translates 
to some $\Q'\pins\Lp^\Gamma(\N)$, where $\OR(\Q')=\OR(\Q)$ and $\Q'$ projects to $\om$, as follows. 
We have $\univ{\Q'}=\univ{\Q}$ and $\hmb^{\Q'}=\hat{\N}$. There is $\alpha>0$ such that 
$\l(\N)+\alpha\leq\l(\Q)$ and for $\beta>\alpha$, $\Q|(\l(\N)+\beta)$ and $\Q'|\beta$ have the 
same active predicates, and for $\beta\in[1,\alpha]$, $\R\eqdef\Q|(\l(\N)+\beta)$ and 
$\R'\eqdef\Q'|\beta$ are both $\hmE$-passive,
and if $\R$ is $\hmP$-active then $\Tt^\R$ is linear, and if $\R'$ is $\hmP$-active then 
$\Tt^{\R'}$ is linear. These are linear iterations at the 
least measurable of $\MFsharp$. Because the iterations are linear, the corresponding predicates are 
trivial, so we can trivially translate between them.\footnote{$\R$ and $\R'$ can
have different predicates, because the definition of spm requires that a particular tree can only 
have a cofinal branch added at at most one segment of the spm. We must have 
$\Sigma^{\Q'|1}=\emptyset$ by definition, but possibly $\Sigma^\N\neq\emptyset$, in which case there 
can be conflict between $\R,\R'$ over which tree should have a branch added. But it is easy to see 
that if $\Q$ is large enough then $\Q$ has a $\g$-closed segment $\R$ such that $\R'$ is also 
$\g$-closed, and beyond which no disagreements arise. (If $\N_0$ is the least $\ZF^-$ level of $\Q$ 
such that $\N\pins\N_0$, and if $\Tt$ is non-linear and via $\Sigma^\N$, then $\Tt$ is not 
making $\N_0$ generically generic, as its linear initial segment is too short. So $\R,\R'$ 
never disagree over non-linear trees.)} It can be that $\Q=\Lp_+^\Gamma(\N)$,
but in this case $\Q$ is not sound, whereas $\Q'$ is sound (recall $\hmb^{\Q'}=\hat{\N})$,
whereas $\hmb^\Q=\hmb^\N$).
\end{remark}

 \begin{comment}
\begin{definition}
 Let $t\in\RR$ and let $\N$ be an $\Fop$-premouse over $t$. We define
$\Lp^{\Fop,\Gamma}_+(\N)$ to be the stack of all $\Fop$-premice such that 
$\N\ins\Q$, $\Q$ projects
$\leq\OR^\N$, and $\Q$ is $(\om,\om_1)$-iterable above $\N$ via a $\Gamma$
strategy.
\end{definition}

Note that in the case that $\N$ above is a strategy premouse,
$\Lp^{\Fop,\Gamma}_+(\N)$ is usually not $\Lp^{\Fop,\Gamma}(\N)$, because
$\Fop^\N\neq\emptyset$ from the perspective of the former, but
$\Fop^\N=\emptyset$ from the perspective of the latter; and also because the
canonical wellorders of mice in the former hierarchy differ from those in the
latter.
\end{comment}

\begin{definition}\label{dfn:k-suitable}
Let $1\leq k\leq\om$. A countable
premouse $\N$ over $A$ is
\emph{$k$-suitable} iff there is a strictly increasing sequence
$\left<\delta_i\right>_{i<k}$ such that
\begin{enumerate}[label=(\alph*)]
 \item For all $\delta\in(\rank(A),\OR(\N))$, we have $\N\sats$``$\delta$ is Woodin'' if and only 
if $\delta=\delta_i$ for some $i<k$.
 \item If $k=\om$ then $\OR(\N)=\sup_{i<\om}\delta_i$, and if $k<\om$ then 
$\OR(\N)=\sup_{i<\om}(\delta_{k-1}^{+i})^\N$.
\item\label{item:cutpoint} If $\N|\eta$ is a  strong 
cutpoint of $\N$ then
$\N|(\eta^+)^\N=\Lp_+^{\Gamma}(\N|\eta)$.
 \item\label{item:Qstructure} Let $\xi\in(\rank(A),\OR(\N))$ be such that $\N\sats$``$\xi$ 
is not Woodin''. Then $C_\Gamma(\N|\xi)\sats$``$\xi$ is not Woodin''.
 \end{enumerate}
We write $\delta^\N_i=\delta_i$ and $\delta_{-1}^\N=0$.
\end{definition}


Let $\N$ be $k$-suitable over $A$ and let $\xi\in(\rank(A),\OR(\N))$ be a limit ordinal 
 such that 
$\N\sats$``$\xi$ isn't Woodin''. Let $\Q\pins\N$ be the Q-structure for 
$\xi$. Let $\alpha$ be such that $\xi=\OR(\N|\alpha)$. Suppose that $\N|\alpha\pins\Q$.
Then $\alpha=\xi$ and $\N|\xi$ is $\g$-closed. In particular, $\N|\xi$ is $\g$-whole,
so $\Lp^\Gamma_+(\N|\xi)$ translates to an initial segment of $\Lp^\Gamma(\N|\xi)$.
Assume that $\N$ is reasonably iterable. If $\xi$ is a strong cutpoint of 
$\Q$, our mouse capturing hypothesis combined 
with \ref{item:Qstructure} therefore gives that $\Q\pins\Lp^{\Gamma}_+(\N|\xi)$. 
Moreover, note that if $\xi$ is a cardinal of $\N$ then $\N|\xi$ \emph{is} a 
strong cutpoint of $\Q$, since $\N$ has only finitely many Woodins. On the other hand, 
if $\xi$ is not a (strong) cutpoint of $\Q$, then one can show that $\Q\notin\Lp_+^\Gamma(\N|\xi)$,
but $\Q$ is coded over $\Lp_+^\Gamma(\N|\xi)$ (here $\Lp_+^\Gamma(\N|\xi)$ translates to a proper 
segment of $\Lp^\Gamma(\N|\xi)$).\footnote{Suppose $\xi$ is not a cutpoint of $\Q$.
Then by definition $\Q\npins\Lp^{\Gamma}_+(\N|\xi)$. Let $E\in\es_+^\Q$ be least overlapping $\xi$ 
and $\kappa=\crit(E)$. Since $\kappa$ is a limit of Woodins in $\Q$, $\kappa$ is not a cardinal of 
$\N$. Let $\P\pins\N$ be least such that $\Q\ins\P$ and $\rho_\om^\P\leq\kappa$,
and let $n<\om$ be such that $\rho_{n+1}^\P\leq\kappa<\rho_n^\P$. We claim that 
$\Lp_+^\Gamma(\N|\xi)=U$ where $U=\Ult_n(\P,E)$ (and note that $U\sats$``$\xi$ is 
Woodin'', but $\Q$ is computable from $U$, as $\Q\ins\P$ and $\P=\core_{n+1}(U)$). For $\xi$ is a 
strong cutpoint of $U$, and $U$ is $\xi$-sound but not fully sound. So it suffices to see that 
there is an above-$\kappa$, $(n,\om_1)$-iteration strategy for $\P$ in $\M|\alpha_0$. Let 
$\R\pins\N$ be least such that $\Q\ins\R$ and $\rho_\om^\R<\kappa$ (so $\P\ins\R$). Note that 
$\kappa$ is a limit of strong cutpoints of $\R$
and of Woodins of $\R$.
Let $\gamma\in(\rho_\om^\R,\kappa)$ be a strong cutpoint of $\R$,
and let $\eta$ be the least Woodin of $\R$ above $\gamma$.
Then $\eta$ is a strong cutpoint of $\R$. Since $C_\Gamma(\N|\eta)\sats$``$\eta$ is not Woodin'',
and by our mouse capturing hypothesis, therefore $\R\pins\Lp_+^\Gamma(\N|\eta)$.
In particular, there is an above-$\eta$ iteration strategy for $\R$ in $\M|\alpha_0$,
which yields the desired strategy.}

\begin{definition}[$\Gamma$-guided] Let $\P$ be
$k$-suitable and $\Tt\in\HC$ be a
normal iteration tree on $\P$. We say $\Tt$ is
\textbf{Q-guided} iff for each limit $\lambda<\lh(\Tt)$,
$\Q=\Q(\Tt\rest\lambda,[0,\lambda]_\Tt)$ exists and 
$\Phi(\Tt\rest\lambda)\conc(\Q,\delta(\Tt))$ is
$(\om,\om_1+1)$-iterable. We say that $\Tt$ is \textbf{$\Gamma$-guided} iff it is 
Q-guided, as witnessed by iteration strategies in $\M|\alpha_0$.\end{definition}

\begin{remark}\label{rem:unique_Q_guided}
Let $\P$ be $k$-suitable. For a normal tree $\Tt$ on $\P$ of limit 
length there is at most one $\Tt$-cofinal branch $b$ such that $\Tt\conc b$ is $\Q$-guided. (Let 
$b_0,b_1$ be distinct such branches; we can successfully compare the phalanxes $\Phi(\Tt\conc b_0)$ 
and $\Phi(\Tt\conc b_1)$. Standard fine structure and the fact that $\P$ has at most $\om$-many 
Woodins then leads to contradiction.) Therefore if $\Tt\conc b$ is normal, via an 
$(\om,\om_1+1)$-iteration 
strategy for $\P$, is based on $[\delta_{i-1}^\P,\delta_i^\P)$ and $\Q(\Tt,b)$ exists, then 
$\Tt\conc b$ is $\Q$-guided.
\end{remark}

\begin{comment}
\begin{lemma} \label{UniquenessOfQStructures}Let
$\P$ be $k$-suitable and let $\Tt$ be a
normal
iteration tree of limit length on $\P$. Suppose $b_0,b_1$ are $\Tt$-cofinal branches and 
$\Q_0,\Q_1$ are such that for each
each $i$, $M(\Tt)\ins \Q_i\ins M^\Tt_{b_i}$, $\rho_\om(\Q_i)\leq\delta=\delta(\Tt)$, 
$\Q_i\sats$``$\delta$ is Woodin'' and
$\Phi(\Tt)\conc Q_i$ is
$(\om,\om_1)$-iterable. Then
either $\Q_0\ins \Q_1$ or $\Q_1\ins \Q_0$.\end{lemma}
\begin{proof}
Suppose not. Compare $\Phi(\Tt\conc b_0)$ with $\Phi(\Tt\conc b_1)$, and use the fact that 
$\P$ has only $\om$-many Woodins, to reach a contradiction.

Let $\Q=\Q_0$. We may 
assume $\delta$ is not a cutpoint of $\Q$. But then the comparis Let
$E\in\es_+(\Q)$ be least such that $\kappa=\crit(E)<\delta$. Let
$\alpha<\lh(\Tt)$ be least such that $\kappa<\nu(E^\Tt_\alpha)$. Let
$\gamma\leq\OR(M^\Tt_\alpha)$ be largest such that $\pow(\kappa)\inter
M^\Tt_\alpha|\gamma=\pow(\kappa)\inter \Q|\lh(E)$. Then:
\begin{enumerate}
 \item Either $[0,\alpha]_\Tt$ drops or $\gamma<\OR(M^\Tt_\alpha)$.
\item $\rho_\om(M^\Tt_\alpha|\gamma)\leq\kappa$ and $M^\Tt_\alpha|\gamma$ is
$\kappa$-sound.
\item $M^\Tt_\alpha|\gamma\sats$``$\kappa$ is a limit of Woodin cardinals and a limit
of cutpoints''.
\item Therefore, $\Tt\rest[\alpha,\lh(\Tt))$ can be considered a normal tree
on $M^\Tt_\alpha|\gamma$, above $\kappa$.
\end{enumerate}
These properties follow from the $k$-suitability of $\P$ and the fact that since
$E$ overlaps $\delta$, $\Q|\lh(E)\sats$``$\kappa$ is a limit of Woodins''.

Let $\Tt'=\Tt\rest[\alpha,\lh(\Tt))$, with
$M^{\Tt'}_\alpha=M^\Tt_\alpha|\gamma$. It follows that a normal tree on
$\Phi(\Tt)\conc\left<\Q_0,\delta\right>$ can be considered a normal tree on
$\Phi(\Tt')\conc\left<\Q_0,\delta\right>$. Likewise for $\Q_1$. The
lemma then follows from comparison and fine structural arguments. Here though,
there is one thing to mention. Because we have not required that
$\Q_0\ins M^\Tt_b$ for some $\Tt$-cofinal branch $b$, we don't know that all
extenders used in $\Uu$ are close to the model to which they apply. Therefore
the theory of \cite{FSIT} doesn't quite give us sufficient fine structural
preservation for this argument. However, we do in fact get enough preservation
in the present context, by \cite{?}.
\end{comment}

\begin{definition}
\label{shortMaximalTrees}
Let $\N$ be a $\g$-whole premouse. We write $\Q^{\Gamma}_\tame(\N)$ 
for the unique $\Q\ins\Lp_+^{\Gamma}(\N)$ such that $\Q$ is a Q-structure for $\N$, if such 
exists.\footnote{The ``$\tame$'' is for \emph{tame}. While $\Q$ might not be tame, $\OR(\N)$ is 
a strong cutpoint of $\Q$.}

Let $k\leq \omega$, $\P$ be $k$-suitable and $\Tt$ a normal, limit length, $\Gamma$-guided tree on 
$\P$. We say that $\T$ is \textbf{short} iff $\Q^\Gamma_\tame(M(\Tt))$ exists; otherwise 
that $\T$ is
\textbf{maximal}.
\end{definition}

\begin{comment}
Note that by Lemma \ref{UniquenessOfQStructures}, if $\T$ is short, then there
is at most one ``good" branch for $\T$ (according to $\M|\beta$). The good
branch is the branch $b$ such
that there is a $\Q\unlhd \M^\T_b$ such that $\Q$ is a $Q$-structure for
$\delta(\T)$ and the phalanx $\Phi(\T)^\smallfrown \langle \Q,\delta(\T) \rangle$
is $(\omega,\omega_1)$-iterable in $\Gamma$. This motivates our next definition.
\end{comment}

\begin{definition}\label{dfn:ss}
Let $\P$ be $k$-suitable. Let $\Tt$ be an iteration tree on $\P$. We say that $\Tt$ is 
\textbf{suitability strict} iff for every $\alpha<\lh(\Tt)$:
\begin{enumerate}[label=(\arabic*)]
 \item If $[0,\alpha]_\Tt$ does not drop then $M^\Tt_\alpha$ is $k$-suitable.
 \item\label{item:ss_drops} If $[0,\alpha]_\Tt$ drops and there are trees 
$\Uu,\Vv$ such that $\Tt\rest\alpha+1=\Uu\conc\Vv$, where 
$\Uu$ has last model $\R$, $b^\Uu$ does not drop, and there is $i\in[0,k)$ such that $\Vv$ is based 
on 
$[\delta_{i-1}^{\R},(\delta_i^{+\om})^{\R})$, then no $\Q\unlhd M^\Tt_\alpha$ is $(i+1)$-suitable.
 \end{enumerate}
 
 Let $\Sigma$ be a (partial) iteration strategy for $\P$. We say that $\Sigma$ is 
\textbf{suitability strict} iff every tree $\Tt$ via $\Sigma$ is suitability strict.
\end{definition}

\begin{definition}\label{shortTreeIterable}
Let $\P$ be $k$-suitable. We say that $\P$ is \textbf{short tree
iterable} iff for every normal $\Gamma$-guided tree $\Tt$ on $\P$, we have:
\begin{enumerate}[label=(\arabic*)]
 \item $\Tt$ is suitability strict.
 \item If $\T$ has limit length and is short then there is $b$ such that $\Tt\conc b$ is a 
$\Gamma$-guided tree.
  \item If $\T$ has successor length then every one-step putative normal extension 
of $\Tt$ is an iteration tree.
\end{enumerate}

Let $\P$ be short tree iterable. The \textbf{short tree strategy} $\Psishort_\P$ for $\P$ is the 
partial 
iteration strategy $\Psi$ for $\P$, such that $\Psi(\Tt)=b$ iff $\Tt$ is 
normal and short and $\Tt\conc b$ is $\Gamma$-guided. (By \ref{rem:unique_Q_guided} this specifies 
$\Psishort_\P$ uniquely.)
\end{definition}

\begin{lemma}\label{lem:short_tree_strat_tracks}Let $\N$ be $k$-suitable.
\begin{enumerate}[label=\tu{(}\arabic*\tu{)}]
\item\label{item:Psi_N_def} The function $\N\mapsto\Psishort_\N$, where $\N$ is short-tree 
iterable, is in $\M$; in fact, $\Psishort_\N$ is $\Gamma(\{\N,z_0\})$-definable, uniformly in 
$\N$.\footnote{But it seems that we might have 
$\Psishort_\N\notin\M|\alpha_0$.}
\item\label{item:full_strat_short_strat} Suppose there is a suitability strict normal 
$(\om,\om_1+1)$-strategy $\Sigma$ for $\N$. Then $\N$ is short tree iterable and 
$\Psishort_\N\sub\Sigma$. Moreover, for any $\Tt$ via $\Sigma$, $\Tt$ is via $\Psishort_\N$ iff for 
every 
limit $\lambda<\lh(\Tt)$, $\Q(\Tt,b)$ exists where $b=[0,\lambda)_\Tt$.
\end{enumerate}
\end{lemma}
\begin{proof}
Part \ref{item:Psi_N_def} follows from the admissibility of $\M|\alpha_0$.

Consider \ref{item:full_strat_short_strat}. Let $\Tt$ on $\N$ be normal, of limit length, via 
both $\Sigma$ and $\Psishort_\N$. Let $b=\Sigma(\Tt)$. It suffices to show that (a) if $\Q(\Tt,b)$ 
exists then $\Tt$ is short, and (b) if $\Tt$ is short then $b=\Psishort_\N(\Tt)$. (Note that if 
$\Q(\Tt,b)$ does not exist then $M^\Tt_b$ is $k$-suitable so $\Tt$ is maximal.)

Consider (a); suppose $\Q=\Q(\Tt,b)$ exists. If $b$ does not drop then $M^\Tt_b$ is suitable 
and $\delta\neq\delta_i(M^\Tt_b)$ for any $i<k$. So $C_\Gamma(M(\Tt))\sats$``$\delta$ is not 
Woodin'', so our mouse capturing hypothesis implies that $\Tt$ is short. So suppose that $b$ drops.
We can't have $C_\Gamma(M(\Tt))\sub\Q$, by suitability strictness. If $\delta$ is a cutpoint of 
$\Q$ (and so a strong cutpoint) we can then compare $\Q$ with $\Lp^\Gamma_+(M(\Tt))$; since the 
comparison is above $\delta$, we get that $\Q\ins\Lp^\Gamma_+(M(\Tt))$, so $\Tt$ is short. So 
suppose 
$\delta$ is not a cutpoint of $\Q$. Let
$E\in\es_+(\Q)$ be least such that $\kappa=\crit(E)<\delta$ and let $\Tt'$ be the normal tree 
given by $\Tt\conc\left<b,E\right>$. Then $M_\infty^{\Tt'}\sats$``$\kappa$ is a limit of Woodins'', 
so 
$b^{\Tt'}$ drops and $C_\Gamma(M(\Tt))\not\sub M_\infty^{\Tt'}$ (by suitability strictness). Also 
$M_\infty^{\Tt'}\sats$``$\delta$ is Woodin'' and $\delta$ is a cutpoint of $M_\infty^{\Tt'}$. So 
$M_\infty^{\Tt'}=\Q^\Gamma_\tame(M(\Tt))$ exists, so $\Tt$ is short.

Consider (b). Since $\Tt$ is short, $\Q=\Q(\Tt,b)$ exists. We claim that 
$\Tt\conc b$ is $\Gamma$-guided, which suffices. For it's easy to reduce to the case that 
$\delta$ is not a cutpoint of $\Q$. Let $\Tt'$ be as above,
let $\lambda=\lh(\Tt)$ and $\alpha=\pred^{\Tt'}(\lambda+1)$. 
Let $M^{*\Tt'}_{\lambda+1}=M^\Tt_\alpha|\gamma$. Then
$M^\Tt_\alpha|\gamma\sats$``$\kappa$ is a limit of cutpoints''. It follows 
that $\Tt\rest[\alpha,\lh(\Tt))$ can be considered an above-$\kappa$, normal tree on 
$M^\Tt_\alpha|\gamma$, and the iterability of the phalanx $\Phi(\Tt)\conc(\Q,\delta)$ reduces to 
the above-$\kappa$ iterability of $M^\Tt_\alpha|\gamma$, which reduces to the 
above-$\delta$ iterability of $M_\infty^{\Tt'}$ (because of the existence of 
$i^{\Tt'}_{\alpha,\lambda+1}$). But $M_\infty^{\Tt'}\ins\Lp_+^\Gamma(M(\Tt))$, so we are done.
\end{proof}

\begin{definition}
Let $A\in\pow(\RR)\inter\M$. We define the phrase $\Tt$ \textbf{respects $A$} as in 
\cite{Scalesweakgap}, except that we also require that $\Tt$ be suitability strict (and making any 
obvious adaptations to our setting). We define $\N$ \textbf{is normally $A$-iterable} as in 
\cite{Scalesweakgap}, except that we also require that $\N$ be short tree iterable. Using these 
definitions, we then define \textbf{(almost, locally) $A$-iterable} as in \cite{Scalesweakgap}.
\end{definition}
\begin{lemma}
\label{Comparisons}
The analogue of \tu{\cite[Lemma 1.9.1]{Scalesweakgap}} holds.
\end{lemma}
\begin{proof}This is mostly an immediate generalization. The proof in \cite{Scalesweakgap} can 
be run inside $\M_\DC$ (in fact, inside $\M$, since $\M\sats\DC_\RR$). Use suitability 
strictness to see that, for example, in the comparison of $\R|0$ with $\N|0$ (notation as in 
\cite{Scalesweakgap}), 
no tree drops on its main branch.\end{proof}
\begin{comment}
Let $\Sigma$ and $\Lambda$ be normal $A$-iteration
strategies of $\P$ and $\Q$ respectively. The restriction of $\Sigma$
($\Lambda$) to short trees witnesses that $\P$ ($\Q$) is short tree iterable.
Also, nondropping $\Sigma$ ($\Lambda$) iterates of $\P$ ($\Q$) are $k$-suitable.
Since we will successively compare
$\P$ and $\Q$ on windows of consecutive Woodin cardinals, we assume $k=1$
without loss of generality. This is just a standard comparison. Let $\T$ and
$\U$ be the comparison trees according to $\Sigma$ and $\Lambda$ respectively.
The only point worth noticing is that there are no drops on the main branches of
$\T$ and $\U$; this follows from the definition of suitability and short-tree
iterability since otherwise, supposing $\T$ drops on the main branch then there
is a dropping iterate of $\P$ (namely the final model $\N^\T$ of $\T$) that
contains a strict initial segment (namely $\N^\U$) which is $1$-suitable; this
contradicts short tree iterability. Also, for each limit $\lambda < $ lh$(\T)$
(similarly for
$\lambda < $ lh$(\U)$), the $Q$-structure $\Q([0,\lambda]_\T,\T\rest \lambda)$
does not have any extender $E$ such that crit$(E) < \delta(\T\rest\lambda) \leq
$ lh$(E)$ since otherwise, the tree $\T$ drops in such a way that we can't undo
the drop; that is, there is some $\alpha<\textrm{lh}(\T)$ and some $\gamma <
o^{\M^\T_\alpha}$ such that $\T\rest [\alpha,\textrm{lh}(\T))$ is a tree based
on $\M^\T_\alpha\rest \gamma$ (this is described in more details in the proof of
Lemma \ref{UniquenessOfQStructures}). But this implies that any cofinal branch
$b$ of $\T$ drops. This contradicts the previous point.
\end{comment}

\begin{remark}
We make a further observation on the comparison above. Let $(\Tt,\Uu)$ be the $\Gamma$-guided 
portion of the comparison of, for example, $(\R|0,\N|0)$. Let $\lambda<\lh(\Tt,\Uu)$ be a limit; 
suppose $\Tt\rest\lambda$ is cofinally non-padded. So $\Q=\Q(\Tt\rest\lambda,[0,\lambda]_\Tt)$ 
exists. Then in fact, $\delta(\Tt\rest\lambda)$ is a strong cutpoint of $\Q$. For otherwise, by
the proof of \ref{lem:short_tree_strat_tracks}, $[0,\lambda]_\Tt$ drops in a manner 
which cannot be undone; i.e., for all $\alpha\geq\lambda$, $[0,\alpha]_\Tt$ drops, a contradiction. 
Similar remarks pertain to genericity iterations on $k$-suitable 
models.
\begin{comment}We remark that in the comparison of, for example, 
$\R|0$ with $\N|0$ above, The discussion in the proof of Lemma \ref{Comparisons} also shows that if 
$\T$
is a genericity iteration tree on a $k$-suitable premouse $\P$ then for no limit
$\lambda\leq \textrm{lh}(\T)$, there is a $Q$-structure $\Q\unlhd \M^\T_\lambda$ for
$\delta(\T\rest\lambda)$ such that there is some $F \in \mathbb{E}_+(\Q)$ such
that crit$(F) < \delta(\T\rest \lambda) \leq $ lh$(F)$ as this would imply that $\T$ drops while 
genericity iteration trees are nowhere dropping.
\end{comment}
\end{remark}

\begin{lemma}\label{lem:exists_A_iterable_mouse}
Let $A\in\M\inter\pow(\RR)$. Then for a cone of $s\in\RR$ 
there is an $\om$-suitable, $A$-iterable premouse over $s$.
\end{lemma}
\begin{proof}
The following proof is based on the sketch given in \cite[1.12.1]{Scalesweakgap}.\footnote{We are 
using $\g$-organized mice as our mice over reals. The authors believe that, had we used a 
hierarchy $Z$ of mice over reals more closely related to $\Theta$-$\g$-organized 
mice, then the proof in \cite[\S 7]{hod_as_core_model} could be adapted to work in the 
present context. (One needs to define $Z$ such that $\Theta$-$\g$-organized mice can be realized as 
derived models of $Z$-mice, in a reasonably level-by-level manner.) Such a proof would have the 
advantage of providing some extra information. However, one would 
need to define and use the relevant Prikry forcing, so it seems to be more work overall, and our 
approach also has the advantage that it is less dependent on the precise hierarchy of mice over 
reals that is used. One might alternatively start out like \cite[\S 
7]{hod_as_core_model}, but instead of using Prikry forcing, finish more like in our present proof.}
We give a full account here, since the 
proof is rather involved and 
the possibility of non-tame mice was not covered explicitly in \cite{Scalesweakgap}. Moreover, 
comparing our proof with the remarks in \cite[Footnote 12]{Scalesweakgap}, we will not manage to 
establish the full Dodd-Jensen property for the 
iteration strategy we construct, but we will obtain a version of the Dodd-Jensen property which 
suffices for our purposes.

Say that a set of reals constituting a counterexample to the theorem is
\textbf{$\Gamma$-bad}. Suppose there is a $\Gamma$-bad set. For other pointclasses $\Gammabar$ we 
define \textbf{$\Gammabar$-bad} analogously.

Let $\zeta_0<\alpha_0$ and $\psi_{\Omega}\in\Sigma_1(\Ll^-)$ be such 
that $\Omega^*$ is definable over $\M|\zeta_0$ from $z_0$ and 
$\M|(\zeta_0+1)\sats\psi_\Omega(z_0)$ but $\M|\zeta_0\sats\neg\psi_\Omega(z_0)$.
Since there is 
$\xi+1\in(\theta,\l(\M))$ such that $\M|\xi\sats\ZF^-$,
 by \ref{Sigma1Elem} there are $\alphabar,\xibar,\betabar$ such that 
$\zeta_0<\alphabar<\xibar<\betabar<\alpha$ and $[\alphabar,\betabar]$ is a $\Sigma_1$ gap of $\M$ 
and 
$\Theta^{\M|\betabar}<\xibar$ and letting
$\Gammabar=\Sigma_1^{\M|\alphabar}$,
$\M|\xibar\sats\ZF^-+$``There is a $\Gammabar$-bad set $A\sub\RR$''. Fixing such a set $A$, note 
that 
$A$ really is $\Gammabar$-bad. We may assume that $\betabar$ is least such that there are 
$\alphabar,\xibar$ as 
above. Then note that $\betabar=\xibar+1$, $\rho_1^{\M|\betabar}=\RR$, 
$p_1^{\M|\betabar}=\{\xibar\}$ and $\betabar$ ends a weak 
gap of $\M$ (the $\Sigma_1$ type of $(\{\xibar\},z_0)$ does not reflect, using the choice of 
$\zeta_0,z_0$). We will show that $A$ is 
\emph{not} $\Gammabar$-bad, a contradiction.
Let $\left<A_i\right>_{i<\om}$ be a self-justifying system at the end of the gap $\M|\betabar$, 
with $A_0=A$. Since $\M\sats\AD$, in $\M|\xibar$ there is a cone of reals $s$ such that 
there is no $\om$-suitable, $A$-iterable premouse over $s$. Let 
$z_1\geq_T z_0$ be a base for this cone, and such that for every $i<\om$ there is 
$\zeta<\Theta^{\M|\betabar}$ such that $A_i$ is definable over $\M|\zeta$ from $z_1$. We write 
$\LpGbgF$ for $\Lp^{\Gammabar}$.

Let $\P\pins\Lp(z_1)$ be least such that $\P$ projects to $\om$ and 
$\Sigma_\P$ is not a $\Gammabar$ 
strategy, where $\Sigma_\P$ is the $(\om,\om_1+1)$-iteration 
strategy for $\P$; by our mouse capturing hypothesis $\P$ exists and is super-small.

We say that a pointclass $\Lambda$ is \textbf{lovely} iff $\Lambda=\Sigma_1^{\M|\zeta}$ for some 
$\zeta<\alpha$. Let $\left<\Gamma_i\right>_{i\in[0,9]}$ be lovely pointclasses such that 
$\Gammabar\sub\Delta_{\Gamma_9}$ and $\Sigma_\P$ is $\Delta_{\Gamma_9}(z_1)$ and for each 
$i\in[1,9]$, 
$\Gamma_i\sub\Delta_{\Gamma_{i-1}}$. 
Let $T_0$ be the tree 
of a scale for a universal $\Gamma_0$ set, with $T_0\in\M$. By Woodin \cite{Woodin_LCFD} there is 
$z_2\in\RR$ such that $z_1\leq_T z_2$ and $H^*=\hod^{L_\xi[T_0,z_2]}_{T_0,z_1}\sats$``$\Delta_0$ is 
Woodin'', where $\Delta_0=\om_2^{L_\xi[T_0,z_2]}$. (We use here that $\M|\xi\sats\ZF$.)

Let $T_i,U_i\in H^*$ be trees projecting respectively to a universal $\Gamma_i$ set and its 
complement. Let $\Delta_i$ be least such that $V_{\Delta_i}^{H^*}$ is $\Gamma_i$-Woodin. Let 
$\lambda<\xi$ be large and such that $(V_\lambda^{H^*},\Delta_9)$ is a coarse premouse.
Let $\pi_H:(H,\Delta)\to(V_\lambda^{H^*},\Delta_9)$ be elementary, with $H$ 
countable, $\pi_H,H\in H^*$, and $z_1,T_i,U_i\in\rg(\pi)$ for each $i\leq 9$ (let 
$U_0=\emptyset$). Let $\pi_H(T^H_i,U^H_i)=(T_i,U_i)$.
Then by arguments in \cite{twms} (using $\M|\xi$ as a background $\ZF+\AD$ model):

\begin{fact}\label{fact:strat_H} In $\M|\alpha$ there is a unique $(\om_1,\om_1+1)$-iteration 
strategy 
$\Lambda_H$ for $(H,\Delta)$ such that for each 
countable successor length tree $\Tt$ via $\Lambda_H$, letting $j=i^\Tt$ and $J=M_\infty^\Tt$, then
\[ p[j(T^H_8)]\sub p[T_8]\ \&\ p[j(U^H_8)]\sub p[U_8].\]
Moreover, the restriction of $\Lambda_H$ to $HC^{H^*}$ is the unique $\pi_H$-realization strategy 
in $H^*$. Further, for $i\geq 1$, $J\sats$``$j(T^H_i),j(U^H_i)$ are 
$\Coll(\om,j(\Delta))$-absolutely complementing''. Moreover,
\[ C^H=C_\Gammabar\rest V_\Delta^H\in H\ \&\ j(C^H)=C_\Gammabar\rest V_{j(\Delta)}^J; \]
\[ \Fop^H=\Fop\rest V_\Delta^H\in H\ \&\ j(\Fop^H)=\Fop\rest i^\Tt(\Fop^H).\]
\end{fact}

\begin{comment}
Since $\M|\alphabar$ is admissible, arguments in \cite{twms} give:

\begin{fact}\label{clm:norm_iter_stacks}
 If $Q$ is a $k+1$-sound g-organized $\Fop$-premouse such that $\rho_{k+1}^Q=\om$, and $Q$ is
$(k,\om_1+1)$-iterable in $\M|\alphabar$, then $Q$ is $(k,\om_1,\om_1+1)$-iterable 
in $\M|\alphabar$.
\end{fact}
\end{comment}

Let $\CC=\left<N_\alpha\right>_{\alpha\leq\Delta}$ be the maximal
fully backgrounded $L^{^\g\Fop}[\es,z_1]$-construction as computed in $H$. The fact that this 
construction does not break down follows from \ref{lem:L[E]_construction} and \ref{fact:strat_H}.
(For $\Lambda_H$ agrees with the $\pi_H$-realization strategy. Also, let $R,N_\alpha$ 
be type 3 and $\pi:R^\sq\to N_\alpha^\sq$ be $\Sigma_0$-elementary. We may assume that 
$\pi$ is cofinal in $\nu(N_\alpha)$, by the ISC. It follows that $R$, and likewise 
$R'=\Hull_1^R(\emptyset)$, are iterable in $\M|\alpha$. So $R'\pins\Lp(z_1)$, so $R'$ is not 
superstrong by our mouse capturing hypothesis, so $R$ is not superstrong. So 
\ref{lem:L[E]_construction} applies.) Also by \ref{fact:strat_H}, for every $\alpha\leq\Delta$ and 
$n<\om$, the $(n,\om_1,\om_1+1)$-strategy for $\core_n(N_\alpha)$ given by resurrection and lifting 
to $\Lambda_H$, is a (${^\g\Fop}$-)strategy.

\begin{claim}
There is $\gamma<\Delta$ and $k<\om$ such that 
$\rho_{k+1}(N_{\gamma})=\om$ and $\core_\om(N_{\gamma})$ is not 
$(k,\om_1+1)$-iterable in $\M|\alphabar$.\end{claim}
\begin{proof}
It suffices to see that $\CC$ reaches 
$\P$.
By the definability of $\P$, $\P\in 
H^*$ and 
$\P\in H$, and letting $\Sigma_\P^H=\Sigma_\P\rest V_\Delta^H$, we have $\Sigma_\P^H\in H$, and 
$\Sigma_\P^H$ is moved correctly by $\Lambda_H$. It follows that the background extenders used in 
$\CC$ all cohere $\Sigma_\P^H$, and so we can apply \ref{lem:back_stat}
(the stationarity of $\CC$ with respect to $\P$). So we just need to rule out the possibility that 
for some normal tree $\Tt$ on $\P$ via $\Sigma_\P$, with last model $\P'$, $N_\Delta\ins\P'$. But 
because $\Sigma_\P$ is a $\Gamma_9$ strategy and $N_\Delta$ is definable over $V_\Delta^H$, 
we have $\Tt\in C_{\Gamma_9}(V_\Delta^H)$. But $C_{\Gamma_9}(V_\Delta^H)\sats$``$\Delta$ is 
Woodin'', so by the universality of $N_\Delta$ (see \cite[Lemma 11.1]{DMATM}), $\Tt\notin 
C_{\Gamma_9}(V_\delta^H)$, contradiction.
\end{proof}


By the previous claim, we may let $(\gamma,m,\eta)\in\Ord^3$ be lexicographically least 
such that, letting $\P=\core_m(N_\gamma)$, $\eta$ is a ${^\g\Fop}$-whole cutpoint of 
$\P$ and $\R=\Hull_{m+1}^{\P}(\eta\un p_{m+1}^\P)$ is $\eta$-sound, and $\R$ is not 
above-$\eta$, $(m,\om_1+1)$-iterable in $\M|\alphabar$. Let $\Sigma_\R$ be the 
$(m,\om_1,\om_1+1)$-iteration 
strategy for $\R$ given by resurrection and lifting to $\Lambda_H$. We take $\pi_0:\R\to\P$ to 
be the base lifting map. Let $\Tt$ be on $\R$ via $\Sigma_\R$ and $\lambda<\lh(\Tt)$, and 
let $\Uu$ be the lifted tree on $H$. Write $\CC_\lambda=i^\Uu_{0,\lambda}(\CC)$. Let 
$n=\deg^\Tt(\lambda)$. Write $\pi_\lambda:M^\Tt_\lambda\to\P_\lambda$ for the lifting map; here 
$\pi_\lambda$ is a weak $n$-embedding 
and $\P_\lambda=\core_n(N^{\CC_\lambda}_\xi)$ for some $\xi\leq i^\Uu_{0,\lambda}(\gamma)$, with 
$\xi=i^\Uu_{0,\lambda}(\gamma)$ iff $[0,\lambda]_\Tt$ does not drop in model.
(Note that the codomain is $i^\Uu_{0,\lambda}(\P)$, not 
$i^\Uu_{0,\lambda}(\R)$, when $[0,\lambda]_\Tt$ does not drop in model.)

Given a premouse $\N$ and $\zeta\in\OR(\N)$, we say that $\N$ is 
\textbf{$(\Gammabar,k,\zeta)$-iterable} 
iff there is an above-$\zeta$, $(k,\om_1+1)$-iteration strategy for $\N$ in $\M|\alphabar$.
We say $\N$ is $(\Gammabar,\zeta)$-iterable iff $\N$ is $(\Gammabar,m,\zeta)$-iterable.

\begin{claim}\label{clm:if_phalanx_not_iter}
Let $\Tt$ be an above-$\eta$ normal tree on $\R$ via $\Sigma_\R$, of length $\lambda+1$ for a limit 
$\lambda$. Let $b=b^\Tt$ and $\Q=\Q(\Tt\rest\lambda,b)$. Let $k=\om$ if $\Q\pins 
M^\Tt_\lambda$ and $k=\deg^\Tt(\lambda)$ otherwise.  Suppose that the phalanx 
$\pP=\Phi(\Tt\rest\lambda)\conc\left<\Q\right>$ is 
not normally $(k,\om_1+1)$-iterable in $\M|\alphabar$ \tu{(}here $k$ indicates the degree for 
$\Q$\tu{)}. Let $\delta=\delta(\Tt\rest\lambda)$ and $M_\Tt=M(\Tt\rest\lambda)$.
Then either:
\begin{enumerate}[label=\tu{(}\alph*\tu{)}]
 \item $\delta$ is a strong cutpoint of $\Q$, $\Q=M^\Tt_\lambda$, $b^\Tt$ does not drop in model or 
degree and $\Q||(\delta^+)^\Q=\LpGbgF(M_\Tt)$;
or
 \item $\delta$ is not a cutpoint of $\Q$, 
and letting $E\in\es_+^\Q$ be such that $\crit(E)<\delta<\lh(E)$, with 
$\lh(E)$ minimal, and letting $\Tt^+$ be the normal tree 
$\Tt\conc\left<E\right>$, then $b^{\Tt^+}$ does not drop in model or degree, 
and $\Q||\lh(E)=\LpGbgF(M_\Tt)$.
\end{enumerate}
\end{claim}
\begin{proof}
Suppose $\delta$ is a cutpoint (hence strong cutpoint) of $\Q$. Because $\delta$ is a 
cutpoint, the difficulty 
in iterating $\pP$ gives that $\Q$ is not $(\Gammabar,k,\delta)$-iterable.
Because $\delta$ is a strong cutpoint and by standard fine structure, 
$\Q\pins\Lp(M_\Tt)$.

We leave the proof that $\Q=M^\Tt_\lambda$ to the reader; assume this. We show that $b$ does not 
drop in model or degree; suppose otherwise. Let $m'=\deg^\Tt(\lambda)$, so 
$\Q=\Hull_{m'+1}^\Q(\delta\un p_{m'+1}^\Q)$. We have $(\gamma',m')<_\lex 
(i^\Uu_{0,\lambda}(\gamma),m)$ where
$\P_\lambda=\core_{m'}(N_{\gamma'}^{\CC_\lambda})$. We have 
$p_{m'+1}^{\P_\lambda}=\pi_{\lambda}(p_{m'+1}^\Q)$ and the $m'+1$-solidity witnesses for 
$(\P_\lambda,p_{m'+1}^{\P_\lambda})$ are in $\rg(\pi_\lambda)$. (The latter is by
the commutativity between the copy and iteration maps.) But 
\[ \rg(\pi_\lambda)\sub\Pbar=\Hull_{m'+1}^{\P_\lambda}(\pi_\lambda(\delta)\un 
p_{m'+1}^{\P_\lambda}).\]
Therefore $\Pbar$ is $\pi_\lambda(\delta)$-sound. Moreover, we have a 
weak $m'$-embedding $\sigma:\Q\to\Pbar$ such that 
$\sigma(\delta)=\pi_\lambda(\delta)$. So $\sigma$ lifts above-$\delta$ trees on $\Q$ to 
above-$\sigma(\delta)$ trees on $\Pbar$. Therefore $\Pbar$ is not 
$(\Gammabar,m',\pi_\lambda(\delta))$-iterable. This contradicts the minimality of 
$(i^\Uu_{0,\lambda}(\gamma),m)$ in $M^\Uu_\lambda$.

So $b^\Tt$ does not drop. An argument similar to the preceding one gives that 
$\Q||(\delta^+)^\Q\sub\LpGbgF(M_\Tt)$. Suppose that $\Q||(\delta^+)^\Q\in\LpGbgF(M_\Tt)$. 
Let $\Q'\pins\LpGbgF(M_\Tt)$ be such that 
$\Q'||(\delta^+)^{\Q'}=\Q||(\delta^+)^\Q$ and $\Q'$ projects to $\delta$. Now $\Q'\down 
z_1$ is $\delta$-sound. For let $n<\om$ be such that $\rho_{n+1}^{\Q'}=M_\Tt\neq\rho_n^{\Q'}$. 
Then 
$\Q'\down z_1$ is $n$-sound, and $p_{n+1}^{\Q'}$ is $(n+1)$-solid for $\Q'\down z_1$, and 
\begin{equation}\label{eqn:Q'=Hull} Q'=\Hull_{n+1}^{Q'}(p_{n+1}^{Q'}),\end{equation}
and so it suffices to see that $\Q'=\K$ where
\[ \K= \Hull_{n+1}^{\Q'\down z_1}(\delta\un p_{n+1}^{\Q'}). \]
By line (\ref{eqn:Q'=Hull}), it suffices to see that $\delta\in\K$. But if not then 
$\delta=\crit(\pi)$ where $\pi$ is the uncollapse embedding, but since $\delta$ is Woodin in 
$\Q$, this implies that $\delta$ is not a cutpoint of $\Q$, a contradiction. 
So comparing $\Q$ with $\Q'\down z_1$, we get $\Q=\Q'\down z_1$. So $\Q$ is 
$(\Gammabar,\delta)$-iterable, a contradiction.

Now suppose $\delta$ is not a cutpoint of $\Q$. Suppose that $b^{\Tt^+}$ drops 
in model or degree. Since $\delta$ is a strong 
cutpoint of $M_\infty^{\Tt^+}$, then as before, by choice of $(\gamma,m)$, 
$M_\infty^{\Tt^+}$ is $(\Gammabar,j,\delta)$-iterable, 
where $j=\deg^{\Tt^+}(M_\infty^{\Tt^+})$. Therefore, letting $\kappa=\crit(E)$ and 
$\lh(\Tt^+)=\xi+1$, 
$M^{*\Tt^+}_{\xi}$ is $(\Gammabar,j,\kappa)$-iterable (we can copy trees using $i_E$). But 
$\kappa$ is a 
cutpoint of $M^{*\Tt^+}_{\xi}$. So 
$\Tt^+=(\Tt\rest\chi+1)\conc\Tt'$, where 
$\chi=\pred^\Tt(\xi)$ and $\Tt'$ is an above-$\kappa$, $j$-maximal tree on 
$M^{*\Tt^+}_\xi$. Thus, the iterability of $\pP$ can be reduced to that of 
$M^{*\Tt^+}_\xi$ above $\kappa$. Therefore $\pP$ is iterable in $\M|\alphabar$, 
a contradiction. So $b^{\Tt^+}$ does not drop. We then get $\Q||\lh(E)=\LpGbgF(M_\Tt)$ 
by the arguments just given.
\end{proof}

Let $\Tt$ be an above-$\eta$ normal tree on $\R$, of limit length. Let $b$ be a $\Tt$-cofinal 
branch. We say that $b$ is \textbf{$\Gammabar$-verified for $\Tt$} iff 
$\Phi(\Tt)\conc\left<Q\right>$ is normally $(k,\om_1+1)$-iterable in 
$\M|\alphabar$, where $Q=Q(\Tt,b)$ and if $Q\pins M^\Tt_b$ then $k=\om$ and if $Q=M^\Tt_b$ then 
$k=\deg^\Tt(b)$.

\begin{claim}\label{clm:partial_strategy}
Let $\Tt$ be as above. Then there is at most one branch $\Gammabar$-verified for $\Tt$.
However, the following partial strategy
$\Psi$ is not an above-$\eta$, $(m,\om_1+1)$-strategy for $\R$: Given 
$\Tt$, let $\Psi(\Tt)$ be the unique branch which is $\Gammabar$-verified for $\Tt$.
\end{claim}
\begin{proof}
Uniqueness follows from the usual comparison and fine structural arguments, 
using the $\eta$-soundness of $\R$.
Suppose existence holds. Then by uniqueness and because $\M|\alphabar$ 
is admissible, $\R$ is $(\Gammabar,\eta)$-iterable,
contradiction.
\end{proof}

\begin{definition}
We define the term \textbf{$\Gammabar$-$k$-suitable} analogously to \emph{$k$-suitable} (cf. 
\ref{dfn:k-suitable}), but 
with $\Gammabar$ replacing $\Gamma$. We likewise define \textbf{$\Gammabar$-$A$-iterable} and 
\textbf{$\Gammabar$-suitability strict}. Let $R$ be $\Gammabar$-$\om$-suitable with $z_1\in R$.
Then $\sigma_i^R$ denotes the $\Coll(\om,\delta_i^R)$-term capturing $A_i$ over $R$ (see 
\cite{twms}). Let $Q$ be a structure and $\pi:Q\to P$. We say that $\pi$ is an 
\textbf{$\Avec$-embedding} iff $\pi$ is $\Sigma_1$-elementary and $\sigma_i^R\in\rg(\pi)$ for all 
$i<\om$.
\end{definition}

\begin{claim}\label{clm:N_om_suitable} \tu{(}i\tu{)} $N_\gamma$ has infinitely many Woodins in 
the 
interval 
$(\eta,\rho_m(N_\gamma))$. Let $\delta_\om$ be the supremum of the first $\om$-many and let 
$N=(N_\gamma|\delta_\om)\down(N_\gamma|\eta)$. Then \tu{(}ii\tu{)} $N$ is
$\Gammabar$-$\om$-suitable.\end{claim}
\begin{proof}
We will construct a $\Gammabar$-$\om$-suitable premouse 
which is an initial segment of a $\Sigma_\R$-iterate of $\R$. This is by 
applying Claim \ref{clm:partial_strategy} and an obvious 
generalization thereof, in tandem with Claim \ref{clm:if_phalanx_not_iter}, up to $\om$ 
many times. So let $\Tt_0$ on $\R_0=\R$ be via $\Sigma_\R$ (so above 
$\delta_{-1}=\eta$), witnessing the failure of ``existence'' in Claim 
\ref{clm:partial_strategy}, with $\Tt_0$ of minimal length. Let $\delta_0=\delta(\Tt_0)$. Let 
$b=\Sigma(\Tt_0)$. So Claim \ref{clm:if_phalanx_not_iter} applies to 
$\Phi(\Tt_0)\conc\left<Q(\Tt_0,b)\right>$. We use notation as there, so write $\Tt=\Tt_0\conc b$ 
and $\delta=\delta_0$.

Suppose first that conclusion (b) of Claim \ref{clm:if_phalanx_not_iter} holds. Let 
$\kappa=\crit(E)$. Since $E$ overlaps 
$\delta$ and $b^{\Tt^+}$ does not drop in model or 
degree, $M_\infty^{\Tt^+}$ has at least $\kappa$-many Woodins $<\delta$, and 
$\delta<\rho_m(M_\infty^{\Tt^+})$. And $M_\infty^{\Tt^+}$ is not $(\Gammabar,\delta)$-iterable. Now 
let 
$\delta^*_\om$ be the supremum of the first $\om$-many Woodins of $M_\infty^{\Tt^+}$ above $\eta$. 
Let 
$\zeta$ be least such that $\delta^*_\om<\lh(E^\Tt_\zeta)$. So 
$M_\infty^{\Tt^+}|\delta^*_\om=M^\Tt_\zeta|\delta^*_\om$. Note that $\delta^*_\om$ is a strong 
cutpoint of $M^\Tt_\zeta$ and $\zeta\in b^{\Tt^+}$, and so $[0,\zeta]_\Tt$ does not drop 
in model or degree. Therefore $M^\Tt_\zeta$ is not $(\Gammabar,\delta^*_\om)$-iterable. Now let 
$\Uu$ be the lifted tree, via $\Sigma_H$, on $H$. We have
$\P_\zeta=i^\Uu_{0,\zeta}(\core_m(N_\gamma))$ and 
$\pi_\zeta(\delta^*_\om)<\rho_m(\P_\zeta)$ and $\pi_\zeta(\delta^*_\om)$ is the sup of the first 
$\om$ Woodins of 
$\P_\zeta$ above $\eta$, and $\P_\zeta$ is not 
$(\Gammabar,\pi_\zeta(\delta^*_\om))$-iterable. By the elementarity of $i^\Uu_{0,\zeta}$, this 
gives (i), and ($*$) $\P=\core_m(N_\gamma)$ is not $(\Gammabar,\delta_\om)$-iterable.

We now verify condition \ref{item:cutpoint} of $\Gammabar$-$\om$-suitability (cf. 
\ref{dfn:k-suitable}). Let $\kappa$ be a cutpoint of $\P|\delta_\om$ with $\eta\leq\kappa$. Let 
$\C_\kappa$ be the $\kappa$-core of $\P$. We claim that ($**$) $\C_\kappa$ is not 
$(\Gammabar,\kappa)$-iterable. For we have $\pi_0:\R\to\P$ is the core map. Let 
$\kappabar\in\OR(\R)$ be least such that $\pi_0(\kappabar)\geq\kappa$, and let 
$\pi_0(\deltabar_\om)=\delta_\om$.

Suppose $\pi_0(\kappabar)=\kappa$. Let $\xi$ be least 
such that $i^{\Tt^+}(\kappabar)<\lh(E^\Tt_\xi)$. Then $M^{\Tt}_\xi$ is not 
$(\Gammabar,i^\Tt_{0,\xi}(\kappabar))$-iterable because $i^{\Tt}_{0,\xi}(\kappabar)$ is a 
cutpoint of $M^\Tt_\xi$, and $M^\Tt_\zeta$ is not 
$(\Gammabar,\delta^*_\om)$-iterable. But then since 
$M^\Tt_\xi$ is $i^\Tt_{0,\xi}(\kappabar)$-sound, $i^\Uu_{0,\xi}(\C_\kappa)$ is not 
$(\Gammabar,i^\Uu_{0,\xi}(\kappa))$-iterable, which gives ($**$).

Now suppose $\pi_0(\kappabar)>\kappa$. Let $\xi$ be least such that 
$\kappa'=\sup i^{\Tt^+}``\kappabar<\lh(E^\Tt_\xi)$. Then $\xi\in b^{\Tt^+}$ and 
$\kappa'\leq\crit(i^{\Tt^+}_{\xi,b^{\Tt^+}})$. One can show that 
$\pi_\xi(\kappa')>i^\Uu_{0,\xi}(\kappa)$; and $\pi_\xi\com 
i^{\Tt}_{0,\xi}``\kappabar\sub i^\Uu_{0,\xi}(\kappa)$. Therefore $\kappa'$ is a cutpoint of 
$M^{\Tt^+}_\xi$; and $M^{\Tt^+}_\xi$ is $\kappa'$-sound. Now argue much as before, giving ($**$).

Now let $\kappa$ be a ${^\g\Fop}$-whole strong cutpoint of $\P|\delta_\om$. Let $\C_{\kappa+1}$ 
be the $(\kappa+1)$-core of $\P$. By  ($**$), the
choice of $\gamma$ and universality for premice over $\P|\kappa$, we have
\[ \P|(\kappa^+)^\P=\P_{\kappa+1}|(\kappa^+)^{\P_{\kappa+1}}=\LpGbgF(\P|\kappa).\]
This gives condition \ref{item:cutpoint} of $\Gammabar$-$\om$-suitability.

It remains to verify condition \ref{item:Qstructure}. So let $\xi<\delta_\om$ with $\xi\geq\eta$ 
and $\xi$ not Woodin in $\P$; we must show that $C_\Gammabar(\P|\xi)\sats$``$\xi$ is not Woodin''. 
We may assume that $\P|\xi$ is ${^\g\Fop}$-whole, and by condition \ref{item:cutpoint}, also that 
$\xi$ is not a strong cutpoint of $\P$. Let $F\in\es^\P$ be least such that 
$\mu=\crit(F)\leq\xi<\lh(F)$. Note that by coherence and the ISC, 
$\mu$ is a limit of cutpoints of $\P|\xi$. So if $\mu=\xi$ then $\P|\xi$ is the 
Q-structure for $\xi$, so we are done. So suppose $\mu<\xi$. We may assume that 
$\P||\lh(F)\sats$``$\xi$ is Woodin'', 
because otherwise there is $\Q\pins\P||\lh(F)$ such that 
$\Q$ is a Q-structure for $\xi$ and $\xi$ is a strong cutpoint of 
$\Q$, and so $\Q\pins\LpGbgF(\P|\xi)$ (by resurrection and the choice of $\gamma$). Therefore 
$\mu$ is not a cardinal of $\P$. Let $\Q\pins\P$ be least such that $\lh(F)\leq\OR(\Q)$ 
and $\rho_\om^\Q<\mu$. Then $\Q$ collapses $\xi$. Let 
$\zeta\in[\rho_\om^\Q,\mu)$ be a ${^\g\Fop}$-whole strong cutpoint of $\Q$. Then 
$\Q\ins\LpGbgF(\P|\zeta)$, so $\Q\in C_\Gammabar(\P|\xi)$, which suffices. This completes 
the proof that $\P|\delta_\om$ is $\Gammabar$-$\om$-suitable in this case.

Now suppose that conclusion (a) of Claim \ref{clm:if_phalanx_not_iter} holds.
Let $\Tt_0^+=\Tt_0\conc\left<b\right>$ and let $\R_1=M_\infty^{\Tt_0^+}$. 
Then $b^{\Tt_0^+}$ does not drop in model or degree. And $\delta_0$ is a strong cutpoint of $\R_1$, 
$\R_1$ is $\delta_0$-sound, projects $<\delta_0$, and is not $(\Gammabar,\delta_0)$-iterable.
So the obvious modification of Claim 
\ref{clm:partial_strategy} applies to $\R_1$ above $\delta_0$. Pick $\Tt_1$ 
on $\R_1$, above $\delta_0$, like before. Again apply Claim 
\ref{clm:if_phalanx_not_iter}. If its conclusion (b) holds proceed as before, and 
otherwise let $\R_1=M_\infty^{\Tt_1^+}$ and pick $\Tt_2$ on $\R_1$, etc.

If the above process produces $\R_n$ and $\Tt_n$ for all $n<\om$, then we get (i) much as before,
and note that, letting $\delta_n$ be the $n^\nth$ Woodin of $\P=\core_m(N_\gamma)$ above $\eta$, 
then $\P$ is not $(\Gammabar,\delta_n)$-iterable. Part (ii) follows much like before.
\end{proof}




\begin{comment}
there is a countable g-organized-$\Fop$-premouse 
$\R$ over $s$ and $\nu<\OR^\R$ such that $\nu$ is a strong cutpoint of $\R$, 
$\R$ is $\nu$-sound, $\rho_{m+1}^\R\leq\nu<\rho_m^\R$, and there is a weak 
$m$-embedding $\pi:\R\to\core_m(N_{\gamma'})$, but $\R$ is not above-$\nu$, 
$(m,\om_1)$-iterable in $\M|\alphabar$. (Thus, $\gamma$ exists 
because $\gamma_1$ is such a $\gamma'$.) Fix $\R,\nu,\pi$ witnessing this.
Also let $\chi$ be large and such that $(V_\chi,\delta)$ is a coarse premouse 
and let $W$ be countable and $\tau:W\to (V_\chi,\delta)$ be elementary, with 
everything relevant in $\rg(\tau)$. Let $\Sigma_W$ be the realization 
strategy for $W$. Let $\Sigma$ be the above-$\nu$,
$(m,\om_1,\om_1)$-strategy for $\R$ given by copying/resurrection to $\Sigma_W$.

Say a countable $m$-maximal stack $\Ttvec$ of countable trees on $\R$ is 
\emph{good} iff every tree $\Tt$ in $\Ttvec$ is above $\nu$, has a last model 
and $b^\Tt$ does not drop in model or degree.
\end{comment}

\begin{claim}\label{clm:term_relation_hull}
Let $P$ be $\Gammabar$-$\om$-suitable and let $\pi:Q\to P$ be an $\Avec$-embedding. Then 
\tu{(}i\tu{)} $Q$ is 
$\Gammabar$-$\om$-suitable and for each $i<\om$, \tu{(}ii\tu{)} $\pi(\sigma^Q_i)=\sigma^P_i$, and 
\tu{(}iii\tu{)} $\rg(\pi)$ is cofinal in $\delta_i^N$.
\end{claim}
\begin{proof}
Parts (i) and (ii) are by condensation of term relations for self-justifying-systems; see 
\cite{twms}.
Consider (iii). If 
$\rg(\pi)\inter\delta_i^P$ is 
bounded in $\delta_i^P$, then we may assume that $\crit(\pi)=\delta_i^Q$, by taking the appropriate 
hull (cf. the first part of the proof of \cite[Lemma 1.16.2]{Scalesweakgap}). 
But then $Q|\delta_i^Q=P|\delta_i^Q$, and $P|\delta_i^Q$ is not $\Gammabar$-Woodin, but 
$Q\sats$``$\delta_i^Q$ is Woodin'', so $Q$ is not $\Gammabar$-$\om$-suitable, contradiction.
\end{proof}

\begin{definition} Let $\Tt=\left<\Tt_\alpha\right>_{\alpha\leq\gamma}$ be a stack of normal 
iteration trees. We say that $\Tt$ is \textbf{relevant} iff for every $\alpha<\gamma$, 
$b^{\Tt_\alpha}$ does not drop. (Here we allow $\Tt_\gamma$ to be trivial, and it might drop.)
The term \textbf{relevantly-$(\om,\om_1,\om_1+1)$-iteration strategy} is defined as is 
\emph{$(\om,\om_1,\om_1+1)$-iteration strategy}, except that the former only acts on 
relevant trees.
\end{definition}

From now on we fix $N$ as defined in Claim \ref{clm:N_om_suitable}. Let $\Sigma_N$ be the 
relevantly-$(\om,\om_1,\om_1+1)$ strategy for $N$ given by resurrection and 
lifting to $\Lambda_H$. The next claim follows from \ref{fact:strat_H}.
\begin{claim}\label{clm:Lambda_H_pres}For any successor length tree $\Uu$ on $H$ via 
$\Lambda_H$, 
$i^\Uu(N)$ is $\Gammabar$-$\om$-suitable and $i^\Uu\rest N:N\to i^\Uu(N)$ is 
an $\Avec$-embedding.
\end{claim}

\begin{claim}\label{clm:Sigma_N_ss}
$\Sigma_N$ is $\Gammabar$-suitability strict. Moreover, let $\Tt$ be via $\Sigma_N$, of successor 
length, such that $b^\Tt$ does not drop. Then $i^\Tt$ is an $\Avec$-embedding.
 \end{claim}
 \begin{comment}
  \item If $\Uu$ is of limit length, via $\Sigma_N$, and is $\Gammabar$-short, then 
$\Sigma_N(\Uu)$ $k<\om$ then $P$ has 
a $k$-suitable segment iff 
``$i^\Tt(\gamma)$'' makes sense, where $\gamma=((\delta_k^N)^+)^N$; that is, letting 
$\alpha_0+1,\ldots,\alpha_j+1$ enumerate the elements of $b^\Tt$ at which $\Tt$ drops in model, in 
increasing order, and $\beta_i=\pred^\Tt(\alpha_i+1)$, and $\alpha_{-1}=-1$, then 
$\gamma\in\dom(\pi)$ where \[ \pi=i^{*\Tt}_{{\alpha_j}+1}\com 
i^{*\Tt}_{\alpha_{j-1}+1,\beta_j}\com\ldots\com 
i^{*\Tt}_{\alpha_0+1,\beta_1}\com i^\Tt_{0,\beta_0}, \]
and in this case, $\pi(N|\gamma)$ is the unique $k$-suitable segment of $P$.
 \item If $b^\Tt$ drops, then letting $k$ be largest such that $P$ has a $k$-suitable segment, the 
tail of $\Sigma_N$ for trees on $P$, above $\delta_k^P$, is the $\Gammabar$-short 
strategy.
 \item If $P$ has a $k$-suitable segment, and $j<k$, and $\alpha<\delta_{j+1}^P$, then the tail of 
$\Sigma_N$ for trees on $P$, based on the interval $[\delta_j^P,\alpha]$, is the $\Gammabar$-short 
strategy.
\end{comment}
\begin{proof}
Let $\Tt$ be via $\Sigma_N$, of successor length. If $b^\Tt$ does not drop, then the 
lemma's conclusions regarding $M_\infty^\Tt$ and $i^\Tt$ follow from \ref{clm:term_relation_hull} 
and
\ref{clm:Lambda_H_pres}.

Suppose $b^\Tt$ drops and that $i<\om$ is as in \ref{dfn:ss}\ref{item:ss_drops}, but some 
$R\ins M_\infty^\Tt$ is $\Gammabar$-$(i+1)$-suitable. For simplicity assume that $\Tt$ consists of 
just one normal tree and that $\Tt$ has minimal possible length. It follows that for every extender 
$E$ used in $\Tt$, 
$\nu(E)<\delta=\delta_i^R$. Let $n=\deg^\Tt(b^\Tt)$. Then $\rho_{n+1}(M_\infty^\Tt)<\OR(R)$ and 
$M_\infty^\Tt$ is $\delta$-sound. So let $Q\ins M_\infty^\Tt$ be least such that $R\ins Q$ and 
$\rho_\om^Q\leq\delta$. So
$R|(\delta^+)^R=\Lp^\Gammabar(R|\delta)=Q|(\delta^+)^Q$. Also $Q\sats$``$\delta$ is Woodin'' and 
$Q$ is $\delta$-sound and $\delta$ is a strong cutpoint of $Q$ (because $\eta$ is a strong cutpoint 
of $N$). So letting $j<\om$ be such that $\rho_{j+1}^Q\leq\delta<\rho_j^Q$, $Q$ is not 
$(\Gammabar,j,\delta)$-iterable. Let $\Uu$ be the $\Lambda_H$-tree on $H$ given by lifting $\Tt$. 
Let $J$ be 
the last model of $\Uu$. Let $\alpha\in\OR(J)$ and 
$\pi:M_\infty^\Tt\to\core_n(N_\alpha^{i^\Uu(\CC)})$ be the lifting map.
Then using $\pi$ and resurrection in $J$, and by choice of $\gamma$, we get that $Q$ is 
$(\Gammabar,j,\delta)$-iterable, a contradiction. (Suppose $M_\infty^\Tt$ is type 3. If 
$\nu(E(M_\infty^\Tt))<\OR(Q)<\OR(M_\infty^\Tt)$ then let $E^*\in J$ be a background extender for 
$N_\alpha^{i^\Uu(\CC)}$ and lift $Q$ to a model in $\Ult(J,E^*)$. If $Q=M_\infty^\Tt$ then 
$\delta<\crit(E^Q)$ so there is no problem.)
\end{proof}



\begin{definition}
Let $Q$ be $\Gammabar$-$\om$-suitable. Let $\Sigma$ be a  relevantly-$(\om,\om_1,\om_1)$ 
iteration strategy for $Q$. We say that $(\Tt,P)$ is a \textbf{$\Sigma$-pair} iff $\Tt$ is a 
countable tree on $Q$ via $\Sigma$, with last model $P$. We say that a $\Sigma$-pair $(\Tt,P)$ is 
\textbf{non-dropping} iff $b^\Tt$ does not drop. We say that $\Sigma$ is
\textbf{$\Avec$-good} iff for every non-dropping $\Sigma$-pair $(\Tt,P)$, $P$ is 
$\Gammabar$-$\om$-suitable and $i^\Tt$ is an $\Avec$-embedding.
If $(\Tt,P)$ is a non-dropping $\Sigma$-pair, we write $\Sigma^\Tt_P$ for the $(\Tt,P)$-tail of 
$\Sigma$ (that is, $\Sigma^\Tt_P$ is the relevantly-$(\om,\om_1,\om_1+1)$ iteration strategy 
$\Lambda$ for $P$ where $\Lambda(\Uu)=\Sigma(\Tt,\Uu)$).
\end{definition}

The following claim is immediate:

\begin{claim}\label{clm:propagate_ss_Ag}
 Let $\Sigma$ be a relevantly-$(\om,\om_1,\om_1+1)$-iteration strategy for $Q$.
 Let $(\Tt,P)$ be a non-dropping $\Sigma$-pair. If $\Sigma$ is suitability strict then 
$\Sigma^\Tt_P$ is suitability strict. If $\Sigma$ is $\Avec$-good then $\Sigma^\Tt_P$ is 
$\Avec$-good.
\end{claim}

\begin{claim}\label{clm:unique_ss_Ag}
Let $Q$ be $\Gammabar$-$\om$-suitable. Then there is at most one suitability strict 
$\Avec$-good relevantly-$(\om,\om_1,\om_1+1)$ iteration strategy for $Q$.\end{claim}
\begin{proof}
Let $\Sigma,\Lambda$ be two such strategies, and let $\Tt$ be of limit length, via 
$\Sigma,\Lambda$, such that $b=\Sigma(\Tt)\neq\Lambda(\Tt)=c$. We may assume that $\Tt$ is 
normal. We can compare the phalanx $\Phi(\Tt)\conc b$ with the phalanx $\Phi(\Tt)\conc c$, forming 
trees $\Uu,\Vv$, using $\Sigma,\Lambda$, respectively. The comparison is successful. By suitability 
strictness, we have $M_\infty^\Uu=P=M_\infty^\Vv$. By standard fine structure, $b^\Uu$ and 
$b^\Vv$ do not drop and $M_\infty^\Uu\sats$``$\delta(\Tt)$ is Woodin''. In particular, 
$\delta(\Tt)=\delta^P_k$ for some $k<\om$. Because $\Sigma,\Lambda$ are $\Avec$-strategies and by 
\ref{clm:term_relation_hull}, therefore $\rg(i^\Uu)\inter\rg(i^\Vv)$ is unbounded in $\delta_k^P$. 
But then $\rg(i^\Tt_b)\inter\rg(i^\Tt_c)$ is unbounded in $\delta_k^P$, so $b=c$. Contradiction.
\end{proof}

We are now in a position to establish a version of 
the Dodd-Jensen property.

\begin{claim}\label{clm:DJ}
 Let $\Sigma$ be an $\Avec$-good, suitability strict strategy for $Q$. Let $(\Tt,P)$ be a 
non-dropping $\Sigma$-pair.
\begin{enumerate}[label=\tu{(}\arabic*\tu{)}]
\item\label{item:pullback} Let $\pi:R\to P$ be an $\Avec$-embedding. Then the $\pi$-pullback 
$\Lambda$ of $\Sigma^\Tt_P$ is $\Avec$-good and suitability strict. Therefore if $R=Q$ then 
$\Lambda=\Sigma$.
\item\label{item:DJ} Let $\pi:Q\to P$ be an $\Avec$-embedding. Then for all $\alpha<\OR(Q)$, 
$i^\Tt(\alpha)\leq\pi(\alpha)$.
\end{enumerate}
\end{claim}
\begin{proof}
The first clause of \ref{item:pullback} is proven like \ref{clm:Sigma_N_ss}. This together with 
\ref{clm:unique_ss_Ag} 
yields the second clause.
For \ref{item:DJ}, the standard proof of the Dodd-Jensen property applies; the copying does 
not break down by \ref{item:pullback}.
\end{proof}

One can now deduce that $N$ is $\Gammabar$-$A$-iterable, because \ref{clm:propagate_ss_Ag} 
and \ref{clm:DJ} apply to $N$ and $\Sigma_N$, which is enough of the Dodd-Jensen property for 
$\Sigma_N$ to apply the proof of 
\cite[Theorem 4.6]{hodlr}. Let $g\sub\Coll(\om,\N|\eta)$ be 
$\N$-generic. Let $x\in\RR\inter\N|(\eta+1)[g]$ code $(\N|\eta,g)$. Then we can 
reorganize $N[x]$ as a premouse $N^*$ over $x$, and $N^*$ is 
$\Gammabar$-$\om$-suitable and $\Gammabar$-$A$-iterable; these facts all follow by 
S-construction.\footnote{S-construction for g-organized $\Fop$-premice; cf. 
\ref{rem:S-construction}. Now $N\down(N|\eta)$ is a premouse 
over $N|\eta$. Using S-construction we can translate back and forth between premice $P$ over 
$N|\eta$ and premice $P^*$ over $x$, where $P^*$ is a reorganization of $P[x]$, and iterates of $P$ 
correspond to iterates of $P^*$, with iteration maps agreeing over $P$.} But $x\geq_T z_1$, 
contradicting the 
choice of $z_1$. This completes the proof of \ref{lem:exists_A_iterable_mouse}.
\end{proof}

Now for simplicity assume $n=1$ and $\beta=\l(\M)$ is a limit ordinal; we allow that 
$X^\M\neq\emptyset$.
Let $p,w_1,W,\Sigma,\left<\beta_i,Y_i,\psi_i\right>_{i<\om}$ be as in the proof of 
\ref{gapInTheMouse}. Claim \ref{claim:union} holds. Let $z = w_1$, $G=p$, 
$X=X^\M$, and $U,U'$ the 
trees of the scales as in \ref{dfn:self-scaled}. Define the language \[ 
\Ll=\Ll_0\un\{\dot{\beta}_i,\dot{\M}_i\}_{i<\om}\un\{\dot{G},\dot{p},\dot{W},\dot{z},
\dot { X } , \dot { 
U},\dot{U'}\};\]
each symbol in $\Ll\cut\Ll_0$ is a constant symbol.  
Relative to these definitions, let $B_0$, $\left<B^i_0\right>_{i<\om}$ and 
$\vec{S}=\left<S_i\right>_{i<\om}$ be as in \cite{Scalesweakgap}. The analogue of \cite[Corollary 
1.14]{Scalesweakgap} holds (since $\left<S_i\right>_{i<\om}\in\J_1(\M)$, its proof works in 
$\M_\DC$; thus, the resulting iterate $\N$ is in $\M$). Regarding \cite[Lemma 
1.15.1]{Scalesweakgap}, see \cite{gaps_LR_derived_model} for details on the process of interleaving 
comparison with genericity iteration.\footnote{The issue is as follows. Let $\Tt$ be 
one of the trees involved in the comparison. Let $\alpha<\lh(\Tt)$; it might be that 
$[0,\alpha]_\Tt$ drops. But then the usual procedure for choosing the least extender on 
$\es_+(\M^\Tt_\alpha)$ producing a bad extender algebra axiom need not make sense, because in 
fact, the relevant extender algebra is not even in $M^\Tt_\alpha$.} Also, in the proof of 
\cite[Lemma 1.15.1]{Scalesweakgap}, with notation as there, instead of demanding $\pi:H\to 
V_\gamma$ we can make do with $\pi:H\to Z$ where $Z\in\opbk$ is transitive and sufficiently large, 
where $\Fop$ is over $\opbk$ (and thus we can find such $\pi,H$). We need to prove the following:
\begin{lemma}
\label{1.16.2}
Let $\N$ be $\omega$-suitable and $\vec{S}$-iterable. Let 
$\pi\maps\Q \rightarrow \N$
be $\Sigma_1$-elementary with $\tau^\N_{i,j} \in \rg(\pi)$ for all
$i,j<\omega$. Then there is some $m<\omega$ such that for all $n\geq m$,
$\rg(\pi)$ is cofinal in $\delta_n^\N$.
\end{lemma}
\begin{proof}
The proof mostly follows that of \cite[1.16.2]{Scalesweakgap}. But consider the proof of its 
Claim; we adopt the same notation. Within that proof, consider the proof that $\M^*=\bar{\M}$. We 
prove this, as things are different here.
Let $X^*,U^*$, etc, be $\dot{X}^{\M^*}$, $\dot{U}^{\M^*}$, etc.
Let $\bar{X}$ be $X^{\bar{\M}}$, etc. Let $X^-=X^{\M^-}$, etc.

First note that $X^*=X\inter\M^*=\bar{X}$, for $\rho^-\com\psi^*$ yields order-preserving maps 
$U^*\to U$ and ${U'}^*\to U'$. Therefore $a^{\M^*}=a^{\bar{\M}}$. So essentially as in the proof of 
\ref{gapInTheMouse}, $\M^*$ is a $1$-sound $\J$-model over $a^{\bar{\M}}$ with 
$\rho_1(\M^*)=\RR^{\M^*}$ and $p_1^{\M^*}=p$.

Because $\rho^*\com\psi^*\maps\Hh^*\to\Hh$ is $\Sigma_1$-elementary, and by 
\ref{lem:gF_props}, $\Hh^*$ is a $(0,\om_1+1)$-iterable g-organized $\Fop$-premouse over 
$T^{\M^*}$ (in $V$).
Likewise for $\Hh^{\M^*|\eta}$ for every $\eta$ such that $\M^*|\eta$ is relevant.
So $\M^*$ is a $(0,\om_1+1)$-iterable $\Theta$-g-organized $\Fop$-premouse over $X^{\bar{\M}}$.

So we can compare $\M^*$ with $\bar{\M}$. 
Because they are both $1$-sound and minimal for realizing $\Sigma$, they are equal.
\begin{comment}
Suppose now we are in Case \ref{case:M_relevant}. Let the notations be as above. The case 
$\dot{B}^\M=\emptyset$ and $\dot{E}^\M\neq \emptyset$ is proved exactly as in \cite[Lemma 
1.16.2]{Scalesweakgap}. Suppose $\dot{B}^\M\neq \emptyset$. The key point is 
that we can define a map $\pi^*\maps\OR(\M^*) \rightarrow \OR(\M)$ which is 
cofinal and 
$\Sigma_1$ elementary with respect to $\Sigma_1$ truth about ordinals and $z^*$ 
in $\M^*$ and about ordinals and $z$ in $\M$. This suffices to give us $\M^*$ 
is 
a $\Theta$-g-organized $\Fop$-premouse (and in this case, soundness of $\M^*$ is automatic because 
$p_1^\M = \emptyset$). The embedding $\pi^*$ can be extended to 
$\Hh^{\dot{\M}_i^{\M^*}}$ if this is defined and gives $0$-iterability 
of $\dot{\M}_i^{\M^*}$; otherwise, $\pi^*$ gives wellfoundedness of 
$\dot{\M}_i^{\M^*}$. We then get $\M^* = \bar{\M}$ as before. 

Otherwise, $\M = \Jop_\gamma(\M|\theta)$ for 
some $\gamma$ and no $\theta < \gamma^* \leq \gamma$ is such that $\M|\gamma^* 
\vDash \textsf{ZF}$. The map $\pi^*$ as in the previous paragraph guarantees 
iterability of $\M^*$ below $\theta^*$. This easily implies $\M^* = \bar{\M}$.

Case \ref{case:M_not_relevant} is dealt with as in the proof of \cite[Lemma 
1.16.2]{Scalesweakgap}.
\end{comment}
\end{proof}

\begin{comment}
Using the above discussion, we get (see 
\cite[Definition 1.17 ]{Scalesweakgap} for \emph{$k$-stability}):
\begin{lemma}
For some $k<\omega$, there is an $k$-stable $\N$
which is $S_i$-iterable for all $i<\omega$.
\end{lemma}

Now armed with a $k$-stable $\N$,}
\end{comment}

We modify the statement of \cite[Lemma 1.20.1]{Scalesweakgap} as follows: Let $\Q$ 
be 
$\om$-suitable, $j$-sound and $j$-realizable. We claim that with respect to trees above 
$\delta_{j-1}^\Q$, $\Q$ is short tree iterable, and the conclusions of \cite[Lemma 
1.20.1]{Scalesweakgap} hold, except with (a)(ii) replaced by 
``$\Q$-to-$\P$ drops'', and (b)(ii) replaced by ``$b$ drops and $\Tt\conc b$ is 
$\Gamma$-guided''. Let us argue that $\Q$ is short tree iterable above 
$\delta_{j-1}^\Q$. Assume $j=0$ for simplicity. First note that whenever $\pi:\Q\to\N$ is a 
$0$-realization, the $\pi$-pullback $(\Psishort_\N)^\pi$ of the short tree strategy $\Psishort_\N$ 
for $\N$ 
is suitability strict. To see this argue like in the proof of \ref{clm:Sigma_N_ss}.
Then, as in the proof of \ref{lem:short_tree_strat_tracks}, it follows that 
$(\Psishort_\N)^\pi$ is precisely the short tree strategy for $\Q$. This suffices.
Now consider the uniqueness of the branch $b$ 
described in \cite[Lemma 1.20.1]{Scalesweakgap}(b) (as modified above). Given two such branches 
$b,c$, we compare 
the phalanxes $\Phi(\Tt\conc b),\Phi(\Tt\conc c)$, producing trees 
$\Uu,\Vv$. If $\Tt$ is short then note that both $\Tt\conc b$ and $\Tt\conc c$ are 
$\Gamma$-guided, so $b=c$. If $\Tt$ is maximal then $b,c$ cannot drop; rule out the possibility 
that, for example, $M_\infty^\Uu\pins M_\infty^\Vv$ and $b^\Vv$ drops, by using suitability 
strictness.

\begin{comment}
Suppose for simplicity that $\Tt$ is based on $\Q|\delta_0^\Q$. Let $\alpha<\lh(\Tt)$ be such that 
$[0,\alpha]_\Tt$ drops and suppose that $M^\Tt_\alpha|\gamma$ is $1$-suitable, with Woodin 
$\delta$. 
Assume that $\alpha$ is least possible. Then all generators used in $[0,\alpha]_\Tt$ are $<\delta$. 
Therefore there is $\R\ins M^\Tt_\alpha$ which is a Q-structure for $\delta$. Since $\delta$ is the 
least Woodin of $\R$, $\delta$ is a cutpoint of $\R$. Let $\sigma:M^\Tt_\alpha\to 
M^{\pi\Tt}_\alpha$ 
be the copy map; assume for simplicity that $M^\Tt_\alpha$ is not type 3. Then $\sigma(\R)$ is the 
Q-structure for $\sigma(\delta)$, and $\sigma(\delta)$ is a cutpoint of $\sigma(\R)$. Since 
$\Psishort_\N$ is suitability strict, therefore $\sigma(\R)$ is above-$\sigma(\delta)$ iterable in 
$\M|\alpha$. But therefore $\R$ is above-$\delta$ iterable in $\M|\alpha$, a 
contradiction.\end{comment}


\begin{comment}
For let $\Tt$ be on 
$\Q$ and via both the short tree strategy and $\Psi^\pi_\N$, of limit length, suitability 
strict, and suppose that $\pi\Tt$ is short. To simplify notation assume that $\Tt$ is based on 
$\Q|\delta_0^\Q$. Let $b=\Psi^\pi_\N(\Tt)$. Let $\sigma:M^\Tt_b\to M^{\pi\Tt}_b$ be the copy map. 
We 
want to see that $\Tt$ is short and $\Tt\conc b$ via the short tree strategy. If 
$\sigma(\delta(\Tt))=\delta(\pi\Tt)$ this is easy so suppose $\sigma(\delta(\Tt))>\delta(\pi\Tt)$. 
Since $\Hull_1^\N(\{\tau^\N_{i,j}\}_{i,j<\om})$ is cofinal in $\delta_0^\N$, note that if $b$ does 
not drop then $\sigma(\delta(\Tt))<\delta_0^{M^{\pi\Tt}_b}$. So in any case, $\R=\Q(\Tt,b)$ exists 
and $\sigma(\R)=\Q(\pi\Tt,b)$. If $\delta$ is a cutpoint of $\R$ then $\sigma(\delta)$ is a 
cutpoint 
of $\sigma(\R)$ and because $\Psi_\N$ is suitability strict, therefore $\sigma(\R)$ is 
above-$\sigma(\delta)$ iterable in $\M|\alpha$, and so likewise $\R$ above $\delta$, which 
suffices. 
If $\delta$ is not a cutpoint of $\R$ use the proof of
\ref{lem:short_tree_strat_tracks} and the fact that $\Tt$ is suitability strict to see that $\Tt$ 
passes through a fatal drop, to a projecting mouse which is iterable in $\M|\alpha$, which 
suffices. If instead, $\pi\Tt$ is maximal, then it is easy to see that $\Tt$ 
is maximal.
\end{comment}



Let $\Sigma,\Q,(F,\prec^*),\Q_\infty$ be defined as in \cite[\S2]{Scalesweakgap}.\footnote{We use 
``$F$'' where \cite{Scalesweakgap} uses ``$\Fop$'' to avoid conflicts of notation.} Note that 
$\Sigma,{(F,{\prec^*})}\in\M_\DC$. We have the analogue of \cite[Lemma 2.1.2]{Scalesweakgap}, but 
we 
mention some points. First, we don't quite need that $\Q_\infty$ is fully wellfounded for the 
proof; it suffices that $\M_\DC\sats$``$\Q_\infty$ is wellfounded in the codes''. But because 
$\M_\DC$ need not have many ordinals beyond $\M$, it seems possible that $\Q_\infty$ be illfounded. 
However, standard arguments show that $\Q_\infty|\delta_0^{\Q_\infty}$ is wellfounded (in fact 
$\delta_0^{\Q_\infty}\leq\Theta^\M$).\footnote{Recall that we assumed at the 
start of the proof that $\M\sats$``$\Theta$ exists''.
This assumption was justified by \ref{?}, which relied on $\M$ being
$\Theta$-g-organized. This is the only point at which there is a problem with the scales 
analysis for g-organized mice.} The latter is enough for the scale construction to go through.
The rest of the argument is essentially as in \cite{Scalesweakgap}. This completes the 
proof.
\end{proof}

\subsection{Scales analysis within core model induction}

We finish by explaining how we use the scale existence theorems in application to the core 
model induction. In such application, $\Fop$ will not just be nice, but \emph{very} nice.

\begin{definition}
Let $\Fop$ be an operator over $\opbk$. We say that $\Fop$ is \textbf{very nice} 
iff $\Fop$ is nice and $\RR\in\opbk$ and letting
$\N=\J_1(\HC,\Fop\rest\HC)$, $\N\sats\AD$ and every set of reals in $\N$ has 
a scale in $\N$.
\end{definition}

\begin{remark}
 Let $\Fop$ be very nice. Let $z\in\RR$ be such that there are scales on $\Fop^\HCc$ and 
$\RR\cut\Fop^\HCc$ which are analytical in $(\Fop^\HCc,z)$. Let $X=\Fop\un\{z\}$. Then using the 
scales existence theorems \ref{passiveGameScale}, \ref{thm:self_anal_coded}, \ref{weak gap from 
MC} together with \ref{rem:non_adm_gap_dealt_with}, we get the scales analysis for 
$\Lp^{^\gTheta\Fop}(\RR,X)$  from optimal determinacy and super-small mouse capturing hypotheses.
This gives the scales analysis for $\Lp^{^\gTheta\Fop}(\RR,\Fop\rest\HC)$, as required. (Note 
that at passive segments the scales are $\Sigma_1(z)$, maybe not $\Sigma_1$.)
\end{remark}

We have dealt with $\Lp^{^\gTheta\Fop}(\RR,\Fop\rest\HC)$ instead of $\Lp^{^\gTheta\Fop}(\RR)$, 
because we seem to need extra assumptions to obtain the scales analysis from optimal assumptions in 
the 
latter. We now discuss what we need for this. In application, \emph{if} there are no 
divergent $\AD$ pointclasses, $\Fop$ will in fact be 
\emph{extremely} nice.

\begin{definition}\label{dfn:extremely}
 Let $\utilde{\Gamma}$ be a boldface pointclass and $X\sub\RR$. We say that $\utilde{\Gamma}$ 
is an \textbf{$\AD$-pointclass} iff $\AD$ holds with respect to all sets in $\utilde{\Gamma}$. We 
say that $\utilde{\Gamma},X$ are \textbf{Wadge compatible} iff $A,X$ are Wadge 
compatible for every $A\in\utilde{\Gamma}$.

Let $\Fop$ be an operator. We say that $\Fop$ is \textbf{extremely nice} iff there is $X\sub\RR$ 
$\Fop$ is very nice, $\Fop\rest\HC$ is projectively equivalent to $X$,
and for every $\AD$-pointclass $\utilde{\Gamma}$, $\utilde{\Gamma},X$ are Wadge 
compatible.
\end{definition}

\begin{remark}\label{rem:application}
Let $\Fop$ be an extremely nice operator.
We want to see that the scales analysis in 
$\Lp^{^\gTheta\Fop}(\RR)$ proceeds from optimal determinacy assumptions. Let 
$\N\pins\Lp^{^\gTheta\Fop}(\RR)$ be such that $\N\sats\AD$ and 
$\N$ ends a gap 
$[\alpha,\beta]$ of $\Lp^{^\gTheta\Fop}(\RR)$, such that $[\alpha,\beta]$ is not strong. Suppose 
that 
if $[\alpha,\beta]$ is weak and $\Fop\rest\HC\in\N|\alpha$ then super-small mouse capturing 
for $\Gamma=\Sigma_1^{\N|\alpha}$ holds on a cone. We claim that one of the scale existence 
theorems 
\ref{passiveGameScale}, 
\ref{gapInTheMouse}, or \ref{weak gap from MC} applies.

For by \ref{rem:non_adm_gap_dealt_with} and the mouse capturing hypothesis, we may assume that the 
gap is admissible, and so weak, and that $\Fop\rest\HC\notin\N|\alpha$, so $X\notin\N|\alpha$. We 
claim that then 
$\J_1(\N)\sats\AD$, so \ref{gapInTheMouse} applies. If every set of reals in $\J_1(\N)$ is 
Wadge below $X$, this is because 
$\J_1(\HC,\Fop\rest\HC)\sats\AD$. So suppose otherwise. Let $\P\ins\N$ be least such that there is 
a 
set $Z\in\J_1(\P)$ such that $Z\not\leq_W X$. If $\P\pins\N$ 
then $\J_1(\P)\sats\AD$, so by the 
Wadge compatibility given by \ref{dfn:extremely}, we have 
$\Fop\rest\HC\in\J_1(\P)$, so 
$\alpha\leq\l(\P)$. We claim that $\Fop\rest\HC\notin\N|\beta$. Because $\Fop$ is extremely nice 
and by 
\ref{InsideGap}, this is clear if $\Th_{\rPi_1}^{\N|\alpha}\leq_W
X$ or $\Th_{\rSigma_1}^{\N|\alpha}\leq_W X$. Otherwise, by Wadge compatibility, 
$X<_W\Th_{\rSigma_1}^{\N|\alpha}$. But then because $\N|\alpha$ is admissible, 
$X\in\N|\alpha$, so $\Fop\rest\HC\in\N|\alpha$, contradiction. So $\P=\N$. 
Since $\N$ ends a 
weak gap, there are sets $X_i\in\pow(\RR)\inter\N$ such that $\pow(\RR)\inter\J_1(\N)$ is exactly 
the sets which are projective in $\oplus_{i<\om}X_i$. It follows that
$\pow(\RR)\inter\J_1(\N)\sub\pow(\RR)\inter\J_1(\RR,X)$, so 
$\J_1(\N)\sats\AD$ (and so $X\in\J_1(\N)$).
\end{remark}



\begin{comment}
 Note then that since $\N\sats\AD$ and $\Fop$ is very nice, for every 
$X\in\pow(\RR)\inter\N|\alpha$, we have $X<_W\Fop\rest\RR$. 

As mentioned above, Theorem \ref{gapInTheMouse} is typically used when $\Fop\rest \textrm{HC}\notin 
\N$, where $\N$ ends a nontrivial weak gap in $\textrm{Lp}^{\gamma\Fop}(\mathbb{R})$. In this case, 
we do need to assume $\Jop_{1}(\N)\vDash \textsf{AD}$. In practice (e.g. in core model induction 
applications), we have $\J_1(\mathbb{R},\Fop\rest \textrm{HC}) \vDash \textsf{AD}$ and it's easy to 
see that every $A\in \powerset(\mathbb{R})\cap \Jop_1(\N)$ belongs to $\J_1(\mathbb{R},\Fop\rest 
\textrm{HC})$; therefore, our determinacy assumption is not unreasonable.
\end{comment}



\begin{comment}
Suppose there is no $E\in\es_+(\N|\eta)$ such that $\crit(E)\leq\xi<\lh(E)$ and
$E$ is total over $\N|\eta$. It follows that $\N|\gamma$ is
passive, that for eventually all $\eta'<\gamma$, $(\N|\eta')^*$ is already
defined, and for all $E\in\es_+(\N|\eta)$ with $\gamma\leq\lh(E)$, we have
$\gamma<\crit(E)$. Suppose $\gamma=\eta'+\om$ for some $\eta'$. Then
$\gamma=\eta$. Then $(\N|\eta')^*$ has already been defined. Moreover,
$\N|\eta'$ needs $J$-information at the next stage iff $(\N|\eta')^*$ does, and
if they do, then letting $\alpha=\alpha(\N|\eta')$, then
$\alpha=\alpha((\N|\eta')^*)$, and letting $\beta=\beta(\N|\eta')$ and
$\beta^*=\beta((\N|\eta')^*)$, then $(\N|\beta)^*=(\N|\eta')^*|\beta^*$ (so
since $\N|\beta$ is interdefinable with $(\N|\beta)^*$, we get
$\alpha(\N|\eta')=\alpha((\N|\eta')^*)$), and
$(\N|\alpha)^*=(\N|\eta')^*|\alpha$, so they're interdefinable, which implies
that $\Tt_{\N|\alpha}=\Tt_{(\N|\eta')^*|\alpha}$. The latter is just because
$\N|\alpha$ and $(\N|\eta')^*|\alpha$ have the same universe, and $\Tt_\M$ only
depends on the universe of $\M$. So by induction,
$(\N|\eta')^*=F_J^{+,\eta'-\alpha}((\N|\alpha)^*)$. So we can set
$(\N|\eta)^*=F_J^{+,\eta-\alpha}((\N|\alpha)^*)$ (which has height $\eta$).

, and
$\eta''\in(\alpha,\eta']$, we can just define $(\N|\eta)$
$\alpha(\N|\eta')=\alpha(\N$
and we set $(\N|\eta)^*=\J_\om((\N|\eta')^*)$.
Suppose $\gamma$ is a limit of limits. If $\gamma=\eta$ let
$(\N|\eta)^*=\sup_{\alpha<\gamma}(\N|\alpha)^*$. Suppose $\gamma<\eta$; so
$(\N|\gamma)^*$ is already defined. Let $(\N|\eta)^*$ be the
$(J,\N|\xi)$-premouse $\M$ of height $\eta$, such that $\M|\gamma=(\N|\gamma)^*$
and above $\gamma$, the extenders on $\es_+(\M)$ are exactly those on
$\es_+(\N|\eta)$.

Now suppose there is $E\in\es_+(\N|\eta)$ such that $\crit(E)\leq\xi<\lh(E)$
and $E$ is total over $\N|\eta$. Let $E$ be such with $\lh(E)$ minimal. Then by
hypothesis, $\rho_\om(\N|\eta)\leq\crit(E)$. Let $k<\om$ be such that
$\rho_{k+1}^{\N|\eta}\leq\crit(E)<\rho_k^{\N|\eta}$. Let $U=\Ult_k(\N|\eta,E)$.
Note that $\lh(E)$ is a strong cutpoint of $U$. Also, either (i)
$\car^U(\xi)=\crit(E)$, $E$ is type 1, and $(\car^U(\xi)^+)^U$ is a strong
cutpoint of $U$; or (ii) $\crit(E)<\car^U(\xi)$ and $\lh(E)=(\car^U(\xi)^+)^U$. 
In either case, let $\zeta$ be least such that $\zeta\geq\xi$ and
$\rho_\om(\N|\zeta)=\car^U(\xi)$. Then for all
$\eta'\in[\zeta,(\car^U(\xi)^+)^U)$ such that $\rho_\om(\N|\eta')=\car^U(\xi)$,
$(\N|\eta')^*$ is already defined.
Let $(\N|\eta)^*$ be the $(J,\N|\xi)$-premouse $\M$ such that
$\M|\lh(E)=\sup_{\eta'<\lh(E)}(\N|\eta')^*$, and above $\lh(E)$, the extenders
on $\es_+(\M)$ are exactly those on $\es_+(U)$.
\end{comment}

%Suppose $\gamma$ is a cutpoint of $\N|\eta$.
%Then $(\N|\eta)^*$ is
%the $(J,\N|\xi)$-premouse $\M$ where (i) $\M|\gamma=(\N|\gamma)^*$; (ii) above
%$\gamma$, the extenders on $\es_+(\M)$ are exactly those on $\es_+(\N|\eta)$.
%This makes sense because $\N|\gamma$ and $(\N|\gamma)^*$ are interdefinable.

%Now suppose $\gamma=\eta$. If $\gamma$ is a limit of limits, this has been
%dealt with by 

%(c) Let $\alpha\in[\gamma,\eta]$ be minimal such that
%$\N|\alpha$ is active and $\crit(F^{\N|\alpha})<\gamma\leq\lh(F^{\N|\alpha})$.
%Let $E=F^{\N|\alpha}$. So $\rho_\om(\N|\eta)\leq\theta\leq\crit(E)$ (in
%fact, $\crit(E)$ is a cutpoint of $\N|\eta$). Let $k<\om$ be such that
%$\rho_{k+1}^{\N|\eta}\leq\crit(E)<\rho_k^{\N|\eta}$. Let $U=\Ult_k(\N|\eta,E)$.
%Note that $\gamma=(\xi^+)^U$ and $U|\gamma$ is passive and is a cutpoint of
%$U$. Let $(\N|\eta,\N|\xi)^*$ be the $(J,\N|\xi)$-premouse $\M$ such that
%$\M|\gamma=(\N|\gamma)^*$ and above $\gamma$, the extenders on $\es_+(\M)$ are
%exactly those on $\es_+(U)$.

%(d) Let $(\N|\eta,\N|\xi)^*=\sup_{\alpha<\eta}(\N|\alpha,\N|\xi)^*$.


%If $\xi$ is a strong cutpoint of $\N|\eta$ then $\N|\eta\approx Q$. (That is,
%that are equal except for the fact that $Q$ is literally an
%$\N|\xi$-$J$-premouse.)

%Suppose $\xi$ is not a cutpoint of $\N|\eta$. Let $E\in\es^{\N|\eta}$ be least
%such that $\kappa=_{\mathrm{def}}\crit(E)<\xi<\lh(E)$. Then
%$\N|\eta\vDash$``$\kappa$ is a limit of Woodins''. Since $\N$ is suitable,
%therefore $\car^\N(\eta)<\kappa$. Let $\gamma\geq\eta$ be least such that
%$\rho_\om(\N|\gamma)\leq\kappa$, and let $n<\om$ be such that
%$\rho_{n+1}(\N|\gamma)=\kappa<\rho_n(\N|\gamma)$. Then
%$\mathrm{Ult}_n(\N|\gamma,E)\approx Q$. So from $(\N|\gamma,\xi)$ we compute
%$Q$.
%Conversely, given $Q$, we can compute $\N|\gamma=\mathcal{C}_\om(Q)$, and $Q$
%specifies $\xi$.

%Finally suppose $\xi$ is a cutpoint, but not a strong cutpoint, of $\N|\eta$.
%Then we translate from $\N|\eta$ to $Q$ by taking ultrapowers by all
%type 1 extenders on \end{comment}
%$\es(\N|\eta)$ having critical point $\xi$.
%We translate in reverse by undoing this process. That is, call a $J$-premouse
%$R$ \emph{relevant} iff $\N|\xi\ins R\ins\N|\eta$ and
%either $\rho_\om(R)\leq\xi$ or $R\sats$``$\kappa$ is the largest cardinal''. We
%define the \emph{$*$-translation} $R^*$ of relevant $J$-premice $R$, by
%induction on $\OR(R)$. The $*$-translation will be a fully sound $J$-premouse
%over $\N|\xi$. We will maintain by induction that if $\N|\xi\ins R\ins\N|\eta$
%and $R\sats$``$\kappa^+$ exists'' then $(R|(\kappa^+)^R)^*$ is
%$\Sigma_1(\{\xi\})$ over $R|(\kappa^+)^R$, and $R|(\kappa^+)^R$ is
%$\Sigma_1(\emptyset)$ over $(R|(\kappa^+)^R)^*$. So let $R$ be relevant.

%If $R\sats$``$\kappa$ is the largest cardinal'' then define
%$R^*=\sup_{\N|\xi\ins S\pins R}S^*$. (Note that $R$ is passive in this case,
%since $\xi$ is a cutpoint.)

%Now suppose $R\sats$``$\kappa^+$ exists''.

%Suppose $(\kappa^+)^R$ is a cutpoint of $R$.
%We define $R^*$ to be the $J$-premouse $R'$ such that
%$\OR(R')=\OR(R)$, $R'|(\kappa^+)^R=(R|(\kappa^+)^R)^*$, and above
%$(\kappa^+)^R$, $\es(R')_+$ consists of exactly the same extenders as does
%$\es(R)_+$. Because $(R|(\kappa^+)^R)$ is interdefinable
%with $(R|(\kappa^+)^R)^*$, this makes sense, and above $(\kappa^+)^R$, the fine
%structure of $R$ corresponds exactly to the fine structure of $R^*$ (though if
%$(\kappa^+)^R<\gamma\leq\OR(R)$ then
%$p_n^{R^*|\gamma}=p_n^{R|\gamma}\cut\{\kappa\}$), so $R^*$ is a sound
%$J$-premouse over $\N|\xi$.

%Now suppose $(\kappa^+)^R$ is not a cutpoint of $R$. Let $E$ be the
%least extender on $\es(R)_+$ witnessing this; so
%$\kappa=\crit(E)$ and $(\kappa^+)^R<\lh(E)$. Let
%$n<\om$ be such that $\rho_{n+1}^R=\kappa<\rho_n^R$. Let $Q=\Ult_n(R,E)$.
%Define $R^*$ from $Q$ just as we defined $R^*$ from $R$ in the previous case.
%Since $E$ is type 1, $R^*$ is sound. To undo the $*$-translation, we just
%compute $Q$ from $R^*$, and find $R=\core_\om(Q)$.

\begin{comment}
\begin{definition}[$*$-translation](***Didn't mention I'd also define
*-translation of $\N||\alpha$ when $\N|\alpha$ is active.***]
Let $\N$ be a $J$-mouse and $\xi<\OR^\N$. Let $\eta\in[\xi,\OR(\N))$, such that
for every $E\in\es_+(\N|\eta)$, if
$\crit(E)\leq\xi<\lh(E)$ and $E$ is total over $\N|\eta$, then
$\rho_\om(\N|\eta)\leq\crit(E)$.
%either (a) $\eta=\xi$; or (b)
%$(\xi^+)^{\N|\eta}$ is a passive level and is a cutpoint of $\N|\eta$; or (c)
%$(\xi^+)^{\N|\eta}$ is either (i) active or (ii) fails to be a cutpoint of
%$\N\|\eta$; and $\rho_\om(\N|\eta)\leq\theta\leq\xi$ for some cutpoint $\theta$
%of $\N|\eta$; or (d)
%$\N|\eta$ is a limit of such levels.
We define the \emph{$*$-translation}
$(\N|\eta,\N|\xi)^*$ (or just $(\N|\eta)^*$ if $\xi$ is understood). The
definition proceeds by recursion on $\eta$. We will maintain that
$(\N|\eta)^*\pins\Lp^J(\N|\xi)$ and
$(\N|\eta,\N|\xi)$ is definably equivalent to $((\N|\eta)^*,\N|\xi)$ (over the
least admissible
structure containing either of these), uniformly in $\eta$. We now
give the definition.

We set $(\N|\xi)^*=\N|\xi$. Similarly, for $\eta>\xi$ such that
$\xi$ is a
strong cutpoint of $\N|\eta$, we similarly set $(\N|\eta)^*\approx\N|\eta$;
that is, $(\N|\eta)^*$ is the 

Suppose $\alpha_0=\alpha>\xi$ is least such that $\N|\alpha$ is active and $\xi$
is not a strong cutpoint of $\N|\alpha$. Let $F=F^{\N|\alpha}$ and
$\kappa_0=\crit(F)$. Let $\eta=\eta_0$ be least such that
$\eta\geq\alpha$ and $\rho_\om(\N|\eta)\leq\kappa_0$, so we must define
$(\N|\eta)^*$. (We need not define $(\N|\gamma)^*$ for
$\gamma\in[\alpha,\eta)$.)

Let $\rho_{k+1}^{\N|\eta}\leq\kappa_0<\rho_k^{\N|\eta}$. Let
$P=\Ult_k(\N|\eta,F)$. We claim that $\lh(F)$ is a cutpoint of $P$. It follows
that $\xi$ is a strong cutpoint of $P$, and so we set $(\N|\eta)^*\approx
P$. (Clearly $P$ can be computed from $(\N|\eta,\N|\xi)$, as just described. To
recover $\N|\eta$ from $P$, we just take the core.) So suppose $\lh(F)$ is not a
cutpoint of $P$. Then by the initial segment condition and the minimality of
$F$, $\nu(F)$ is a limit cardinal and $\nu(F)=\crit(E)$ for any $E\in\es^P$
overlapping $\lh(F)$. Let $E$ be the least. Then $\kappa_0$ is strong below
$\nu(F)$ in $\N|\lh(E)$ (as witnessed by $\es^\N$). But then by applying $E$,
and the initial segment condition, $\kappa_0$ is strong below $\lh(E)$,
contradiction.

For $\eta>\eta_0$ such that $\N|\eta=\J_{\eta-\eta_0}(\N|\eta_0)$, just set
$(\N|\eta)^*=\J_{\eta-\eta_0}((\N|\eta_0)^*)$. Then for $\eta$ least such that
$\N|\eta$ is admissible, $\N|\eta$ has the same universe as $(\N|\eta)^*$ (and
$(\N|\eta)^*$ is the least admissible structure containing $(\N|\eta_0)^*$).

So for $\eta>\eta_0$ such that $\xi$ is a strong cutpoint of $\N|\eta$
(equivalently, $\kappa_0$ is a strong cutpoint, or $\eta_0$ is a strong
cutpoint), we can literally copy extenders across to define $(\N|\eta)^*$.
Let $\alpha_1>\eta_0$ be least such that $\kappa_0$ is not a strong cutpoint of
$\N|\alpha_1$. Let $F=F^{\N|\alpha_1}$.

Suppose $\kappa_0$ is a cardinal of
$\N|\alpha_1$. Then $\kappa_0=\crit(F)$, because otherwise $\crit(F)$ would be
strong below $\kappa_0$ in $\N|\kappa_0$, and we would get a contradiction like
before. Therefore, since $\N|\eta_0$ projects to $\kappa_0$, also $F$ is type 1.
Now choose $\eta_1\geq\alpha_1$ least such that $\N|\eta_1$ projects to
$\kappa_0$ and define $(\N|\eta_1)^*$ by:
$(\N|\eta_1)^*||\alpha_1=(\N||\alpha_1)^*$, and above $\alpha_1$, the extender
sequence of $(\N|\eta_1)^*$ is given by copying extenders from
$\Ult_k(\N|\eta_1,F)$, where $k$ is chosen as before.

We carry on in this way, defining pairs $\alpha_\gamma,\eta_\gamma$,
until reaching the lea\end{enumerate}
st $\gamma$ such that $\kappa_0$ is not a cardinal of
$\N|\alpha_\gamma$, and we have defined $(\N||\alpha_\gamma)^*$. Let
$\kappa'=\crit(F^{\N|\alpha_\gamma})$.

For $\eta\geq\eta_\gamma$, define $(\N|\eta)^*$ (when required) by:
$(\N|\eta)^*|\alpha_\gamma=(\N||\alpha_\gamma)^*$, and the extender sequence
above $\alpha_\gamma$ is given by copying $(\N|\eta,\N|\kappa')^*$. (Note that
$(\N||\alpha_\gamma,\N|\kappa)^*\approx\N||\alpha_\gamma$, so is
inter-computable with $(\N||\alpha_\gamma,\N|\xi)^*$. Moreover, for
$\eta\geq\alpha_\gamma$, $(\N|\eta)^*=(\N|\eta,\N|\xi)^*$ is defined iff
$(\N|\eta,\N|\kappa')^*$ is defined.)\end{definition}
\end{comment}

\begin{comment}
\begin{theorem}
\label{gapInTheMouse}
Let $\M$ be a $J$-mouse over $\mathbb{R}^\M$. Suppose $\M \vDash \textsf{AD}^+$
and $[\alpha,\beta]$ is a weak gap in $\M$ and $\omega\beta < o(\M)$. Let $n$ be
the least such that $\rho_n(\M|\beta) = \mathbb{R}^\M$. Then $\M \vDash
``r\utilde{\Sigma}^{\M|\beta}_n$ has the scale property".
\end{theorem}
\begin{proof}[Proof Sketch]
Since the proof is almost the same as that of \cite[Theorem 4.16]{ScalesK(R)},
we only sketch it here, focusing on a new case. There are three main cases:
\begin{enumerate}
\item $\M|\beta$ is passive;
\item $\M|\beta$ is active with $\dot{E}^{\M|\beta}\neq \emptyset$;
\item\label{passive_active_cases_3} $\M|\beta$ is active with
$\dot{B}^{\M|\beta}\neq \emptyset$.
\end{enumerate}
Case \ref{passive_active_cases_3} is new here so we'll focus on it. The other
cases are handled just like
in the proof of Theor\end{enumerate}
em 4.16 in \cite{ScalesK(R)}. To simplify the notation, we
assume $n=1$. Note that $\beta$ is a successor ordinal. Suppose $\Sigma = 
\Sigma_a^{1,\M}$ is a
non-reflecting type, where $a=\langle G, w_1\rangle$ for some real $w_1$ and a
finite set of ordinals $G$. We take $G$ to be $<_{\textrm{lex}}$-least. 

Let $\eta<\beta$ be largest such that $\M|\eta$ is whole. So
$\M|\beta\ins\BBB(\M|\eta,\Tt,b)$ for some $\Tt,b$.
Suppose $\M|\beta = (\lpole\M|\beta\rpole,\in,\emptyset,B,S,\l,\RR^\M)$ for some
$B,S,\l$. We define a sequence $(\beta_i \ | \ i<\omega)$ as in the proof of
\cite[Theorem 4.16]{ScalesK(R)}. Let $\beta_0 = \max\{\eta,
\max\{G\}\}$.\end{enumerate}

Suppose $\beta_i<\beta$ is defined. For $\gamma<\beta$ let
\[
\R_{\gamma}=(\lpole\M|\gamma\rpole,\in,\emptyset,B\inter\gamma,S^{\M|\gamma}
,\l^{\M|\gamma},a). \]
Let
\[
Y_i = \{ a \ | \ a \textrm{ is definable over } \R_{\beta_i} \textrm{ from }
\mathbb{R}^\M\cup\{G, \beta_0,\dots,\beta_{i-1}\}\}.
\]
Let $\psi_i$ be the least $\psi\in \Sigma$ such that $\R_{\beta_i} \vDash \neg
\psi[\langle G,w_1\rangle]$. Let 
\begin{center}
$\beta_{i+1}$ = least $\gamma$ such that $\R_\gamma \vDash \psi_i[\langle
G,w_1\rangle]$.
\end{center}
\noindent \textbf{Claim:} $\cup_{i<\omega} Y_i = \M|\beta$. In particular, the
$\beta_i$'s are cofinal in $\beta$.
\begin{proof}
Let $N$ be the transitive collapse of $\cup_{i<\omega} Y_i$ and let $\pi: N
\rightarrow \cup_{i\end{enumerate}
<\omega} Y_i$. Then $N = \mathcal{C}_0(\N)$ for some
$J$-premouse $\N$ over $\mathbb{R}^\M$. This uses that $J$ condenses well. Since
trees on $\N$ can be lifted to trees on $\M$ via $\pi$, $\N$ is $0$-countably
iterable. This implies $\N\lhd \M$. Since $\N$ realizes $\Sigma$, $\N = \M$.
This proves the claim.
\end{proof}
The rest of the proof is just as in the proof of
\cite[Theorem 4.16]{ScalesK(R)}. This completes our sketch of the theorem.
\end{proof}
A corollary of the proof of Theorem \ref{gapInTheMouse} is the following
theorem.
\begin{theorem}\end{enumerate}

\label{GapPassiveMouse}
Let $\M$ be a $J$-mouse over $\mathbb{R}^\M$ and $[\alpha,\beta]$ is a weak gap
in $\M$. Suppose either $\Theta^\M$ doesn't exist or sup$\{ \gamma < l(\M) \ | \
\M|\gamma \textrm{ is active}\} < l(\M)$. Letting $n$ be least such that
$\rho_n(\M|\beta)=\mathbb{R}^\M$, then $\M \vDash
``\utilde{\Sigma}^{\M|\beta}_n$ has the scale property". 
\end{theorem}
\begin{proof}[Sketch]
Note that $\beta$ could be $l(\M)$. The proof of this theorem follows from that
of Theorem \ref{gapInTheMouse} without significant changes. The point worth
mentioning is the following. Using the notation of the proof of Theorem 4.16 in
\cite{ScalesK(R)}, the condition (v) in the definition of $x$-honest becomes
\\
\noindent (v') \inde\end{enumerate}
nt if $\sigma_0,\dots, \sigma_n$ enumerates those
$B_0$-formulae $\sigma$ of one free variable such that $n(\sigma)\in
\textrm{dom}(u)$ and 
\begin{center}
$(|\M|\beta|,\in,I_u) \vDash i v \sigma(v) \in \textrm{OR}$,
\end{center}  
and if $\delta_m < o(\M|\beta)$ is such that 
\begin{center}
$(|\M|\beta|,\in,I_u) \vDash i v \sigma_m(v) = \delta_m$,
\end{center}  
for all $m\leq n$, then the map $\pi(\delta_m)= \eta_{n(\sigma_m)}$ for $m\leq
n$ is well-defined and for each $k<\omega$, $\pi$ is extendable to an
order-preserving map $\pi_k:o(\M|\beta_k)\rightarrow o(\M|\beta_k)$ such that
\begin{center}
$\M|\beta_k \vDash \theta[\gamma,w_1,w_2] \Leftrightarrow
\theta[\pi_k(\gamma),w_1,w_2]$.
\end{center}
\end{enumerate}

Note then that determinacy of $\M|\beta$ is enough to compute this aspect of
honesty. The rest of the proof is the same as before. 
\end{proof}
\end{comment}
\begin{comment}
 \item\label{item:local_cutpoint} Let $\eta<\xi<\OR^\N$ be such that $\eta$ is 
a strong cutpoint of
$\N|\xi$ and $\rho_\om(\N|\xi)\leq\eta$. Then
$\N|\xi\ins\Lp^{J,\Gamma}_+(\N|\eta)$.
\end{comment}
\begin{comment}
 \begin{definition}
  Let $t\in\RR$ and $1\leq k\leq\om$. A $J$-premouse $\N$ over $t$ is
\emph{$k$-suitable\end{enumerate}
} iff there is a strictly increasing sequence
$\left<\delta_i\right>_{i<k}$ such that \cite[1.2(a),(b),(d)]{Scalesweakgap}
hold (call these conditions (a),(b),(d)), along with: (c) Let $\xi\in\OR(\N)$
and let $\xibar=\car^\N(\xi)$. Among those extenders $E\in\es(\N)$ such that
$\xi<\lh(E)$, let $E$ be the extender for which $(\crit(E),\lh(E))$ is
$<_\lex$-minimal. Let $\kappa=\crit(E)$. 
 \begin{enumerate}
  \item Suppose $\kappa<\car^\N(\xi)$ (so $E$ is total over $\N$). Then
$\Lp^{J,\Gamma}(\N|\xi)=\N||\lh(E)$.
\item Suppose $\car^\N(\xi)\leq\kappa$. Then
$\Lp^{J,\Gamma}(\N|\xi)=(\N|(\xi^+)^\N,\N|\xi)^*$.
 \end{enumerate}
\end{definition}
For each $i\leq k$, we will write $\delta^\N_i$ for the $\delta_i$ in the above
definition. In the context of $k$-suitability, we omit the phrase ``over
$t$'', but all relevant premice will implicitly be over $t$ for some fixed $t$.
\end{comment}
\begin{comment}
Consider comparing $M^\Tt_b$ with the least
$\P\pins\Lp^{J,\Gamma}_+(M(\Tt))$ such that $\P$ projects to
$\delta(\Tt)$ and $\P\notin M^\Tt_b$, producing trees $\Uu,\Vv$ on
$M^\Tt_b,\P$. 

 Since $\P$ projects to $\delta(\Tt)$, $b^\Uu$ does
not drop. But then $\N$ is $\Gamma$-iterable, since the last model of $\Vv$ is
$\Gamma$-iterable (here we use that $\Lp^{J,\Gamma}_+(M(\Tt))$ is iterable for
finite stacks of normal trees). This is a contradiction. So if $i$ is least
such that $\Tt$ is based on $\N|\delta_i^\N$, then
$i^\Tt_b(\delta_i^\N)>\delta(\Tt)$. Therefore there is a Q-structure
$Q(\Tt,b)\ins M^\Tt_b$. If $Q(\Tt,b)$ does not overlap $\delta(\Tt)$ then we
can compare $Q(\Tt,b)$ with the Q-structure $Q\pins\Lp^{J,\Gamma}_+(M(\Tt))$,
as before, and therefore $Q(\Tt,b)=Q$, and we are done. Suppose $Q(\Tt,b)$
overlaps $\delta(\T\end{enumerate}
t)$.
\end{comment}

\begin{comment}
 Wfd'ness of $Q_\infty$ is not clear without $\RR=\RR^\M$. We do have wellfoundedness through 
$\Theta^\M$ tho. Regarding Lemma 2.1.2, it's okay as the linear chain gets in $\M_\DC$, so those 
iterates can all be compared inside $\M_\DC$.
\end{comment}

\begin{comment}
 Let $\Fop$ be an operator. We say that $\Fop$ is \textbf{extremely nice} iff there is a sequence 
of 
sets 
of reals 
$\left<A_i\right>_{i<\om\beta}$ for some $\beta$ such that:
\begin{enumerate}[label=(\arabic*)]
 \item $\Fop$ is very nice;
 \item for each $i<\beta$, $\left<A_{\omega i+n}\right>_{n<\om}$ is a self-justifying system;
 \item for each $i<\beta$, $n,m<\omega$, there is no scale on $A_{\om i + n}$ which is Wadge below 
$A_{\omega i + m}$, and $A_{\omega i + n}<_W 
A_{\omega i + k}$ for some $k<\om$;
\item for $i<j<\beta$, $A_{\omega i + n} <_W A_{\omega j}$ for all $n<\omega$;
 \item \label{item:ProjEqui}$\Fop\rest\HC$ is projectively equivalent to a set of 
Wadge rank sup$_{i<\beta}w(A_{\om i})$; and
 \item For every $\AD$-pointclass $\utilde{\Gamma}$, $\utilde{\Gamma},\Fop\rest\HC$ are Wadge 
compatible.
\begin{comment}and every $i<\beta$, $\utilde{\Gamma},A_{\omega 
i}$ are 
Wadge compatible.
\qedhere\end{enumerate}

\end{enumerate}
\end{definition}

\begin{remark}\label{rem:application}
Let $\Fop$ be an extremely nice operator.
We want to see that the scales analysis in 
$\Lp^{^\gTheta\Fop}(\RR)$ proceeds from optimal determinacy assumptions. Let 
$\N\pins\Lp^{^\gThe
ta\Fop}(\RR)$ be such that $\N\sats\AD$ and 
$\N$ ends a gap 
$[\alpha,\beta]$ of $\Lp^{^\gTheta\Fop}(\RR)$, such that $[\alpha,\beta]$ is not strong. Suppose 
that 
if $[\alpha,\beta]$ is weak and $\Fop\rest\HC\in\N|\alpha$ then super-small mouse capturing 
for $\Gamma=\Sigma_1^{\N|\alpha}$ holds on a cone. We claim that one of the scale existence 
theorems 
\ref{passiveGameScale}, 
\ref{gapInTheMou\end{enumerate}
se}, or \ref{weak gap from MC} applies.

For by \ref{rem:non_adm_gap_dealt_with} and the mouse capturing hypothesis, we may assume that the 
gap is admissible, and so weak, and that $\Fop\rest\HC\notin\N|\alpha$. We claim that then 
$\J_1(\N)\sats\AD$, so \ref{gapInTheMouse} applies. If every set of reals in $\J_1(\N)$ is Wadge 
below $A_{\om i}$ for some $i<\beta$, then this follows immediately because 
$\J_1(\HC,\Fop\rest\HC)\sats\AD$. So suppose otherwise. Let $\P\ins\N$ be least such that there is 
a 
set $X\in\J_1(\P)$ with $X$ not Wadge below any $A_{\om i}$. If $\P\pins\N$ then $\J_1(\P)\sats\AD$, 
so by 
Wadge compatibility (i.e. \ref{dfn:extremely}\ref{item:ProjEqui}), we have 
$\Fop\rest\HC\in\J_1(\P)$, so 
$\alpha\leq\l(\P)$. Now we claim that $\Fop\rest\HC\notin\N|\beta$. Because $\Fop$ is very nice 
and by 
\ref{InsideGap}, this is clear if $\Th_{\rPi_1}^{\N|\alpha}\leq_W
\Fop\rest\HC$ or $\Th_{\rSigma_1}^{\N|\alpha}\leq_W\Fop\rest\HC$. Otherwise, by Wadge 
compatibility, 
$\Fop\rest\HC<_W\Th_{\rSigma_1}^{\N|\alpha}$. But then because $\N|\alpha$ is 
admissible, 
$\Fop\rest\HC\in\N|\alpha$, contradiction. So $\P=\N$. 
Since $\N$ ends a 
weak gap, there are sets $X_i\in\pow(\RR)\inter\N$ such that $\pow(\RR)\inter\J_1(\N)$ is exactly 
the sets which are projective in $\oplus_{i<\om}X_i$. It follows that
$\pow(\RR)\inter\J_1(\N)=\pow(\RR)\inter\J_1(\HC,\Fop\rest\HC)$, so $\J_1(\N)\sats\AD$, as required.

%Let $T=\Th_{\rPi_1}^{\N|\alpha}(\RR)$; so $T\in\N$, so by Wadge compatibility, 
%either $T<_W A_{\om i}$ for some $i<\beta$ or $A_{\omega i}\leq_W T$ for all $i<\beta$. But if 
$T<_W A_{\omega i}$ then because $\Fop$ 
%is very nice, there is a scale on $T$ in $\J_1(\P)$, contradicting \ref{InsideGap}. So 
%$A_{\om i}\leq_W T$ for all $i<\beta$, and so $A_{\omega i} \leq_W\neg T$ for all $i<\beta$.


%Therefore $A_0<_W\neg T$, which 
%implies $A_0\in\N|\alpha$ because $\N|\alpha$ is admissible. But then there is a scale $S$ for 
$A_0$ 
%in $\N|\alpha$, so $S$ is not Wadge below any $A_i$, contradiction. 
\end{remark}

\end{comment}

